The Impact of Exposed Passwords on Honeyword Efficacy

Honeywords are decoy passwords that can be added to a credential database; if a login attempt uses a honeyword, this indicates that the site's credential database has been leaked. In this paper we explore the basic requirements for honeywords to be effective, in a threat model where the attacker knows passwords for the same users at other sites. First, we show that for user-chosen (vs. algorithmically generated, i.e., by a password manager) passwords, existing honeyword-generation algorithms do not simultaneously achieve false-positive and false-negative rates near their ideals of $\approx 0$ and $\approx \frac{1}{1+n}$, respectively, in this threat model, where $n$ is the number of honeywords per account. Second, we show that for users leveraging algorithmically generated passwords, state-of-the-art methods for honeyword generation will produce honeywords that are not sufficiently deceptive, yielding many false negatives. Instead, we find that only a honeyword-generation algorithm that uses the \textit{same} password generator as the user can provide deceptive honeywords in this case. However, when the defender's ability to infer the generator from the (one) account password is less accurate than the attacker's ability to infer the generator from potentially many, this deception can again wane. Taken together, our results provide a cautionary note for the state of honeyword research and pose new challenges to the field.

==> figure/mixed_0.33/CBTr/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.285899847745895 0.478500008583069
0.310899257659912 0.445400297641754
0.326100617647171 0.431899696588516
0.339499533176422 0.420900046825409
0.351800322532654 0.411700278520584
0.362800449132919 0.403700828552246
0.374600172042847 0.39849990606308
0.386000633239746 0.394400149583817
0.396400362253189 0.389099776744843
0.40629979968071 0.383900165557861
0.415600001811981 0.379999667406082
0.423299521207809 0.375499665737152
0.432400345802307 0.371200203895569
0.440899938344955 0.366800218820572
0.448000013828278 0.364000380039215
0.455600053071976 0.359199851751328
0.464300185441971 0.353800088167191
0.471599996089935 0.350199669599533
0.480299949645996 0.347700208425522
0.486099988222122 0.345599740743637
0.49210000038147 0.343299448490143
0.498699694871902 0.340699523687363
0.504800140857697 0.338899880647659
0.510700821876526 0.336899995803833
0.517799437046051 0.334899514913559
0.524200320243835 0.332499772310257
0.5316002368927 0.330700159072876
0.539398968219757 0.328500121831894
0.546002447605133 0.327099502086639
0.55270117521286 0.324500322341919
0.559199750423431 0.322200685739517
0.565599083900452 0.314500421285629
0.572399854660034 0.309200763702393
0.577998399734497 0.305799663066864
0.583300471305847 0.3030004799366
0.589798927307129 0.301099896430969
0.595799922943115 0.299100309610367
0.602500140666962 0.297300547361374
0.607997894287109 0.295999526977539
0.613400042057037 0.294899642467499
0.620099008083344 0.293599814176559
0.626802682876587 0.292500138282776
0.633098900318146 0.29169949889183
0.64029848575592 0.290600299835205
0.646801292896271 0.289500385522842
0.65339982509613 0.288701117038727
0.660400390625 0.287100106477737
0.666600167751312 0.284700304269791
0.673399448394775 0.281998574733734
0.680699110031128 0.280099153518677
0.68729841709137 0.278699159622192
0.693199872970581 0.276699811220169
0.6989985704422 0.275198817253113
0.7041996717453 0.27320072054863
0.711299180984497 0.271501004695892
0.716900229454041 0.269599914550781
0.723000109195709 0.267598807811737
0.729499101638794 0.26650071144104
0.735599339008331 0.265600442886353
0.743601024150848 0.264799982309341
0.749098896980286 0.2639000415802
0.754699468612671 0.262900501489639
0.760700166225433 0.262200325727463
0.768100202083588 0.233200028538704
0.774099290370941 0.223700001835823
0.781798660755157 0.221499904990196
0.789300143718719 0.220299899578094
0.794999837875366 0.218600049614906
0.801199436187744 0.217499807476997
0.807100415229797 0.216499999165535
0.813000082969666 0.215100094676018
0.818799197673798 0.213400050997734
0.823899388313293 0.211400091648102
0.829800367355347 0.209999904036522
0.834998905658722 0.208899706602097
0.841199994087219 0.207700178027153
0.847300171852112 0.206999465823174
0.852399528026581 0.205400094389915
0.858199596405029 0.203100010752678
0.864900171756744 0.201300159096718
0.869400382041931 0.199299767613411
0.876299798488617 0.196799844503403
0.882700204849243 0.195399880409241
0.888499975204468 0.193799898028374
0.894299924373627 0.192700237035751
0.902199983596802 0.191599979996681
0.90790057182312 0.190800115466118
0.914300203323364 0.190199956297874
0.920199632644653 0.189599722623825
0.925999999046326 0.188900366425514
0.932600080966949 0.187200129032135
0.939199805259705 0.184300035238266
0.94489997625351 0.182000160217285
0.95169997215271 0.179299905896187
0.958100020885468 0.174999907612801
0.964999914169312 0.1721001714468
0.972400009632111 0.169900149106979
0.978799998760223 0.16860020160675
0.988099992275238 0.16480016708374
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.982417583465576 0.478500008583069
0.984615385532379 0.445400297641754
0.985494494438171 0.431899696588516
0.98593407869339 0.420900046825409
0.986813187599182 0.411700278520584
0.986813187599182 0.403700828552246
0.986813187599182 0.39849990606308
0.987692296504974 0.394400149583817
0.988131880760193 0.389099776744843
0.988571405410767 0.383900165557861
0.988571405410767 0.379999667406082
0.988571405410767 0.375499665737152
0.989010989665985 0.371200203895569
0.989010989665985 0.366800218820572
0.989010989665985 0.364000380039215
0.989010989665985 0.359199851751328
0.989450573921204 0.353800088167191
0.989450573921204 0.350199669599533
0.989450573921204 0.347700208425522
0.989450573921204 0.345599740743637
0.989450573921204 0.343299448490143
0.989450573921204 0.340699523687363
0.989890098571777 0.338899880647659
0.989890098571777 0.336899995803833
0.989890098571777 0.334899514913559
0.989890098571777 0.332499772310257
0.990329682826996 0.330700159072876
0.990329682826996 0.328500121831894
0.990329682826996 0.327099502086639
0.990329682826996 0.324500322341919
0.990329682826996 0.322200685739517
0.99076920747757 0.314500421285629
0.991208791732788 0.309200763702393
0.991208791732788 0.305799663066864
0.991208791732788 0.3030004799366
0.991648375988007 0.301099896430969
0.991648375988007 0.299100309610367
0.991648375988007 0.297300547361374
0.991648375988007 0.295999526977539
0.99208790063858 0.294899642467499
0.99208790063858 0.293599814176559
0.99208790063858 0.292500138282776
0.99208790063858 0.29169949889183
0.992527484893799 0.290600299835205
0.992967009544373 0.289500385522842
0.993406593799591 0.288701117038727
0.993406593799591 0.287100106477737
0.993406593799591 0.284700304269791
0.993406593799591 0.281998574733734
0.99384617805481 0.280099153518677
0.99384617805481 0.278699159622192
0.99384617805481 0.276699811220169
0.99384617805481 0.275198817253113
0.994285702705383 0.27320072054863
0.994285702705383 0.271501004695892
0.994285702705383 0.269599914550781
0.994285702705383 0.267598807811737
0.994725286960602 0.26650071144104
0.994725286960602 0.265600442886353
0.994725286960602 0.264799982309341
0.994725286960602 0.2639000415802
0.994725286960602 0.262900501489639
0.994725286960602 0.262200325727463
0.995164811611176 0.233200028538704
0.995164811611176 0.223700001835823
0.995164811611176 0.221499904990196
0.995164811611176 0.220299899578094
0.995164811611176 0.218600049614906
0.996043980121613 0.217499807476997
0.996043980121613 0.216499999165535
0.996043980121613 0.215100094676018
0.996923089027405 0.213400050997734
0.996923089027405 0.211400091648102
0.997362613677979 0.209999904036522
0.997362613677979 0.208899706602097
0.997802197933197 0.207700178027153
0.997802197933197 0.206999465823174
0.998241782188416 0.205400094389915
0.998241782188416 0.203100010752678
0.998241782188416 0.201300159096718
0.998241782188416 0.199299767613411
0.998241782188416 0.196799844503403
0.998241782188416 0.195399880409241
0.998241782188416 0.193799898028374
0.998241782188416 0.192700237035751
0.998241782188416 0.191599979996681
0.998241782188416 0.190800115466118
0.998241782188416 0.190199956297874
0.998241782188416 0.189599722623825
0.998241782188416 0.188900366425514
0.998241782188416 0.187200129032135
0.998241782188416 0.184300035238266
0.998241782188416 0.182000160217285
0.998241782188416 0.179299905896187
0.998681306838989 0.174999907612801
0.998681306838989 0.1721001714468
0.998681306838989 0.169900149106979
0.998681306838989 0.16860020160675
0.999120891094208 0.16480016708374
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.263013899326324 0.478500008583069
0.333333164453506 0.445400297641754
0.366209894418716 0.431899696588516
0.385388195514679 0.420900046825409
0.407305836677551 0.411700278520584
0.429223716259003 0.403700828552246
0.452968060970306 0.39849990606308
0.469406455755234 0.394400149583817
0.488584697246552 0.389099776744843
0.499543994665146 0.383900165557861
0.514154970645905 0.379999667406082
0.521461129188538 0.375499665737152
0.534246146678925 0.371200203895569
0.547031879425049 0.366800218820572
0.554338216781616 0.364000380039215
0.559817373752594 0.359199851751328
0.571689605712891 0.353800088167191
0.581735074520111 0.350199669599533
0.589954555034637 0.347700208425522
0.597260117530823 0.345599740743637
0.601826548576355 0.343299448490143
0.606392860412598 0.340699523687363
0.610959112644196 0.338899880647659
0.615525186061859 0.336899995803833
0.621917724609375 0.334899514913559
0.627397119998932 0.332499772310257
0.635616838932037 0.330700159072876
0.645662009716034 0.328500121831894
0.652054727077484 0.327099502086639
0.659360527992249 0.324500322341919
0.66483998298645 0.322200685739517
0.670319736003876 0.314500421285629
0.675799071788788 0.309200763702393
0.682192087173462 0.305799663066864
0.687671065330505 0.3030004799366
0.692237555980682 0.301099896430969
0.695890545845032 0.299100309610367
0.70319652557373 0.297300547361374
0.71050226688385 0.295999526977539
0.715068280696869 0.294899642467499
0.71963495016098 0.293599814176559
0.726027369499207 0.292500138282776
0.726941049098969 0.29169949889183
0.729680061340332 0.290600299835205
0.735159993171692 0.289500385522842
0.740639328956604 0.288701117038727
0.746118664741516 0.287100106477737
0.749771237373352 0.284700304269791
0.757077813148499 0.281998574733734
0.76621001958847 0.280099153518677
0.768949508666992 0.278699159622192
0.774429202079773 0.276699811220169
0.780821681022644 0.275198817253113
0.781735181808472 0.27320072054863
0.785388231277466 0.271501004695892
0.78904116153717 0.269599914550781
0.794520199298859 0.267598807811737
0.801826536655426 0.26650071144104
0.808219194412231 0.265600442886353
0.814611911773682 0.264799982309341
0.817351818084717 0.2639000415802
0.82283091545105 0.262900501489639
0.830137014389038 0.262200325727463
0.839269757270813 0.233200028538704
0.845661878585815 0.223700001835823
0.852967619895935 0.221499904990196
0.861187219619751 0.220299899578094
0.866666734218597 0.218600049614906
0.867579996585846 0.217499807476997
0.870319902896881 0.216499999165535
0.873059272766113 0.215100094676018
0.875799179077148 0.213400050997734
0.880365490913391 0.211400091648102
0.884018182754517 0.209999904036522
0.886757850646973 0.208899706602097
0.890411019325256 0.207700178027153
0.892237663269043 0.206999465823174
0.894977152347565 0.205400094389915
0.898630082607269 0.203100010752678
0.902283310890198 0.201300159096718
0.905936002731323 0.199299767613411
0.908675789833069 0.196799844503403
0.910502254962921 0.195399880409241
0.915981709957123 0.193799898028374
0.917808294296265 0.192700237035751
0.922374427318573 0.191599979996681
0.926027476787567 0.190800115466118
0.930593729019165 0.190199956297874
0.937899649143219 0.189599722623825
0.94063925743103 0.188900366425514
0.943379104137421 0.187200129032135
0.947945177555084 0.184300035238266
0.948858320713043 0.182000160217285
0.956164360046387 0.179299905896187
0.960730612277985 0.174999907612801
0.965296804904938 0.1721001714468
0.970776259899139 0.169900149106979
0.978995442390442 0.16860020160675
0.984474897384644 0.16480016708374
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0506787300109863 0.478500008583069
0.0760180577635765 0.445400297641754
0.0932127237319946 0.431899696588516
0.11010555177927 0.420900046825409
0.124736152589321 0.411700278520584
0.137707442045212 0.403700828552246
0.151583909988403 0.39849990606308
0.165761694312096 0.394400149583817
0.178129523992538 0.389099776744843
0.19110107421875 0.383900165557861
0.202714934945107 0.379999667406082
0.213122054934502 0.375499665737152
0.224585294723511 0.371200203895569
0.235294103622437 0.366800218820572
0.244796365499496 0.364000380039215
0.255354970693588 0.359199851751328
0.266364634037018 0.353800088167191
0.275716990232468 0.350199669599533
0.28748145699501 0.347700208425522
0.295022904872894 0.345599740743637
0.303317964076996 0.343299448490143
0.312518537044525 0.340699523687363
0.320815294981003 0.338899880647659
0.328959226608276 0.336899995803833
0.338612526655197 0.334899514913559
0.347360730171204 0.332499772310257
0.357013761997223 0.330700159072876
0.367119014263153 0.328500121831894
0.376017868518829 0.327099502086639
0.384916752576828 0.324500322341919
0.393816083669662 0.322200685739517
0.402413129806519 0.314500421285629
0.411613881587982 0.309200763702393
0.419004410505295 0.305799663066864
0.426093518733978 0.3030004799366
0.434992223978043 0.301099896430969
0.443439066410065 0.299100309610367
0.452337861061096 0.297300547361374
0.45942685008049 0.295999526977539
0.466666668653488 0.294899642467499
0.476018011569977 0.293599814176559
0.485067874193192 0.292500138282776
0.494419306516647 0.29169949889183
0.504675030708313 0.290600299835205
0.513423323631287 0.289500385522842
0.522323668003082 0.288701117038727
0.531975209712982 0.287100106477737
0.540723741054535 0.284700304269791
0.549774289131165 0.281998574733734
0.55912572145462 0.280099153518677
0.568628370761871 0.278699159622192
0.576619625091553 0.276699811220169
0.584312081336975 0.275198817253113
0.591853559017181 0.27320072054863
0.601962089538574 0.271501004695892
0.609804451465607 0.269599914550781
0.618100166320801 0.267598807811737
0.626544594764709 0.26650071144104
0.634691953659058 0.265600442886353
0.645699977874756 0.264799982309341
0.653545677661896 0.2639000415802
0.661085903644562 0.262900501489639
0.66892808675766 0.262200325727463
0.678430914878845 0.233200028538704
0.686425626277924 0.223700001835823
0.696832954883575 0.221499904990196
0.706786870956421 0.220299899578094
0.714480102062225 0.218600049614906
0.723378598690033 0.217499807476997
0.731825172901154 0.216499999165535
0.740272104740143 0.215100094676018
0.748265027999878 0.213400050997734
0.755204141139984 0.211400091648102
0.763348042964935 0.209999904036522
0.770739376544952 0.208899706602097
0.779335618019104 0.207700178027153
0.788235604763031 0.206999465823174
0.795324444770813 0.205400094389915
0.803468286991119 0.203100010752678
0.81297105550766 0.201300159096718
0.819155216217041 0.199299767613411
0.829109489917755 0.196799844503403
0.838461518287659 0.195399880409241
0.846304774284363 0.193799898028374
0.854751288890839 0.192700237035751
0.865912199020386 0.191599979996681
0.873906493186951 0.190800115466118
0.882805585861206 0.190199956297874
0.89049756526947 0.189599722623825
0.89879322052002 0.188900366425514
0.908295631408691 0.187200129032135
0.917496502399445 0.184300035238266
0.925942540168762 0.182000160217285
0.934992253780365 0.179299905896187
0.943740487098694 0.174999907612801
0.953393757343292 0.1721001714468
0.963650047779083 0.169900149106979
0.971945583820343 0.16860020160675
0.984917044639587 0.16480016708374
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/CHM/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.261500924825668 0.675799608230591
0.283099800348282 0.675702393054962
0.304098963737488 0.675702393054962
0.319500058889389 0.675601899623871
0.333299994468689 0.675300359725952
0.345000028610229 0.674799203872681
0.356400400400162 0.674299597740173
0.368100047111511 0.67330002784729
0.379499644041061 0.67180061340332
0.391099840402603 0.670098841190338
0.401900380849838 0.668198823928833
0.411499500274658 0.664001047611237
0.422100007534027 0.659900069236755
0.430099755525589 0.653601109981537
0.439600199460983 0.646000504493713
0.448799908161163 0.636501491069794
0.456900149583817 0.62690132856369
0.465300142765045 0.614100754261017
0.474200010299683 0.602600932121277
0.481000006198883 0.589898705482483
0.490000009536743 0.575498998165131
0.497499644756317 0.561297357082367
0.505299389362335 0.547499418258667
0.513700306415558 0.534400224685669
0.52130138874054 0.52190101146698
0.528600811958313 0.505599975585938
0.536401152610779 0.49210000038147
0.543499052524567 0.475600033998489
0.551600754261017 0.458599895238876
0.558499097824097 0.439499765634537
0.566198885440826 0.419200301170349
0.573398947715759 0.398899674415588
0.581700623035431 0.377599686384201
0.588900625705719 0.359300136566162
0.596700370311737 0.335599631071091
0.603899836540222 0.312599837779999
0.610701620578766 0.288699626922607
0.61770236492157 0.26849952340126
0.624800801277161 0.246700003743172
0.634100615978241 0.22779980301857
0.642301559448242 0.207900196313858
0.649600565433502 0.189999729394913
0.655999779701233 0.170799970626831
0.663002371788025 0.15159983932972
0.669201493263245 0.132200285792351
0.675800263881683 0.115900009870529
0.683499395847321 0.101800076663494
0.689500093460083 0.0876999497413635
0.696300804615021 0.0747999176383018
0.702898263931274 0.0646000653505325
0.708901047706604 0.0542000122368336
0.71599930524826 0.0457000508904457
0.721899092197418 0.0386999100446701
0.7277991771698 0.0317000485956669
0.734000146389008 0.026399988681078
0.739899575710297 0.0209000129252672
0.746198832988739 0.0152000123634934
0.753499269485474 0.0105000045150518
0.759600043296814 0.00829998590052128
0.767300605773926 0.00579999946057796
0.774400591850281 0.0045999912545085
0.780000388622284 0.00350000197067857
0.787299752235413 0.00299998978152871
0.794400870800018 0.00249999645166099
0.799999296665192 0.00199999078176916
0.807199537754059 0.00160000112373382
0.814200580120087 0.000999995390884578
0.819800019264221 0.000299999344861135
0.826399385929108 9.99997646431439e-05
0.831900119781494 9.99997646431439e-05
0.838399529457092 9.99997646431439e-05
0.844300389289856 0
0.849400758743286 0
0.855100572109222 0
0.86069929599762 0
0.866698443889618 0
0.871900022029877 0
0.877000570297241 0
0.883000075817108 0
0.887800216674805 0
0.891799986362457 0
0.898300409317017 0
0.905099809169769 0
0.911000370979309 0
0.916000008583069 0
0.922399818897247 0
0.929199993610382 0
0.935299634933472 0
0.940099775791168 0
0.945999801158905 0
0.951600015163422 0
0.958500027656555 0
0.963399887084961 0
0.968800008296967 0
0.97409999370575 0
0.979399979114532 0
0.984899997711182 0
0.990899980068207 0
0.995100021362305 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.977242887020111 0.675799608230591
0.982932150363922 0.675702393054962
0.98730856180191 0.675702393054962
0.989934325218201 0.675601899623871
0.991684913635254 0.675300359725952
0.992122530937195 0.674799203872681
0.992122530937195 0.674299597740173
0.992560148239136 0.67330002784729
0.992997825145721 0.67180061340332
0.992997825145721 0.670098841190338
0.993435442447662 0.668198823928833
0.993435442447662 0.664001047611237
0.993435442447662 0.659900069236755
0.993435442447662 0.653601109981537
0.993435442447662 0.646000504493713
0.993873059749603 0.636501491069794
0.994310736656189 0.62690132856369
0.994310736656189 0.614100754261017
0.994310736656189 0.602600932121277
0.994310736656189 0.589898705482483
0.994310736656189 0.575498998165131
0.994310736656189 0.561297357082367
0.994310736656189 0.547499418258667
0.994310736656189 0.534400224685669
0.994310736656189 0.52190101146698
0.994310736656189 0.505599975585938
0.994310736656189 0.49210000038147
0.994310736656189 0.475600033998489
0.994310736656189 0.458599895238876
0.994310736656189 0.439499765634537
0.994310736656189 0.419200301170349
0.994310736656189 0.398899674415588
0.994310736656189 0.377599686384201
0.994310736656189 0.359300136566162
0.994310736656189 0.335599631071091
0.994310736656189 0.312599837779999
0.994310736656189 0.288699626922607
0.994310736656189 0.26849952340126
0.994310736656189 0.246700003743172
0.99474835395813 0.22779980301857
0.99474835395813 0.207900196313858
0.99474835395813 0.189999729394913
0.99474835395813 0.170799970626831
0.995185971260071 0.15159983932972
0.995623648166656 0.132200285792351
0.996061265468597 0.115900009870529
0.996061265468597 0.101800076663494
0.996061265468597 0.0876999497413635
0.996061265468597 0.0747999176383018
0.996061265468597 0.0646000653505325
0.996061265468597 0.0542000122368336
0.996061265468597 0.0457000508904457
0.996061265468597 0.0386999100446701
0.996498882770538 0.0317000485956669
0.996498882770538 0.026399988681078
0.996498882770538 0.0209000129252672
0.996498882770538 0.0152000123634934
0.996936559677124 0.0105000045150518
0.996936559677124 0.00829998590052128
0.996936559677124 0.00579999946057796
0.996936559677124 0.0045999912545085
0.996936559677124 0.00350000197067857
0.996936559677124 0.00299998978152871
0.996936559677124 0.00249999645166099
0.996936559677124 0.00199999078176916
0.996936559677124 0.00160000112373382
0.996936559677124 0.000999995390884578
0.996936559677124 0.000299999344861135
0.997811794281006 9.99997646431439e-05
0.997811794281006 9.99997646431439e-05
0.997811794281006 9.99997646431439e-05
0.998249471187592 0
0.998249471187592 0
0.998249471187592 0
0.998249471187592 0
0.998687088489532 0
0.998687088489532 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999124705791473 0
0.999562382698059 0
0.999562382698059 0
0.999562382698059 0
0.999562382698059 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.181981936097145 0.675799608230591
0.265765905380249 0.675702393054962
0.352252095937729 0.675702393054962
0.413513571023941 0.675601899623871
0.454955011606216 0.675300359725952
0.491892218589783 0.674799203872681
0.525225639343262 0.674299597740173
0.563063204288483 0.67330002784729
0.590090394020081 0.67180061340332
0.624324202537537 0.670098841190338
0.636936843395233 0.668198823928833
0.652252078056335 0.664001047611237
0.663062930107117 0.659900069236755
0.674774646759033 0.653601109981537
0.686486542224884 0.646000504493713
0.694595038890839 0.636501491069794
0.703603863716125 0.62690132856369
0.711711645126343 0.614100754261017
0.722522497177124 0.602600932121277
0.72792774438858 0.589898705482483
0.736036241054535 0.575498998165131
0.737837910652161 0.561297357082367
0.743243217468262 0.547499418258667
0.750450372695923 0.534400224685669
0.758558750152588 0.52190101146698
0.764864921569824 0.505599975585938
0.768468379974365 0.49210000038147
0.776576459407806 0.475600033998489
0.783783853054047 0.458599895238876
0.793693661689758 0.439499765634537
0.798198282718658 0.419200301170349
0.804504573345184 0.398899674415588
0.809009313583374 0.377599686384201
0.812612652778625 0.359300136566162
0.818918943405151 0.335599631071091
0.825225234031677 0.312599837779999
0.831531643867493 0.288699626922607
0.838738858699799 0.26849952340126
0.847747921943665 0.246700003743172
0.851351261138916 0.22779980301857
0.854954957962036 0.207900196313858
0.858558595180511 0.189999729394913
0.859459519386292 0.170799970626831
0.860360383987427 0.15159983932972
0.862161993980408 0.132200285792351
0.866666913032532 0.115900009870529
0.867567837238312 0.101800076663494
0.870270371437073 0.0876999497413635
0.872072041034698 0.0747999176383018
0.87567549943924 0.0646000653505325
0.878378331661224 0.0542000122368336
0.88468474149704 0.0457000508904457
0.88738751411438 0.0386999100446701
0.889189302921295 0.0317000485956669
0.890990972518921 0.026399988681078
0.893693685531616 0.0209000129252672
0.896396398544312 0.0152000123634934
0.899999916553497 0.0105000045150518
0.903603374958038 0.00829998590052128
0.904504477977753 0.00579999946057796
0.905405461788177 0.0045999912545085
0.907207012176514 0.00350000197067857
0.911711871623993 0.00299998978152871
0.913513660430908 0.00249999645166099
0.918018043041229 0.00199999078176916
0.920720756053925 0.00160000112373382
0.92522519826889 0.000999995390884578
0.927927911281586 0.000299999344861135
0.930630505084991 9.99997646431439e-05
0.932432413101196 9.99997646431439e-05
0.936036050319672 9.99997646431439e-05
0.937837839126587 0
0.939639508724213 0
0.941441416740417 0
0.945045053958893 0
0.946846842765808 0
0.948648631572723 0
0.950450479984283 0
0.952252268791199 0
0.953153133392334 0
0.955855846405029 0
0.957657635211945 0
0.959459483623505 0
0.962162137031555 0
0.963963985443115 0
0.967567563056946 0
0.970270276069641 0
0.972972989082336 0
0.979279279708862 0
0.979279279708862 0
0.981081068515778 0
0.981981992721558 0
0.982882857322693 0
0.986486494541168 0
0.990090072154999 0
0.990990996360779 0
0.995495498180389 0
0.997297286987305 0
0.998198211193085 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0272520687431097 0.675799608230591
0.043906144797802 0.675702393054962
0.0596516989171505 0.675702393054962
0.0717639103531837 0.675601899623871
0.0850870162248611 0.675300359725952
0.0964421853423119 0.674799203872681
0.108099929988384 0.674299597740173
0.119303613901138 0.67330002784729
0.131869718432426 0.67180061340332
0.143679603934288 0.670098841190338
0.157759234309196 0.668198823928833
0.169719949364662 0.664001047611237
0.183951497077942 0.659900069236755
0.194095313549042 0.653601109981537
0.206510439515114 0.646000504493713
0.218925014138222 0.636501491069794
0.229523122310638 0.62690132856369
0.240878090262413 0.614100754261017
0.252536207437515 0.602600932121277
0.261922717094421 0.589898705482483
0.274186223745346 0.575498998165131
0.285238832235336 0.561297357082367
0.296139657497406 0.547499418258667
0.307646125555038 0.534400224685669
0.3177889585495 0.52190101146698
0.32778137922287 0.505599975585938
0.338985532522202 0.49210000038147
0.348372370004654 0.475600033998489
0.359424740076065 0.458599895238876
0.368206053972244 0.439499765634537
0.379107028245926 0.419200301170349
0.388947755098343 0.398899674415588
0.400756925344467 0.377599686384201
0.411052167415619 0.359300136566162
0.421801745891571 0.335599631071091
0.431642532348633 0.312599837779999
0.440878123044968 0.288699626922607
0.450265049934387 0.26849952340126
0.459500372409821 0.246700003743172
0.472823530435562 0.22779980301857
0.484632849693298 0.207900196313858
0.495079338550568 0.189999729394913
0.504617094993591 0.170799970626831
0.514912784099579 0.15159983932972
0.523846507072449 0.132200285792351
0.532929718494415 0.115900009870529
0.544438242912292 0.101800076663494
0.553065955638885 0.0876999497413635
0.563055753707886 0.0747999176383018
0.572445452213287 0.0646000653505325
0.581075489521027 0.0542000122368336
0.590763509273529 0.0457000508904457
0.599242925643921 0.0386999100446701
0.607721328735352 0.0317000485956669
0.61680543422699 0.026399988681078
0.625285506248474 0.0209000129252672
0.634367167949677 0.0152000123634934
0.644665062427521 0.0105000045150518
0.653293311595917 0.00829998590052128
0.664799749851227 0.00579999946057796
0.675397992134094 0.0045999912545085
0.683572173118591 0.00350000197067857
0.69386899471283 0.00299998978152871
0.704315662384033 0.00249999645166099
0.712036311626434 0.00199999078176916
0.722482204437256 0.00160000112373382
0.73232364654541 0.000999995390884578
0.740348756313324 0.000299999344861135
0.749583959579468 9.99997646431439e-05
0.757607161998749 9.99997646431439e-05
0.766842722892761 9.99997646431439e-05
0.775322616100311 0
0.782739460468292 0
0.79106730222702 0
0.798940181732178 0
0.807570397853851 0
0.815139770507812 0
0.822406828403473 0
0.831188201904297 0
0.838303744792938 0
0.843905806541443 0
0.853444278240204 0
0.863436341285706 0
0.871915280818939 0
0.879182159900665 0
0.888266146183014 0
0.898107469081879 0
0.906888544559479 0
0.913096308708191 0
0.92202889919281 0
0.930204451084137 0
0.940499484539032 0
0.947766780853271 0
0.95533686876297 0
0.962604105472565 0
0.970476925373077 0
0.978046953678131 0
0.986828148365021 0
0.992884159088135 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/List/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.375600010156631 0.674200654029846
0.395699918270111 0.661402225494385
0.411800295114517 0.622997879981995
0.423999905586243 0.549498617649078
0.437600195407867 0.44200000166893
0.447600394487381 0.322399944067001
0.458399802446365 0.20829975605011
0.46849998831749 0.120199978351593
0.480500012636185 0.0618998110294342
0.490899711847305 0.0306000113487244
0.50110137462616 0.0127000026404858
0.511399328708649 0.00499998638406396
0.520899534225464 0.00149999489076436
0.528400421142578 0.000499999907333404
0.537100672721863 0
0.547900319099426 0
0.556598961353302 0
0.564200162887573 0
0.573099792003632 0
0.580998778343201 0
0.588898122310638 0
0.596301674842834 0
0.604699730873108 0
0.613500356674194 0
0.62120109796524 0
0.62790048122406 0
0.633499145507812 0
0.640299439430237 0
0.64730030298233 0
0.654599487781525 0
0.660600483417511 0
0.667099595069885 0
0.673800051212311 0
0.680299401283264 0
0.687400460243225 0
0.693798899650574 0
0.700200855731964 0
0.707300126552582 0
0.713099777698517 0
0.720500290393829 0
0.725899159908295 0
0.733300507068634 0
0.738799691200256 0
0.744599223136902 0
0.749700009822845 0
0.756000876426697 0
0.762199223041534 0
0.76829981803894 0
0.774199843406677 0
0.779900372028351 0
0.786198854446411 0
0.792800486087799 0
0.798200070858002 0
0.803300440311432 0
0.808700799942017 0
0.814599454402924 0
0.819100379943848 0
0.824400365352631 0
0.828999638557434 0
0.835399329662323 0
0.841799974441528 0
0.846699416637421 0
0.851900279521942 0
0.856099605560303 0
0.861099600791931 0
0.866400361061096 0
0.871999979019165 0
0.87619960308075 0
0.880399882793427 0
0.88500040769577 0
0.889798820018768 0
0.893600285053253 0
0.896999716758728 0
0.901399791240692 0
0.907000005245209 0
0.911100208759308 0
0.9154993891716 0
0.919400215148926 0
0.925099790096283 0
0.929699420928955 0
0.933700382709503 0
0.938100099563599 0
0.941899538040161 0
0.945700109004974 0
0.948800206184387 0
0.953599810600281 0
0.95770001411438 0
0.961299896240234 0
0.96450001001358 0
0.967899799346924 0
0.971200168132782 0
0.975499987602234 0
0.97979998588562 0
0.98360002040863 0
0.985899984836578 0
0.988900005817413 0
0.991900026798248 0
0.994499981403351 0
0.997099995613098 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.982796669006348 0.674200654029846
0.987207770347595 0.661402225494385
0.988089978694916 0.622997879981995
0.988972187042236 0.549498617649078
0.989413321018219 0.44200000166893
0.989413321018219 0.322399944067001
0.989413321018219 0.20829975605011
0.989854454994202 0.120199978351593
0.989854454994202 0.0618998110294342
0.989854454994202 0.0306000113487244
0.989854454994202 0.0127000026404858
0.989854454994202 0.00499998638406396
0.989854454994202 0.00149999489076436
0.989854454994202 0.000499999907333404
0.989854454994202 0
0.989854454994202 0
0.99029552936554 0
0.990736663341522 0
0.990736663341522 0
0.990736663341522 0
0.990736663341522 0
0.990736663341522 0
0.990736663341522 0
0.991177797317505 0
0.991618871688843 0
0.991618871688843 0
0.991618871688843 0
0.991618871688843 0
0.991618871688843 0
0.991618871688843 0
0.992060005664825 0
0.992060005664825 0
0.992060005664825 0
0.992501080036163 0
0.992501080036163 0
0.992501080036163 0
0.992501080036163 0
0.992501080036163 0
0.992501080036163 0
0.992942214012146 0
0.992942214012146 0
0.993383347988129 0
0.993383347988129 0
0.993824422359467 0
0.994265556335449 0
0.994706690311432 0
0.994706690311432 0
0.994706690311432 0
0.99514776468277 0
0.99514776468277 0
0.99514776468277 0
0.99514776468277 0
0.99514776468277 0
0.995588898658752 0
0.995588898658752 0
0.995588898658752 0
0.995588898658752 0
0.99602997303009 0
0.99602997303009 0
0.99602997303009 0
0.99602997303009 0
0.99602997303009 0
0.99602997303009 0
0.99602997303009 0
0.996471107006073 0
0.996471107006073 0
0.996471107006073 0
0.996471107006073 0
0.997353315353394 0
0.997353315353394 0
0.997353315353394 0
0.997794449329376 0
0.997794449329376 0
0.997794449329376 0
0.997794449329376 0
0.998235583305359 0
0.998235583305359 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.998676657676697 0
0.999117791652679 0
0.999558866024017 0
0.999558866024017 0
0.999558866024017 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.513615369796753 0.674200654029846
0.541604220867157 0.661402225494385
0.563540637493134 0.622997879981995
0.577154934406281 0.549498617649078
0.586989343166351 0.44200000166893
0.596066355705261 0.322399944067001
0.611195087432861 0.20829975605011
0.620272219181061 0.120199978351593
0.632375240325928 0.0618998110294342
0.641452252864838 0.0306000113487244
0.653555750846863 0.0127000026404858
0.662632167339325 0.00499998638406396
0.670952916145325 0.00149999489076436
0.68002986907959 0.000499999907333404
0.687594413757324 0
0.689863681793213 0
0.695159196853638 0
0.701966047286987 0
0.711800277233124 0
0.717095196247101 0
0.723902940750122 0
0.725416600704193 0
0.730710625648499 0
0.738274931907654 0
0.745839893817902 0
0.754160404205322 0
0.757942914962769 0
0.765507102012634 0
0.773827314376831 0
0.779878973960876 0
0.783661007881165 0
0.788199901580811 0
0.791225612163544 0
0.795764207839966 0
0.80181485414505 0
0.807866930961609 0
0.810136079788208 0
0.817700564861298 0
0.824508666992188 0
0.830559968948364 0
0.834342002868652 0
0.838880121707916 0
0.839636385440826 0
0.841150164604187 0
0.844175279140472 0
0.845687985420227 0
0.848714649677277 0
0.850983381271362 0
0.853252649307251 0
0.858547449111938 0
0.863842666149139 0
0.86989426612854 0
0.873676240444183 0
0.876701772212982 0
0.879727840423584 0
0.882753789424896 0
0.885022580623627 0
0.891074061393738 0
0.893343448638916 0
0.894099771976471 0
0.897882342338562 0
0.899394869804382 0
0.905446290969849 0
0.907715559005737 0
0.910741090774536 0
0.914523363113403 0
0.91906201839447 0
0.922843992710114 0
0.924357056617737 0
0.925869703292847 0
0.928895592689514 0
0.930408477783203 0
0.931921243667603 0
0.934947073459625 0
0.937972784042358 0
0.940998673439026 0
0.942511320114136 0
0.945537149906158 0
0.948562800884247 0
0.950075447559357 0
0.953101336956024 0
0.955370664596558 0
0.956883490085602 0
0.960665643215179 0
0.962178528308868 0
0.965204238891602 0
0.969742834568024 0
0.972012102603912 0
0.977307021617889 0
0.977307021617889 0
0.980332851409912 0
0.982602119445801 0
0.985627830028534 0
0.988653540611267 0
0.990922868251801 0
0.991679251194 0
0.995461404323578 0
0.996974289417267 0
0.997730731964111 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0394633300602436 0.674200654029846
0.0664482265710831 0.661402225494385
0.0889097228646278 0.622997879981995
0.108407445251942 0.549498617649078
0.130400523543358 0.44200000166893
0.146779417991638 0.322399944067001
0.16346937417984 0.20829975605011
0.178287208080292 0.120199978351593
0.196693196892738 0.0618998110294342
0.213383242487907 0.0306000113487244
0.228045552968979 0.0127000026404858
0.244111642241478 0.00499998638406396
0.258306413888931 0.00149999489076436
0.270473331212997 0.000499999907333404
0.284822851419449 0
0.303073555231094 0
0.317423433065414 0
0.329122304916382 0
0.343471556901932 0
0.357198297977448 0
0.369676798582077 0
0.382467418909073 0
0.396193653345108 0
0.409452497959137 0
0.421619236469269 0
0.43206986784935 0
0.44298854470253 0
0.451567530632019 0
0.461550533771515 0
0.473561078310013 0
0.483699828386307 0
0.494618386030197 0
0.50569361448288 0
0.515831291675568 0
0.527531385421753 0
0.537356793880463 0
0.547808468341827 0
0.558102667331696 0
0.565746963024139 0
0.577600598335266 0
0.586024463176727 0
0.597099483013153 0
0.606300890445709 0
0.615192532539368 0
0.623146295547485 0
0.633130788803101 0
0.64389181137085 0
0.653876066207886 0
0.664172530174255 0
0.672594368457794 0
0.681952893733978 0
0.691778600215912 0
0.70113867521286 0
0.708468735218048 0
0.716736078262329 0
0.726095795631409 0
0.732803821563721 0
0.740134000778198 0
0.747309923171997 0
0.758852422237396 0
0.768834054470062 0
0.77632200717926 0
0.783965229988098 0
0.790203511714935 0
0.797535181045532 0
0.80517852306366 0
0.813133835792542 0
0.819061160087585 0
0.825300514698029 0
0.832319617271423 0
0.83918297290802 0
0.845422029495239 0
0.85072523355484 0
0.85680878162384 0
0.865387618541718 0
0.871159076690674 0
0.878177762031555 0
0.883325636386871 0
0.891904532909393 0
0.898923873901367 0
0.904850900173187 0
0.911402344703674 0
0.917485415935516 0
0.92310094833374 0
0.927780389785767 0
0.934643507003784 0
0.940103113651276 0
0.945250272750854 0
0.94914984703064 0
0.95445328950882 0
0.959288716316223 0
0.965839982032776 0
0.971923232078552 0
0.977226555347443 0
0.980034291744232 0
0.984401822090149 0
0.988301336765289 0
0.992044925689697 0
0.995944499969482 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/List/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    % ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.430800348520279 0.456900000572205
0.484199911355972 0.193799719214439
0.533602178096771 0.0598000138998032
0.578299343585968 0.01490000449121
0.619299530982971 0.00150000141002238
0.650498986244202 0.000199999529286288
0.686900019645691 0
0.719199001789093 0
0.748800456523895 0
0.778799295425415 0
0.80269992351532 0
0.829500377178192 0
0.855000615119934 0
0.88120049238205 0
0.904800176620483 0
0.928600192070007 0
0.948599636554718 0
0.966799974441528 0
0.983900010585785 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.996877789497375 0.456900000572205
0.99732381105423 0.193799719214439
0.99732381105423 0.0598000138998032
0.99732381105423 0.01490000449121
0.99732381105423 0.00150000141002238
0.997769832611084 0.000199999529286288
0.998215854167938 0
0.998215854167938 0
0.998215854167938 0
0.998215854167938 0
0.998661935329437 0
0.998661935329437 0
0.998661935329437 0
0.998661935329437 0
0.999107956886292 0
0.999107956886292 0
0.999107956886292 0
0.999107956886292 0
0.999553978443146 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.749999761581421 0.456900000572205
0.797520577907562 0.193799719214439
0.832644522190094 0.0598000138998032
0.858471214771271 0.01490000449121
0.873966932296753 0.00150000141002238
0.888429641723633 0.000199999529286288
0.900826454162598 0
0.912190020084381 0
0.9194216132164 0
0.929752051830292 0
0.934917330741882 0
0.93904972076416 0
0.946281015872955 0
0.96074378490448 0
0.971074402332306 0
0.976239681243896 0
0.983471095561981 0
0.985537171363831 0
0.991735517978668 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.122091345489025 0.456900000572205
0.207069233059883 0.193799719214439
0.283358931541443 0.0598000138998032
0.357436984777451 0.01490000449121
0.423416793346405 0.00150000141002238
0.471281379461288 0.000199999529286288
0.529307961463928 0
0.579822897911072 0
0.626214146614075 0
0.67334258556366 0
0.710456669330597 0
0.752577841281891 0
0.791016280651093 0
0.828130185604095 0
0.862150490283966 0
0.897054493427277 0
0.926214993000031 0
0.953313708305359 0
0.977614164352417 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/List_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.309600353240967 0.670598983764648
0.326099574565887 0.65679919719696
0.338400423526764 0.627800941467285
0.347799956798553 0.585299730300903
0.359998911619186 0.534500658512115
0.369700729846954 0.46769991517067
0.378699988126755 0.402300328016281
0.389100313186646 0.339999347925186
0.397399812936783 0.285199999809265
0.406999975442886 0.24480003118515
0.417100578546524 0.213699832558632
0.424899905920029 0.190700352191925
0.433700054883957 0.167200058698654
0.443000108003616 0.146899819374084
0.450799703598022 0.129299908876419
0.459500044584274 0.111299984157085
0.469700008630753 0.0913998484611511
0.477299898862839 0.0769998878240585
0.486399948596954 0.0627000853419304
0.493600010871887 0.0509000346064568
0.500899374485016 0.042199932038784
0.5086989402771 0.0341000966727734
0.514900684356689 0.0276999995112419
0.521201074123383 0.0233000069856644
0.528599202632904 0.019799992442131
0.535100102424622 0.0170999355614185
0.542599380016327 0.015299997292459
0.551200151443481 0.0135999955236912
0.560100436210632 0.0121999932453036
0.567300856113434 0.0107999965548515
0.573199331760406 0.00960002280771732
0.580300867557526 0.00849997997283936
0.586700022220612 0.00769999856129289
0.59330290555954 0.00710000144317746
0.600299775600433 0.00609999289736152
0.60780143737793 0.00469999667257071
0.614900290966034 0.00430001458153129
0.622300505638123 0.00350000197067857
0.629299700260162 0.00330000161193311
0.636900246143341 0.00249999901279807
0.644099652767181 0.00180000357795507
0.65179967880249 0.0015000025741756
0.658100545406342 0.00129999872297049
0.665299296379089 0.000899998471140862
0.672097444534302 0.000800001143943518
0.679699778556824 0.000600000552367419
0.687402009963989 0.000399999669753015
0.693500876426697 0.000299999490380287
0.700300514698029 0.000199999834876508
0.706598579883575 9.99997646431439e-05
0.71310031414032 9.99997646431439e-05
0.719500958919525 0
0.725799918174744 0
0.731799721717834 0
0.737200558185577 0
0.743600249290466 0
0.748800456523895 0
0.755699098110199 0
0.76139909029007 0
0.769599437713623 0
0.777100324630737 0
0.783200204372406 0
0.789599895477295 0
0.797401666641235 0
0.804199159145355 0
0.811099827289581 0
0.818099617958069 0
0.823698997497559 0
0.829899787902832 0
0.835700392723083 0
0.841399788856506 0
0.848300099372864 0
0.85379958152771 0
0.858499825000763 0
0.863900005817413 0
0.869399607181549 0
0.874600172042847 0
0.880099833011627 0
0.885499596595764 0
0.891199827194214 0
0.895899534225464 0
0.902700185775757 0
0.90910017490387 0
0.914600014686584 0
0.918900012969971 0
0.925199389457703 0
0.930899798870087 0
0.936200082302094 0
0.942000269889832 0
0.946699976921082 0
0.952100217342377 0
0.957899987697601 0
0.962100207805634 0
0.967599987983704 0
0.973600089550018 0
0.978399991989136 0
0.983699917793274 0
0.989499986171722 0
0.995100021362305 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.989809453487396 0.670598983764648
0.990695595741272 0.65679919719696
0.991138696670532 0.627800941467285
0.991581737995148 0.585299730300903
0.992024838924408 0.534500658512115
0.992024838924408 0.46769991517067
0.992024838924408 0.402300328016281
0.992467880249023 0.339999347925186
0.992467880249023 0.285199999809265
0.992467880249023 0.24480003118515
0.992910921573639 0.213699832558632
0.992910921573639 0.190700352191925
0.992910921573639 0.167200058698654
0.992910921573639 0.146899819374084
0.992910921573639 0.129299908876419
0.992910921573639 0.111299984157085
0.993354022502899 0.0913998484611511
0.993354022502899 0.0769998878240585
0.993354022502899 0.0627000853419304
0.993354022502899 0.0509000346064568
0.993354022502899 0.042199932038784
0.993354022502899 0.0341000966727734
0.993354022502899 0.0276999995112419
0.993354022502899 0.0233000069856644
0.993354022502899 0.019799992442131
0.993354022502899 0.0170999355614185
0.993797063827515 0.015299997292459
0.993797063827515 0.0135999955236912
0.993797063827515 0.0121999932453036
0.993797063827515 0.0107999965548515
0.993797063827515 0.00960002280771732
0.993797063827515 0.00849997997283936
0.993797063827515 0.00769999856129289
0.993797063827515 0.00710000144317746
0.993797063827515 0.00609999289736152
0.993797063827515 0.00469999667257071
0.993797063827515 0.00430001458153129
0.993797063827515 0.00350000197067857
0.993797063827515 0.00330000161193311
0.994240164756775 0.00249999901279807
0.994240164756775 0.00180000357795507
0.994240164756775 0.0015000025741756
0.994240164756775 0.00129999872297049
0.99468320608139 0.000899998471140862
0.995126247406006 0.000800001143943518
0.995569348335266 0.000600000552367419
0.995569348335266 0.000399999669753015
0.995569348335266 0.000299999490380287
0.995569348335266 0.000199999834876508
0.995569348335266 9.99997646431439e-05
0.995569348335266 9.99997646431439e-05
0.995569348335266 0
0.995569348335266 0
0.996012389659882 0
0.996012389659882 0
0.996012389659882 0
0.996012389659882 0
0.996455490589142 0
0.996455490589142 0
0.996455490589142 0
0.996455490589142 0
0.996455490589142 0
0.996455490589142 0
0.996455490589142 0
0.996898531913757 0
0.996898531913757 0
0.996898531913757 0
0.996898531913757 0
0.997784674167633 0
0.997784674167633 0
0.997784674167633 0
0.998227715492249 0
0.998227715492249 0
0.998227715492249 0
0.998227715492249 0
0.998670816421509 0
0.998670816421509 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999113857746124 0
0.999556958675385 0
0.999556958675385 0
0.999556958675385 0
0.999556958675385 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.519631147384644 0.670598983764648
0.548114001750946 0.65679919719696
0.562740802764893 0.627800941467285
0.581986427307129 0.585299730300903
0.597383081912994 0.534500658512115
0.610469818115234 0.46769991517067
0.62047678232193 0.402300328016281
0.627406001091003 0.339999347925186
0.635873675346375 0.285199999809265
0.64665162563324 0.24480003118515
0.658198595046997 0.213699832558632
0.663587331771851 0.190700352191925
0.672825276851654 0.167200058698654
0.685142934322357 0.146899819374084
0.689761102199554 0.129299908876419
0.692840874195099 0.111299984157085
0.702078580856323 0.0913998484611511
0.709007263183594 0.0769998878240585
0.715934932231903 0.0627000853419304
0.72209370136261 0.0509000346064568
0.729792654514313 0.042199932038784
0.732101857662201 0.0341000966727734
0.735950589179993 0.0276999995112419
0.743649125099182 0.0233000069856644
0.746728301048279 0.019799992442131
0.751347124576569 0.0170999355614185
0.755966246128082 0.015299997292459
0.765203595161438 0.0135999955236912
0.772132575511932 0.0121999932453036
0.779060244560242 0.0107999965548515
0.783679962158203 0.00960002280771732
0.787528872489929 0.00849997997283936
0.791377902030945 0.00769999856129289
0.795227289199829 0.00710000144317746
0.802155435085297 0.00609999289736152
0.806774437427521 0.00469999667257071
0.81216299533844 0.00430001458153129
0.817551970481873 0.00350000197067857
0.823710381984711 0.00330000161193311
0.826789855957031 0.00249999901279807
0.829099595546722 0.00180000357795507
0.835258007049561 0.0015000025741756
0.836027503013611 0.00129999872297049
0.836797714233398 0.000899998471140862
0.83910721540451 0.000800001143943518
0.840646862983704 0.000600000552367419
0.844495594501495 0.000399999669753015
0.849114537239075 0.000299999490380287
0.852963447570801 0.000199999834876508
0.857582747936249 9.99997646431439e-05
0.859122395515442 9.99997646431439e-05
0.863741159439087 0
0.866820812225342 0
0.868360161781311 0
0.872209370136261 0
0.8760586977005 0
0.880677461624146 0
0.884526371955872 0
0.888375699520111 0
0.889145493507385 0
0.891455173492432 0
0.894534230232239 0
0.899153172969818 0
0.903771936893463 0
0.907621264457703 0
0.910700559616089 0
0.914549648761749 0
0.91762912273407 0
0.919168770313263 0
0.922247707843781 0
0.927636623382568 0
0.930715918540955 0
0.934565126895905 0
0.936104714870453 0
0.937644183635712 0
0.93841415643692 0
0.940723657608032 0
0.942263305187225 0
0.946112394332886 0
0.949191689491272 0
0.953810632228851 0
0.955350279808044 0
0.956120073795319 0
0.959199368953705 0
0.960739016532898 0
0.963818311691284 0
0.968437254428864 0
0.970746755599976 0
0.976905286312103 0
0.977675139904022 0
0.979214787483215 0
0.982294082641602 0
0.983063876628876 0
0.986913025379181 0
0.989992320537567 0
0.990762114524841 0
0.993841409683228 0
0.995381057262421 0
0.997690558433533 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0290192291140556 0.670598983764648
0.0485722683370113 0.65679919719696
0.0645562931895256 0.627800941467285
0.075108677148819 0.585299730300903
0.090782105922699 0.534500658512115
0.103196807205677 0.46769991517067
0.115146026015282 0.402300328016281
0.129733011126518 0.339999347925186
0.140906512737274 0.285199999809265
0.153631120920181 0.24480003118515
0.166822209954262 0.213699832558632
0.177840128540993 0.190700352191925
0.189633876085281 0.167200058698654
0.201582998037338 0.146899819374084
0.212756097316742 0.129299908876419
0.225636273622513 0.111299984157085
0.239447295665741 0.0913998484611511
0.249845400452614 0.0769998878240585
0.262569934129715 0.0627000853419304
0.272501349449158 0.0509000346064568
0.282277256250381 0.042199932038784
0.293917000293732 0.0341000966727734
0.302762567996979 0.0276999995112419
0.310986369848251 0.0233000069856644
0.321850001811981 0.019799992442131
0.33100625872612 0.0170999355614185
0.341558486223221 0.015299997292459
0.353041887283325 0.0135999955236912
0.365456312894821 0.0121999932453036
0.375232458114624 0.0107999965548515
0.383457243442535 0.00960002280771732
0.393699496984482 0.00849997997283936
0.40285524725914 0.00769999856129289
0.412321627140045 0.00710000144317746
0.421787798404694 0.00609999289736152
0.432495415210724 0.00469999667257071
0.442427039146423 0.00430001458153129
0.452824324369431 0.00350000197067857
0.462445765733719 0.00330000161193311
0.47346368432045 0.00249999901279807
0.484171330928802 0.00180000357795507
0.494878858327866 0.0015000025741756
0.504502236843109 0.00129999872297049
0.515363991260529 0.000899998471140862
0.525294065475464 0.000800001143943518
0.536622166633606 0.000600000552367419
0.547795653343201 0.000399999669753015
0.556331157684326 0.000299999490380287
0.566107630729675 0.000199999834876508
0.574953496456146 9.99997646431439e-05
0.584729373455048 9.99997646431439e-05
0.593731045722961 0
0.602888405323029 0
0.611732006072998 0
0.619336724281311 0
0.628491222858429 0
0.635630190372467 0
0.645407021045685 0
0.653475701808929 0
0.666046440601349 0
0.677219748497009 0
0.686064839363098 0
0.695065379142761 0
0.706237435340881 0
0.715859472751617 0
0.72594678401947 0
0.736032783985138 0
0.744102716445923 0
0.753103792667389 0
0.761483490467072 0
0.769243478775024 0
0.7791748046875 0
0.786933660507202 0
0.7939173579216 0
0.801986932754517 0
0.810210824012756 0
0.817814290523529 0
0.825884461402893 0
0.833488523960114 0
0.84171336889267 0
0.848075807094574 0
0.858317494392395 0
0.868094205856323 0
0.876007914543152 0
0.882371187210083 0
0.891527056694031 0
0.899441480636597 0
0.907200515270233 0
0.914959788322449 0
0.92209792137146 0
0.930167675018311 0
0.938547432422638 0
0.944909989833832 0
0.952669203281403 0
0.96120423078537 0
0.968497812747955 0
0.976101815700531 0
0.984792053699493 0
0.992861568927765 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/List_/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    % ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.353899627923965 0.52440071105957
0.405799329280853 0.33380001783371
0.449100196361542 0.193300172686577
0.491499990224838 0.109300024807453
0.530699551105499 0.059799998998642
0.570199072360992 0.0313999578356743
0.606299936771393 0.0153999999165535
0.641799747943878 0.00740000139921904
0.674399614334106 0.00369999930262566
0.70790034532547 0.00230000750161707
0.742899775505066 0.000399999669753015
0.77419912815094 9.99999174382538e-05
0.805300176143646 0
0.837300598621368 0
0.866200268268585 0
0.89459902048111 0
0.923799812793732 0
0.949299991130829 0
0.97460001707077 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.996434926986694 0.52440071105957
0.99688059091568 0.33380001783371
0.99688059091568 0.193300172686577
0.99688059091568 0.109300024807453
0.99688059091568 0.059799998998642
0.997771859169006 0.0313999578356743
0.997771859169006 0.0153999999165535
0.997771859169006 0.00740000139921904
0.997771859169006 0.00369999930262566
0.997771859169006 0.00230000750161707
0.998217463493347 0.000399999669753015
0.998217463493347 9.99999174382538e-05
0.998217463493347 0
0.998217463493347 0
0.998663127422333 0
0.999108731746674 0
0.999108731746674 0
0.999108731746674 0
0.999554395675659 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.749219417572021 0.52440071105957
0.79188334941864 0.33380001783371
0.818938732147217 0.193300172686577
0.843912601470947 0.109300024807453
0.861602663993835 0.059799998998642
0.878251850605011 0.0313999578356743
0.89594179391861 0.0153999999165535
0.908428728580475 0.00740000139921904
0.918834686279297 0.00369999930262566
0.928199768066406 0.00230000750161707
0.933402717113495 0.000399999669753015
0.938605606555939 9.99999174382538e-05
0.946930289268494 0
0.957336127758026 0
0.965660750865936 0
0.973985433578491 0
0.981269538402557 0
0.983350694179535 0
0.992715895175934 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0857985988259315 0.52440071105957
0.155996918678284 0.33380001783371
0.215894043445587 0.193300172686577
0.274760186672211 0.109300024807453
0.329948306083679 0.059799998998642
0.385430693626404 0.0313999578356743
0.436055988073349 0.0153999999165535
0.486534297466278 0.00740000139921904
0.533038675785065 0.00369999930262566
0.581016361713409 0.00230000750161707
0.631641209125519 0.000399999669753015
0.676967918872833 9.99999174382538e-05
0.721559822559357 0
0.767181873321533 0
0.808387994766235 0
0.848859369754791 0
0.890802204608917 0
0.92803543806076 0
0.96379691362381 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/List_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.263800621032715 0.675699234008789
0.287500590085983 0.675600171089172
0.305900990962982 0.675399363040924
0.322099983692169 0.672300636768341
0.337799787521362 0.663300633430481
0.350800007581711 0.6409991979599
0.363499671220779 0.605498850345612
0.376099556684494 0.54459947347641
0.386900037527084 0.466499805450439
0.398800224065781 0.37070044875145
0.408499866724014 0.276000291109085
0.418300092220306 0.190800100564957
0.428800255060196 0.123200014233589
0.438600301742554 0.0723001733422279
0.44789981842041 0.0404999926686287
0.458299815654755 0.020399970933795
0.466700196266174 0.010500006377697
0.47530010342598 0.00520001025870442
0.484800010919571 0.00199999962933362
0.49219998717308 0.000599998980760574
0.499697417020798 0.000199999834876508
0.507900476455688 9.99997646431439e-05
0.514701724052429 9.99997646431439e-05
0.521998107433319 0
0.529497742652893 0
0.536701381206512 0
0.544000446796417 0
0.552599847316742 0
0.561101257801056 0
0.567701041698456 0
0.575800836086273 0
0.582401096820831 0
0.590899050235748 0
0.597699880599976 0
0.604100406169891 0
0.611199975013733 0
0.618301272392273 0
0.625101029872894 0
0.632599830627441 0
0.639901101589203 0
0.646800518035889 0
0.653899490833282 0
0.660200893878937 0
0.66810005903244 0
0.675800025463104 0
0.681600153446198 0
0.688400983810425 0
0.695599138736725 0
0.702798843383789 0
0.710000395774841 0
0.716399610042572 0
0.723199546337128 0
0.728400826454163 0
0.734799981117249 0
0.741400897502899 0
0.747999727725983 0
0.753899216651917 0
0.760801315307617 0
0.767600059509277 0
0.775399565696716 0
0.782000005245209 0
0.787398993968964 0
0.795200169086456 0
0.800999999046326 0
0.80670040845871 0
0.814799666404724 0
0.821300804615021 0
0.827300608158112 0
0.833499610424042 0
0.83930104970932 0
0.845400214195251 0
0.851199686527252 0
0.855900287628174 0
0.861199975013733 0
0.867399990558624 0
0.872699439525604 0
0.877300322055817 0
0.883399605751038 0
0.889599919319153 0
0.895699977874756 0
0.900399684906006 0
0.906499624252319 0
0.912700176239014 0
0.918700397014618 0
0.92330002784729 0
0.929199635982513 0
0.934699833393097 0
0.940599918365479 0
0.946199834346771 0
0.952300190925598 0
0.957499980926514 0
0.962499976158142 0
0.966299593448639 0
0.972000002861023 0
0.976499974727631 0
0.981500029563904 0
0.986400008201599 0
0.990700006484985 0
0.995400011539459 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.968982100486755 0.675699234008789
0.977282643318176 0.675600171089172
0.980340778827667 0.675399363040924
0.982962012290955 0.672300636768341
0.987767577171326 0.663300633430481
0.988641321659088 0.6409991979599
0.989078223705292 0.605498850345612
0.989951968193054 0.54459947347641
0.990388810634613 0.466499805450439
0.990388810634613 0.37070044875145
0.991262555122375 0.276000291109085
0.991699457168579 0.190800100564957
0.991699457168579 0.123200014233589
0.991699457168579 0.0723001733422279
0.991699457168579 0.0404999926686287
0.991699457168579 0.020399970933795
0.992136299610138 0.010500006377697
0.992573201656342 0.00520001025870442
0.992573201656342 0.00199999962933362
0.9930100440979 0.000599998980760574
0.9930100440979 0.000199999834876508
0.9930100440979 9.99997646431439e-05
0.993446946144104 9.99997646431439e-05
0.993446946144104 0
0.993446946144104 0
0.993446946144104 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.993883788585663 0
0.994320690631866 0
0.994320690631866 0
0.994320690631866 0
0.994320690631866 0
0.994757533073425 0
0.995194435119629 0
0.995631277561188 0
0.995631277561188 0
0.995631277561188 0
0.995631277561188 0
0.995631277561188 0
0.995631277561188 0
0.995631277561188 0
0.995631277561188 0
0.996068179607391 0
0.996068179607391 0
0.996068179607391 0
0.996068179607391 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.99650502204895 0
0.997378766536713 0
0.997378766536713 0
0.997378766536713 0
0.997815668582916 0
0.997815668582916 0
0.997815668582916 0
0.997815668582916 0
0.998252511024475 0
0.998252511024475 0
0.998689413070679 0
0.998689413070679 0
0.998689413070679 0
0.998689413070679 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999126255512238 0
0.999563157558441 0
0.999563157558441 0
0.999563157558441 0
0.999563157558441 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.234701782464981 0.675699234008789
0.325329065322876 0.675600171089172
0.397366285324097 0.675399363040924
0.437645196914673 0.672300636768341
0.477149486541748 0.663300633430481
0.511232316493988 0.6409991979599
0.536018133163452 0.605498850345612
0.567777276039124 0.54459947347641
0.584043323993683 0.466499805450439
0.601083755493164 0.37070044875145
0.615027129650116 0.276000291109085
0.627420425415039 0.190800100564957
0.639040112495422 0.123200014233589
0.651433348655701 0.0723001733422279
0.657629787921906 0.0404999926686287
0.664601027965546 0.020399970933795
0.675445318222046 0.010500006377697
0.683191061019897 0.00520001025870442
0.688612997531891 0.00199999962933362
0.698683142662048 0.000599998980760574
0.70565402507782 0.000199999834876508
0.710302114486694 9.99997646431439e-05
0.713400602340698 9.99997646431439e-05
0.721921324729919 0
0.7281174659729 0
0.732765138149261 0
0.738187253475189 0
0.745933055877686 0
0.750580847263336 0
0.756777584552765 0
0.762974500656128 0
0.766072750091553 0
0.771495282649994 0
0.776917099952698 0
0.784663259983063 0
0.790859878063202 0
0.797830939292908 0
0.804027915000916 0
0.812548696994781 0
0.816421270370483 0
0.821069300174713 0
0.824941694736481 0
0.826490879058838 0
0.82804000377655 0
0.829589247703552 0
0.830363869667053 0
0.834237396717072 0
0.838884592056274 0
0.841208338737488 0
0.84663051366806 0
0.849728882312775 0
0.854376375675201 0
0.858249604701996 0
0.861347615718842 0
0.86444616317749 0
0.867544531822205 0
0.872966706752777 0
0.875290632247925 0
0.879163444042206 0
0.883811116218567 0
0.886134684085846 0
0.889232993125916 0
0.895429790019989 0
0.896979093551636 0
0.901626646518707 0
0.907048881053925 0
0.911696374416351 0
0.914794743061066 0
0.916343927383423 0
0.918667793273926 0
0.921766102313995 0
0.925639033317566 0
0.927962839603424 0
0.92873740196228 0
0.931835770606995 0
0.934159576892853 0
0.935708820819855 0
0.938032627105713 0
0.938807129859924 0
0.941905498504639 0
0.945003867149353 0
0.947327673435211 0
0.949651420116425 0
0.95352441072464 0
0.958171963691711 0
0.962044954299927 0
0.966692507266998 0
0.972114622592926 0
0.976762175559998 0
0.979860544204712 0
0.98218435049057 0
0.984508156776428 0
0.985282719135284 0
0.9891557097435 0
0.991479456424713 0
0.991479456424713 0
0.994577825069427 0
0.997676193714142 0
0.998450815677643 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0182243064045906 0.675699234008789
0.033956415951252 0.675600171089172
0.047040518373251 0.675399363040924
0.0632398575544357 0.672300636768341
0.078037291765213 0.663300633430481
0.0911214649677277 0.6409991979599
0.105763211846352 0.605498850345612
0.118691608309746 0.54459947347641
0.132087022066116 0.466499805450439
0.147196158766747 0.37070044875145
0.15919004380703 0.276000291109085
0.171806961297989 0.190800100564957
0.185825347900391 0.123200014233589
0.198598131537437 0.0723001733422279
0.21183805167675 0.0404999926686287
0.226635470986366 0.020399970933795
0.237383171916008 0.010500006377697
0.249065652489662 0.00520001025870442
0.262772083282471 0.00199999962933362
0.272118449211121 0.000599998980760574
0.282398670911789 0.000199999834876508
0.294237017631531 9.99997646431439e-05
0.304049700498581 9.99997646431439e-05
0.313707649707794 0
0.32414323091507 0
0.334423512220383 0
0.344547986984253 0
0.356386661529541 0
0.368691504001617 0
0.377725929021835 0
0.389096736907959 0
0.398753970861435 0
0.410903036594391 0
0.420404762029648 0
0.428816199302673 0
0.438629060983658 0
0.448286443948746 0
0.45763236284256 0
0.467601209878922 0
0.478037387132645 0
0.487850457429886 0
0.498131096363068 0
0.507632553577423 0
0.519470274448395 0
0.530996561050415 0
0.539719521999359 0
0.549531936645508 0
0.559813022613525 0
0.570559859275818 0
0.580686688423157 0
0.590031027793884 0
0.599688231945038 0
0.607008814811707 0
0.616198897361755 0
0.625856518745422 0
0.635513007640839 0
0.643613755702972 0
0.653739631175995 0
0.663550972938538 0
0.674766600131989 0
0.684578120708466 0
0.692366659641266 0
0.703271150588989 0
0.711993873119354 0
0.719938457012177 0
0.731463968753815 0
0.740653455257416 0
0.749376356601715 0
0.758410811424255 0
0.766977608203888 0
0.775857150554657 0
0.78395676612854 0
0.790809750556946 0
0.798909783363342 0
0.807943642139435 0
0.815576255321503 0
0.822429478168488 0
0.831308722496033 0
0.840809047222137 0
0.849689364433289 0
0.856386363506317 0
0.865264713764191 0
0.874454617500305 0
0.883021652698517 0
0.889252364635468 0
0.897663414478302 0
0.905295312404633 0
0.913395881652832 0
0.92118364572525 0
0.930062174797058 0
0.937694728374481 0
0.945015549659729 0
0.950778901576996 0
0.958878517150879 0
0.965264797210693 0
0.973052978515625 0
0.980062305927277 0
0.986137092113495 0
0.993146419525146 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/List_target/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    % ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.327600747346878 0.599800229072571
0.389499932527542 0.421099692583084
0.441000044345856 0.229499995708466
0.484800010919571 0.0947997942566872
0.526901245117188 0.0289000179618597
0.5647993683815 0.00669999839738011
0.603299796581268 0.00140000157989562
0.640698611736298 0.000199999834876508
0.675198137760162 0
0.708999156951904 0
0.740399539470673 0
0.774199366569519 0
0.804700970649719 0
0.835500299930573 0
0.867300093173981 0
0.896399974822998 0
0.925000011920929 0
0.950600206851959 0
0.977199971675873 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.992003560066223 0.599800229072571
0.995557546615601 0.421099692583084
0.996446013450623 0.229499995708466
0.996446013450623 0.0947997942566872
0.996446013450623 0.0289000179618597
0.996890246868134 0.00669999839738011
0.996890246868134 0.00140000157989562
0.997334539890289 0.000199999834876508
0.9977787733078 0
0.9977787733078 0
0.998223006725311 0
0.998223006725311 0
0.998223006725311 0
0.998223006725311 0
0.998667240142822 0
0.998667240142822 0
0.998667240142822 0
0.999111533164978 0
0.999555766582489 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.562105417251587 0.599800229072571
0.728421330451965 0.421099692583084
0.808421313762665 0.229499995708466
0.846315801143646 0.0947997942566872
0.872631430625916 0.0289000179618597
0.884210407733917 0.00669999839738011
0.90105265378952 0.00140000157989562
0.909473657608032 0.000199999834876508
0.918947458267212 0
0.92736828327179 0
0.929473578929901 0
0.936842083930969 0
0.945263147354126 0
0.956842124462128 0
0.967368423938751 0
0.976842105388641 0
0.985263168811798 0
0.986315786838531 0
0.994736850261688 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0748637691140175 0.599800229072571
0.141491174697876 0.421099692583084
0.205765590071678 0.229499995708466
0.264891773462296 0.0947997942566872
0.323135226964951 0.0289000179618597
0.37711438536644 0.00669999839738011
0.431387156248093 0.00140000157989562
0.485071271657944 0.000199999834876508
0.534343898296356 0
0.582879066467285 0
0.628621995449066 0
0.677305459976196 0
0.720989227294922 0
0.764671683311462 0
0.809824824333191 0
0.851300895214081 0
0.892189621925354 0
0.929548442363739 0
0.967348158359528 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/Markov/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.384699642658234 0.669499635696411
0.404100209474564 0.634200692176819
0.420100182294846 0.546099781990051
0.433799892663956 0.425200134515762
0.447400063276291 0.286700040102005
0.458999812602997 0.164900422096252
0.470200151205063 0.0837999731302261
0.480399936437607 0.0384998992085457
0.490500062704086 0.0155000071972609
0.502201437950134 0.0054999990388751
0.51110315322876 0.00190000096336007
0.521200239658356 0.000499997695442289
0.529898226261139 0.000299999344861135
0.538099706172943 9.99997646431439e-05
0.54619950056076 0
0.555499315261841 0
0.565501153469086 0
0.572299480438232 0
0.580499351024628 0
0.587298989295959 0
0.59429919719696 0
0.601700365543365 0
0.609999477863312 0
0.616299033164978 0
0.623699724674225 0
0.629798948764801 0
0.635300099849701 0
0.643800616264343 0
0.651000022888184 0
0.657301187515259 0
0.663999736309052 0
0.670798897743225 0
0.678801417350769 0
0.684700608253479 0
0.691700875759125 0
0.697200775146484 0
0.703601002693176 0
0.70989990234375 0
0.715399384498596 0
0.722400069236755 0
0.728699326515198 0
0.736701190471649 0
0.743499875068665 0
0.749100506305695 0
0.754600465297699 0
0.761501491069794 0
0.76669979095459 0
0.773000717163086 0
0.778100073337555 0
0.783498883247375 0
0.788898944854736 0
0.794099152088165 0
0.799000084400177 0
0.803500711917877 0
0.809101045131683 0
0.814199209213257 0
0.819000959396362 0
0.82329922914505 0
0.828499436378479 0
0.834000766277313 0
0.838799595832825 0
0.843100309371948 0
0.848000168800354 0
0.853100121021271 0
0.858199715614319 0
0.863699793815613 0
0.869599580764771 0
0.874599993228912 0
0.879900574684143 0
0.883499979972839 0
0.887399971485138 0
0.89130038022995 0
0.89520001411438 0
0.898800194263458 0
0.904399991035461 0
0.909300208091736 0
0.913500010967255 0
0.91729998588562 0
0.921000182628632 0
0.92490017414093 0
0.929299831390381 0
0.934699833393097 0
0.938700020313263 0
0.941399991512299 0
0.945300102233887 0
0.949599921703339 0
0.953400015830994 0
0.95740020275116 0
0.9617999792099 0
0.96560001373291 0
0.969299793243408 0
0.973100185394287 0
0.975899994373322 0
0.979900121688843 0
0.982800185680389 0
0.986199975013733 0
0.989700019359589 0
0.99370002746582 0
0.996800005435944 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.988505721092224 0.669499635696411
0.989389896392822 0.634200692176819
0.99027407169342 0.546099781990051
0.99027407169342 0.425200134515762
0.990716159343719 0.286700040102005
0.990716159343719 0.164900422096252
0.990716159343719 0.0837999731302261
0.991158246994019 0.0384998992085457
0.991158246994019 0.0155000071972609
0.991158246994019 0.0054999990388751
0.991158246994019 0.00190000096336007
0.991158246994019 0.000499997695442289
0.991158246994019 0.000299999344861135
0.991158246994019 9.99997646431439e-05
0.991158246994019 0
0.991158246994019 0
0.992042422294617 0
0.992484509944916 0
0.992484509944916 0
0.992926597595215 0
0.992926597595215 0
0.992926597595215 0
0.992926597595215 0
0.992926597595215 0
0.992926597595215 0
0.992926597595215 0
0.992926597595215 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993368685245514 0
0.993810772895813 0
0.993810772895813 0
0.993810772895813 0
0.993810772895813 0
0.994252860546112 0
0.994694948196411 0
0.99513703584671 0
0.99513703584671 0
0.99513703584671 0
0.99513703584671 0
0.99513703584671 0
0.99513703584671 0
0.99513703584671 0
0.99513703584671 0
0.995579123497009 0
0.996021211147308 0
0.996021211147308 0
0.996021211147308 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.996463298797607 0
0.997347474098206 0
0.997347474098206 0
0.997347474098206 0
0.997789561748505 0
0.997789561748505 0
0.997789561748505 0
0.997789561748505 0
0.998673737049103 0
0.998673737049103 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999115824699402 0
0.999557912349701 0
0.999557912349701 0
0.999557912349701 0
0.999557912349701 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.519637644290924 0.669499635696411
0.552115380764008 0.634200692176819
0.572507679462433 0.546099781990051
0.589124083518982 0.425200134515762
0.601963400840759 0.286700040102005
0.618580043315887 0.164900422096252
0.632930397987366 0.0837999731302261
0.639728128910065 0.0384998992085457
0.645014822483063 0.0155000071972609
0.655588984489441 0.0054999990388751
0.66314172744751 0.00190000096336007
0.670694708824158 0.000499997695442289
0.680513620376587 0.000299999344861135
0.693353652954102 9.99997646431439e-05
0.69788521528244 0
0.701661467552185 0
0.709214568138123 0
0.714501619338989 0
0.723564982414246 0
0.728096425533295 0
0.732628047466278 0
0.737915933132172 0
0.742447435855865 0
0.747733950614929 0
0.752265512943268 0
0.75906366109848 0
0.762840449810028 0
0.770392417907715 0
0.77492493391037 0
0.78172242641449 0
0.784743547439575 0
0.790785491466522 0
0.793807208538055 0
0.799848675727844 0
0.805136144161224 0
0.808912456035614 0
0.814199566841125 0
0.820241510868073 0
0.825528979301453 0
0.828550219535828 0
0.830816149711609 0
0.835347056388855 0
0.838368773460388 0
0.842145204544067 0
0.844411075115204 0
0.846676766872406 0
0.848942756652832 0
0.851963996887207 0
0.857250571250916 0
0.863292694091797 0
0.865558743476868 0
0.870846092700958 0
0.874622285366058 0
0.876132726669312 0
0.878398597240448 0
0.880664825439453 0
0.88368558883667 0
0.886707127094269 0
0.891238510608673 0
0.89274924993515 0
0.895014941692352 0
0.896525681018829 0
0.901057243347168 0
0.903323471546173 0
0.906344413757324 0
0.910876393318176 0
0.916163325309753 0
0.91918420791626 0
0.920694708824158 0
0.924471318721771 0
0.929758429527283 0
0.932779431343079 0
0.935045301914215 0
0.935800611972809 0
0.93806654214859 0
0.940332114696503 0
0.944108843803406 0
0.945619344711304 0
0.947885096073151 0
0.949395775794983 0
0.951661646366119 0
0.953172206878662 0
0.956193327903748 0
0.958459198474884 0
0.961480379104614 0
0.9645015001297 0
0.96752268075943 0
0.972054362297058 0
0.976586103439331 0
0.977341413497925 0
0.98036253452301 0
0.981117844581604 0
0.982628405094147 0
0.987915396690369 0
0.990936577320099 0
0.991691827774048 0
0.993957698345184 0
0.996223568916321 0
0.998489439487457 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0512940473854542 0.669499635696411
0.0795134529471397 0.634200692176819
0.101808585226536 0.546099781990051
0.124415144324303 0.425200134515762
0.145463317632675 0.286700040102005
0.162301391363144 0.164900422096252
0.178827747702599 0.0837999731302261
0.19426266849041 0.0384998992085457
0.210788905620575 0.0155000071972609
0.228250667452812 0.0054999990388751
0.241971030831337 0.00190000096336007
0.257249772548676 0.000499997695442289
0.270345419645309 0.000299999344861135
0.282973766326904 9.99997646431439e-05
0.297007143497467 0
0.312285482883453 0
0.328187793493271 0
0.338478475809097 0
0.351886719465256 0
0.363423615694046 0
0.375272810459137 0
0.387433439493179 0
0.400997847318649 0
0.411443799734116 0
0.42391636967659 0
0.433582752943039 0
0.442625433206558 0
0.453850954771042 0
0.465232461690903 0
0.47458690404892 0
0.486435920000076 0
0.496725678443909 0
0.50997793674469 0
0.519643545150757 0
0.532583117485046 0
0.54131543636322 0
0.55144989490509 0
0.560961186885834 0
0.568755507469177 0
0.580759942531586 0
0.590896248817444 0
0.602117896080017 0
0.613502383232117 0
0.621296942234039 0
0.629872381687164 0
0.641565501689911 0
0.650609195232391 0
0.661055028438568 0
0.668538331985474 0
0.675865292549133 0
0.684440970420837 0
0.692547857761383 0
0.701278388500214 0
0.707982540130615 0
0.71655797958374 0
0.724976480007172 0
0.731991469860077 0
0.738541126251221 0
0.746335864067078 0
0.756470859050751 0
0.763953685760498 0
0.770970046520233 0
0.778608858585358 0
0.786248683929443 0
0.794668078422546 0
0.802619278430939 0
0.811038076877594 0
0.818210303783417 0
0.826161801815033 0
0.83146196603775 0
0.83645087480545 0
0.842064261436462 0
0.848144292831421 0
0.853445589542389 0
0.861864805221558 0
0.868724822998047 0
0.874961197376251 0
0.880729496479034 0
0.886186718940735 0
0.892267048358917 0
0.898659348487854 0
0.907078206539154 0
0.912847340106964 0
0.916588544845581 0
0.922201335430145 0
0.928593873977661 0
0.933894634246826 0
0.939039587974548 0
0.945120215415955 0
0.950888693332672 0
0.956345617771149 0
0.962426006793976 0
0.966479599475861 0
0.971624553203583 0
0.975210547447205 0
0.980355501174927 0
0.985344529151917 0
0.991113185882568 0
0.995322704315186 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/Markov/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.440099596977234 0.387699753046036
0.49670073390007 0.132599845528603
0.539099395275116 0.0319000445306301
0.582000970840454 0.00509999832138419
0.622799873352051 0.000399999058572575
0.656901776790619 0.000199999529286288
0.690901637077332 0
0.723300278186798 0
0.749500572681427 0
0.776398897171021 0
0.803499579429626 0
0.829300105571747 0
0.85619980096817 0
0.881600201129913 0
0.904000282287598 0
0.926600217819214 0
0.94780021905899 0
0.966000199317932 0
0.985300004482269 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.996877789497375 0.387699753046036
0.997769832611084 0.132599845528603
0.997769832611084 0.0319000445306301
0.997769832611084 0.00509999832138419
0.997769832611084 0.000399999058572575
0.998215854167938 0.000199999529286288
0.998215854167938 0
0.998215854167938 0
0.998215854167938 0
0.998215854167938 0
0.998661935329437 0
0.998661935329437 0
0.998661935329437 0
0.998661935329437 0
0.999107956886292 0
0.999107956886292 0
0.999107956886292 0
0.999107956886292 0
0.999553978443146 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.761706531047821 0.387699753046036
0.805411040782928 0.132599845528603
0.827263534069061 0.0319000445306301
0.855359137058258 0.00509999832138419
0.870967626571655 0.000399999058572575
0.886576473712921 0.000199999529286288
0.901144683361053 0
0.911550402641296 0
0.920915722846985 0
0.931321561336517 0
0.935483872890472 0
0.940686762332916 0
0.947970807552338 0
0.959417283535004 0
0.967741906642914 0
0.976066589355469 0
0.982310116291046 0
0.984391272068024 0
0.990634739398956 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.133000209927559 0.387699753046036
0.221715405583382 0.132599845528603
0.292776882648468 0.0319000445306301
0.361335635185242 0.00509999832138419
0.425481766462326 0.000399999058572575
0.481830209493637 0.000199999529286288
0.535971283912659 0
0.586877584457397 0
0.628071308135986 0
0.669855058193207 0
0.711343467235565 0
0.751360476016998 0
0.792260527610779 0
0.829336643218994 0
0.861850678920746 0
0.894365012645721 0
0.925408124923706 0
0.952037751674652 0
0.979843974113464 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/Markov_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.311099618673325 0.624300181865692
0.329000145196915 0.586199462413788
0.342899948358536 0.541900992393494
0.353700160980225 0.477400004863739
0.36620032787323 0.399699479341507
0.377099573612213 0.321400254964828
0.389200061559677 0.252099871635437
0.398299962282181 0.195500165224075
0.409100234508514 0.157800063490868
0.418200194835663 0.129600495100021
0.427900284528732 0.104499898850918
0.436300009489059 0.0842999964952469
0.445300400257111 0.0654998868703842
0.455200254917145 0.0489000082015991
0.46329990029335 0.036800105124712
0.471000134944916 0.0249999836087227
0.480199962854385 0.0187000297009945
0.48649999499321 0.0136000048369169
0.496200621128082 0.010900005698204
0.50370067358017 0.00849997997283936
0.510799944400787 0.00700000440701842
0.517700731754303 0.006100008264184
0.5253005027771 0.00440000696107745
0.530499637126923 0.00360000086948276
0.539400160312653 0.00310000427998602
0.547098278999329 0.00259999558329582
0.555199146270752 0.00189999956637621
0.563601493835449 0.00119999598246068
0.571401417255402 0.00099999934900552
0.578198254108429 0.000399999669753015
0.583700895309448 0.000199999834876508
0.590598821640015 9.99999174382538e-05
0.597599148750305 9.99999174382538e-05
0.604399740695953 0
0.6118004322052 0
0.618500232696533 0
0.625000953674316 0
0.631199836730957 0
0.636699974536896 0
0.643099308013916 0
0.650701344013214 0
0.657400071620941 0
0.66449910402298 0
0.671100556850433 0
0.67799985408783 0
0.685500264167786 0
0.693399965763092 0
0.699399828910828 0
0.70499849319458 0
0.712099492549896 0
0.718100309371948 0
0.724299311637878 0
0.730300605297089 0
0.735499620437622 0
0.74090051651001 0
0.747198760509491 0
0.752799987792969 0
0.759498834609985 0
0.76519912481308 0
0.772900760173798 0
0.779499769210815 0
0.784799814224243 0
0.792400658130646 0
0.799501180648804 0
0.804999887943268 0
0.811900615692139 0
0.819200396537781 0
0.825299322605133 0
0.832099199295044 0
0.836800217628479 0
0.84279990196228 0
0.848899900913239 0
0.854101359844208 0
0.859599828720093 0
0.865600287914276 0
0.871900379657745 0
0.877299189567566 0
0.88250058889389 0
0.888000190258026 0
0.893299400806427 0
0.897200584411621 0
0.903700113296509 0
0.910700082778931 0
0.916099786758423 0
0.921999990940094 0
0.927899897098541 0
0.933200001716614 0
0.938199818134308 0
0.943999826908112 0
0.949299991130829 0
0.954299926757812 0
0.958899974822998 0
0.963900029659271 0
0.969200015068054 0
0.97460001707077 0
0.980199992656708 0
0.984799981117249 0
0.990499973297119 0
0.995599985122681 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.991130828857422 0.624300181865692
0.991574287414551 0.586199462413788
0.992461204528809 0.541900992393494
0.992461204528809 0.477400004863739
0.992461204528809 0.399699479341507
0.992461204528809 0.321400254964828
0.992461204528809 0.252099871635437
0.992904663085938 0.195500165224075
0.992904663085938 0.157800063490868
0.992904663085938 0.129600495100021
0.992904663085938 0.104499898850918
0.992904663085938 0.0842999964952469
0.992904663085938 0.0654998868703842
0.992904663085938 0.0489000082015991
0.992904663085938 0.036800105124712
0.992904663085938 0.0249999836087227
0.993348121643066 0.0187000297009945
0.993348121643066 0.0136000048369169
0.993348121643066 0.010900005698204
0.993791580200195 0.00849997997283936
0.993791580200195 0.00700000440701842
0.993791580200195 0.006100008264184
0.993791580200195 0.00440000696107745
0.993791580200195 0.00360000086948276
0.993791580200195 0.00310000427998602
0.993791580200195 0.00259999558329582
0.993791580200195 0.00189999956637621
0.993791580200195 0.00119999598246068
0.993791580200195 0.00099999934900552
0.993791580200195 0.000399999669753015
0.993791580200195 0.000199999834876508
0.993791580200195 9.99999174382538e-05
0.993791580200195 9.99999174382538e-05
0.993791580200195 0
0.993791580200195 0
0.993791580200195 0
0.993791580200195 0
0.993791580200195 0
0.993791580200195 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994678497314453 0
0.995121955871582 0
0.995565414428711 0
0.995565414428711 0
0.995565414428711 0
0.995565414428711 0
0.995565414428711 0
0.995565414428711 0
0.995565414428711 0
0.995565414428711 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.997339248657227 0
0.997339248657227 0
0.997339248657227 0
0.997782707214355 0
0.997782707214355 0
0.998226165771484 0
0.998226165771484 0
0.998669624328613 0
0.998669624328613 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999556541442871 0
0.999556541442871 0
0.999556541442871 0
0.999556541442871 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.517215013504028 0.624300181865692
0.551645219326019 0.586199462413788
0.575363278388977 0.541900992393494
0.591430604457855 0.477400004863739
0.601377308368683 0.399699479341507
0.613619446754456 0.321400254964828
0.628156006336212 0.252099871635437
0.636572301387787 0.195500165224075
0.649578928947449 0.157800063490868
0.657995522022247 0.129600495100021
0.664881885051727 0.104499898850918
0.670237481594086 0.0842999964952469
0.678652763366699 0.0654998868703842
0.689365029335022 0.0489000082015991
0.692425429821014 0.036800105124712
0.697016179561615 0.0249999836087227
0.703902244567871 0.0187000297009945
0.710788369178772 0.0136000048369169
0.720734536647797 0.010900005698204
0.724559724330902 0.00849997997283936
0.729150533676147 0.00700000440701842
0.73221081495285 0.006100008264184
0.736801743507385 0.00440000696107745
0.742158114910126 0.00360000086948276
0.746748089790344 0.00310000427998602
0.75133866071701 0.00259999558329582
0.753634393215179 0.00189999956637621
0.760520219802856 0.00119999598246068
0.765876054763794 0.00099999934900552
0.774292171001434 0.000399999669753015
0.77735310792923 0.000199999834876508
0.783473968505859 9.99999174382538e-05
0.788064241409302 9.99999174382538e-05
0.79341983795166 0
0.797245800495148 0
0.801836669445038 0
0.804896831512451 0
0.81254780292511 0
0.818668305873871 0
0.820199310779572 0
0.827084898948669 0
0.830910563468933 0
0.83320564031601 0
0.834736049175262 0
0.836266100406647 0
0.842387318611145 0
0.845447599887848 0
0.846977829933167 0
0.848507642745972 0
0.853098690509796 0
0.856159150600433 0
0.861514627933502 0
0.865340292453766 0
0.869166195392609 0
0.871461570262909 0
0.875286996364594 0
0.878346979618073 0
0.885233521461487 0
0.888293623924255 0
0.890589118003845 0
0.892119348049164 0
0.894414484500885 0
0.900535583496094 0
0.903595805168152 0
0.908186674118042 0
0.910481810569763 0
0.912777245044708 0
0.915072619915009 0
0.917367994785309 0
0.919663369655609 0
0.921958804130554 0
0.924253821372986 0
0.928079545497894 0
0.931905150413513 0
0.93649560213089 0
0.937260985374451 0
0.939556241035461 0
0.941851556301117 0
0.944146871566772 0
0.944912016391754 0
0.94720733165741 0
0.950267791748047 0
0.951797902584076 0
0.954858481884003 0
0.957918882369995 0
0.961744427680969 0
0.964804887771606 0
0.967865347862244 0
0.975516438484192 0
0.976281583309174 0
0.97704666852951 0
0.977811753749847 0
0.978576898574829 0
0.983932673931122 0
0.986993134021759 0
0.987758219242096 0
0.990818679332733 0
0.994644224643707 0
0.996939539909363 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0310655366629362 0.624300181865692
0.0517241396009922 0.586199462413788
0.06818887591362 0.541900992393494
0.0817023664712906 0.477400004863739
0.0990991741418839 0.399699479341507
0.113544598221779 0.321400254964828
0.129388123750687 0.252099871635437
0.141658902168274 0.195500165224075
0.15579380095005 0.157800063490868
0.168219715356827 0.129600495100021
0.181888476014137 0.104499898850918
0.193848997354507 0.0842999964952469
0.206119909882545 0.0654998868703842
0.219322919845581 0.0489000082015991
0.231283009052277 0.036800105124712
0.242311581969261 0.0249999836087227
0.255047291517258 0.0187000297009945
0.263435840606689 0.0136000048369169
0.27648201584816 0.010900005698204
0.287200719118118 0.00849997997283936
0.297297775745392 0.00700000440701842
0.307394176721573 0.006100008264184
0.318266481161118 0.00440000696107745
0.325255960226059 0.00360000086948276
0.338148534297943 0.00310000427998602
0.349176913499832 0.00259999558329582
0.361292541027069 0.00189999956637621
0.372941970825195 0.00119999598246068
0.383970201015472 0.00099999934900552
0.392823785543442 0.000399999669753015
0.400745391845703 0.000199999834876508
0.41022065281868 9.99999174382538e-05
0.420161306858063 9.99999174382538e-05
0.42963644862175 0
0.440354228019714 0
0.449829071760178 0
0.459304094314575 0
0.467381209135056 0
0.474681615829468 0
0.484156578779221 0
0.494563162326813 0
0.504194617271423 0
0.514756917953491 0
0.524542033672333 0
0.534793317317963 0
0.545044422149658 0
0.556695520877838 0
0.565706074237823 0
0.574088990688324 0
0.584187388420105 0
0.592886686325073 0
0.601430356502533 0
0.609973132610321 0
0.617118000984192 0
0.625038683414459 0
0.634049236774445 0
0.642123699188232 0
0.650979161262512 0
0.659209847450256 0
0.67070460319519 0
0.680645704269409 0
0.688412427902222 0
0.698974668979645 0
0.709380030632019 0
0.716992616653442 0
0.727244257926941 0
0.738117933273315 0
0.747125685214996 0
0.756912231445312 0
0.763745307922363 0
0.772600173950195 0
0.781454265117645 0
0.788754105567932 0
0.796365201473236 0
0.804753184318542 0
0.814228653907776 0
0.822150588035583 0
0.82960569858551 0
0.837682485580444 0
0.845759391784668 0
0.85135143995285 0
0.860826373100281 0
0.871388554573059 0
0.879155337810516 0
0.887698471546173 0
0.896085917949677 0
0.90369713306427 0
0.910841703414917 0
0.91829788684845 0
0.926374495029449 0
0.933985531330109 0
0.940975487232208 0
0.948586523532867 0
0.955731749534607 0
0.963342666625977 0
0.971885681152344 0
0.978409469127655 0
0.986486494541168 0
0.993786871433258 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/Markov_/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.357599914073944 0.449300110340118
0.40699976682663 0.250500380992889
0.452200084924698 0.117199949920177
0.494200199842453 0.0516000352799892
0.532701134681702 0.0187000092118979
0.571800410747528 0.00630000419914722
0.605800330638885 0.00179999426472932
0.640000104904175 0.000800000212620944
0.67589807510376 0.000299999490380287
0.70710027217865 0
0.740799188613892 0
0.772600173950195 0
0.801699817180634 0
0.833700954914093 0
0.864599883556366 0
0.89260059595108 0
0.920999586582184 0
0.948300123214722 0
0.974900007247925 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.997768878936768 0.449300110340118
0.997768878936768 0.250500380992889
0.997768878936768 0.117199949920177
0.997768878936768 0.0516000352799892
0.997768878936768 0.0187000092118979
0.998215079307556 0.00630000419914722
0.998215079307556 0.00179999426472932
0.998215079307556 0.000800000212620944
0.998215079307556 0.000299999490380287
0.998215079307556 0
0.99866133928299 0
0.99866133928299 0
0.99866133928299 0
0.99866133928299 0
0.999107539653778 0
0.999107539653778 0
0.999107539653778 0
0.999107539653778 0
0.999553799629211 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.750258147716522 0.449300110340118
0.795665621757507 0.250500380992889
0.832817316055298 0.117199949920177
0.859649121761322 0.0516000352799892
0.877192974090576 0.0187000092118979
0.895768761634827 0.00630000419914722
0.907120704650879 0.00179999426472932
0.914344668388367 0.000800000212620944
0.923632740974426 0.000299999490380287
0.933952510356903 0
0.937048494815826 0
0.945304453372955 0
0.951496362686157 0
0.960784316062927 0
0.968008279800415 0
0.976264178752899 0
0.983488142490387 0
0.984520137310028 0
0.991744041442871 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0902798771858215 0.449300110340118
0.156553462147713 0.250500380992889
0.217820346355438 0.117199949920177
0.275846391916275 0.0516000352799892
0.330043971538544 0.0187000092118979
0.384830862283707 0.00630000419914722
0.433284252882004 0.00179999426472932
0.482621490955353 0.000800000212620944
0.534167468547821 0.000299999490380287
0.578644454479218 0
0.62768679857254 0
0.673343598842621 0
0.7153160572052 0
0.76111912727356 0
0.805449545383453 0
0.845508456230164 0
0.886303663253784 0
0.92636239528656 0
0.964359402656555 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/Markov_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.26860037446022 0.675699234008789
0.296600699424744 0.675399899482727
0.317500174045563 0.673598945140839
0.335299998521805 0.665399193763733
0.350900143384933 0.645499110221863
0.365100353956223 0.604999780654907
0.378800749778748 0.542300641536713
0.391200095415115 0.45410019159317
0.403599768877029 0.356099784374237
0.414699524641037 0.258099883794785
0.424200445413589 0.169600456953049
0.431300282478333 0.106200039386749
0.44080001115799 0.0606000013649464
0.448699951171875 0.0320998765528202
0.458800405263901 0.0150999892503023
0.467199891805649 0.00660000694915652
0.476499915122986 0.0026999965775758
0.483699887990952 0.00150000222492963
0.492799997329712 0.000999999814666808
0.500500082969666 0.000199999951291829
0.507601261138916 9.9999931990169e-05
0.515701174736023 9.9999931990169e-05
0.52240002155304 9.9999931990169e-05
0.529700100421906 0
0.536998987197876 0
0.544802188873291 0
0.553100347518921 0
0.560398876667023 0
0.568499386310577 0
0.575901687145233 0
0.582401096820831 0
0.588601291179657 0
0.595198214054108 0
0.602598607540131 0
0.608799576759338 0
0.617599904537201 0
0.624197661876678 0
0.631000697612762 0
0.637799441814423 0
0.645398259162903 0
0.653499841690063 0
0.661000847816467 0
0.667298495769501 0
0.673901200294495 0
0.679598927497864 0
0.685901641845703 0
0.693100929260254 0
0.699301540851593 0
0.705699384212494 0
0.711801469326019 0
0.718100488185883 0
0.723999559879303 0
0.728901147842407 0
0.735099196434021 0
0.741299569606781 0
0.747199833393097 0
0.753100216388702 0
0.760299861431122 0
0.765899538993835 0
0.774199426174164 0
0.781299650669098 0
0.787498891353607 0
0.794200360774994 0
0.80059951543808 0
0.806498825550079 0
0.813400208950043 0
0.820701003074646 0
0.82620096206665 0
0.83300119638443 0
0.838500797748566 0
0.844401359558105 0
0.849700391292572 0
0.855099618434906 0
0.860199987888336 0
0.865899980068207 0
0.871798634529114 0
0.876199424266815 0
0.881400406360626 0
0.886099994182587 0
0.891100287437439 0
0.896000385284424 0
0.903499901294708 0
0.90919953584671 0
0.913800120353699 0
0.919000029563904 0
0.925999820232391 0
0.931199789047241 0
0.936800003051758 0
0.942099809646606 0
0.947699785232544 0
0.953399896621704 0
0.958700001239777 0
0.96319991350174 0
0.969200193881989 0
0.97460001707077 0
0.979700028896332 0
0.985099971294403 0
0.990499973297119 0
0.995500028133392 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.974583566188812 0.675699234008789
0.983347952365875 0.675399899482727
0.98510080575943 0.673598945140839
0.986853659152985 0.665399193763733
0.990359306335449 0.645499110221863
0.991235733032227 0.604999780654907
0.992112159729004 0.542300641536713
0.992550373077393 0.45410019159317
0.992550373077393 0.356099784374237
0.992550373077393 0.258099883794785
0.992550373077393 0.169600456953049
0.992550373077393 0.106200039386749
0.992550373077393 0.0606000013649464
0.992550373077393 0.0320998765528202
0.992550373077393 0.0150999892503023
0.992550373077393 0.00660000694915652
0.992988586425781 0.0026999965775758
0.992988586425781 0.00150000222492963
0.992988586425781 0.000999999814666808
0.992988586425781 0.000199999951291829
0.992988586425781 9.9999931990169e-05
0.992988586425781 9.9999931990169e-05
0.992988586425781 9.9999931990169e-05
0.992988586425781 0
0.992988586425781 0
0.992988586425781 0
0.992988586425781 0
0.992988586425781 0
0.992988586425781 0
0.99342679977417 0
0.99342679977417 0
0.99342679977417 0
0.99342679977417 0
0.99342679977417 0
0.99342679977417 0
0.99342679977417 0
0.99342679977417 0
0.99342679977417 0
0.99342679977417 0
0.993865013122559 0
0.993865013122559 0
0.993865013122559 0
0.993865013122559 0
0.994303226470947 0
0.994741439819336 0
0.995179653167725 0
0.995179653167725 0
0.995179653167725 0
0.995179653167725 0
0.995179653167725 0
0.995179653167725 0
0.995179653167725 0
0.995179653167725 0
0.995617866516113 0
0.995617866516113 0
0.995617866516113 0
0.995617866516113 0
0.996056079864502 0
0.996056079864502 0
0.996056079864502 0
0.996056079864502 0
0.996056079864502 0
0.996056079864502 0
0.996494293212891 0
0.996494293212891 0
0.996494293212891 0
0.996494293212891 0
0.996494293212891 0
0.997370719909668 0
0.997370719909668 0
0.997370719909668 0
0.997808933258057 0
0.997808933258057 0
0.997808933258057 0
0.997808933258057 0
0.998247146606445 0
0.998247146606445 0
0.998685359954834 0
0.998685359954834 0
0.998685359954834 0
0.998685359954834 0
0.998685359954834 0
0.998685359954834 0
0.998685359954834 0
0.999123573303223 0
0.999123573303223 0
0.999123573303223 0
0.999123573303223 0
0.999123573303223 0
0.999123573303223 0
0.999123573303223 0
0.999123573303223 0
0.999123573303223 0
0.999123573303223 0
0.999561786651611 0
0.999561786651611 0
0.999561786651611 0
0.999561786651611 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.240310072898865 0.675699234008789
0.346511512994766 0.675399899482727
0.416278868913651 0.673598945140839
0.474418610334396 0.665399193763733
0.507751941680908 0.645499110221863
0.5395348072052 0.604999780654907
0.562790393829346 0.542300641536713
0.585271298885345 0.45410019159317
0.604650735855103 0.356099784374237
0.624030828475952 0.258099883794785
0.641085803508759 0.169600456953049
0.648836612701416 0.106200039386749
0.66124016046524 0.0606000013649464
0.672092854976654 0.0320998765528202
0.682170748710632 0.0150999892503023
0.687596797943115 0.00660000694915652
0.695348918437958 0.0026999965775758
0.699999630451202 0.00150000222492963
0.704651534557343 0.000999999814666808
0.71007764339447 0.000199999951291829
0.71395355463028 9.9999931990169e-05
0.720154941082001 9.9999931990169e-05
0.724806308746338 9.9999931990169e-05
0.729457437992096 0
0.73333340883255 0
0.742635548114777 0
0.748837232589722 0
0.755813956260681 0
0.761240363121033 0
0.767442107200623 0
0.76976752281189 0
0.777519226074219 0
0.781395852565765 0
0.786046385765076 0
0.791472911834717 0
0.799224734306335 0
0.80232560634613 0
0.808527052402496 0
0.817054450511932 0
0.819379866123199 0
0.82325541973114 0
0.826356410980225 0
0.827131867408752 0
0.830232858657837 0
0.834108650684357 0
0.837209045886993 0
0.840310633182526 0
0.842635452747345 0
0.844961225986481 0
0.850387573242188 0
0.852713167667389 0
0.858914613723755 0
0.861240029335022 0
0.865116119384766 0
0.868992269039154 0
0.873643577098846 0
0.877519547939301 0
0.880620181560516 0
0.884495913982391 0
0.886821806430817 0
0.88837206363678 0
0.890698075294495 0
0.896123945713043 0
0.898449540138245 0
0.903100788593292 0
0.906201720237732 0
0.91162770986557 0
0.916278958320618 0
0.91782945394516 0
0.920155107975006 0
0.923255622386932 0
0.924806177616119 0
0.92790699005127 0
0.929457366466522 0
0.932558059692383 0
0.934108316898346 0
0.935658931732178 0
0.937984704971313 0
0.940310060977936 0
0.941860377788544 0
0.945736408233643 0
0.948837220668793 0
0.950387477874756 0
0.952713191509247 0
0.958914756774902 0
0.962790668010712 0
0.965116262435913 0
0.967441856861115 0
0.975193798542023 0
0.976744174957275 0
0.978294551372528 0
0.979069769382477 0
0.980620145797729 0
0.985271334648132 0
0.98992246389389 0
0.990697681903839 0
0.994573652744293 0
0.996124029159546 0
0.998449623584747 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0236465316265821 0.675699234008789
0.042781550437212 0.675399899482727
0.0606719888746738 0.673598945140839
0.0760733783245087 0.665399193763733
0.0924082547426224 0.645499110221863
0.107809603214264 0.604999780654907
0.12414412945509 0.542300641536713
0.13876785337925 0.45410019159317
0.154169321060181 0.356099784374237
0.167548537254333 0.258099883794785
0.178904816508293 0.169600456953049
0.188394472002983 0.106200039386749
0.200684443116188 0.0606000013649464
0.210796475410461 0.0320998765528202
0.22448655962944 0.0150999892503023
0.236465618014336 0.00660000694915652
0.24922189116478 0.0026999965775758
0.259489566087723 0.00150000222492963
0.27271294593811 0.000999999814666808
0.283603519201279 0.000199999951291829
0.293870210647583 9.9999931990169e-05
0.305226594209671 9.9999931990169e-05
0.314716845750809 9.9999931990169e-05
0.325140476226807 0
0.335719078779221 0
0.345986068248749 0
0.357654273509979 0
0.367610335350037 0
0.379122585058212 0
0.389234632253647 0
0.398880213499069 0
0.406969279050827 0
0.416459023952484 0
0.4270378947258 0
0.435594260692596 0
0.447728604078293 0
0.457374155521393 0
0.466708064079285 0
0.475575655698776 0
0.48677721619606 0
0.498600155115128 0
0.509645581245422 0
0.519288778305054 0
0.528778076171875 0
0.536714971065521 0
0.545738697052002 0
0.556315660476685 0
0.565494894981384 0
0.574984014034271 0
0.583385467529297 0
0.592719733715057 0
0.600653529167175 0
0.607809484004974 0
0.61652272939682 0
0.62538880109787 0
0.633637309074402 0
0.642035007476807 0
0.6524578332901 0
0.660391271114349 0
0.672837436199188 0
0.683572471141815 0
0.692750751972198 0
0.702085256576538 0
0.711418330669403 0
0.719663381576538 0
0.72977614402771 0
0.740043699741364 0
0.747667133808136 0
0.757623493671417 0
0.765712678432465 0
0.774268209934235 0
0.782047152519226 0
0.789825737476349 0
0.797449111938477 0
0.805693507194519 0
0.814405560493469 0
0.820940852165222 0
0.828407287597656 0
0.835251808166504 0
0.842719435691833 0
0.849563598632812 0
0.860609352588654 0
0.869166195392609 0
0.87585586309433 0
0.882544815540314 0
0.892656981945038 0
0.900280177593231 0
0.908525228500366 0
0.915214538574219 0
0.923615753650665 0
0.932171702384949 0
0.94026118516922 0
0.946950912475586 0
0.955351650714874 0
0.962663173675537 0
0.970441818237305 0
0.978064715862274 0
0.986154317855835 0
0.993310511112213 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/Markov_target/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.336100578308105 0.577000677585602
0.400899976491928 0.373800128698349
0.452300041913986 0.18240025639534
0.494500011205673 0.0623000375926495
0.535000324249268 0.0179000589996576
0.571699678897858 0.00389999896287918
0.610899209976196 0.000399999058572575
0.644501626491547 0
0.678099811077118 0
0.710399925708771 0
0.743500709533691 0
0.774800002574921 0
0.804899930953979 0
0.835699617862701 0
0.864100873470306 0
0.894900023937225 0
0.922999918460846 0
0.950500190258026 0
0.976600110530853 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.993769466876984 0.577000677585602
0.995549619197845 0.373800128698349
0.996439695358276 0.18240025639534
0.996884763240814 0.0623000375926495
0.996884763240814 0.0179000589996576
0.997329771518707 0.00389999896287918
0.997329771518707 0.000399999058572575
0.997329771518707 0
0.997329771518707 0
0.997329771518707 0
0.998219847679138 0
0.998664915561676 0
0.998664915561676 0
0.998664915561676 0
0.999109923839569 0
0.999109923839569 0
0.999109923839569 0
0.999109923839569 0
0.999554991722107 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.572764813899994 0.577000677585602
0.72037410736084 0.373800128698349
0.800415933132172 0.18240025639534
0.85446971654892 0.0623000375926495
0.880457282066345 0.0179000589996576
0.893970906734467 0.00389999896287918
0.905405402183533 0.000399999058572575
0.916839897632599 0
0.927234947681427 0
0.938669443130493 0
0.941787958145142 0
0.946985423564911 0
0.954261958599091 0
0.963617444038391 0
0.972972989082336 0
0.977130949497223 0
0.98336797952652 0
0.985446989536285 0
0.994802474975586 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0849654600024223 0.577000677585602
0.158886551856995 0.373800128698349
0.222942039370537 0.18240025639534
0.277278661727905 0.0623000375926495
0.333235114812851 0.0179000589996576
0.385215640068054 0.00389999896287918
0.441319316625595 0.000399999058572575
0.48917692899704 0
0.537181377410889 0
0.583121776580811 0
0.631129443645477 0
0.676336169242859 0
0.719628214836121 0
0.76365852355957 0
0.80400538444519 0
0.848770558834076 0
0.88926500082016 0
0.929465353488922 0
0.966426253318787 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/PCFG/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.391899794340134 0.673900127410889
0.409300565719604 0.658599436283112
0.425100207328796 0.616800427436829
0.43870010972023 0.540301084518433
0.450700104236603 0.424700498580933
0.461700111627579 0.297900646924973
0.471300005912781 0.185299873352051
0.482300013303757 0.103500172495842
0.493600279092789 0.0564000010490417
0.502099931240082 0.0260000005364418
0.51179963350296 0.0125000039115548
0.520399630069733 0.00489999353885651
0.529100358486176 0.00119999900925905
0.538202106952667 0.000199999529286288
0.546300292015076 0
0.555799603462219 0
0.565399289131165 0
0.573301136493683 0
0.580701589584351 0
0.588098466396332 0
0.59420108795166 0
0.601999342441559 0
0.608400046825409 0
0.615899503231049 0
0.623099625110626 0
0.629799783229828 0
0.636398553848267 0
0.645599722862244 0
0.652901351451874 0
0.657799422740936 0
0.66390061378479 0
0.672301769256592 0
0.67919909954071 0
0.685100436210632 0
0.691000461578369 0
0.696598947048187 0
0.702999234199524 0
0.708200395107269 0
0.714099824428558 0
0.719999730587006 0
0.725598990917206 0
0.732398748397827 0
0.73860114812851 0
0.745300650596619 0
0.750500082969666 0
0.756900370121002 0
0.762999296188354 0
0.76840078830719 0
0.773300409317017 0
0.779500663280487 0
0.784999847412109 0
0.790998756885529 0
0.795999884605408 0
0.80220103263855 0
0.807400226593018 0
0.811900556087494 0
0.817000448703766 0
0.821899592876434 0
0.826000213623047 0
0.830998837947845 0
0.836401581764221 0
0.841000080108643 0
0.846299231052399 0
0.851600587368011 0
0.856300711631775 0
0.860098898410797 0
0.864399790763855 0
0.869499802589417 0
0.873300194740295 0
0.877299785614014 0
0.881200015544891 0
0.885500609874725 0
0.889700591564178 0
0.893999636173248 0
0.898500084877014 0
0.902700364589691 0
0.907899796962738 0
0.91250079870224 0
0.917699635028839 0
0.922400116920471 0
0.926599979400635 0
0.933499991893768 0
0.936999797821045 0
0.941500008106232 0
0.944800317287445 0
0.949299812316895 0
0.954000174999237 0
0.957799971103668 0
0.961900174617767 0
0.964100003242493 0
0.967999815940857 0
0.9721999168396 0
0.976300001144409 0
0.980199992656708 0
0.983799993991852 0
0.987900018692017 0
0.991100013256073 0
0.994199991226196 0
0.997399985790253 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.99025684595108 0.673900127410889
0.991142630577087 0.658599436283112
0.991585493087769 0.616800427436829
0.99202835559845 0.540301084518433
0.99202835559845 0.424700498580933
0.99202835559845 0.297900646924973
0.99202835559845 0.185299873352051
0.992471218109131 0.103500172495842
0.992471218109131 0.0564000010490417
0.992471218109131 0.0260000005364418
0.992471218109131 0.0125000039115548
0.992471218109131 0.00489999353885651
0.992471218109131 0.00119999900925905
0.992471218109131 0.000199999529286288
0.992471218109131 0
0.992914080619812 0
0.993356943130493 0
0.993356943130493 0
0.993356943130493 0
0.993356943130493 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.993799805641174 0
0.994242668151855 0
0.994242668151855 0
0.994242668151855 0
0.994242668151855 0
0.994685590267181 0
0.995128452777863 0
0.995571315288544 0
0.995571315288544 0
0.995571315288544 0
0.995571315288544 0
0.995571315288544 0
0.995571315288544 0
0.995571315288544 0
0.995571315288544 0
0.996014177799225 0
0.996014177799225 0
0.996014177799225 0
0.996014177799225 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.996457040309906 0
0.997342765331268 0
0.997342765331268 0
0.997342765331268 0
0.998228549957275 0
0.998228549957275 0
0.998228549957275 0
0.998228549957275 0
0.998671412467957 0
0.998671412467957 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999114274978638 0
0.999557137489319 0
0.999557137489319 0
0.999557137489319 0
0.999557137489319 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.54754364490509 0.673900127410889
0.581616520881653 0.658599436283112
0.603803694248199 0.616800427436829
0.623613178730011 0.540301084518433
0.635499358177185 0.424700498580933
0.64659321308136 0.297900646924973
0.65610146522522 0.185299873352051
0.663232743740082 0.103500172495842
0.671949565410614 0.0564000010490417
0.676703453063965 0.0260000005364418
0.682250559329987 0.0125000039115548
0.690173983573914 0.00489999353885651
0.696513473987579 0.00119999900925905
0.709984123706818 0.000199999529286288
0.714739263057709 0
0.719493091106415 0
0.729001462459564 0
0.735340654850006 0
0.744056701660156 0
0.748811483383179 0
0.751981437206268 0
0.753566145896912 0
0.756735384464264 0
0.759112477302551 0
0.762282192707062 0
0.767036139965057 0
0.770998358726501 0
0.777337431907654 0
0.784469068050385 0
0.791600704193115 0
0.792392909526825 0
0.798731863498688 0
0.805071532726288 0
0.809825420379639 0
0.812202572822571 0
0.817749798297882 0
0.820126891136169 0
0.824088752269745 0
0.831219911575317 0
0.834389567375183 0
0.837559819221497 0
0.843106210231781 0
0.847067952156067 0
0.850237727165222 0
0.85261470079422 0
0.853407382965088 0
0.854991972446442 0
0.857369184494019 0
0.859746515750885 0
0.86370837688446 0
0.86767053604126 0
0.872424364089966 0
0.876386523246765 0
0.878764033317566 0
0.881933748722076 0
0.885102808475494 0
0.889856994152069 0
0.893819153308868 0
0.897781312465668 0
0.899366199970245 0
0.9001584649086 0
0.902535855770111 0
0.907290041446686 0
0.909667372703552 0
0.912836790084839 0
0.916006326675415 0
0.918383419513702 0
0.922345399856567 0
0.925515055656433 0
0.927099823951721 0
0.931061804294586 0
0.932646572589874 0
0.935023784637451 0
0.938985764980316 0
0.941362917423248 0
0.942947685718536 0
0.944532513618469 0
0.946909666061401 0
0.948494434356689 0
0.950079143047333 0
0.952456414699554 0
0.954041182994843 0
0.954833626747131 0
0.957210779190063 0
0.958795547485352 0
0.965134680271149 0
0.970681428909302 0
0.973058640956879 0
0.977813005447388 0
0.978605389595032 0
0.98019015789032 0
0.983359754085541 0
0.984152138233185 0
0.98811411857605 0
0.991283655166626 0
0.992868483066559 0
0.994453251361847 0
0.996038019657135 0
0.998415231704712 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.061882808804512 0.673900127410889
0.0859567895531654 0.658599436283112
0.108024694025517 0.616800427436829
0.12885770201683 0.540301084518433
0.147839784622192 0.424700498580933
0.165123581886292 0.297900646924973
0.180555611848831 0.185299873352051
0.198302581906319 0.103500172495842
0.216049462556839 0.0564000010490417
0.231790125370026 0.0260000005364418
0.24845664203167 0.0125000039115548
0.261729329824448 0.00489999353885651
0.2745361328125 0.00119999900925905
0.287963062524796 0.000199999529286288
0.301543712615967 0
0.316820681095123 0
0.331017881631851 0
0.343518167734146 0
0.355092585086823 0
0.36743837594986 0
0.377161085605621 0
0.390277922153473 0
0.402006089687347 0
0.414814889431 0
0.427777916193008 0
0.438734710216522 0
0.449845641851425 0
0.46296301484108 0
0.473919749259949 0
0.481018602848053 0
0.492129921913147 0
0.504783034324646 0
0.515587449073792 0
0.525154709815979 0
0.535339772701263 0
0.54382598400116 0
0.554628789424896 0
0.562808811664581 0
0.570987820625305 0
0.580399215221405 0
0.590123295783997 0
0.599536240100861 0
0.609105169773102 0
0.619290471076965 0
0.627469778060913 0
0.638272941112518 0
0.648917973041534 0
0.657716870307922 0
0.66543173789978 0
0.674383401870728 0
0.682716965675354 0
0.691666066646576 0
0.700000286102295 0
0.708949506282806 0
0.716976046562195 0
0.723611176013947 0
0.730400919914246 0
0.737500309944153 0
0.743828356266022 0
0.752469301223755 0
0.761419534683228 0
0.768518805503845 0
0.776389122009277 0
0.784413456916809 0
0.791666984558105 0
0.797222077846527 0
0.803703844547272 0
0.810956716537476 0
0.815895080566406 0
0.82191401720047 0
0.827160775661469 0
0.833487331867218 0
0.840123176574707 0
0.845833241939545 0
0.852468907833099 0
0.858950316905975 0
0.867129683494568 0
0.873610973358154 0
0.881635725498199 0
0.88858026266098 0
0.894753754138947 0
0.905709803104401 0
0.910956621170044 0
0.917438447475433 0
0.922530770301819 0
0.928394913673401 0
0.934567928314209 0
0.939814686775208 0
0.945216119289398 0
0.948456943035126 0
0.954629600048065 0
0.960648119449615 0
0.966820895671844 0
0.972067892551422 0
0.976697504520416 0
0.982716023921967 0
0.987345695495605 0
0.9919753074646 0
0.996296286582947 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/PCFG_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.318000376224518 0.670899927616119
0.336299866437912 0.656699657440186
0.349400192499161 0.629401683807373
0.361000210046768 0.585398972034454
0.373000115156174 0.530201375484467
0.383099973201752 0.46659979224205
0.393000215291977 0.401799827814102
0.403400361537933 0.332000762224197
0.412900328636169 0.267200112342834
0.422500669956207 0.211300149559975
0.431499719619751 0.163999646902084
0.439500391483307 0.126299828290939
0.448800086975098 0.0949000641703606
0.45740008354187 0.0683998465538025
0.465800046920776 0.0509999580681324
0.474900037050247 0.0342999473214149
0.483700007200241 0.0216999799013138
0.490300089120865 0.0144999995827675
0.498300194740295 0.0084999967366457
0.505101144313812 0.00519999768584967
0.51240062713623 0.00310000218451023
0.519500017166138 0.00119999796152115
0.525001287460327 0.000700000789947808
0.530799388885498 0.000199999834876508
0.538300216197968 0
0.546600818634033 0
0.553099870681763 0
0.560699760913849 0
0.568500936031342 0
0.575399935245514 0
0.582898020744324 0
0.590599656105042 0
0.596900105476379 0
0.602701783180237 0
0.608800947666168 0
0.614799618721008 0
0.621099889278412 0
0.627300322055817 0
0.633598029613495 0
0.640001118183136 0
0.646800577640533 0
0.654100120067596 0
0.66109973192215 0
0.668000459671021 0
0.674399375915527 0
0.679300248622894 0
0.685600459575653 0
0.692899584770203 0
0.698901116847992 0
0.705800712108612 0
0.711599290370941 0
0.718200027942657 0
0.723099410533905 0
0.72960102558136 0
0.736100137233734 0
0.742699503898621 0
0.748401165008545 0
0.753900647163391 0
0.759400486946106 0
0.768200278282166 0
0.775799810886383 0
0.780599534511566 0
0.788599133491516 0
0.795099854469299 0
0.800401031970978 0
0.807699501514435 0
0.814601540565491 0
0.820499420166016 0
0.826799392700195 0
0.831799983978271 0
0.837500393390656 0
0.843800008296967 0
0.849299192428589 0
0.855400025844574 0
0.860199630260468 0
0.865400612354279 0
0.871300756931305 0
0.877599775791168 0
0.883099615573883 0
0.888500213623047 0
0.892899811267853 0
0.89900016784668 0
0.905499696731567 0
0.911199927330017 0
0.917100608348846 0
0.922699630260468 0
0.929099917411804 0
0.934599816799164 0
0.939800381660461 0
0.946399927139282 0
0.951900005340576 0
0.957800209522247 0
0.962399780750275 0
0.968000173568726 0
0.974100112915039 0
0.980000019073486 0
0.985099911689758 0
0.989600002765656 0
0.995299994945526 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.991574287414551 0.670899927616119
0.992461204528809 0.656699657440186
0.992904663085938 0.629401683807373
0.992904663085938 0.585398972034454
0.992904663085938 0.530201375484467
0.992904663085938 0.46659979224205
0.992904663085938 0.401799827814102
0.993348121643066 0.332000762224197
0.993348121643066 0.267200112342834
0.993348121643066 0.211300149559975
0.993348121643066 0.163999646902084
0.993348121643066 0.126299828290939
0.993348121643066 0.0949000641703606
0.993791580200195 0.0683998465538025
0.993791580200195 0.0509999580681324
0.993791580200195 0.0342999473214149
0.994235038757324 0.0216999799013138
0.994235038757324 0.0144999995827675
0.994235038757324 0.0084999967366457
0.994235038757324 0.00519999768584967
0.994235038757324 0.00310000218451023
0.994235038757324 0.00119999796152115
0.994235038757324 0.000700000789947808
0.994235038757324 0.000199999834876508
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994678497314453 0
0.994678497314453 0
0.994678497314453 0
0.994678497314453 0
0.995121955871582 0
0.995565414428711 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.997782707214355 0
0.997782707214355 0
0.997782707214355 0
0.998226165771484 0
0.998226165771484 0
0.998226165771484 0
0.998226165771484 0
0.998669624328613 0
0.998669624328613 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999556541442871 0
0.999556541442871 0
0.999556541442871 0
0.999556541442871 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.551199734210968 0.670899927616119
0.582399964332581 0.656699657440186
0.603999972343445 0.629401683807373
0.616799831390381 0.585398972034454
0.626400172710419 0.530201375484467
0.637600481510162 0.46659979224205
0.649599194526672 0.401799827814102
0.656799733638763 0.332000762224197
0.663200259208679 0.267200112342834
0.671200215816498 0.211300149559975
0.6776003241539 0.163999646902084
0.685599744319916 0.126299828290939
0.69279956817627 0.0949000641703606
0.700000047683716 0.0683998465538025
0.708799839019775 0.0509999580681324
0.715199887752533 0.0342999473214149
0.722400069236755 0.0216999799013138
0.730400085449219 0.0144999995827675
0.734399616718292 0.0084999967366457
0.738399922847748 0.00519999768584967
0.741600334644318 0.00310000218451023
0.744800388813019 0.00119999796152115
0.747199952602386 0.000700000789947808
0.750400066375732 0.000199999834876508
0.75599992275238 0
0.76559990644455 0
0.768800377845764 0
0.774400293827057 0
0.779199600219727 0
0.784800052642822 0
0.788800120353699 0
0.791999936103821 0
0.794400215148926 0
0.800800383090973 0
0.805600166320801 0
0.810400068759918 0
0.814399719238281 0
0.820799827575684 0
0.82800018787384 0
0.830400168895721 0
0.832799971103668 0
0.837599813938141 0
0.841600179672241 0
0.843199789524078 0
0.847199976444244 0
0.851199984550476 0
0.853600025177002 0
0.857599973678589 0
0.859999775886536 0
0.864800214767456 0
0.867199778556824 0
0.871999800205231 0
0.875999629497528 0
0.879999816417694 0
0.882400214672089 0
0.887199997901917 0
0.889599978923798 0
0.891999781131744 0
0.896000027656555 0
0.897599995136261 0
0.899200081825256 0
0.901600003242493 0
0.905600011348724 0
0.907999992370605 0
0.911999881267548 0
0.916000187397003 0
0.91839998960495 0
0.921599984169006 0
0.922399997711182 0
0.925599992275238 0
0.928799986839294 0
0.930399894714355 0
0.932799994945526 0
0.933599829673767 0
0.936000108718872 0
0.937600076198578 0
0.939999997615814 0
0.943199992179871 0
0.944000005722046 0
0.944800019264221 0
0.948800027370453 0
0.951200008392334 0
0.953599989414215 0
0.957599997520447 0
0.960799992084503 0
0.964800000190735 0
0.967199981212616 0
0.970399975776672 0
0.976000010967255 0
0.978399991989136 0
0.980799973011017 0
0.982400000095367 0
0.983200013637543 0
0.986400008201599 0
0.990400016307831 0
0.991999983787537 0
0.995199978351593 0
0.996800005435944 0
0.997600018978119 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0392610505223274 0.670899927616119
0.0611240677535534 0.656699657440186
0.076982244849205 0.629401683807373
0.0923788845539093 0.585398972034454
0.109006963670254 0.530201375484467
0.122402235865593 0.46659979224205
0.135334804654121 0.401799827814102
0.149807900190353 0.332000762224197
0.163202628493309 0.267200112342834
0.176443591713905 0.211300149559975
0.189068660140038 0.163999646902084
0.199845924973488 0.126299828290939
0.21277891099453 0.0949000641703606
0.224480301141739 0.0683998465538025
0.235719725489616 0.0509999580681324
0.248498842120171 0.0342999473214149
0.260508000850677 0.0216999799013138
0.269130021333694 0.0144999995827675
0.280677080154419 0.0084999967366457
0.290377825498581 0.00519999768584967
0.301000982522964 0.00310000218451023
0.311316430568695 0.00119999796152115
0.319322258234024 0.000700000789947808
0.327636271715164 0.000199999834876508
0.338106125593185 0
0.349037557840347 0
0.358429402112961 0
0.369053184986115 0
0.380138516426086 0
0.389684230089188 0
0.400461733341217 0
0.411701381206512 0
0.420939117670059 0
0.428637534379959 0
0.437105357646942 0
0.445419698953629 0
0.454349547624588 0
0.462663590908051 0
0.470977663993835 0
0.480215549468994 0
0.490222901105881 0
0.500537812709808 0
0.51054722070694 0
0.520708501338959 0
0.529637634754181 0
0.536258161067963 0
0.545496940612793 0
0.555966138839722 0
0.564741969108582 0
0.57444167137146 0
0.582909762859344 0
0.592148065567017 0
0.598921537399292 0
0.60800713300705 0
0.617552399635315 0
0.626789450645447 0
0.635104596614838 0
0.642955243587494 0
0.650654196739197 0
0.663895010948181 0
0.675287485122681 0
0.682217538356781 0
0.693764269351959 0
0.703310549259186 0
0.710699319839478 0
0.721170663833618 0
0.731330454349518 0
0.739799082279205 0
0.749036967754364 0
0.756120085716248 0
0.764280498027802 0
0.773518562316895 0
0.78152471780777 0
0.790761649608612 0
0.797690510749817 0
0.805234968662262 0
0.813856899738312 0
0.822786808013916 0
0.831100702285767 0
0.839260995388031 0
0.845266044139862 0
0.854196012020111 0
0.863741338253021 0
0.871747672557831 0
0.88021594285965 0
0.888067901134491 0
0.897459745407104 0
0.905311763286591 0
0.912240266799927 0
0.921940088272095 0
0.92994624376297 0
0.938722252845764 0
0.945650339126587 0
0.953656673431396 0
0.962124705314636 0
0.97090071439743 0
0.978137016296387 0
0.984757483005524 0
0.993225574493408 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/PCFG_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.266399323940277 0.675799608230591
0.292900502681732 0.67530220746994
0.312800109386444 0.674000322818756
0.331199496984482 0.666099548339844
0.346999824047089 0.650498270988464
0.361000210046768 0.616099953651428
0.37229973077774 0.559798896312714
0.384499818086624 0.47540009021759
0.395999550819397 0.383199870586395
0.404999017715454 0.284299790859222
0.413999766111374 0.196299850940704
0.422399520874023 0.122399941086769
0.432200103998184 0.0702999010682106
0.44099959731102 0.0382999405264854
0.450299948453903 0.0202999766916037
0.459800094366074 0.00869999267160892
0.470699906349182 0.00370000372640789
0.477299988269806 0.0015000025741756
0.486600011587143 0.000599998980760574
0.49409955739975 0.000299999490380287
0.501299679279327 0.000299999490380287
0.510400354862213 0.000199999529286288
0.518400013446808 0
0.526100754737854 0
0.535599708557129 0
0.542499601840973 0
0.55100154876709 0
0.558699369430542 0
0.56669956445694 0
0.5748011469841 0
0.581699728965759 0
0.587699174880981 0
0.595200657844543 0
0.602899134159088 0
0.609501242637634 0
0.616799533367157 0
0.622798800468445 0
0.628797292709351 0
0.634701251983643 0
0.64179939031601 0
0.648899793624878 0
0.655201196670532 0
0.662100493907928 0
0.670399367809296 0
0.676900446414948 0
0.683099746704102 0
0.690400660037994 0
0.695500254631042 0
0.701799333095551 0
0.708700180053711 0
0.715601682662964 0
0.722199141979218 0
0.729099631309509 0
0.735200941562653 0
0.741800904273987 0
0.748498737812042 0
0.754200041294098 0
0.761200606822968 0
0.766100764274597 0
0.773800671100616 0
0.780800879001617 0
0.787299931049347 0
0.794300556182861 0
0.800199925899506 0
0.806500911712646 0
0.814299643039703 0
0.820900976657867 0
0.826099097728729 0
0.83219963312149 0
0.83750057220459 0
0.84399825334549 0
0.850899815559387 0
0.856799602508545 0
0.863400101661682 0
0.868700087070465 0
0.874799907207489 0
0.879899799823761 0
0.884700000286102 0
0.88999992609024 0
0.895600199699402 0
0.900000214576721 0
0.906499922275543 0
0.912400364875793 0
0.918299794197083 0
0.922699928283691 0
0.928800165653229 0
0.934499979019165 0
0.939099788665771 0
0.945299983024597 0
0.950500190258026 0
0.956100165843964 0
0.961600005626678 0
0.965600192546844 0
0.970600008964539 0
0.975599825382233 0
0.980799973011017 0
0.984999895095825 0
0.989700019359589 0
0.995500028133392 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.972854614257812 0.675799608230591
0.98161119222641 0.67530220746994
0.986427307128906 0.674000322818756
0.988178610801697 0.666099548339844
0.989929974079132 0.650498270988464
0.990805625915527 0.616099953651428
0.991243422031403 0.559798896312714
0.992119073867798 0.47540009021759
0.992556929588318 0.383199870586395
0.992556929588318 0.284299790859222
0.992556929588318 0.196299850940704
0.992556929588318 0.122399941086769
0.992556929588318 0.0702999010682106
0.992556929588318 0.0382999405264854
0.992994725704193 0.0202999766916037
0.992994725704193 0.00869999267160892
0.993432581424713 0.00370000372640789
0.993432581424713 0.0015000025741756
0.993432581424713 0.000599998980760574
0.993432581424713 0.000299999490380287
0.993432581424713 0.000299999490380287
0.993432581424713 0.000199999529286288
0.993432581424713 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.993870377540588 0
0.994308233261108 0
0.994308233261108 0
0.994308233261108 0
0.994746088981628 0
0.995183885097504 0
0.995621740818024 0
0.996059536933899 0
0.996059536933899 0
0.996059536933899 0
0.996059536933899 0
0.996059536933899 0
0.996059536933899 0
0.996059536933899 0
0.996059536933899 0
0.996497392654419 0
0.996497392654419 0
0.996497392654419 0
0.996497392654419 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.996935188770294 0
0.997810840606689 0
0.997810840606689 0
0.997810840606689 0
0.998248696327209 0
0.998248696327209 0
0.998248696327209 0
0.998248696327209 0
0.998686492443085 0
0.998686492443085 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.999124348163605 0
0.99956214427948 0
0.99956214427948 0
0.99956214427948 0
0.99956214427948 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.232378005981445 0.675799608230591
0.332300543785095 0.67530220746994
0.403563141822815 0.674000322818756
0.463981509208679 0.666099548339844
0.499613165855408 0.650498270988464
0.529047250747681 0.616099953651428
0.553059756755829 0.559798896312714
0.577847123146057 0.47540009021759
0.591015160083771 0.383199870586395
0.604182302951813 0.284299790859222
0.617351233959198 0.196299850940704
0.626646101474762 0.122399941086769
0.637490034103394 0.0702999010682106
0.651432812213898 0.0382999405264854
0.660728335380554 0.0202999766916037
0.67157244682312 0.00869999267160892
0.679318308830261 0.00370000372640789
0.687838733196259 0.0015000025741756
0.697133898735046 0.000599998980760574
0.699457943439484 0.000299999490380287
0.704880058765411 0.000299999490380287
0.707978308200836 0.000199999529286288
0.7149498462677 0
0.724244892597198 0
0.72966730594635 0
0.735088407993317 0
0.741285800933838 0
0.749806344509125 0
0.758326828479767 0
0.76452374458313 0
0.766847431659698 0
0.773043990135193 0
0.77769148349762 0
0.780790269374847 0
0.784663498401642 0
0.789310693740845 0
0.792409181594849 0
0.797831118106842 0
0.805577099323273 0
0.809449672698975 0
0.812548220157623 0
0.815646409988403 0
0.820293962955475 0
0.82184374332428 0
0.82571679353714 0
0.828815162181854 0
0.82958984375 0
0.832687735557556 0
0.836560904979706 0
0.843531966209412 0
0.849728584289551 0
0.855925798416138 0
0.862122356891632 0
0.865995168685913 0
0.869093716144562 0
0.87529045343399 0
0.877614319324493 0
0.882262170314789 0
0.886134684085846 0
0.887683868408203 0
0.890782356262207 0
0.894655287265778 0
0.898528158664703 0
0.902401328086853 0
0.906274020671844 0
0.909372568130493 0
0.913245558738708 0
0.918667674064636 0
0.920216858386993 0
0.922540664672852 0
0.92486447095871 0
0.928737580776215 0
0.930286586284637 0
0.933384954929352 0
0.93570876121521 0
0.938807249069214 0
0.941905498504639 0
0.943454682826996 0
0.94655305147171 0
0.948102056980133 0
0.950426042079926 0
0.951975107192993 0
0.95352441072464 0
0.958946526050568 0
0.960495710372925 0
0.965917885303497 0
0.969790875911713 0
0.972889244556427 0
0.977536797523499 0
0.978311359882355 0
0.981409788131714 0
0.98218435049057 0
0.985282719135284 0
0.9891557097435 0
0.991479456424713 0
0.992254078388214 0
0.994577825069427 0
0.996901631355286 0
0.998450815677643 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0221011601388454 0.675799608230591
0.040155652910471 0.67530220746994
0.0550972670316696 0.674000322818756
0.0709727257490158 0.666099548339844
0.0877821743488312 0.650498270988464
0.10334624350071 0.616099953651428
0.115953303873539 0.559798896312714
0.129649639129639 0.47540009021759
0.144747242331505 0.383199870586395
0.156109094619751 0.284299790859222
0.16747073829174 0.196299850940704
0.178677082061768 0.122399941086769
0.191750973463058 0.0702999010682106
0.202645793557167 0.0382999405264854
0.215097233653069 0.0202999766916037
0.227704241871834 0.00869999267160892
0.24295711517334 0.00370000372640789
0.251516968011856 0.0015000025741756
0.264124751091003 0.000599998980760574
0.275330126285553 0.000299999490380287
0.285447210073471 0.000299999490380287
0.298988968133926 0.000199999529286288
0.310039222240448 0
0.319999426603317 0
0.33369642496109 0
0.343345910310745 0
0.355330973863602 0
0.365602999925613 0
0.376342803239822 0
0.387704819440842 0
0.397976875305176 0
0.406069993972778 0
0.416809499263763 0
0.428171128034592 0
0.437665432691574 0
0.448093384504318 0
0.456809461116791 0
0.465058356523514 0
0.472684979438782 0
0.482801556587219 0
0.493229418992996 0
0.502412021160126 0
0.51206374168396 0
0.524513423442841 0
0.533697068691254 0
0.542568147182465 0
0.553775191307068 0
0.56108957529068 0
0.57011616230011 0
0.579455375671387 0
0.588948607444763 0
0.597975552082062 0
0.607468664646149 0
0.616032183170319 0
0.625678598880768 0
0.634863913059235 0
0.643268227577209 0
0.653073787689209 0
0.659921705722809 0
0.671595633029938 0
0.681866466999054 0
0.691206097602844 0
0.701321125030518 0
0.709726989269257 0
0.718753218650818 0
0.730273962020874 0
0.739766240119934 0
0.746770858764648 0
0.755641996860504 0
0.763423979282379 0
0.773074865341187 0
0.782878994941711 0
0.79175066947937 0
0.801399946212769 0
0.80918288230896 0
0.817898392677307 0
0.825213730335236 0
0.83221834897995 0
0.839844524860382 0
0.848249316215515 0
0.854630351066589 0
0.86443567276001 0
0.873307466506958 0
0.881400942802429 0
0.887937486171722 0
0.896342098712921 0
0.904435634613037 0
0.910972893238068 0
0.919688820838928 0
0.927626311779022 0
0.935719847679138 0
0.944124519824982 0
0.949727654457092 0
0.956731617450714 0
0.96389102935791 0
0.971828699111938 0
0.977898836135864 0
0.984747052192688 0
0.993307411670685 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/RNN/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.378199547529221 0.672300815582275
0.396100074052811 0.653799533843994
0.410999804735184 0.600000858306885
0.424600154161453 0.506100714206696
0.43849989771843 0.38380041718483
0.447599798440933 0.25629985332489
0.45989990234375 0.154799625277519
0.470099985599518 0.0834000557661057
0.481200039386749 0.0414000079035759
0.491299986839294 0.0175999812781811
0.499699085950851 0.00679999543353915
0.507899403572083 0.00169999804347754
0.518001079559326 0.000599998980760574
0.526899337768555 0.000299999490380287
0.534701406955719 9.99997646431439e-05
0.544900000095367 0
0.554300904273987 0
0.563600361347198 0
0.573501288890839 0
0.581399917602539 0
0.590600430965424 0
0.597900927066803 0
0.603098034858704 0
0.611700057983398 0
0.620700180530548 0
0.628099918365479 0
0.635698854923248 0
0.642900705337524 0
0.649800777435303 0
0.656299293041229 0
0.661500513553619 0
0.668400168418884 0
0.676398754119873 0
0.681600034236908 0
0.688499629497528 0
0.694500207901001 0
0.699999332427979 0
0.705799698829651 0
0.711999833583832 0
0.719400227069855 0
0.727000892162323 0
0.734800755977631 0
0.74139940738678 0
0.748002052307129 0
0.75270015001297 0
0.7588991522789 0
0.764200508594513 0
0.770698606967926 0
0.776300728321075 0
0.782899439334869 0
0.788200855255127 0
0.794000267982483 0
0.798598766326904 0
0.803500950336456 0
0.809700131416321 0
0.816699624061584 0
0.823201179504395 0
0.827901363372803 0
0.832099616527557 0
0.837499618530273 0
0.842601180076599 0
0.846901059150696 0
0.851999998092651 0
0.856799602508545 0
0.862299025058746 0
0.867199778556824 0
0.872799634933472 0
0.877400875091553 0
0.881600499153137 0
0.884900271892548 0
0.888800024986267 0
0.89339953660965 0
0.897099792957306 0
0.901599586009979 0
0.906199812889099 0
0.911699712276459 0
0.915000557899475 0
0.91899973154068 0
0.9241002202034 0
0.92879980802536 0
0.933000028133392 0
0.93779981136322 0
0.941999971866608 0
0.945699989795685 0
0.949000000953674 0
0.953100085258484 0
0.957499921321869 0
0.96099990606308 0
0.96450001001358 0
0.968100011348724 0
0.972000122070312 0
0.976599991321564 0
0.978999972343445 0
0.98309999704361 0
0.986299991607666 0
0.989400029182434 0
0.991999983787537 0
0.994400024414062 0
0.997600018978119 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.986754953861237 0.672300815582275
0.988079488277435 0.653799533843994
0.988962471485138 0.600000858306885
0.989403963088989 0.506100714206696
0.989403963088989 0.38380041718483
0.989845454692841 0.25629985332489
0.989845454692841 0.154799625277519
0.990286946296692 0.0834000557661057
0.990286946296692 0.0414000079035759
0.990286946296692 0.0175999812781811
0.990728497505188 0.00679999543353915
0.990728497505188 0.00169999804347754
0.991169989109039 0.000599998980760574
0.991169989109039 0.000299999490380287
0.991169989109039 9.99997646431439e-05
0.991169989109039 0
0.991611480712891 0
0.991611480712891 0
0.991611480712891 0
0.991611480712891 0
0.991611480712891 0
0.991611480712891 0
0.991611480712891 0
0.991611480712891 0
0.991611480712891 0
0.991611480712891 0
0.992052972316742 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992494463920593 0
0.992935955524445 0
0.992935955524445 0
0.992935955524445 0
0.992935955524445 0
0.993377506732941 0
0.993818998336792 0
0.994260489940643 0
0.994260489940643 0
0.994701981544495 0
0.994701981544495 0
0.994701981544495 0
0.994701981544495 0
0.994701981544495 0
0.994701981544495 0
0.995143473148346 0
0.995584964752197 0
0.995584964752197 0
0.995584964752197 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.996026515960693 0
0.997350990772247 0
0.997350990772247 0
0.997350990772247 0
0.997792482376099 0
0.997792482376099 0
0.997792482376099 0
0.997792482376099 0
0.99823397397995 0
0.99823397397995 0
0.998675525188446 0
0.998675525188446 0
0.998675525188446 0
0.998675525188446 0
0.998675525188446 0
0.998675525188446 0
0.998675525188446 0
0.998675525188446 0
0.998675525188446 0
0.998675525188446 0
0.999117016792297 0
0.999117016792297 0
0.999117016792297 0
0.999117016792297 0
0.999117016792297 0
0.999117016792297 0
0.999117016792297 0
0.999558508396149 0
0.999558508396149 0
0.999558508396149 0
0.999558508396149 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.520848453044891 0.672300815582275
0.550417363643646 0.653799533843994
0.567854881286621 0.600000858306885
0.580742835998535 0.506100714206696
0.592873275279999 0.38380041718483
0.601212799549103 0.25629985332489
0.617892205715179 0.154799625277519
0.628506541252136 0.0834000557661057
0.63684618473053 0.0414000079035759
0.644427597522736 0.0175999812781811
0.650492548942566 0.00679999543353915
0.656558036804199 0.00169999804347754
0.66565614938736 0.000599998980760574
0.679302453994751 0.000299999490380287
0.68536788225174 9.99997646431439e-05
0.693707644939423 0
0.701288640499115 0
0.706596732139587 0
0.716452717781067 0
0.723275423049927 0
0.727824032306671 0
0.732373178005219 0
0.735405564308167 0
0.740712463855743 0
0.749052464962006 0
0.755117475986481 0
0.761182606220245 0
0.766489923000336 0
0.773313283920288 0
0.780894637107849 0
0.782410621643066 0
0.786201477050781 0
0.793025553226471 0
0.796057462692261 0
0.804397642612457 0
0.808946251869202 0
0.81349515914917 0
0.820318222045898 0
0.825625479221344 0
0.830174028873444 0
0.8354811668396 0
0.8407883644104 0
0.843062818050385 0
0.84533703327179 0
0.846853494644165 0
0.851402699947357 0
0.854434967041016 0
0.858984053134918 0
0.862016499042511 0
0.866565406322479 0
0.868840038776398 0
0.874147057533264 0
0.876421332359314 0
0.879453957080841 0
0.886277675628662 0
0.889310002326965 0
0.892342567443848 0
0.895375490188599 0
0.896891593933105 0
0.900682330131531 0
0.902198553085327 0
0.905231237411499 0
0.909021973609924 0
0.911296546459198 0
0.91660350561142 0
0.919636249542236 0
0.923426866531372 0
0.927217781543732 0
0.928734004497528 0
0.93025016784668 0
0.932524621486664 0
0.934799075126648 0
0.937073171138763 0
0.939348101615906 0
0.941622614860535 0
0.943896889686584 0
0.945413112640381 0
0.948445796966553 0
0.949962079524994 0
0.95147830247879 0
0.954510986804962 0
0.956027269363403 0
0.958301723003387 0
0.961334347724915 0
0.962850630283356 0
0.967399537563324 0
0.972706615924835 0
0.974981069564819 0
0.979529917240143 0
0.981046259403229 0
0.98256254196167 0
0.983320713043213 0
0.983320713043213 0
0.988627731800079 0
0.991660356521606 0
0.992418527603149 0
0.995451092720032 0
0.996967375278473 0
0.997725546360016 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0394326597452164 0.672300815582275
0.0637468621134758 0.653799533843994
0.0868143290281296 0.600000858306885
0.108946405351162 0.506100714206696
0.131078287959099 0.38380041718483
0.145729497075081 0.25629985332489
0.163809448480606 0.154799625277519
0.17877185344696 0.0834000557661057
0.197630941867828 0.0414000079035759
0.214931473135948 0.0175999812781811
0.228647172451019 0.00679999543353915
0.241272106766701 0.00169999804347754
0.256234854459763 0.000599998980760574
0.269950091838837 0.000299999490380287
0.283821761608124 9.99997646431439e-05
0.299251228570938 0
0.313278585672379 0
0.328397184610367 0
0.343983441591263 0
0.358168333768845 0
0.373130023479462 0
0.384975224733353 0
0.394638448953629 0
0.408977568149567 0
0.422069907188416 0
0.43375951051712 0
0.446072161197662 0
0.456514954566956 0
0.467425107955933 0
0.477088451385498 0
0.485972583293915 0
0.497818410396576 0
0.509819626808167 0
0.518080413341522 0
0.529458343982697 0
0.538966059684753 0
0.548005998134613 0
0.556421518325806 0
0.564994931221008 0
0.576527416706085 0
0.588838934898376 0
0.599282264709473 0
0.610348641872406 0
0.620633840560913 0
0.627961397171021 0
0.637312889099121 0
0.645884990692139 0
0.65554815530777 0
0.664900422096252 0
0.675031006336212 0
0.683448255062103 0
0.692954480648041 0
0.701215088367462 0
0.708698511123657 0
0.717425644397736 0
0.728334903717041 0
0.73862236738205 0
0.745480358600616 0
0.751714706420898 0
0.760442614555359 0
0.768391311168671 0
0.774470508098602 0
0.782419383525848 0
0.790212571620941 0
0.797849118709564 0
0.805330395698547 0
0.813902258872986 0
0.820448875427246 0
0.82621556520462 0
0.831047356128693 0
0.836658954620361 0
0.84398365020752 0
0.849595010280609 0
0.856140673160553 0
0.863154292106628 0
0.871415138244629 0
0.876558423042297 0
0.88294905424118 0
0.890898108482361 0
0.898067235946655 0
0.904145956039429 0
0.911471307277679 0
0.917549848556519 0
0.922849297523499 0
0.927992343902588 0
0.933603465557098 0
0.939526319503784 0
0.94420200586319 0
0.948566079139709 0
0.953865349292755 0
0.960099816322327 0
0.96726930141449 0
0.971009969711304 0
0.976309239864349 0
0.980361580848694 0
0.985037386417389 0
0.988622188568115 0
0.992051124572754 0
0.996726930141449 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/RNN/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.428500294685364 0.434599995613098
0.482900083065033 0.175599634647369
0.528202176094055 0.0494000166654587
0.569900512695312 0.00960000418126583
0.610699117183685 0.00119999772869051
0.652000844478607 0
0.684900283813477 0
0.716900229454041 0
0.746598541736603 0
0.775799512863159 0
0.802700042724609 0
0.829300224781036 0
0.855200111865997 0
0.878700613975525 0
0.902700960636139 0
0.925100028514862 0
0.947600126266479 0
0.966099917888641 0
0.984499990940094 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.99732381105423 0.434599995613098
0.997769832611084 0.175599634647369
0.997769832611084 0.0494000166654587
0.997769832611084 0.00960000418126583
0.997769832611084 0.00119999772869051
0.998215854167938 0
0.998215854167938 0
0.998215854167938 0
0.998215854167938 0
0.998215854167938 0
0.998661935329437 0
0.998661935329437 0
0.998661935329437 0
0.998661935329437 0
0.999107956886292 0
0.999107956886292 0
0.999107956886292 0
0.999107956886292 0
0.999553978443146 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.753926813602448 0.434599995613098
0.80418872833252 0.175599634647369
0.826178073883057 0.0494000166654587
0.855497241020203 0.00960000418126583
0.877486765384674 0.00119999772869051
0.89319372177124 0
0.904712021350861 0
0.914136111736298 0
0.921465992927551 0
0.92879581451416 0
0.931937158107758 0
0.938219904899597 0
0.948691070079803 0
0.95811516046524 0
0.968586385250092 0
0.9759162068367 0
0.985340297222137 0
0.98848170042038 0
0.99371725320816 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.116272322833538 0.434599995613098
0.202410742640495 0.175599634647369
0.276054859161377 0.0494000166654587
0.341760993003845 0.00960000418126583
0.406879037618637 0.00119999772869051
0.472438633441925 0
0.526092350482941 0
0.57680481672287 0
0.62413626909256 0
0.669409990310669 0
0.711157560348511 0
0.751873970031738 0
0.790239214897156 0
0.82434219121933 0
0.858885586261749 0
0.891959428787231 0
0.924738943576813 0
0.951638996601105 0
0.97824490070343 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/RNN_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.308899432420731 0.642897307872772
0.324000477790833 0.605198919773102
0.336400747299194 0.55709981918335
0.347399890422821 0.503799438476562
0.358899831771851 0.438000202178955
0.368800282478333 0.374299913644791
0.378699779510498 0.318599790334702
0.387699812650681 0.271800696849823
0.397500425577164 0.234099999070168
0.407200157642365 0.205499798059464
0.415999710559845 0.185399889945984
0.42389965057373 0.165900066494942
0.432999819517136 0.149100288748741
0.441000282764435 0.132399991154671
0.450899809598923 0.114999949932098
0.460499912500381 0.0986999422311783
0.469799906015396 0.0832000970840454
0.47859999537468 0.0697998777031898
0.486699998378754 0.0545999892055988
0.494499891996384 0.0458999536931515
0.502700448036194 0.0379000864923
0.510900318622589 0.0302000176161528
0.518501281738281 0.0242999885231256
0.524899899959564 0.0205999612808228
0.533200323581696 0.0174000412225723
0.539898991584778 0.015399994328618
0.54679924249649 0.014000004157424
0.555100440979004 0.0124999834224582
0.563599050045013 0.0110999960452318
0.570700287818909 0.00999998580664396
0.577398657798767 0.00880000367760658
0.58420068025589 0.00789999589323997
0.591901004314423 0.00680000241845846
0.598900496959686 0.00549999671056867
0.606000363826752 0.00439998414367437
0.613801419734955 0.00309999985620379
0.620201289653778 0.00220000371336937
0.626399576663971 0.00169999885838479
0.632098972797394 0.00150000141002238
0.638099730014801 0.00139999948441982
0.644900500774384 0.000899999518878758
0.653000235557556 0.000499999092426151
0.659798979759216 0.000399999582441524
0.66790109872818 0.000299999432172626
0.674899876117706 9.99997646431439e-05
0.680900454521179 9.99997646431439e-05
0.688700079917908 0
0.695199549198151 0
0.701499998569489 0
0.708000063896179 0
0.714899241924286 0
0.721101582050323 0
0.726200103759766 0
0.732100069522858 0
0.739400088787079 0
0.745701193809509 0
0.751999616622925 0
0.759898900985718 0
0.766201257705688 0
0.773598790168762 0
0.780499637126923 0
0.78750067949295 0
0.794399201869965 0
0.801699817180634 0
0.807599008083344 0
0.815399825572968 0
0.82219934463501 0
0.82739919424057 0
0.833800792694092 0
0.839900195598602 0
0.846300184726715 0
0.85219931602478 0
0.8572998046875 0
0.861699819564819 0
0.867400407791138 0
0.87300056219101 0
0.877799391746521 0
0.882800757884979 0
0.888600170612335 0
0.894400000572205 0
0.898899435997009 0
0.90559983253479 0
0.911799788475037 0
0.916999876499176 0
0.92220002412796 0
0.927599906921387 0
0.932599902153015 0
0.937300086021423 0
0.943199813365936 0
0.948099970817566 0
0.954399824142456 0
0.960300028324127 0
0.964199900627136 0
0.970099985599518 0
0.976499974727631 0
0.98199999332428 0
0.986199975013733 0
0.99099999666214 0
0.995500028133392 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.990691483020782 0.642897307872772
0.991578042507172 0.605198919773102
0.992021262645721 0.55709981918335
0.992021262645721 0.503799438476562
0.992464542388916 0.438000202178955
0.992464542388916 0.374299913644791
0.992464542388916 0.318599790334702
0.992907822132111 0.271800696849823
0.992907822132111 0.234099999070168
0.992907822132111 0.205499798059464
0.992907822132111 0.185399889945984
0.992907822132111 0.165900066494942
0.992907822132111 0.149100288748741
0.992907822132111 0.132399991154671
0.992907822132111 0.114999949932098
0.992907822132111 0.0986999422311783
0.99335104227066 0.0832000970840454
0.99335104227066 0.0697998777031898
0.993794322013855 0.0545999892055988
0.993794322013855 0.0458999536931515
0.993794322013855 0.0379000864923
0.993794322013855 0.0302000176161528
0.993794322013855 0.0242999885231256
0.993794322013855 0.0205999612808228
0.993794322013855 0.0174000412225723
0.993794322013855 0.015399994328618
0.993794322013855 0.014000004157424
0.993794322013855 0.0124999834224582
0.993794322013855 0.0110999960452318
0.993794322013855 0.00999998580664396
0.993794322013855 0.00880000367760658
0.993794322013855 0.00789999589323997
0.993794322013855 0.00680000241845846
0.993794322013855 0.00549999671056867
0.993794322013855 0.00439998414367437
0.993794322013855 0.00309999985620379
0.993794322013855 0.00220000371336937
0.99423760175705 0.00169999885838479
0.99423760175705 0.00150000141002238
0.994680821895599 0.00139999948441982
0.994680821895599 0.000899999518878758
0.994680821895599 0.000499999092426151
0.994680821895599 0.000399999582441524
0.995124101638794 0.000299999432172626
0.995567381381989 9.99997646431439e-05
0.996010661125183 9.99997646431439e-05
0.996010661125183 0
0.996010661125183 0
0.996010661125183 0
0.996010661125183 0
0.996010661125183 0
0.996010661125183 0
0.996010661125183 0
0.996453881263733 0
0.996453881263733 0
0.996453881263733 0
0.996453881263733 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.996897161006927 0
0.997783660888672 0
0.997783660888672 0
0.997783660888672 0
0.998226940631866 0
0.998226940631866 0
0.998226940631866 0
0.998226940631866 0
0.998670220375061 0
0.998670220375061 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999113500118256 0
0.999556720256805 0
0.999556720256805 0
0.999556720256805 0
0.999556720256805 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.511485755443573 0.642897307872772
0.549770593643188 0.605198919773102
0.565849959850311 0.55709981918335
0.578101098537445 0.503799438476562
0.59111762046814 0.438000202178955
0.60260397195816 0.374299913644791
0.616385638713837 0.318599790334702
0.627870738506317 0.271800696849823
0.635527908802032 0.234099999070168
0.642419934272766 0.205499798059464
0.649310529232025 0.185399889945984
0.655436277389526 0.165900066494942
0.664624810218811 0.149100288748741
0.673813283443451 0.132399991154671
0.68223637342453 0.114999949932098
0.687595546245575 0.0986999422311783
0.693721294403076 0.0832000970840454
0.699846863746643 0.0697998777031898
0.7059725522995 0.0545999892055988
0.710566639900208 0.0458999536931515
0.71516078710556 0.0379000864923
0.720520257949829 0.0302000176161528
0.725880801677704 0.0242999885231256
0.733538031578064 0.0205999612808228
0.741194188594818 0.0174000412225723
0.74578857421875 0.015399994328618
0.751914441585541 0.014000004157424
0.759571135044098 0.0124999834224582
0.766462743282318 0.0110999960452318
0.772588074207306 0.00999998580664396
0.775650918483734 0.00880000367760658
0.78330785036087 0.00789999589323997
0.787902355194092 0.00680000241845846
0.793261468410492 0.00549999671056867
0.796324729919434 0.00439998414367437
0.800918936729431 0.00309999985620379
0.805513203144073 0.00220000371336937
0.810107171535492 0.00169999885838479
0.816998660564423 0.00150000141002238
0.818529665470123 0.00139999948441982
0.821592628955841 0.000899999518878758
0.826952874660492 0.000499999092426151
0.827718198299408 0.000399999582441524
0.831546902656555 0.000299999432172626
0.833844006061554 9.99997646431439e-05
0.836906611919403 9.99997646431439e-05
0.840734899044037 0
0.846094965934753 0
0.849923253059387 0
0.855282843112946 0
0.857580125331879 0
0.863705992698669 0
0.866768598556519 0
0.870597422122955 0
0.872128427028656 0
0.877488315105438 0
0.88131707906723 0
0.885911166667938 0
0.891271412372589 0
0.893568336963654 0
0.896630764007568 0
0.900459408760071 0
0.905819594860077 0
0.91041374206543 0
0.915773332118988 0
0.918836116790771 0
0.921899020671844 0
0.924961686134338 0
0.925727248191833 0
0.927258789539337 0
0.929555892944336 0
0.932618677616119 0
0.934915781021118 0
0.935681462287903 0
0.937978565692902 0
0.938744068145752 0
0.94180703163147 0
0.943338453769684 0
0.944104135036469 0
0.947166919708252 0
0.952526807785034 0
0.956355273723602 0
0.957120954990387 0
0.9609494805336 0
0.962480843067169 0
0.966309368610382 0
0.969372153282166 0
0.97166919708252 0
0.980091869831085 0
0.980091869831085 0
0.981623291969299 0
0.982388973236084 0
0.982388973236084 0
0.986217439174652 0
0.991577327251434 0
0.993108749389648 0
0.995405793190002 0
0.997702896595001 0
0.998468577861786 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.028890959918499 0.642897307872772
0.0442683808505535 0.605198919773102
0.0601118355989456 0.55709981918335
0.0747126266360283 0.503799438476562
0.0897794887423515 0.438000202178955
0.102826930582523 0.374299913644791
0.115408509969711 0.318599790334702
0.126902684569359 0.271800696849823
0.140571534633636 0.234099999070168
0.154240757226944 0.205499798059464
0.166511163115501 0.185399889945984
0.177539527416229 0.165900066494942
0.189810276031494 0.149100288748741
0.200372919440269 0.132399991154671
0.214041545987129 0.114999949932098
0.227865859866142 0.0986999422311783
0.240913406014442 0.0832000970840454
0.25333908200264 0.0697998777031898
0.264523923397064 0.0545999892055988
0.275707483291626 0.0458999536931515
0.287511616945267 0.0379000864923
0.299161523580551 0.0302000176161528
0.309878647327423 0.0242999885231256
0.318266153335571 0.0205999612808228
0.329606026411057 0.0174000412225723
0.339080601930618 0.015399994328618
0.34855580329895 0.014000004157424
0.359894603490829 0.0124999834224582
0.371698975563049 0.0110999960452318
0.381484717130661 0.00999998580664396
0.391270518302917 0.00880000367760658
0.40027928352356 0.00789999589323997
0.411307722330093 0.00680000241845846
0.421093344688416 0.00549999671056867
0.431500315666199 0.00439998414367437
0.44268387556076 0.00309999985620379
0.45169323682785 0.00220000371336937
0.460236102342606 0.00169999885838479
0.467691779136658 0.00150000141002238
0.476545423269272 0.00139999948441982
0.486486524343491 0.000899999518878758
0.497980743646622 0.000499999092426151
0.508386850357056 0.000399999582441524
0.520037114620209 0.000299999432172626
0.530288517475128 9.99997646431439e-05
0.538830816745758 9.99997646431439e-05
0.550170421600342 0
0.559180378913879 0
0.568188369274139 0
0.577199339866638 0
0.587449193000793 0
0.595835387706757 0
0.603137135505676 0
0.611370503902435 0
0.622398734092712 0
0.631097733974457 0
0.640105605125427 0
0.65129029750824 0
0.659988045692444 0
0.671015739440918 0
0.681111991405487 0
0.691208899021149 0
0.700837731361389 0
0.711245715618134 0
0.71932315826416 0
0.730816960334778 0
0.740757465362549 0
0.748214542865753 0
0.757688164710999 0
0.766853213310242 0
0.776328027248383 0
0.784715473651886 0
0.792171359062195 0
0.798850893974304 0
0.807238399982452 0
0.815626204013824 0
0.822461009025574 0
0.82976096868515 0
0.838614344596863 0
0.847001731395721 0
0.852904677391052 0
0.862534821033478 0
0.872009813785553 0
0.879310250282288 0
0.887076735496521 0
0.89468777179718 0
0.90183287858963 0
0.908667087554932 0
0.91612309217453 0
0.923734068870544 0
0.933209240436554 0
0.942218244075775 0
0.948276042938232 0
0.956663548946381 0
0.965361893177032 0
0.973594307899475 0
0.979652166366577 0
0.986641824245453 0
0.993320882320404 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/RNN_/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.35370010137558 0.469300001859665
0.404899805784225 0.285699814558029
0.449200093746185 0.163100212812424
0.491500049829483 0.0921000093221664
0.531501591205597 0.050099965184927
0.569199979305267 0.0272000189870596
0.605500280857086 0.0137999895960093
0.640598654747009 0.00759999826550484
0.676799535751343 0.0035999973770231
0.709500670433044 0.00130000081844628
0.74370014667511 0.000499999267049134
0.775300264358521 0.000199999834876508
0.806401073932648 9.99997646431439e-05
0.835799992084503 0
0.865600168704987 0
0.89410001039505 0
0.923299789428711 0
0.952100098133087 0
0.978299975395203 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.99732381105423 0.469300001859665
0.99732381105423 0.285699814558029
0.99732381105423 0.163100212812424
0.997769832611084 0.0921000093221664
0.997769832611084 0.050099965184927
0.998215854167938 0.0272000189870596
0.998215854167938 0.0137999895960093
0.998215854167938 0.00759999826550484
0.998215854167938 0.0035999973770231
0.998215854167938 0.00130000081844628
0.998661935329437 0.000499999267049134
0.998661935329437 0.000199999834876508
0.998661935329437 9.99997646431439e-05
0.998661935329437 0
0.999107956886292 0
0.999107956886292 0
0.999107956886292 0
0.999107956886292 0
0.999553978443146 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.757067978382111 0.469300001859665
0.812565445899963 0.285699814558029
0.835602104663849 0.163100212812424
0.857591688632965 0.0921000093221664
0.876439809799194 0.050099965184927
0.89319372177124 0.0272000189870596
0.904712021350861 0.0137999895960093
0.913088977336884 0.00759999826550484
0.925654411315918 0.0035999973770231
0.934031367301941 0.00130000081844628
0.935078620910645 0.000499999267049134
0.940314114093781 0.000199999834876508
0.949738204479218 9.99997646431439e-05
0.959162294864655 0
0.967539250850677 0
0.973821997642517 0
0.98219895362854 0
0.986387431621552 0
0.992670178413391 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0849623531103134 0.469300001859665
0.152432605624199 0.285699814558029
0.214317217469215 0.163100212812424
0.273261576890945 0.0921000093221664
0.329414010047913 0.050099965184927
0.382331430912018 0.0272000189870596
0.434073239564896 0.0137999895960093
0.484492003917694 0.00759999826550484
0.535940945148468 0.0035999973770231
0.582831084728241 0.00130000081844628
0.632808744907379 0.000499999267049134
0.678524315357208 0.000199999834876508
0.722915947437286 9.99997646431439e-05
0.764809131622314 0
0.807290971279144 0
0.848302364349365 0
0.890048563480377 0
0.931794941425323 0
0.969278275966644 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/RNN_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.26469948887825 0.675799608230591
0.291000217199326 0.675600171089172
0.30890080332756 0.674299597740173
0.324599921703339 0.669800043106079
0.340499758720398 0.652199566364288
0.353699535131454 0.621699631214142
0.36729970574379 0.571700751781464
0.378299683332443 0.498000234365463
0.390799790620804 0.406999796628952
0.402100056409836 0.306999981403351
0.411000102758408 0.216499909758568
0.419800490140915 0.139199748635292
0.43049955368042 0.0822999849915504
0.441199958324432 0.0471999384462833
0.449699848890305 0.0241999868303537
0.459500193595886 0.0104000009596348
0.469799906015396 0.00499999802559614
0.476900011301041 0.00230000261217356
0.485799998044968 0.000599998980760574
0.492000013589859 0.000399999669753015
0.500200748443604 9.99997646431439e-05
0.507400214672089 9.99997646431439e-05
0.515299201011658 0
0.522900938987732 0
0.532001495361328 0
0.539400458335876 0
0.547499716281891 0
0.555398404598236 0
0.562901318073273 0
0.570100784301758 0
0.576599299907684 0
0.58309930562973 0
0.590200126171112 0
0.597599864006042 0
0.604099929332733 0
0.610500574111938 0
0.617198467254639 0
0.625400304794312 0
0.632100462913513 0
0.639099717140198 0
0.646300137042999 0
0.65500009059906 0
0.66190105676651 0
0.669200122356415 0
0.675499439239502 0
0.682400524616241 0
0.689399719238281 0
0.695800125598907 0
0.70160037279129 0
0.709599614143372 0
0.715400516986847 0
0.721700549125671 0
0.727499127388 0
0.733299434185028 0
0.739600896835327 0
0.745400905609131 0
0.751399755477905 0
0.759399831295013 0
0.765999436378479 0
0.774401187896729 0
0.781999707221985 0
0.787100076675415 0
0.79520046710968 0
0.801599085330963 0
0.8081995844841 0
0.814400434494019 0
0.821499288082123 0
0.826799631118774 0
0.832500755786896 0
0.839100182056427 0
0.845100402832031 0
0.851200759410858 0
0.857099831104279 0
0.862400472164154 0
0.867499828338623 0
0.873000025749207 0
0.878200173377991 0
0.883300602436066 0
0.888199925422668 0
0.894600808620453 0
0.898700892925262 0
0.904699981212616 0
0.910699784755707 0
0.915399789810181 0
0.921099781990051 0
0.925999879837036 0
0.932400107383728 0
0.937399983406067 0
0.942200183868408 0
0.948099970817566 0
0.953699827194214 0
0.959500014781952 0
0.964100182056427 0
0.969600081443787 0
0.975099980831146 0
0.979899883270264 0
0.985300004482269 0
0.990299999713898 0
0.995899975299835 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.973753273487091 0.675799608230591
0.981627285480499 0.675600171089172
0.984251976013184 0.674299597740173
0.98468941450119 0.669800043106079
0.986439168453217 0.652199566364288
0.989063858985901 0.621699631214142
0.989938735961914 0.571700751781464
0.990813672542572 0.498000234365463
0.990813672542572 0.406999796628952
0.990813672542572 0.306999981403351
0.991251111030579 0.216499909758568
0.991251111030579 0.139199748635292
0.991251111030579 0.0822999849915504
0.991251111030579 0.0471999384462833
0.991251111030579 0.0241999868303537
0.991251111030579 0.0104000009596348
0.991688549518585 0.00499999802559614
0.991688549518585 0.00230000261217356
0.991688549518585 0.000599998980760574
0.991688549518585 0.000399999669753015
0.992125988006592 9.99997646431439e-05
0.992125988006592 9.99997646431439e-05
0.992125988006592 0
0.992563426494598 0
0.993000864982605 0
0.993000864982605 0
0.993000864982605 0
0.993000864982605 0
0.993438303470612 0
0.993438303470612 0
0.993438303470612 0
0.993438303470612 0
0.993438303470612 0
0.993438303470612 0
0.993875741958618 0
0.993875741958618 0
0.993875741958618 0
0.993875741958618 0
0.993875741958618 0
0.99431324005127 0
0.99431324005127 0
0.99431324005127 0
0.99431324005127 0
0.994750678539276 0
0.995188117027283 0
0.995625555515289 0
0.995625555515289 0
0.995625555515289 0
0.995625555515289 0
0.995625555515289 0
0.995625555515289 0
0.995625555515289 0
0.995625555515289 0
0.996062994003296 0
0.996062994003296 0
0.996062994003296 0
0.996062994003296 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.996500432491302 0
0.997375309467316 0
0.997375309467316 0
0.997375309467316 0
0.997812747955322 0
0.997812747955322 0
0.997812747955322 0
0.997812747955322 0
0.998250246047974 0
0.998250246047974 0
0.99868768453598 0
0.99868768453598 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999125123023987 0
0.999562561511993 0
0.999562561511993 0
0.999562561511993 0
0.999562561511993 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.230109199881554 0.675799608230591
0.343213647603989 0.675600171089172
0.409516394138336 0.674299597740173
0.460998445749283 0.669800043106079
0.49922040104866 0.652199566364288
0.536661744117737 0.621699631214142
0.563182413578033 0.571700751781464
0.57878303527832 0.498000234365463
0.595163643360138 0.406999796628952
0.60920512676239 0.306999981403351
0.623245000839233 0.216499909758568
0.634945511817932 0.139199748635292
0.645865440368652 0.0822999849915504
0.658346652984619 0.0471999384462833
0.665366530418396 0.0241999868303537
0.674726963043213 0.0104000009596348
0.681746900081635 0.00499999802559614
0.69266802072525 0.00230000261217356
0.702028393745422 0.000599998980760574
0.705928266048431 0.000399999669753015
0.712948381900787 9.99997646431439e-05
0.716068863868713 9.99997646431439e-05
0.72230851650238 0
0.72698962688446 0
0.730889320373535 0
0.737909615039825 0
0.744929730892181 0
0.752729833126068 0
0.759750366210938 0
0.765990376472473 0
0.772231161594391 0
0.77535092830658 0
0.781591296195984 0
0.78939151763916 0
0.794071614742279 0
0.799531996250153 0
0.801871716976166 0
0.8096724152565 0
0.818252325057983 0
0.819813072681427 0
0.82293313741684 0
0.829173386096954 0
0.830733418464661 0
0.830733418464661 0
0.833073496818542 0
0.834633588790894 0
0.83541339635849 0
0.840093433856964 0
0.842433869838715 0
0.847893893718719 0
0.851793766021729 0
0.858034729957581 0
0.863494515419006 0
0.867394685745239 0
0.871294677257538 0
0.875975251197815 0
0.878315389156342 0
0.88221538066864 0
0.886895298957825 0
0.890795648097992 0
0.892355620861053 0
0.895475625991821 0
0.902496099472046 0
0.904056251049042 0
0.910296618938446 0
0.913416564464569 0
0.916536450386047 0
0.920436918735504 0
0.921996891498566 0
0.925117015838623 0
0.929017186164856 0
0.932137310504913 0
0.933697164058685 0
0.936817586421967 0
0.938377559185028 0
0.939157664775848 0
0.942277669906616 0
0.944617807865143 0
0.945397794246674 0
0.948517918586731 0
0.952418088912964 0
0.953978180885315 0
0.956318259239197 0
0.958658337593079 0
0.96099841594696 0
0.964898586273193 0
0.970358788967133 0
0.974258899688721 0
0.978939175605774 0
0.981279253959656 0
0.982059299945831 0
0.982839286327362 0
0.983619332313538 0
0.987519502639771 0
0.992199659347534 0
0.992199659347534 0
0.995319783687592 0
0.996879875659943 0
0.998439908027649 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0195895731449127 0.675799608230591
0.0351367630064487 0.675600171089172
0.0488183796405792 0.674299597740173
0.0628108531236649 0.669800043106079
0.0792910233139992 0.652199566364288
0.0914178341627121 0.621699631214142
0.10696517676115 0.571700751781464
0.120646610856056 0.498000234365463
0.136815831065178 0.406999796628952
0.151586085557938 0.306999981403351
0.162468567490578 0.216499909758568
0.173818290233612 0.139199748635292
0.188277319073677 0.0822999849915504
0.202425375580788 0.0471999384462833
0.214241296052933 0.0241999868303537
0.227611914277077 0.0104000009596348
0.24207104742527 0.00499999802559614
0.250932693481445 0.00230000261217356
0.262904047966003 0.000599998980760574
0.271766096353531 0.000399999669753015
0.282959938049316 9.99997646431439e-05
0.293533056974411 9.99997646431439e-05
0.304571568965912 0
0.315298289060593 0
0.328512936830521 0
0.338619142770767 0
0.349813401699066 0
0.360541045665741 0
0.37064653635025 0
0.380597501993179 0
0.389459252357483 0
0.398942798376083 0
0.408737570047379 0
0.418687671422958 0
0.427705138921738 0
0.436567276716232 0
0.44651734828949 0
0.457711428403854 0
0.466417908668518 0
0.476834565401077 0
0.487406730651855 0
0.499689370393753 0
0.510105669498444 0
0.521299004554749 0
0.53047388792038 0
0.540734827518463 0
0.551462590694427 0
0.560480654239655 0
0.569029569625854 0
0.580377876758575 0
0.588619947433472 0
0.597169995307922 0
0.605100035667419 0
0.613183438777924 0
0.622201502323151 0
0.630286693572998 0
0.639148235321045 0
0.650653600692749 0
0.659981489181519 0
0.672264575958252 0
0.683768630027771 0
0.69107574224472 0
0.702269911766052 0
0.711910128593445 0
0.720927119255066 0
0.729944109916687 0
0.74036055803299 0
0.747823536396027 0
0.75606381893158 0
0.765701770782471 0
0.774252831935883 0
0.782960832118988 0
0.791822016239166 0
0.799440443515778 0
0.80705863237381 0
0.815298974514008 0
0.822761356830597 0
0.830068171024323 0
0.837531387805939 0
0.846704065799713 0
0.852300643920898 0
0.861317753791809 0
0.870180070400238 0
0.877021431922913 0
0.885416805744171 0
0.892257213592529 0
0.901119351387024 0
0.908116042613983 0
0.914645493030548 0
0.923352003097534 0
0.931903123855591 0
0.940764784812927 0
0.947761118412018 0
0.955534815788269 0
0.962997496128082 0
0.970460176467896 0
0.978233814239502 0
0.985696494579315 0
0.993936538696289 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/RNN_target/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.333099067211151 0.586398601531982
0.395000010728836 0.390500277280807
0.444199651479721 0.199900224804878
0.491199910640717 0.0767998546361923
0.532100021839142 0.0233999695628881
0.572299122810364 0.00609999289736152
0.607300996780396 0.00109999882988632
0.64329981803894 9.9999931990169e-05
0.678099811077118 9.9999931990169e-05
0.710200071334839 0
0.744398415088654 0
0.773698925971985 0
0.806200921535492 0
0.8370001912117 0
0.86680018901825 0
0.896999597549438 0
0.92519998550415 0
0.952000081539154 0
0.976999998092651 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.991566777229309 0.586398601531982
0.995117604732513 0.390500277280807
0.996449172496796 0.199900224804878
0.996893048286438 0.0767998546361923
0.997336864471436 0.0233999695628881
0.997780740261078 0.00609999289736152
0.997780740261078 0.00109999882988632
0.997780740261078 9.9999931990169e-05
0.997780740261078 9.9999931990169e-05
0.997780740261078 0
0.99822461605072 0
0.99822461605072 0
0.998668432235718 0
0.998668432235718 0
0.99911230802536 0
0.99911230802536 0
0.99911230802536 0
0.99911230802536 0
0.999556124210358 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.576882541179657 0.586398601531982
0.733828127384186 0.390500277280807
0.803817629814148 0.199900224804878
0.851537525653839 0.0767998546361923
0.873806893825531 0.0233999695628881
0.882290482521057 0.00609999289736152
0.896076381206512 0.00109999882988632
0.907741248607635 9.9999931990169e-05
0.917285263538361 9.9999931990169e-05
0.928950130939484 0
0.931071043014526 0
0.935312807559967 0
0.942735970020294 0
0.957582175731659 0
0.969247102737427 0
0.97560977935791 0
0.981972455978394 0
0.986214220523834 0
0.993637323379517 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0812759026885033 0.586398601531982
0.149323984980583 0.390500277280807
0.211493164300919 0.199900224804878
0.273809462785721 0.0767998546361923
0.33068773150444 0.0233999695628881
0.388447910547256 0.00609999289736152
0.437977522611618 0.00109999882988632
0.489271074533463 9.9999931990169e-05
0.539094984531403 9.9999931990169e-05
0.58465451002121 0
0.634479403495789 0
0.676954388618469 0
0.723545670509338 0
0.766755223274231 0
0.808789134025574 0
0.852292597293854 0
0.89285671710968 0
0.931657731533051 0
0.967225134372711 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/Tweak/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.259999811649323 0.481899815797806
0.278600603342056 0.429700005054474
0.291199654340744 0.392100036144257
0.303300380706787 0.352300012111664
0.31499981880188 0.320799964666367
0.325299739837646 0.28680008649826
0.336700439453125 0.260700064897537
0.34750097990036 0.236099997162819
0.357600539922714 0.211499996483326
0.367299139499664 0.187300005555153
0.374699831008911 0.165800000727177
0.382200300693512 0.146200004220009
0.390799880027771 0.125700011849403
0.401499927043915 0.11010000705719
0.410099893808365 0.0930000051856041
0.417500376701355 0.077899993956089
0.427499711513519 0.0641000013798475
0.435600012540817 0.0525999985635281
0.4441998898983 0.0433999918401241
0.451499789953232 0.0347000025212765
0.458999991416931 0.0268000012263656
0.466600000858307 0.0194000011309981
0.475600093603134 0.01539999935776
0.483599990606308 0.0117000013589859
0.491800010204315 0.00939999893307686
0.500900506973267 0.00720000038854778
0.508899629116058 0.0056000005453825
0.516602218151093 0.00399999944493175
0.525299191474915 0.00319999903440475
0.534401416778564 0.00259999909903854
0.541599214076996 0.00219999916153029
0.549700319766998 0.00159999969182536
0.557698667049408 0.00109999928390607
0.566400468349457 0.00049999967450276
0.573899626731873 0.00049999967450276
0.58260041475296 0.000399999739602208
0.590199947357178 0.000299999699927866
0.596901535987854 0.000199999869801104
0.605199098587036 0.000199999869801104
0.613599181175232 0.000199999869801104
0.622199833393097 9.9999934900552e-05
0.630599617958069 9.9999934900552e-05
0.638800024986267 0
0.646998703479767 0
0.65550035238266 0
0.662301540374756 0
0.669299483299255 0
0.677400290966034 0
0.684698700904846 0
0.692499339580536 0
0.69959968328476 0
0.706599295139313 0
0.712798655033112 0
0.719099342823029 0
0.725100934505463 0
0.732200026512146 0
0.738498985767365 0
0.746899604797363 0
0.752900004386902 0
0.763300955295563 0
0.77150022983551 0
0.77720057964325 0
0.783800363540649 0
0.791400671005249 0
0.798400342464447 0
0.806600511074066 0
0.814199328422546 0
0.820900201797485 0
0.827199220657349 0
0.834300994873047 0
0.840799808502197 0
0.846499800682068 0
0.852300763130188 0
0.858399212360382 0
0.863999247550964 0
0.870300114154816 0
0.876300394535065 0
0.882599413394928 0
0.888900995254517 0
0.895000100135803 0
0.899800598621368 0
0.905699610710144 0
0.911499440670013 0
0.916900277137756 0
0.921700179576874 0
0.928399622440338 0
0.934000194072723 0
0.938600122928619 0
0.943700075149536 0
0.949799776077271 0
0.955400168895721 0
0.961499810218811 0
0.965299904346466 0
0.971199989318848 0
0.976100027561188 0
0.981400012969971 0
0.985700011253357 0
0.990800023078918 0
0.995599985122681 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.933109164237976 0.481899815797806
0.950778305530548 0.429700005054474
0.957088768482208 0.392100036144257
0.964240550994873 0.352300012111664
0.966344118118286 0.320799964666367
0.969709694385529 0.28680008649826
0.972654581069946 0.260700064897537
0.9743372797966 0.236099997162819
0.977282285690308 0.211499996483326
0.978544354438782 0.187300005555153
0.978965103626251 0.165800000727177
0.979806482791901 0.146200004220009
0.98064786195755 0.125700011849403
0.98064786195755 0.11010000705719
0.981909990310669 0.0930000051856041
0.981909990310669 0.077899993956089
0.983172059059143 0.0641000013798475
0.983172059059143 0.0525999985635281
0.983592748641968 0.0433999918401241
0.984013438224792 0.0347000025212765
0.984854876995087 0.0268000012263656
0.985696256160736 0.0194000011309981
0.986537635326385 0.01539999935776
0.98695832490921 0.0117000013589859
0.98695832490921 0.00939999893307686
0.987799763679504 0.00720000038854778
0.988220453262329 0.0056000005453825
0.988220453262329 0.00399999944493175
0.988641142845154 0.00319999903440475
0.989482522010803 0.00259999909903854
0.989903211593628 0.00219999916153029
0.989903211593628 0.00159999969182536
0.990323960781097 0.00109999928390607
0.990323960781097 0.00049999967450276
0.990323960781097 0.00049999967450276
0.990323960781097 0.000399999739602208
0.990744650363922 0.000299999699927866
0.991165339946747 0.000199999869801104
0.991165339946747 0.000199999869801104
0.991586029529572 0.000199999869801104
0.991586029529572 9.9999934900552e-05
0.992006719112396 9.9999934900552e-05
0.992006719112396 0
0.992427408695221 0
0.993268847465515 0
0.99368953704834 0
0.99368953704834 0
0.994110226631165 0
0.994110226631165 0
0.994110226631165 0
0.994110226631165 0
0.994530916213989 0
0.994530916213989 0
0.994951605796814 0
0.994951605796814 0
0.994951605796814 0
0.994951605796814 0
0.995372295379639 0
0.995372295379639 0
0.995372295379639 0
0.995372295379639 0
0.995372295379639 0
0.995372295379639 0
0.995793044567108 0
0.995793044567108 0
0.995793044567108 0
0.995793044567108 0
0.995793044567108 0
0.996634423732758 0
0.996634423732758 0
0.996634423732758 0
0.997475802898407 0
0.997896492481232 0
0.997896492481232 0
0.997896492481232 0
0.998317182064056 0
0.998317182064056 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.998737931251526 0
0.999158620834351 0
0.999158620834351 0
0.999158620834351 0
0.999158620834351 0
0.999158620834351 0
0.999158620834351 0
0.999579310417175 0
0.999579310417175 0
0.999579310417175 0
0.999579310417175 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.245778724551201 0.481899815797806
0.301125764846802 0.429700005054474
0.332082539796829 0.392100036144257
0.354596465826035 0.352300012111664
0.382739186286926 0.320799964666367
0.398686587810516 0.28680008649826
0.423076987266541 0.260700064897537
0.445590943098068 0.236099997162819
0.456848055124283 0.211499996483326
0.472795516252518 0.187300005555153
0.48592871427536 0.165800000727177
0.499061465263367 0.146200004220009
0.512195110321045 0.125700011849403
0.529081225395203 0.11010000705719
0.539399445056915 0.0930000051856041
0.54596608877182 0.077899993956089
0.557223260402679 0.0641000013798475
0.56754207611084 0.0525999985635281
0.577861309051514 0.0433999918401241
0.585365653038025 0.0347000025212765
0.596622943878174 0.0268000012263656
0.604127943515778 0.0194000011309981
0.610694766044617 0.01539999935776
0.617261052131653 0.0117000013589859
0.622889220714569 0.00939999893307686
0.633208513259888 0.00720000038854778
0.64258873462677 0.0056000005453825
0.653846323490143 0.00399999944493175
0.663226902484894 0.00319999903440475
0.677298069000244 0.00259999909903854
0.682926833629608 0.00219999916153029
0.690431475639343 0.00159999969182536
0.695121586322784 0.00109999928390607
0.702626883983612 0.00049999967450276
0.707316994667053 0.00049999967450276
0.715759754180908 0.000399999739602208
0.723264515399933 0.000299999699927866
0.732645452022552 0.000199999869801104
0.741087913513184 0.000199999869801104
0.746716558933258 0.000199999869801104
0.753282845020294 9.9999934900552e-05
0.763602197170258 9.9999934900552e-05
0.767354428768158 0
0.770168721675873 0
0.778611838817596 0
0.783302366733551 0
0.788930356502533 0
0.795496881008148 0
0.799249529838562 0
0.805816113948822 0
0.810506463050842 0
0.818011224269867 0
0.825516104698181 0
0.831144452095032 0
0.836773097515106 0
0.844277679920197 0
0.846153676509857 0
0.852720379829407 0
0.858349025249481 0
0.862101256847382 0
0.867729842662811 0
0.869606018066406 0
0.876172423362732 0
0.879924893379211 0
0.884615421295166 0
0.888367712497711 0
0.893058061599731 0
0.896810472011566 0
0.898686707019806 0
0.904315173625946 0
0.909943640232086 0
0.911819756031036 0
0.913696050643921 0
0.915572226047516 0
0.921200811862946 0
0.923076987266541 0
0.926829278469086 0
0.929643452167511 0
0.933395981788635 0
0.936210155487061 0
0.941838681697845 0
0.944652915000916 0
0.947467088699341 0
0.951219499111176 0
0.95403379201889 0
0.959662318229675 0
0.96341460943222 0
0.96810507774353 0
0.97467166185379 0
0.97560977935791 0
0.977485954761505 0
0.97842401266098 0
0.97842401266098 0
0.98592871427536 0
0.991557240486145 0
0.991557240486145 0
0.994371473789215 0
0.99624764919281 0
0.998123824596405 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0183010846376419 0.481899815797806
0.031264204531908 0.429700005054474
0.0431599356234074 0.392100036144257
0.0553606785833836 0.352300012111664
0.067866250872612 0.320799964666367
0.0797619596123695 0.28680008649826
0.0921152606606483 0.260700064897537
0.104316085577011 0.236099997162819
0.116821698844433 0.211499996483326
0.128565222024918 0.187300005555153
0.137563288211823 0.165800000727177
0.146560579538345 0.146200004220009
0.157236590981483 0.125700011849403
0.170810043811798 0.11010000705719
0.181790560483932 0.0930000051856041
0.192008584737778 0.077899993956089
0.204971790313721 0.0641000013798475
0.215647339820862 0.0525999985635281
0.226932972669601 0.0433999918401241
0.236693561077118 0.0347000025212765
0.245996743440628 0.0268000012263656
0.25606232881546 0.0194000011309981
0.268415242433548 0.01539999935776
0.279395312070847 0.0117000013589859
0.29098641872406 0.00939999893307686
0.302882075309753 0.00720000038854778
0.313405454158783 0.0056000005453825
0.32331770658493 0.00399999944493175
0.334909111261368 0.00319999903440475
0.346194565296173 0.00259999909903854
0.356107950210571 0.00219999916153029
0.367241114377975 0.00159999969182536
0.378527283668518 0.00109999928390607
0.390574842691422 0.00049999967450276
0.401250571012497 0.00049999967450276
0.413146257400513 0.000399999739602208
0.423364460468292 0.000299999699927866
0.431905061006546 0.000199999869801104
0.443190485239029 0.000199999869801104
0.45493358373642 0.000199999869801104
0.466981828212738 9.9999934900552e-05
0.477962493896484 9.9999934900552e-05
0.4898581802845 0
0.501754879951477 0
0.513038277626038 0
0.522496223449707 0
0.532255887985229 0
0.543389499187469 0
0.553912043571472 0
0.564737975597382 0
0.574806571006775 0
0.584108948707581 0
0.592343389987946 0
0.600886285305023 0
0.609121024608612 0
0.618728458881378 0
0.628031313419342 0
0.639621317386627 0
0.647856652736664 0
0.663106501102448 0
0.674698054790497 0
0.683087348937988 0
0.692084789276123 0
0.702912330627441 0
0.71282571554184 0
0.724720120429993 0
0.735548913478851 0
0.745157837867737 0
0.754156410694122 0
0.764068782329559 0
0.773066818714142 0
0.781149923801422 0
0.789538025856018 0
0.798535943031311 0
0.806161224842072 0
0.815312027931213 0
0.823852837085724 0
0.832849621772766 0
0.841849148273468 0
0.850694358348846 0
0.857099592685699 0
0.865640223026276 0
0.874027669429779 0
0.881653189659119 0
0.888515949249268 0
0.897819340229034 0
0.905749440193176 0
0.912002444267273 0
0.918560028076172 0
0.927710771560669 0
0.935946345329285 0
0.945096850395203 0
0.950892090797424 0
0.958670139312744 0
0.965075492858887 0
0.973158478736877 0
0.979258716106415 0
0.986731708049774 0
0.993594646453857 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/chaffing3/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.289699226617813 0.550799489021301
0.311599940061569 0.452100187540054
0.328200668096542 0.402699917554855
0.342099338769913 0.373500257730484
0.35569965839386 0.353199809789658
0.365899682044983 0.342900395393372
0.376400142908096 0.335199952125549
0.387600392103195 0.331099510192871
0.396199554204941 0.329300582408905
0.405600100755692 0.32830074429512
0.414700001478195 0.327400684356689
0.423000037670135 0.326600581407547
0.431600302457809 0.324399799108505
0.440300285816193 0.32169970870018
0.447299897670746 0.318199872970581
0.456299901008606 0.312500715255737
0.464299917221069 0.304800301790237
0.471500098705292 0.29650029540062
0.480500012636185 0.286200404167175
0.486999988555908 0.275599747896194
0.492599993944168 0.265100181102753
0.499000579118729 0.256800174713135
0.506900072097778 0.25109937787056
0.514098942279816 0.244200006127357
0.522199213504791 0.239099949598312
0.52940046787262 0.235499933362007
0.536400139331818 0.233699902892113
0.543899834156036 0.231999978423119
0.551199197769165 0.231099933385849
0.557500183582306 0.230600044131279
0.563298463821411 0.229800030589104
0.569699883460999 0.229000151157379
0.577501118183136 0.228799909353256
0.584798634052277 0.228100001811981
0.591601490974426 0.2277000695467
0.598098754882812 0.2274000197649
0.604800224304199 0.226800054311752
0.611001014709473 0.226499885320663
0.617101192474365 0.225999996066093
0.62410181760788 0.225699946284294
0.631801128387451 0.225600093603134
0.639298677444458 0.225499853491783
0.646399021148682 0.225499853491783
0.653300404548645 0.225300043821335
0.659699499607086 0.225300043821335
0.665701150894165 0.225300043821335
0.672399878501892 0.225300043821335
0.678699910640717 0.225300043821335
0.684500098228455 0.225300043821335
0.691300094127655 0.225300043821335
0.696199893951416 0.225300043821335
0.702899992465973 0.225300043821335
0.709200739860535 0.225300043821335
0.714999735355377 0.225300043821335
0.721499681472778 0.225300043821335
0.728399276733398 0.225300043821335
0.734299957752228 0.225300043821335
0.741300821304321 0.225300043821335
0.74699878692627 0.225300043821335
0.755199909210205 0.225300043821335
0.761698067188263 0.225300043821335
0.766800463199615 0.225300043821335
0.773400664329529 0.225300043821335
0.781400442123413 0.225300043821335
0.787200093269348 0.225300043821335
0.795000076293945 0.225300043821335
0.803400099277496 0.225300043821335
0.808499932289124 0.225300043821335
0.814299523830414 0.225300043821335
0.819799482822418 0.225300043821335
0.825999200344086 0.225300043821335
0.832500219345093 0.225300043821335
0.838199615478516 0.225300043821335
0.844300091266632 0.225300043821335
0.848999440670013 0.225300043821335
0.854100167751312 0.225300043821335
0.860100209712982 0.225300043821335
0.865699708461761 0.225300043821335
0.870900809764862 0.225300043821335
0.875699043273926 0.225300043821335
0.880700469017029 0.225300043821335
0.886500120162964 0.225300043821335
0.893099904060364 0.225300043821335
0.899499595165253 0.225300043821335
0.905099987983704 0.225300043821335
0.911200165748596 0.225300043821335
0.917499423027039 0.225300043821335
0.924000203609467 0.225300043821335
0.930400013923645 0.225300043821335
0.936799824237823 0.225300043821335
0.943400382995605 0.225300043821335
0.949200093746185 0.225300043821335
0.954900205135345 0.225300043821335
0.96069997549057 0.225300043821335
0.967100203037262 0.225300043821335
0.972600102424622 0.225300043821335
0.978399813175201 0.225300043821335
0.984399974346161 0.225300043821335
0.991800010204315 0.225300043821335
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.992895185947418 0.550799489021301
0.992895185947418 0.452100187540054
0.993339240550995 0.402699917554855
0.993339240550995 0.373500257730484
0.993339240550995 0.353199809789658
0.993339240550995 0.342900395393372
0.993339240550995 0.335199952125549
0.993783295154572 0.331099510192871
0.993783295154572 0.329300582408905
0.993783295154572 0.32830074429512
0.993783295154572 0.327400684356689
0.993783295154572 0.326600581407547
0.993783295154572 0.324399799108505
0.993783295154572 0.32169970870018
0.993783295154572 0.318199872970581
0.993783295154572 0.312500715255737
0.994227349758148 0.304800301790237
0.994227349758148 0.29650029540062
0.994227349758148 0.286200404167175
0.994227349758148 0.275599747896194
0.994227349758148 0.265100181102753
0.994227349758148 0.256800174713135
0.994227349758148 0.25109937787056
0.994227349758148 0.244200006127357
0.994227349758148 0.239099949598312
0.994227349758148 0.235499933362007
0.994227349758148 0.233699902892113
0.994227349758148 0.231999978423119
0.994227349758148 0.231099933385849
0.994227349758148 0.230600044131279
0.994227349758148 0.229800030589104
0.994227349758148 0.229000151157379
0.994227349758148 0.228799909353256
0.994227349758148 0.228100001811981
0.994227349758148 0.2277000695467
0.994227349758148 0.2274000197649
0.994227349758148 0.226800054311752
0.994227349758148 0.226499885320663
0.994227349758148 0.225999996066093
0.994671404361725 0.225699946284294
0.994671404361725 0.225600093603134
0.994671404361725 0.225499853491783
0.994671404361725 0.225499853491783
0.995115458965302 0.225300043821335
0.995559513568878 0.225300043821335
0.996003568172455 0.225300043821335
0.996003568172455 0.225300043821335
0.996003568172455 0.225300043821335
0.996003568172455 0.225300043821335
0.996003568172455 0.225300043821335
0.996003568172455 0.225300043821335
0.996003568172455 0.225300043821335
0.996003568172455 0.225300043821335
0.996447622776031 0.225300043821335
0.996447622776031 0.225300043821335
0.996447622776031 0.225300043821335
0.996447622776031 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.996891677379608 0.225300043821335
0.997779726982117 0.225300043821335
0.997779726982117 0.225300043821335
0.997779726982117 0.225300043821335
0.998223781585693 0.225300043821335
0.998223781585693 0.225300043821335
0.998223781585693 0.225300043821335
0.998223781585693 0.225300043821335
0.99866783618927 0.225300043821335
0.99866783618927 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999111890792847 0.225300043821335
0.999555945396423 0.225300043821335
0.999555945396423 0.225300043821335
0.999555945396423 0.225300043821335
0.999555945396423 0.225300043821335
1 0.225300043821335
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.381040722131729 0.550799489021301
0.452602237462997 0.452100187540054
0.49442395567894 0.402699917554855
0.515799283981323 0.373500257730484
0.532527208328247 0.353199809789658
0.546468496322632 0.342900395393372
0.563197135925293 0.335199952125549
0.580855071544647 0.331099510192871
0.587361335754395 0.329300582408905
0.600371778011322 0.32830074429512
0.607806384563446 0.327400684356689
0.614312410354614 0.326600581407547
0.625465154647827 0.324399799108505
0.633828818798065 0.32169970870018
0.639405846595764 0.318199872970581
0.646840155124664 0.312500715255737
0.654275059700012 0.304800301790237
0.662639439105988 0.29650029540062
0.671003401279449 0.286200404167175
0.673791527748108 0.275599747896194
0.676580190658569 0.265100181102753
0.678438663482666 0.256800174713135
0.685873627662659 0.25109937787056
0.691449820995331 0.244200006127357
0.698884963989258 0.239099949598312
0.704460918903351 0.235499933362007
0.712825298309326 0.233699902892113
0.723977565765381 0.231999978423119
0.730482935905457 0.231099933385849
0.73698890209198 0.230600044131279
0.741635382175446 0.229800030589104
0.749070823192596 0.229000151157379
0.751858651638031 0.228799909353256
0.755576074123383 0.228100001811981
0.761152803897858 0.2277000695467
0.768587589263916 0.2274000197649
0.772305250167847 0.226800054311752
0.778810381889343 0.226499885320663
0.788104116916656 0.225999996066093
0.791821718215942 0.225699946284294
0.797397971153259 0.225600093603134
0.801115274429321 0.225499853491783
0.803903460502625 0.225499853491783
0.803903460502625 0.225300043821335
0.807620942592621 0.225300043821335
0.809479355812073 0.225300043821335
0.813197076320648 0.225300043821335
0.817843914031982 0.225300043821335
0.820632040500641 0.225300043821335
0.824349582195282 0.225300043821335
0.826208293437958 0.225300043821335
0.83178436756134 0.225300043821335
0.836431205272675 0.225300043821335
0.837360620498657 0.225300043821335
0.842007339000702 0.225300043821335
0.845724940299988 0.225300043821335
0.848512947559357 0.225300043821335
0.85316002368927 0.225300043821335
0.856877446174622 0.225300043821335
0.858736157417297 0.225300043821335
0.862453639507294 0.225300043821335
0.866171002388 0.225300043821335
0.872676610946655 0.225300043821335
0.8773233294487 0.225300043821335
0.881970345973969 0.225300043821335
0.885687828063965 0.225300043821335
0.890334486961365 0.225300043821335
0.894052028656006 0.225300043821335
0.895910799503326 0.225300043821335
0.899628281593323 0.225300043821335
0.902416348457336 0.225300043821335
0.906133770942688 0.225300043821335
0.907992660999298 0.225300043821335
0.908921957015991 0.225300043821335
0.910780668258667 0.225300043821335
0.911710023880005 0.225300043821335
0.916356861591339 0.225300043821335
0.919145107269287 0.225300043821335
0.922862470149994 0.225300043821335
0.92657995223999 0.225300043821335
0.931226789951324 0.225300043821335
0.936802983283997 0.225300043821335
0.939590990543365 0.225300043821335
0.945167243480682 0.225300043821335
0.949814200401306 0.225300043821335
0.956319689750671 0.225300043821335
0.95910781621933 0.225300043821335
0.962825298309326 0.225300043821335
0.969330847263336 0.225300043821335
0.970260202884674 0.225300043821335
0.973048210144043 0.225300043821335
0.975836455821991 0.225300043821335
0.977695167064667 0.225300043821335
0.982342004776001 0.225300043821335
0.986988842487335 0.225300043821335
0.986988842487335 0.225300043821335
0.991635680198669 0.225300043821335
0.994423806667328 0.225300043821335
0.996282517910004 0.225300043821335
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0376199334859848 0.550799489021301
0.0589029416441917 0.452100187540054
0.0768887624144554 0.402699917554855
0.0942745804786682 0.373500257730484
0.111960485577583 0.353199809789658
0.124999545514584 0.342900395393372
0.138039246201515 0.335199952125549
0.151827901601791 0.331099510192871
0.163669496774673 0.329300582408905
0.175659149885178 0.32830074429512
0.18809974193573 0.327400684356689
0.199490189552307 0.326600581407547
0.210581436753273 0.324399799108505
0.222272261977196 0.32169970870018
0.231864526867867 0.318199872970581
0.244154423475266 0.312500715255737
0.254796028137207 0.304800301790237
0.264237701892853 0.29650029540062
0.276378452777863 0.286200404167175
0.285671383142471 0.275599747896194
0.293614685535431 0.265100181102753
0.302907317876816 0.256800174713135
0.313549160957336 0.25109937787056
0.323440730571747 0.244200006127357
0.334382385015488 0.239099949598312
0.344275087118149 0.235499933362007
0.353417336940765 0.233699902892113
0.362859845161438 0.231999978423119
0.372752159833908 0.231099933385849
0.381145119667053 0.230600044131279
0.389088988304138 0.229800030589104
0.397481709718704 0.229000151157379
0.408723086118698 0.228799909353256
0.419064462184906 0.228100001811981
0.428357362747192 0.2277000695467
0.436900347471237 0.2274000197649
0.446342885494232 0.226800054311752
0.454586207866669 0.226499885320663
0.462230265140533 0.225999996066093
0.471972435712814 0.225699946284294
0.482613861560822 0.225600093603134
0.493255436420441 0.225499853491783
0.503446638584137 0.225499853491783
0.513639211654663 0.225300043821335
0.522484302520752 0.225300043821335
0.531024873256683 0.225300043821335
0.540468752384186 0.225300043821335
0.549159646034241 0.225300043821335
0.557403087615967 0.225300043821335
0.5669966340065 0.225300043821335
0.574041306972504 0.225300043821335
0.583182275295258 0.225300043821335
0.591875493526459 0.225300043821335
0.600269079208374 0.225300043821335
0.60926228761673 0.225300043821335
0.619004845619202 0.225300043821335
0.62739759683609 0.225300043821335
0.636991560459137 0.225300043821335
0.644933819770813 0.225300043821335
0.656926512718201 0.225300043821335
0.666066467761993 0.225300043821335
0.673111379146576 0.225300043821335
0.681954801082611 0.225300043821335
0.693195521831512 0.225300043821335
0.701139807701111 0.225300043821335
0.71222996711731 0.225300043821335
0.72407066822052 0.225300043821335
0.731114566326141 0.225300043821335
0.739208459854126 0.225300043821335
0.746852815151215 0.225300043821335
0.755695521831512 0.225300043821335
0.764688849449158 0.225300043821335
0.772930979728699 0.225300043821335
0.781924486160278 0.225300043821335
0.788668632507324 0.225300043821335
0.796013176441193 0.225300043821335
0.804257154464722 0.225300043821335
0.812050700187683 0.225300043821335
0.819244801998138 0.225300043821335
0.825838983058929 0.225300043821335
0.832584083080292 0.225300043821335
0.840377390384674 0.225300043821335
0.84982043504715 0.225300043821335
0.858513474464417 0.225300043821335
0.866156756877899 0.225300043821335
0.874250471591949 0.225300043821335
0.883243083953857 0.225300043821335
0.892386376857758 0.225300043821335
0.900929093360901 0.225300043821335
0.910371541976929 0.225300043821335
0.919814229011536 0.225300043821335
0.928057551383972 0.225300043821335
0.936300933361053 0.225300043821335
0.944244623184204 0.225300043821335
0.952937662601471 0.225300043821335
0.961181044578552 0.225300043821335
0.969124674797058 0.225300043821335
0.97766786813736 0.225300043821335
0.988309323787689 0.225300043821335
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/chaffing3/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.343300670385361 0.402500867843628
0.395400017499924 0.335199266672134
0.441099911928177 0.305500060319901
0.481700092554092 0.279700666666031
0.519600629806519 0.258600443601608
0.555598855018616 0.243300005793571
0.591200232505798 0.233800023794174
0.624100029468536 0.228499948978424
0.654600501060486 0.226400002837181
0.687199413776398 0.225899994373322
0.718699276447296 0.225499853491783
0.751100361347198 0.225300043821335
0.781699597835541 0.225300043821335
0.816299319267273 0.225300043821335
0.848300576210022 0.225300043821335
0.877600371837616 0.225300043821335
0.908499896526337 0.225300043821335
0.937699794769287 0.225300043821335
0.968800008296967 0.225300043821335
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.997768878936768 0.402500867843628
0.997768878936768 0.335199266672134
0.997768878936768 0.305500060319901
0.997768878936768 0.279700666666031
0.997768878936768 0.258600443601608
0.998215079307556 0.243300005793571
0.998215079307556 0.233800023794174
0.998215079307556 0.228499948978424
0.998215079307556 0.226400002837181
0.998215079307556 0.225899994373322
0.99866133928299 0.225499853491783
0.99866133928299 0.225300043821335
0.99866133928299 0.225300043821335
0.99866133928299 0.225300043821335
0.999107539653778 0.225300043821335
0.999107539653778 0.225300043821335
0.999107539653778 0.225300043821335
0.999107539653778 0.225300043821335
0.999553799629211 0.225300043821335
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.573319315910339 0.402500867843628
0.671444714069366 0.335199266672134
0.716648578643799 0.305500060319901
0.749724090099335 0.279700666666031
0.777287840843201 0.258600443601608
0.799338757991791 0.243300005793571
0.818081498146057 0.233800023794174
0.841234683990479 0.228499948978424
0.855567753314972 0.226400002837181
0.867695689201355 0.225899994373322
0.876515865325928 0.225499853491783
0.8886439204216 0.225300043821335
0.898566722869873 0.225300043821335
0.919514894485474 0.225300043821335
0.930540263652802 0.225300043821335
0.941565573215485 0.225300043821335
0.96361631155014 0.225300043821335
0.974641680717468 0.225300043821335
0.986769556999207 0.225300043821335
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0988032892346382 0.402500867843628
0.161850735545158 0.335199266672134
0.222562715411186 0.305500060319901
0.277437269687653 0.279700666666031
0.329100459814072 0.258600443601608
0.37857574224472 0.243300005793571
0.428050130605698 0.233800023794174
0.473000466823578 0.228499948978424
0.515616893768311 0.226400002837181
0.561588287353516 0.225899994373322
0.606245338916779 0.225499853491783
0.65192711353302 0.225300043821335
0.695271730422974 0.225300043821335
0.742995023727417 0.225300043821335
0.788091778755188 0.225300043821335
0.829392731189728 0.225300043821335
0.871570348739624 0.225300043821335
0.91272634267807 0.225300043821335
0.956363201141357 0.225300043821335
};
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/chaffing4/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.302199721336365 0.274699330329895
0.325200438499451 0.225300043821335
0.341300249099731 0.205700054764748
0.353499501943588 0.192499652504921
0.365200102329254 0.183899968862534
0.375900059938431 0.176200076937675
0.386599957942963 0.164900302886963
0.396499752998352 0.146499842405319
0.406599789857864 0.125900089740753
0.415600478649139 0.101899996399879
0.423699915409088 0.0794001072645187
0.431499511003494 0.0564999803900719
0.439599990844727 0.0366000272333622
0.446999907493591 0.0228000469505787
0.455699890851974 0.0133999921381474
0.464000105857849 0.00719998404383659
0.471700102090836 0.00310000218451023
0.477899938821793 0.00109999882988632
0.485799998044968 0.000399999058572575
0.492699891328812 0.000199999529286288
0.498400151729584 9.99997646431439e-05
0.504400730133057 0
0.511200189590454 0
0.517798900604248 0
0.524999797344208 0
0.532901763916016 0
0.540498614311218 0
0.548500418663025 0
0.556698679924011 0
0.563600540161133 0
0.570201396942139 0
0.576299548149109 0
0.582498848438263 0
0.589002251625061 0
0.59449976682663 0
0.601599514484406 0
0.607901811599731 0
0.614298045635223 0
0.620999813079834 0
0.627199590206146 0
0.633401274681091 0
0.640298843383789 0
0.646099805831909 0
0.653799891471863 0
0.660200119018555 0
0.666000008583069 0
0.671799600124359 0
0.67790013551712 0
0.6842001080513 0
0.69100022315979 0
0.697600185871124 0
0.703399419784546 0
0.70930027961731 0
0.715699553489685 0
0.721999049186707 0
0.727698087692261 0
0.734400808811188 0
0.740900158882141 0
0.746200025081635 0
0.75379878282547 0
0.76000052690506 0
0.765600264072418 0
0.773098945617676 0
0.779999613761902 0
0.78519994020462 0
0.792999923229218 0
0.799499452114105 0
0.803698360919952 0
0.809902310371399 0
0.815099656581879 0
0.821200609207153 0
0.827600181102753 0
0.833000004291534 0
0.838199615478516 0
0.844399631023407 0
0.850098848342896 0
0.856499791145325 0
0.861699819564819 0
0.867800176143646 0
0.874599635601044 0
0.880099892616272 0
0.885999798774719 0
0.892200589179993 0
0.897800087928772 0
0.903999805450439 0
0.910099804401398 0
0.916099488735199 0
0.921799778938293 0
0.928099811077118 0
0.933600008487701 0
0.939899981021881 0
0.947399795055389 0
0.951899826526642 0
0.958999931812286 0
0.965299785137177 0
0.972899973392487 0
0.979200124740601 0
0.986800014972687 0
0.993099987506866 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.992895185947418 0.274699330329895
0.992895185947418 0.225300043821335
0.993339240550995 0.205700054764748
0.993339240550995 0.192499652504921
0.993339240550995 0.183899968862534
0.993339240550995 0.176200076937675
0.993339240550995 0.164900302886963
0.993783295154572 0.146499842405319
0.993783295154572 0.125900089740753
0.993783295154572 0.101899996399879
0.993783295154572 0.0794001072645187
0.993783295154572 0.0564999803900719
0.993783295154572 0.0366000272333622
0.993783295154572 0.0228000469505787
0.993783295154572 0.0133999921381474
0.993783295154572 0.00719998404383659
0.994227349758148 0.00310000218451023
0.994227349758148 0.00109999882988632
0.994227349758148 0.000399999058572575
0.994227349758148 0.000199999529286288
0.994227349758148 9.99997646431439e-05
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994227349758148 0
0.994671404361725 0
0.994671404361725 0
0.994671404361725 0
0.994671404361725 0
0.995115458965302 0
0.995559513568878 0
0.996003568172455 0
0.996003568172455 0
0.996003568172455 0
0.996003568172455 0
0.996003568172455 0
0.996003568172455 0
0.996003568172455 0
0.996003568172455 0
0.996447622776031 0
0.996447622776031 0
0.996447622776031 0
0.996447622776031 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.996891677379608 0
0.997779726982117 0
0.997779726982117 0
0.997779726982117 0
0.998223781585693 0
0.998223781585693 0
0.998223781585693 0
0.998223781585693 0
0.99866783618927 0
0.99866783618927 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999111890792847 0
0.999555945396423 0
0.999555945396423 0
0.999555945396423 0
0.999555945396423 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.464879930019379 0.274699330329895
0.527726411819458 0.225300043821335
0.55267995595932 0.205700054764748
0.566543638706207 0.192499652504921
0.580406725406647 0.183899968862534
0.593345403671265 0.176200076937675
0.606284856796265 0.164900302886963
0.611829459667206 0.146499842405319
0.623844563961029 0.125900089740753
0.634011089801788 0.101899996399879
0.640480697154999 0.0794001072645187
0.646026134490967 0.0564999803900719
0.656191885471344 0.0366000272333622
0.666358411312103 0.0228000469505787
0.671903908252716 0.0133999921381474
0.680221676826477 0.00719998404383659
0.685767352581024 0.00310000218451023
0.692236423492432 0.00109999882988632
0.698706328868866 0.000399999058572575
0.703327417373657 0.000199999529286288
0.705175817012787 9.99997646431439e-05
0.707948327064514 0
0.712569296360016 0
0.717190563678741 0
0.722735583782196 0
0.73012900352478 0
0.735674679279327 0
0.743992269039154 0
0.747689187526703 0
0.754159033298492 0
0.758779942989349 0
0.762476742267609 0
0.767097890377045 0
0.769870400428772 0
0.774491369724274 0
0.784658193588257 0
0.786506354808807 0
0.79390025138855 0
0.800369620323181 0
0.804066836833954 0
0.806839287281036 0
0.811460256576538 0
0.811460256576538 0
0.813308537006378 0
0.81608122587204 0
0.817005515098572 0
0.817929685115814 0
0.819778323173523 0
0.82439923286438 0
0.829020440578461 0
0.830868780612946 0
0.835489928722382 0
0.841035306453705 0
0.841959178447723 0
0.846580266952515 0
0.851201236248016 0
0.8548983335495 0
0.857671022415161 0
0.860443651676178 0
0.86136782169342 0
0.863216400146484 0
0.865988969802856 0
0.871534109115601 0
0.874306857585907 0
0.878927826881409 0
0.882624626159668 0
0.885397374629974 0
0.888169944286346 0
0.889094352722168 0
0.892791211605072 0
0.895563662052155 0
0.899260640144348 0
0.902033150196075 0
0.903881907463074 0
0.909426808357239 0
0.911275386810303 0
0.917744934558868 0
0.919593274593353 0
0.922365963459015 0
0.925138771533966 0
0.93068391084671 0
0.934380769729614 0
0.939925968647003 0
0.94454699754715 0
0.94916820526123 0
0.954713463783264 0
0.958410322666168 0
0.962107181549072 0
0.968576729297638 0
0.96950089931488 0
0.971349358558655 0
0.972273588180542 0
0.97319769859314 0
0.976894617080688 0
0.983364164829254 0
0.986136794090271 0
0.989833652973175 0
0.994454741477966 0
0.996303141117096 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0424541980028152 0.274699330329895
0.0667566359043121 0.225300043821335
0.0867087095975876 0.205700054764748
0.102760300040245 0.192499652504921
0.118061758577824 0.183899968862534
0.132013201713562 0.176200076937675
0.145964965224266 0.164900302886963
0.159766048192978 0.146499842405319
0.172967284917831 0.125900089740753
0.184818372130394 0.101899996399879
0.195919632911682 0.0794001072645187
0.206720739603043 0.0564999803900719
0.21722187101841 0.0366000272333622
0.226672664284706 0.0228000469505787
0.238823875784874 0.0133999921381474
0.249925911426544 0.00719998404383659
0.260426700115204 0.00310000218451023
0.268676459789276 0.00109999882988632
0.279477953910828 0.000399999058572575
0.289079278707504 0.000199999529286288
0.297329276800156 9.99997646431439e-05
0.305881053209305 0
0.315331518650055 0
0.324482440948486 0
0.334382742643356 0
0.345034658908844 0
0.355535447597504 0
0.366186589002609 0
0.37788799405098 0
0.387188732624054 0
0.396339625120163 0
0.404890209436417 0
0.413441270589828 0
0.42274209856987 0
0.430242925882339 0
0.439244002103806 0
0.44839483499527 0
0.45679560303688 0
0.465796500444412 0
0.474347442388535 0
0.483198314905167 0
0.492799252271652 0
0.501500010490417 0
0.512600362300873 0
0.521603047847748 0
0.5300013422966 0
0.538554251194 0
0.547407329082489 0
0.556104838848114 0
0.565556108951569 0
0.575157284736633 0
0.583108603954315 0
0.591059029102325 0
0.60036039352417 0
0.609059989452362 0
0.616860926151276 0
0.626314163208008 0
0.635465025901794 0
0.642964005470276 0
0.654214978218079 0
0.663215577602386 0
0.671167254447937 0
0.681519031524658 0
0.691417992115021 0
0.698469400405884 0
0.709572434425354 0
0.718871891498566 0
0.724722445011139 0
0.733572602272034 0
0.740774154663086 0
0.749475240707397 0
0.758326768875122 0
0.765976369380951 0
0.773477613925934 0
0.781877756118774 0
0.789979875087738 0
0.79852968454361 0
0.805880010128021 0
0.814581036567688 0
0.824333012104034 0
0.831682860851288 0
0.839934408664703 0
0.848334550857544 0
0.855985283851624 0
0.864536464214325 0
0.872787594795227 0
0.881188094615936 0
0.88913905620575 0
0.897539973258972 0
0.905640721321106 0
0.914791345596313 0
0.92589259147644 0
0.932493090629578 0
0.942544281482697 0
0.95079517364502 0
0.961746156215668 0
0.970597088336945 0
0.981248140335083 0
0.990249037742615 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/combination/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.381300151348114 0.672300815582275
0.40350005030632 0.654898822307587
0.419600188732147 0.60140073299408
0.432600110769272 0.511098682880402
0.446600049734116 0.3915995657444
0.456200301647186 0.265998989343643
0.466199994087219 0.161499932408333
0.477500051259995 0.0861999616026878
0.488000005483627 0.0430999584496021
0.497800529003143 0.0186999924480915
0.507598996162415 0.00799999851733446
0.517098069190979 0.00290000275708735
0.527200996875763 0.000999999232590199
0.534899115562439 9.99997646431439e-05
0.544100821018219 9.99997646431439e-05
0.554798483848572 0
0.564200162887573 0
0.570399045944214 0
0.578001499176025 0
0.58449798822403 0
0.592498302459717 0
0.598500430583954 0
0.608398973941803 0
0.615902602672577 0
0.624300062656403 0
0.630701541900635 0
0.636898458003998 0
0.64439994096756 0
0.650799691677094 0
0.657300114631653 0
0.663499712944031 0
0.670200705528259 0
0.676898658275604 0
0.682599425315857 0
0.688400030136108 0
0.693399965763092 0
0.699701249599457 0
0.705600559711456 0
0.711099743843079 0
0.71820056438446 0
0.72390079498291 0
0.731201171875 0
0.738099098205566 0
0.744199216365814 0
0.750000178813934 0
0.75510036945343 0
0.761100649833679 0
0.767001390457153 0
0.772900223731995 0
0.777799785137177 0
0.78279983997345 0
0.789400219917297 0
0.793000519275665 0
0.796700835227966 0
0.802698314189911 0
0.808999538421631 0
0.814100623130798 0
0.820699036121368 0
0.825899004936218 0
0.831900000572205 0
0.837301552295685 0
0.841400027275085 0
0.846599400043488 0
0.852700591087341 0
0.856699824333191 0
0.861299633979797 0
0.86679881811142 0
0.871900200843811 0
0.877000272274017 0
0.881300568580627 0
0.886399388313293 0
0.891099810600281 0
0.895699977874756 0
0.899699211120605 0
0.90449982881546 0
0.907700181007385 0
0.911500215530396 0
0.915899813175201 0
0.921400189399719 0
0.925800025463104 0
0.930099785327911 0
0.93500030040741 0
0.939300119876862 0
0.942600071430206 0
0.945699989795685 0
0.94980001449585 0
0.954500019550323 0
0.958199918270111 0
0.961900174617767 0
0.964999794960022 0
0.969200015068054 0
0.97350001335144 0
0.976599812507629 0
0.980099976062775 0
0.983799874782562 0
0.98769998550415 0
0.991599977016449 0
0.994700014591217 0
0.997600018978119 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.985008835792542 0.672300815582275
0.987654328346252 0.654898822307587
0.988095223903656 0.60140073299408
0.988095223903656 0.511098682880402
0.988977074623108 0.3915995657444
0.989417970180511 0.265998989343643
0.989417970180511 0.161499932408333
0.990299820899963 0.0861999616026878
0.990740716457367 0.0430999584496021
0.990740716457367 0.0186999924480915
0.991181671619415 0.00799999851733446
0.991622567176819 0.00290000275708735
0.991622567176819 0.000999999232590199
0.991622567176819 9.99997646431439e-05
0.992063462734222 9.99997646431439e-05
0.992063462734222 0
0.992504417896271 0
0.992504417896271 0
0.992504417896271 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.992945313453674 0
0.993386268615723 0
0.993386268615723 0
0.993386268615723 0
0.993827164173126 0
0.993827164173126 0
0.993827164173126 0
0.993827164173126 0
0.99426805973053 0
0.994709014892578 0
0.995149910449982 0
0.995149910449982 0
0.995149910449982 0
0.995149910449982 0
0.995149910449982 0
0.995149910449982 0
0.995149910449982 0
0.995149910449982 0
0.995590806007385 0
0.995590806007385 0
0.995590806007385 0
0.995590806007385 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.996472656726837 0
0.997354507446289 0
0.997354507446289 0
0.997795403003693 0
0.998236358165741 0
0.998236358165741 0
0.998236358165741 0
0.998236358165741 0
0.998677253723145 0
0.998677253723145 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999118149280548 0
0.999559104442596 0
0.999559104442596 0
0.999559104442596 0
0.999559104442596 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.525151968002319 0.672300815582275
0.563262522220612 0.654898822307587
0.583078920841217 0.60140073299408
0.597560703754425 0.511098682880402
0.608231961727142 0.3915995657444
0.61814022064209 0.265998989343643
0.631859540939331 0.161499932408333
0.644054591655731 0.0861999616026878
0.651676714420319 0.0430999584496021
0.659298777580261 0.0186999924480915
0.669207155704498 0.00799999851733446
0.674543082714081 0.00290000275708735
0.682164788246155 0.000999999232590199
0.695122241973877 9.99997646431439e-05
0.700457990169525 9.99997646431439e-05
0.705793261528015 0
0.711889386177063 0
0.716463565826416 0
0.722561180591583 0
0.724847555160522 0
0.727896451950073 0
0.727896451950073 0
0.734755575656891 0
0.74009120464325 0
0.746189653873444 0
0.753811001777649 0
0.760671079158783 0
0.7690549492836 0
0.775152325630188 0
0.782773852348328 0
0.785823345184326 0
0.790395975112915 0
0.798018097877502 0
0.802590906620026 0
0.805640816688538 0
0.810213625431061 0
0.815548598766327 0
0.819359958171844 0
0.824695289134979 0
0.830030739307404 0
0.833079159259796 0
0.837652504444122 0
0.841463208198547 0
0.842225611209869 0
0.844512224197388 0
0.846036970615387 0
0.84908539056778 0
0.852133989334106 0
0.855945110321045 0
0.861280500888824 0
0.863566875457764 0
0.869664430618286 0
0.873475611209869 0
0.875762462615967 0
0.878048598766327 0
0.883383989334106 0
0.886432766914368 0
0.889481604099274 0
0.891006112098694 0
0.893292486667633 0
0.895579278469086 0
0.897865831851959 0
0.903201401233673 0
0.90625 0
0.909298956394196 0
0.91158539056778 0
0.915396630764008 0
0.917682945728302 0
0.918445110321045 0
0.920731723308563 0
0.924542784690857 0
0.926829278469086 0
0.929115772247314 0
0.93064022064209 0
0.935213387012482 0
0.936737775802612 0
0.940548956394196 0
0.94283539056778 0
0.944359660148621 0
0.945121943950653 0
0.948932766914368 0
0.951981604099274 0
0.954268276691437 0
0.957317054271698 0
0.958841443061829 0
0.96341460943222 0
0.967987775802612 0
0.971036612987518 0
0.975609660148621 0
0.976371884346008 0
0.978658556938171 0
0.980182945728302 0
0.983231723308563 0
0.986280500888824 0
0.989329278469086 0
0.990853667259216 0
0.993902444839478 0
0.996951222419739 0
0.996951222419739 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0451713651418686 0.672300815582275
0.0758566856384277 0.654898822307587
0.0987538546323776 0.60140073299408
0.119158737361431 0.511098682880402
0.14143317937851 0.3915995657444
0.156697943806648 0.265998989343643
0.17149506509304 0.161499932408333
0.189096614718437 0.0861999616026878
0.206853702664375 0.0430999584496021
0.222897201776505 0.0186999924480915
0.237850576639175 0.00799999851733446
0.253427356481552 0.00290000275708735
0.269003421068192 0.000999999232590199
0.279594987630844 9.99997646431439e-05
0.296261370182037 9.99997646431439e-05
0.313396275043488 0
0.328192412853241 0
0.337851077318192 0
0.350311607122421 0
0.362461298704147 0
0.376946955919266 0
0.387850403785706 0
0.40404999256134 0
0.415264785289764 0
0.428660422563553 0
0.439252227544785 0
0.448753893375397 0
0.459034264087677 0
0.469158947467804 0
0.478660434484482 0
0.488940924406052 0
0.499844133853912 0
0.510281264781952 0
0.517757058143616 0
0.528348386287689 0
0.536292672157288 0
0.545795321464539 0
0.554986536502838 0
0.562770843505859 0
0.573676645755768 0
0.58317643404007 0
0.593613266944885 0
0.604516804218292 0
0.614329278469086 0
0.623364686965942 0
0.63162088394165 0
0.641122162342072 0
0.650935113430023 0
0.660591423511505 0
0.668223679065704 0
0.675700485706329 0
0.685670375823975 0
0.69158923625946 0
0.697508454322815 0
0.707008898258209 0
0.716042995452881 0
0.724143326282501 0
0.734267354011536 0
0.743301808834076 0
0.752959072589874 0
0.761994063854218 0
0.768068850040436 0
0.775700151920319 0
0.784891426563263 0
0.790809750556946 0
0.797662794589996 0
0.805918991565704 0
0.813707232475281 0
0.821339845657349 0
0.827570080757141 0
0.835046827793121 0
0.842211842536926 0
0.849221408367157 0
0.854984402656555 0
0.861526310443878 0
0.866199672222137 0
0.871807336807251 0
0.878348886966705 0
0.886915981769562 0
0.893769443035126 0
0.89984393119812 0
0.907009482383728 0
0.913707137107849 0
0.918379902839661 0
0.923052966594696 0
0.928660452365875 0
0.935202777385712 0
0.940342664718628 0
0.945171177387238 0
0.949999988079071 0
0.956386268138885 0
0.962928354740143 0
0.967289626598358 0
0.972118377685547 0
0.976947069168091 0
0.982710182666779 0
0.988317728042603 0
0.992523372173309 0
0.996884763240814 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/combination_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.311399936676025 0.666599333286285
0.327299684286118 0.645500481128693
0.339299947023392 0.610400021076202
0.350099802017212 0.56150233745575
0.362399458885193 0.50080019235611
0.373499929904938 0.437599986791611
0.384499996900558 0.365899711847305
0.393399387598038 0.303199887275696
0.403699606657028 0.244999945163727
0.412999898195267 0.197400093078613
0.420999467372894 0.164300099015236
0.430000305175781 0.13670040667057
0.438999712467194 0.114200010895729
0.447699695825577 0.0963999480009079
0.455599904060364 0.0770998671650887
0.465000003576279 0.060300026088953
0.475700050592422 0.0450998693704605
0.483000099658966 0.0338000133633614
0.490600049495697 0.0250999815762043
0.49719974398613 0.0170999858528376
0.50519996881485 0.0113000040873885
0.511899173259735 0.00729999830946326
0.518599271774292 0.00470001250505447
0.526202440261841 0.00380000146105886
0.534102320671082 0.00269999913871288
0.54059773683548 0.00129999942146242
0.546798408031464 0.000899998878594488
0.555001735687256 0.000299999490380287
0.563199877738953 0
0.571101069450378 0
0.576799035072327 0
0.583698689937592 0
0.589800417423248 0
0.597000539302826 0
0.603500306606293 0
0.611599266529083 0
0.618898212909698 0
0.625400841236115 0
0.63150030374527 0
0.638799846172333 0
0.646001040935516 0
0.654201328754425 0
0.661300957202911 0
0.667799353599548 0
0.674499213695526 0
0.681399047374725 0
0.688500046730042 0
0.69489973783493 0
0.701000273227692 0
0.708398461341858 0
0.71390026807785 0
0.720399439334869 0
0.726099371910095 0
0.731900334358215 0
0.737998247146606 0
0.744700610637665 0
0.749899983406067 0
0.756499886512756 0
0.762099385261536 0
0.770199000835419 0
0.776800692081451 0
0.782001733779907 0
0.789099991321564 0
0.796001255512238 0
0.80269992351532 0
0.809499382972717 0
0.817499160766602 0
0.822700798511505 0
0.828700184822083 0
0.834699213504791 0
0.840300798416138 0
0.846400022506714 0
0.851999580860138 0
0.85699999332428 0
0.862000584602356 0
0.866999506950378 0
0.873400211334229 0
0.878399789333344 0
0.884500205516815 0
0.890600383281708 0
0.896100103855133 0
0.902999997138977 0
0.909000217914581 0
0.914499998092651 0
0.919299602508545 0
0.925399780273438 0
0.930899977684021 0
0.936299800872803 0
0.941700100898743 0
0.947499930858612 0
0.953900218009949 0
0.959299981594086 0
0.962900221347809 0
0.9689000248909 0
0.973900020122528 0
0.978500008583069 0
0.98470002412796 0
0.990000009536743 0
0.995100021362305 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.991130828857422 0.666599333286285
0.99201774597168 0.645500481128693
0.992904663085938 0.610400021076202
0.992904663085938 0.56150233745575
0.992904663085938 0.50080019235611
0.992904663085938 0.437599986791611
0.992904663085938 0.365899711847305
0.993348121643066 0.303199887275696
0.993348121643066 0.244999945163727
0.993348121643066 0.197400093078613
0.993348121643066 0.164300099015236
0.993348121643066 0.13670040667057
0.993348121643066 0.114200010895729
0.993348121643066 0.0963999480009079
0.993348121643066 0.0770998671650887
0.993348121643066 0.060300026088953
0.993791580200195 0.0450998693704605
0.993791580200195 0.0338000133633614
0.993791580200195 0.0250999815762043
0.994235038757324 0.0170999858528376
0.994235038757324 0.0113000040873885
0.994235038757324 0.00729999830946326
0.994235038757324 0.00470001250505447
0.994235038757324 0.00380000146105886
0.994235038757324 0.00269999913871288
0.994235038757324 0.00129999942146242
0.994235038757324 0.000899998878594488
0.994235038757324 0.000299999490380287
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994235038757324 0
0.994678497314453 0
0.994678497314453 0
0.994678497314453 0
0.994678497314453 0
0.995121955871582 0
0.995565414428711 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.99600887298584 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996452331542969 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.996895790100098 0
0.997782707214355 0
0.997782707214355 0
0.997782707214355 0
0.998226165771484 0
0.998226165771484 0
0.998226165771484 0
0.998226165771484 0
0.998669624328613 0
0.998669624328613 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999113082885742 0
0.999556541442871 0
0.999556541442871 0
0.999556541442871 0
0.999556541442871 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.517162442207336 0.666599333286285
0.540045559406281 0.645500481128693
0.561403214931488 0.610400021076202
0.576659083366394 0.56150233745575
0.588863968849182 0.50080019235611
0.603356182575226 0.437599986791611
0.615561068058014 0.365899711847305
0.622425556182861 0.303199887275696
0.630053699016571 0.244999945163727
0.637680888175964 0.197400093078613
0.648360192775726 0.164300099015236
0.655987977981567 0.13670040667057
0.664378523826599 0.114200010895729
0.677345514297485 0.0963999480009079
0.682685256004333 0.0770998671650887
0.689549505710602 0.060300026088953
0.698703289031982 0.0450998693704605
0.704805970191956 0.0338000133633614
0.710908055305481 0.0250999815762043
0.714721500873566 0.0170999858528376
0.72082382440567 0.0113000040873885
0.721586465835571 0.00729999830946326
0.727688848972321 0.00470001250505447
0.734553694725037 0.00380000146105886
0.740655839443207 0.00269999913871288
0.747520565986633 0.00129999942146242
0.751335203647614 0.000899998878594488
0.759725332260132 0.000299999490380287
0.765827476978302 0
0.774217903614044 0
0.777269661426544 0
0.781083166599274 0
0.782609045505524 0
0.788711071014404 0
0.790999412536621 0
0.798626899719238 0
0.806255042552948 0
0.811594367027283 0
0.817696392536163 0
0.819985330104828 0
0.823798656463623 0
0.827612519264221 0
0.829900920391083 0
0.831426382064819 0
0.83371490240097 0
0.836765944957733 0
0.839816927909851 0
0.843630790710449 0
0.845918774604797 0
0.85125857591629 0
0.854309499263763 0
0.861937284469604 0
0.8642258644104 0
0.868039667606354 0
0.87109112739563 0
0.874904274940491 0
0.879481494426727 0
0.883295178413391 0
0.888634741306305 0
0.889397621154785 0
0.891685724258423 0
0.895499706268311 0
0.900839030742645 0
0.902364611625671 0
0.908466815948486 0
0.913043677806854 0
0.916094601154327 0
0.920671343803406 0
0.921434044837952 0
0.924485146999359 0
0.926773428916931 0
0.929824590682983 0
0.934401035308838 0
0.935163974761963 0
0.93745231628418 0
0.93821507692337 0
0.941266417503357 0
0.942791759967804 0
0.94431734085083 0
0.945842862129211 0
0.948893964290619 0
0.951945066452026 0
0.954233407974243 0
0.958810091018677 0
0.960335612297058 0
0.964912295341492 0
0.96872615814209 0
0.972540020942688 0
0.978642284870148 0
0.979405045509338 0
0.982456147670746 0
0.983981668949127 0
0.983981668949127 0
0.98779559135437 0
0.992372214794159 0
0.992372214794159 0
0.995423316955566 0
0.996948897838593 0
0.997711658477783 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0312402416020632 0.666599333286285
0.0509791523218155 0.645500481128693
0.0649674236774445 0.610400021076202
0.0786446779966354 0.56150233745575
0.0952751189470291 0.50080019235611
0.109574191272259 0.437599986791611
0.124184019863605 0.365899711847305
0.13646274805069 0.303199887275696
0.150917142629623 0.244999945163727
0.163817465305328 0.197400093078613
0.174075186252594 0.164300099015236
0.186509013175964 0.13670040667057
0.198787733912468 0.114200010895729
0.209667384624481 0.0963999480009079
0.220857948064804 0.0770998671650887
0.234069004654884 0.060300026088953
0.248678773641586 0.0450998693704605
0.258781999349594 0.0338000133633614
0.269349992275238 0.0250999815762043
0.278676271438599 0.0170999858528376
0.289866358041763 0.0113000040873885
0.30012372136116 0.00729999830946326
0.309294283390045 0.00470001250505447
0.319707244634628 0.00380000146105886
0.330742955207825 0.00269999913871288
0.339446842670441 0.00129999942146242
0.348306000232697 0.000899998878594488
0.359341084957123 0.000299999490380287
0.370842099189758 0
0.381411164999008 0
0.38964918255806 0
0.399595737457275 0
0.408766090869904 0
0.418712645769119 0
0.42834946513176 0
0.439384549856186 0
0.449176281690598 0
0.458190858364105 0
0.466428339481354 0
0.477152615785599 0
0.48756605386734 0
0.499533504247665 0
0.510103404521942 0
0.519740045070648 0
0.529529809951782 0
0.539477944374084 0
0.549891769886017 0
0.559062123298645 0
0.568076014518738 0
0.578489422798157 0
0.586416959762573 0
0.594965040683746 0
0.603355586528778 0
0.611437857151031 0
0.620298027992249 0
0.629934191703796 0
0.63708484172821 0
0.64640873670578 0
0.654024481773376 0
0.666458249092102 0
0.676252543926239 0
0.683555960655212 0
0.693502426147461 0
0.703915119171143 0
0.713086903095245 0
0.722722828388214 0
0.734534621238708 0
0.741685509681702 0
0.750544667243958 0
0.759247004985809 0
0.767485558986664 0
0.776190221309662 0
0.783960044384003 0
0.791576147079468 0
0.798880338668823 0
0.806341767311096 0
0.815666437149048 0
0.822972297668457 0
0.832142114639282 0
0.841311573982239 0
0.849238872528076 0
0.859341025352478 0
0.868200242519379 0
0.875816106796265 0
0.88296502828598 0
0.891513347625732 0
0.899285018444061 0
0.906900584697723 0
0.9140505194664 0
0.922909557819366 0
0.932234704494476 0
0.940317094326019 0
0.94591224193573 0
0.954460501670837 0
0.961143910884857 0
0.968293428421021 0
0.977308034896851 0
0.985234677791595 0
0.992850482463837 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/combination_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.265599608421326 0.675799608230591
0.290700435638428 0.675699234008789
0.310299634933472 0.674398899078369
0.329699993133545 0.667600393295288
0.342499643564224 0.652199923992157
0.356199741363525 0.622399389743805
0.372400343418121 0.569900751113892
0.384600043296814 0.495400011539459
0.397099763154984 0.401900142431259
0.407400250434875 0.300999879837036
0.418299704790115 0.21160002052784
0.426699936389923 0.138999968767166
0.437300086021423 0.0875000581145287
0.446699887514114 0.0458000302314758
0.457500159740448 0.0233000498265028
0.466899901628494 0.0115999942645431
0.475299894809723 0.00520000327378511
0.482900083065033 0.00260000163689256
0.491300046443939 0.00140000053215772
0.497400403022766 0.000299999490380287
0.506299197673798 9.99997646431439e-05
0.513399541378021 0
0.521401107311249 0
0.527600467205048 0
0.536899983882904 0
0.545899927616119 0
0.55400162935257 0
0.562100172042847 0
0.569600284099579 0
0.576799392700195 0
0.582399964332581 0
0.589899837970734 0
0.596799731254578 0
0.602899193763733 0
0.610000848770142 0
0.617199718952179 0
0.623800098896027 0
0.630299866199493 0
0.636698484420776 0
0.643600225448608 0
0.651598691940308 0
0.659699499607086 0
0.666802048683167 0
0.674199759960175 0
0.680899500846863 0
0.687701284885406 0
0.695199966430664 0
0.702300667762756 0
0.708499908447266 0
0.715200126171112 0
0.720599830150604 0
0.72719943523407 0
0.732299208641052 0
0.738799512386322 0
0.745499849319458 0
0.751698851585388 0
0.758099555969238 0
0.764301538467407 0
0.769200086593628 0
0.77720046043396 0
0.784800410270691 0
0.790599703788757 0
0.797699987888336 0
0.803900361061096 0
0.80959814786911 0
0.816500604152679 0
0.823400378227234 0
0.829199433326721 0
0.835900008678436 0
0.842100203037262 0
0.84829968214035 0
0.854400217533112 0
0.859000027179718 0
0.865099906921387 0
0.870300590991974 0
0.875600516796112 0
0.880200207233429 0
0.885699391365051 0
0.891600072383881 0
0.896500706672668 0
0.900500178337097 0
0.906700670719147 0
0.91290020942688 0
0.917499780654907 0
0.922300398349762 0
0.928900182247162 0
0.935199618339539 0
0.939500093460083 0
0.945200026035309 0
0.951600015163422 0
0.956799924373627 0
0.961399793624878 0
0.966000199317932 0
0.970700204372406 0
0.975899994373322 0
0.981400012969971 0
0.986199975013733 0
0.99099999666214 0
0.995599985122681 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.97251307964325 0.675799608230591
0.979493916034698 0.675699234008789
0.983856916427612 0.674398899078369
0.986038386821747 0.667600393295288
0.987347304821014 0.652199923992157
0.988656222820282 0.622399389743805
0.988656222820282 0.569900751113892
0.989965081214905 0.495400011539459
0.990837693214417 0.401900142431259
0.991273999214172 0.300999879837036
0.991273999214172 0.21160002052784
0.991273999214172 0.138999968767166
0.991273999214172 0.0875000581145287
0.991273999214172 0.0458000302314758
0.991273999214172 0.0233000498265028
0.991273999214172 0.0115999942645431
0.991710305213928 0.00520000327378511
0.991710305213928 0.00260000163689256
0.991710305213928 0.00140000053215772
0.991710305213928 0.000299999490380287
0.991710305213928 9.99997646431439e-05
0.992146611213684 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.99258291721344 0
0.993455469608307 0
0.993891775608063 0
0.993891775608063 0
0.993891775608063 0
0.994328081607819 0
0.994764387607574 0
0.99520069360733 0
0.99520069360733 0
0.99520069360733 0
0.99520069360733 0
0.99520069360733 0
0.99520069360733 0
0.99520069360733 0
0.99520069360733 0
0.995636999607086 0
0.995636999607086 0
0.995636999607086 0
0.995636999607086 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996073305606842 0
0.996945917606354 0
0.996945917606354 0
0.99738222360611 0
0.997818470001221 0
0.997818470001221 0
0.997818470001221 0
0.997818470001221 0
0.998691082000732 0
0.998691082000732 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999127388000488 0
0.999563694000244 0
0.999563694000244 0
0.999563694000244 0
0.999563694000244 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.236966818571091 0.675799608230591
0.348341077566147 0.675699234008789
0.412322282791138 0.674398899078369
0.474723547697067 0.667600393295288
0.5055291056633 0.652199923992157
0.533965408802032 0.622399389743805
0.565560936927795 0.569900751113892
0.586887955665588 0.495400011539459
0.603475689888 0.401900142431259
0.614534139633179 0.300999879837036
0.626382052898407 0.21160002052784
0.638230621814728 0.138999968767166
0.649288833141327 0.0875000581145287
0.658767819404602 0.0458000302314758
0.672195971012115 0.0233000498265028
0.679305255413055 0.0115999942645431
0.687994003295898 0.00520000327378511
0.698262214660645 0.00260000163689256
0.704581499099731 0.00140000053215772
0.709320247173309 0.000299999490380287
0.718799293041229 9.99997646431439e-05
0.720379233360291 0
0.725118577480316 0
0.732227563858032 0
0.740126729011536 0
0.751185059547424 0
0.754344701766968 0
0.76145339012146 0
0.766192555427551 0
0.773301899433136 0
0.77409154176712 0
0.780410647392273 0
0.782780289649963 0
0.78672993183136 0
0.792259156703949 0
0.801737785339355 0
0.804107546806335 0
0.810426652431488 0
0.815165877342224 0
0.818325340747833 0
0.820695221424103 0
0.826224327087402 0
0.827803909778595 0
0.83017361164093 0
0.834913015365601 0
0.837282776832581 0
0.838862955570221 0
0.84281188249588 0
0.846761465072632 0
0.849921226501465 0
0.85308039188385 0
0.859399676322937 0
0.863349199295044 0
0.868088483810425 0
0.871248304843903 0
0.875197291374207 0
0.879936814308167 0
0.88309633731842 0
0.886256098747253 0
0.887045621871948 0
0.89099508523941 0
0.89415454864502 0
0.899684250354767 0
0.901263833045959 0
0.905213296413422 0
0.90837299823761 0
0.913902044296265 0
0.917061507701874 0
0.921011030673981 0
0.924960494041443 0
0.928120076656342 0
0.930489718914032 0
0.932069540023804 0
0.932859480381012 0
0.936018764972687 0
0.937598764896393 0
0.940758287906647 0
0.943127989768982 0
0.944707751274109 0
0.946287512779236 0
0.950236976146698 0
0.951816737651825 0
0.954976320266724 0
0.958135843276978 0
0.961295425891876 0
0.96445494890213 0
0.968404412269592 0
0.970774114131927 0
0.978672981262207 0
0.981042683124542 0
0.982622444629669 0
0.984202206134796 0
0.98499208688736 0
0.988941550254822 0
0.992891013622284 0
0.992891013622284 0
0.995260655879974 0
0.996840417385101 0
0.99763035774231 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0197143722325563 0.675799608230591
0.0343060344457626 0.675699234008789
0.0506053827702999 0.674398899078369
0.0676809549331665 0.667600393295288
0.0810306444764137 0.652199923992157
0.0962434485554695 0.622399389743805
0.115181662142277 0.569900751113892
0.129463240504265 0.495400011539459
0.145296543836594 0.401900142431259
0.158956825733185 0.300999879837036
0.173548474907875 0.21160002052784
0.184259653091431 0.138999968767166
0.198540791869164 0.0875000581145287
0.211269557476044 0.0458000302314758
0.225395873188972 0.0233000498265028
0.238590493798256 0.0115999942645431
0.249767318367958 0.00520000327378511
0.259547024965286 0.00260000163689256
0.2713443338871 0.00140000053215772
0.279882073402405 0.000299999490380287
0.291834503412247 9.99997646431439e-05
0.302390247583389 0
0.31372207403183 0
0.321950525045395 0
0.334833949804306 0
0.346631407737732 0
0.358583986759186 0
0.369760483503342 0
0.38047194480896 0
0.390251159667969 0
0.398789346218109 0
0.409189701080322 0
0.419435143470764 0
0.428127944469452 0
0.438062787055969 0
0.447376668453217 0
0.45715606212616 0
0.466004461050034 0
0.475007772445679 0
0.484787255525589 0
0.496585249900818 0
0.50807249546051 0
0.518782615661621 0
0.52964860200882 0
0.538962304592133 0
0.548898100852966 0
0.560230612754822 0
0.570476889610291 0
0.579322755336761 0
0.58910346031189 0
0.59686416387558 0
0.605868518352509 0
0.613008141517639 0
0.622011303901672 0
0.631791532039642 0
0.640641212463379 0
0.649642825126648 0
0.658489942550659 0
0.665476500988007 0
0.67773973941803 0
0.688761532306671 0
0.697144210338593 0
0.707078874111176 0
0.716392397880554 0
0.724464476108551 0
0.734554052352905 0
0.744178295135498 0
0.75256073474884 0
0.761874139308929 0
0.770723581314087 0
0.77957147359848 0
0.788419306278229 0
0.795249938964844 0
0.804564118385315 0
0.812014758586884 0
0.81962126493454 0
0.826141536235809 0
0.834057807922363 0
0.842905700206757 0
0.850202262401581 0
0.855635046958923 0
0.864948451519012 0
0.87395191192627 0
0.88047206401825 0
0.887302458286285 0
0.896926641464233 0
0.905929625034332 0
0.912139058113098 0
0.919434666633606 0
0.928904056549072 0
0.9366654753685 0
0.943495750427246 0
0.950481235980988 0
0.957000851631165 0
0.964141547679901 0
0.972679316997528 0
0.979664623737335 0
0.986805319786072 0
0.993635535240173 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/gpt/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.272262364625931 0.236496344208717
0.298539966344833 0.169099777936935
0.313138574361801 0.133090242743492
0.329927235841751 0.114111930131912
0.343795597553253 0.101459868252277
0.356204360723495 0.0934306904673576
0.364233165979385 0.088321141898632
0.375912398099899 0.0836983174085617
0.387104690074921 0.0766424536705017
0.397080272436142 0.071046270430088
0.409489005804062 0.0642335191369057
0.418004989624023 0.0610705986618996
0.424574255943298 0.0574209280312061
0.434792995452881 0.0530413463711739
0.441849261522293 0.051824826747179
0.449391782283783 0.0503649488091469
0.460097312927246 0.0481751747429371
0.465936690568924 0.0474452488124371
0.474695831537247 0.0464720278978348
0.481995165348053 0.0445255488157272
0.48564475774765 0.0433090031147003
0.493430823087692 0.0420924946665764
0.499514162540436 0.0411191806197166
0.505838930606842 0.0408759191632271
0.514598309993744 0.0401459783315659
0.521654486656189 0.0399026796221733
0.528953671455383 0.0389293879270554
0.536982297897339 0.0377128906548023
0.546471834182739 0.0364963933825493
0.553283929824829 0.0352798476815224
0.560583472251892 0.0340632945299149
0.567152917385101 0.0326033793389797
0.575426518917084 0.0318734794855118
0.581021666526794 0.0313868559896946
0.587347447872162 0.0304136779159307
0.593674540519714 0.0294403899461031
0.601946234703064 0.0282238461077213
0.609732508659363 0.0270073004066944
0.614598274230957 0.0257907547056675
0.623843967914581 0.0253041405230761
0.630900263786316 0.0248175244778395
0.638442575931549 0.0236009806394577
0.645742237567902 0.0216544810682535
0.652797222137451 0.0206812303513288
0.658150613307953 0.0187347996979952
0.662773609161377 0.0182481836527586
0.669829726219177 0.0175182726234198
0.676399409770966 0.0158150997012854
0.681995153427124 0.015328461304307
0.689294755458832 0.0143552115187049
0.696836173534393 0.0136253172531724
0.70413613319397 0.0131386881694198
0.709732413291931 0.012652070261538
0.714355945587158 0.0111922211945057
0.719707548618317 0.0104622961953282
0.724087476730347 0.0104622961953282
0.732359766960144 0.0102189872413874
0.740632891654968 0.0099756782874465
0.746472120285034 0.00875913631170988
0.754257917404175 0.00827250722795725
0.763017416000366 0.00754258036613464
0.768370449542999 0.00729927653446794
0.775912523269653 0.00729927653446794
0.784914910793304 0.00632603419944644
0.790024518966675 0.00510948989540339
0.799026548862457 0.00510948989540339
0.80754280090332 0.00462286453694105
0.813868761062622 0.00437956675887108
0.821654736995697 0.00389294093474746
0.827250599861145 0.00291971582919359
0.835036754608154 0.00218978244811296
0.840632319450378 0.00218978244811296
0.847444951534271 0.00194647524040192
0.853771150112152 0.00170316069852561
0.861313998699188 0.00170316069852561
0.86496365070343 0.00170316069852561
0.870073199272156 0.00170316069852561
0.874695837497711 0.00145985721610487
0.879562079906464 0.00121654639951885
0.884671628475189 0.00121654639951885
0.889051258563995 0.000973234651610255
0.896350383758545 0.000973234651610255
0.901216328144073 0.000973234651610255
0.908272445201874 0.000729926978237927
0.912408709526062 0.000729926978237927
0.916058540344238 0.000729926978237927
0.920924603939056 0.000729926978237927
0.926764130592346 0.000486617325805128
0.93284672498703 0.000243308662902564
0.939659476280212 0.000243308662902564
0.946228802204132 0.000243308662902564
0.951581478118896 0
0.955474376678467 0
0.962043762207031 0
0.966910004615784 0
0.972992718219757 0
0.977615594863892 0
0.985158145427704 0
0.99148416519165 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.913921356201172 0.236496344208717
0.943676948547363 0.169099777936935
0.953241229057312 0.133090242743492
0.96174281835556 0.114111930131912
0.964930951595306 0.101459868252277
0.965993642807007 0.0934306904673576
0.969181716442108 0.088321141898632
0.971307098865509 0.0836983174085617
0.972369790077209 0.0766424536705017
0.972369790077209 0.071046270430088
0.973432540893555 0.0642335191369057
0.974495232105255 0.0610705986618996
0.975557923316956 0.0574209280312061
0.977683305740356 0.0530413463711739
0.977683305740356 0.051824826747179
0.977683305740356 0.0503649488091469
0.979808688163757 0.0481751747429371
0.980871438980103 0.0474452488124371
0.981934130191803 0.0464720278978348
0.981934130191803 0.0445255488157272
0.981934130191803 0.0433090031147003
0.981934130191803 0.0420924946665764
0.981934130191803 0.0411191806197166
0.981934130191803 0.0408759191632271
0.984059512615204 0.0401459783315659
0.984059512615204 0.0399026796221733
0.984059512615204 0.0389293879270554
0.984059512615204 0.0377128906548023
0.984059512615204 0.0364963933825493
0.984059512615204 0.0352798476815224
0.984059512615204 0.0340632945299149
0.984059512615204 0.0326033793389797
0.985122203826904 0.0318734794855118
0.986184895038605 0.0313868559896946
0.986184895038605 0.0304136779159307
0.986184895038605 0.0294403899461031
0.986184895038605 0.0282238461077213
0.986184895038605 0.0270073004066944
0.986184895038605 0.0257907547056675
0.98831033706665 0.0253041405230761
0.989373028278351 0.0248175244778395
0.989373028278351 0.0236009806394577
0.990435719490051 0.0216544810682535
0.991498410701752 0.0206812303513288
0.991498410701752 0.0187347996979952
0.992561101913452 0.0182481836527586
0.993623793125153 0.0175182726234198
0.993623793125153 0.0158150997012854
0.993623793125153 0.015328461304307
0.993623793125153 0.0143552115187049
0.993623793125153 0.0136253172531724
0.993623793125153 0.0131386881694198
0.993623793125153 0.012652070261538
0.994686484336853 0.0111922211945057
0.994686484336853 0.0104622961953282
0.994686484336853 0.0104622961953282
0.994686484336853 0.0102189872413874
0.994686484336853 0.0099756782874465
0.995749175548553 0.00875913631170988
0.995749175548553 0.00827250722795725
0.995749175548553 0.00754258036613464
0.995749175548553 0.00729927653446794
0.995749175548553 0.00729927653446794
0.995749175548553 0.00632603419944644
0.995749175548553 0.00510948989540339
0.996811926364899 0.00510948989540339
0.996811926364899 0.00462286453694105
0.996811926364899 0.00437956675887108
0.9989373087883 0.00389294093474746
0.9989373087883 0.00291971582919359
0.9989373087883 0.00218978244811296
0.9989373087883 0.00218978244811296
0.9989373087883 0.00194647524040192
0.9989373087883 0.00170316069852561
0.9989373087883 0.00170316069852561
0.9989373087883 0.00170316069852561
0.9989373087883 0.00170316069852561
0.9989373087883 0.00145985721610487
0.9989373087883 0.00121654639951885
0.9989373087883 0.00121654639951885
0.9989373087883 0.000973234651610255
0.9989373087883 0.000973234651610255
0.9989373087883 0.000973234651610255
0.9989373087883 0.000729926978237927
0.9989373087883 0.000729926978237927
0.9989373087883 0.000729926978237927
0.9989373087883 0.000729926978237927
0.9989373087883 0.000486617325805128
0.9989373087883 0.000243308662902564
0.9989373087883 0.000243308662902564
0.9989373087883 0.000243308662902564
0.9989373087883 0
0.9989373087883 0
0.9989373087883 0
0.9989373087883 0
0.9989373087883 0
0.9989373087883 0
0.9989373087883 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.290167838335037 0.236496344208717
0.347721815109253 0.169099777936935
0.381294965744019 0.133090242743492
0.441247016191483 0.114111930131912
0.458033561706543 0.101459868252277
0.472422093153 0.0934306904673576
0.486810356378555 0.088321141898632
0.513189494609833 0.0836983174085617
0.527578115463257 0.0766424536705017
0.537170052528381 0.071046270430088
0.549160659313202 0.0642335191369057
0.551558613777161 0.0610705986618996
0.558752834796906 0.0574209280312061
0.57314121723175 0.0530413463711739
0.585131883621216 0.051824826747179
0.59232634305954 0.0503649488091469
0.604316592216492 0.0481751747429371
0.609112441539764 0.0474452488124371
0.618704974651337 0.0464720278978348
0.625899016857147 0.0445255488157272
0.625899016857147 0.0433090031147003
0.628296971321106 0.0420924946665764
0.630695581436157 0.0411191806197166
0.642685830593109 0.0408759191632271
0.645083904266357 0.0401459783315659
0.652277886867523 0.0399026796221733
0.659472286701202 0.0389293879270554
0.673861086368561 0.0377128906548023
0.688249349594116 0.0364963933825493
0.697841882705688 0.0352798476815224
0.702637732028961 0.0340632945299149
0.707433998584747 0.0326033793389797
0.719424486160278 0.0318734794855118
0.719424486160278 0.0313868559896946
0.721822679042816 0.0304136779159307
0.729016959667206 0.0294403899461031
0.73141485452652 0.0282238461077213
0.748201429843903 0.0270073004066944
0.757793784141541 0.0257907547056675
0.764988005161285 0.0253041405230761
0.767386078834534 0.0248175244778395
0.774580359458923 0.0236009806394577
0.776978433132172 0.0216544810682535
0.77937650680542 0.0206812303513288
0.77937650680542 0.0187347996979952
0.77937650680542 0.0182481836527586
0.781774580478668 0.0175182726234198
0.784172654151917 0.0158150997012854
0.784172654151917 0.015328461304307
0.793765068054199 0.0143552115187049
0.798560976982117 0.0136253172531724
0.808153390884399 0.0131386881694198
0.82014387845993 0.012652070261538
0.822541892528534 0.0111922211945057
0.824939966201782 0.0104622961953282
0.829736113548279 0.0104622961953282
0.832134127616882 0.0102189872413874
0.844124674797058 0.0099756782874465
0.848920881748199 0.00875913631170988
0.851318955421448 0.00827250722795725
0.853717029094696 0.00754258036613464
0.853717029094696 0.00729927653446794
0.860911250114441 0.00729927653446794
0.863309323787689 0.00632603419944644
0.870503604412079 0.00510948989540339
0.877697944641113 0.00510948989540339
0.887290179729462 0.00462286453694105
0.892086327075958 0.00437956675887108
0.892086327075958 0.00389294093474746
0.896882474422455 0.00291971582919359
0.906474828720093 0.00218978244811296
0.906474828720093 0.00218978244811296
0.913669049739838 0.00194647524040192
0.916067123413086 0.00170316069852561
0.918465256690979 0.00170316069852561
0.918465256690979 0.00170316069852561
0.923261404037476 0.00170316069852561
0.925659477710724 0.00145985721610487
0.928057551383972 0.00121654639951885
0.93045562505722 0.00121654639951885
0.932853698730469 0.000973234651610255
0.93764990568161 0.000973234651610255
0.940047979354858 0.000973234651610255
0.947242200374603 0.000729926978237927
0.9520383477211 0.000729926978237927
0.954436421394348 0.000729926978237927
0.956834554672241 0.000729926978237927
0.961630702018738 0.000486617325805128
0.964028775691986 0.000243308662902564
0.964028775691986 0.000243308662902564
0.966426849365234 0.000243308662902564
0.968824923038483 0
0.968824923038483 0
0.978417277336121 0
0.983213424682617 0
0.983213424682617 0
0.988009572029114 0
0.992805778980255 0
0.997601926326752 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0501453392207623 0.236496344208717
0.070494182407856 0.169099777936935
0.0839389562606812 0.133090242743492
0.0970203280448914 0.114111930131912
0.114098839461803 0.101459868252277
0.130087226629257 0.0934306904673576
0.138808056712151 0.088321141898632
0.151526287198067 0.0836983174085617
0.165697649121284 0.0766424536705017
0.17914243042469 0.071046270430088
0.195494249463081 0.0642335191369057
0.207485422492027 0.0610705986618996
0.215843051671982 0.0574209280312061
0.228197693824768 0.0530413463711739
0.23691862821579 0.051824826747179
0.247093066573143 0.0503649488091469
0.260537803173065 0.0481751747429371
0.268168956041336 0.0474452488124371
0.279432684183121 0.0464720278978348
0.289244502782822 0.0445255488157272
0.294694602489471 0.0433090031147003
0.305959224700928 0.0420924946665764
0.314680218696594 0.0411191806197166
0.322310835123062 0.0408759191632271
0.334302365779877 0.0401459783315659
0.343750178813934 0.0399026796221733
0.353561460971832 0.0389293879270554
0.363371998071671 0.0377128906548023
0.375363647937775 0.0364963933825493
0.38408425450325 0.0352798476815224
0.394258618354797 0.0340632945299149
0.403343111276627 0.0326033793389797
0.413517534732819 0.0318734794855118
0.421511441469193 0.0313868559896946
0.430595695972443 0.0304136779159307
0.438953578472137 0.0294403899461031
0.450944691896439 0.0282238461077213
0.460029065608978 0.0270073004066944
0.465843081474304 0.0257907547056675
0.477834314107895 0.0253041405230761
0.487645357847214 0.0248175244778395
0.497819900512695 0.0236009806394577
0.507994592189789 0.0216544810682535
0.517805218696594 0.0206812303513288
0.525799810886383 0.0187347996979952
0.532339334487915 0.0182481836527586
0.542151093482971 0.0175182726234198
0.551598191261292 0.0158150997012854
0.559956133365631 0.015328461304307
0.569404065608978 0.0143552115187049
0.579941868782043 0.0136253172531724
0.589389324188232 0.0131386881694198
0.59592992067337 0.012652070261538
0.602107763290405 0.0111922211945057
0.609737694263458 0.0104622961953282
0.615552127361298 0.0104622961953282
0.627542614936829 0.0102189872413874
0.638081908226013 0.0099756782874465
0.645712077617645 0.00875913631170988
0.656976938247681 0.00827250722795725
0.669694364070892 0.00754258036613464
0.677688837051392 0.00729927653446794
0.687862694263458 0.00729927653446794
0.700944304466248 0.00632603419944644
0.70748496055603 0.00510948989540339
0.719476878643036 0.00510948989540339
0.7307408452034 0.00462286453694105
0.739462375640869 0.00437956675887108
0.750363707542419 0.00389294093474746
0.757994532585144 0.00291971582919359
0.768167555332184 0.00218978244811296
0.776526510715485 0.00218978244811296
0.785609662532806 0.00194647524040192
0.794694781303406 0.00170316069852561
0.805596649646759 0.00170316069852561
0.811046540737152 0.00170316069852561
0.817950785160065 0.00170316069852561
0.824491083621979 0.00145985721610487
0.831395149230957 0.00121654639951885
0.838663160800934 0.00121654639951885
0.844840586185455 0.000973234651610255
0.855014204978943 0.000973234651610255
0.861919164657593 0.000973234651610255
0.871366262435913 0.000729926978237927
0.876816868782043 0.000729926978237927
0.881904065608978 0.000729926978237927
0.888808131217957 0.000729926978237927
0.896802484989166 0.000486617325805128
0.905523240566254 0.000243308662902564
0.915697753429413 0.000243308662902564
0.925145268440247 0.000243308662902564
0.93277633190155 0
0.938590407371521 0
0.946947693824768 0
0.953488349914551 0
0.962572693824768 0
0.96875 0
0.979287803173065 0
0.987645328044891 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.33/pass2path/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.253401279449463 0.656900078058243
0.279599875211716 0.641199886798859
0.296800404787064 0.628199887275696
0.309699565172195 0.612600010633469
0.3231001496315 0.596200078725815
0.334699779748917 0.577099943161011
0.347699671983719 0.553600120544434
0.358700156211853 0.526800107955933
0.37089991569519 0.492799991369247
0.382399499416351 0.460500019788742
0.393599659204483 0.41649996638298
0.403999865055084 0.377499979734421
0.413800209760666 0.338400003314018
0.421699702739716 0.30300005376339
0.430600196123123 0.271199983358383
0.441100001335144 0.242800000309944
0.450700014829636 0.212899994850159
0.458899915218353 0.189699985086918
0.469600051641464 0.167399969696999
0.477499961853027 0.145299965143204
0.484599947929382 0.127099993079901
0.493400305509567 0.108700004965067
0.501398801803589 0.0940000012516975
0.509101092815399 0.0813999947160482
0.517999470233917 0.0702999927103519
0.526099324226379 0.0613999888300896
0.534700155258179 0.0528000071644783
0.542299389839172 0.0458999957889318
0.54990017414093 0.0384999971836805
0.558299362659454 0.0335000041872263
0.565000414848328 0.0292000094428658
0.572701454162598 0.0246000036597252
0.580900728702545 0.0210999950766563
0.588397920131683 0.0186000010930002
0.594801485538483 0.0163000041618943
0.602799892425537 0.0148000007495284
0.610699653625488 0.0136999996379018
0.617099463939667 0.0125999985262752
0.624999105930328 0.0119999990798533
0.632399499416351 0.0111999987624586
0.641098618507385 0.0107000004965812
0.648400247097015 0.0100999998860061
0.655299782752991 0.00980000053532422
0.663300216197968 0.00889999778009951
0.670700669288635 0.00839999811723828
0.677498757839203 0.00809999858029187
0.684398710727692 0.00729999770410359
0.691100120544434 0.0066999982111156
0.697299718856812 0.00609999790322036
0.704100370407104 0.00519999966491014
0.711599111557007 0.00449999878183007
0.717699825763702 0.00409999839030206
0.724199831485748 0.00309999897144735
0.730199337005615 0.00239999890327454
0.737099289894104 0.00179999913088977
0.744102239608765 0.00139999899547547
0.751100778579712 0.00109999910928309
0.757102131843567 0.000599999353289604
0.76250159740448 0.000299999699927866
0.769799649715424 0.000199999765027314
0.776899755001068 0.000199999765027314
0.782999932765961 0.000199999765027314
0.79099977016449 9.9999934900552e-05
0.797599375247955 9.9999934900552e-05
0.802799820899963 9.9999934900552e-05
0.810100078582764 9.9999934900552e-05
0.816500425338745 9.9999934900552e-05
0.82220059633255 0
0.828899443149567 0
0.834301173686981 0
0.840599119663239 0
0.846799790859222 0
0.852500021457672 0
0.858099579811096 0
0.864799916744232 0
0.870999872684479 0
0.876100361347198 0
0.88150018453598 0
0.887499809265137 0
0.892399728298187 0
0.897900223731995 0
0.904099822044373 0
0.91049998998642 0
0.915799677371979 0
0.920100092887878 0
0.926700174808502 0
0.932399988174438 0
0.937600374221802 0
0.942699790000916 0
0.947200000286102 0
0.951699793338776 0
0.957700073719025 0
0.962499797344208 0
0.967599630355835 0
0.974199891090393 0
0.98009991645813 0
0.984200000762939 0
0.98989999294281 0
0.995199978351593 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.903383612632751 0.656900078058243
0.936812043190002 0.641199886798859
0.949857234954834 0.628199887275696
0.95964103937149 0.612600010633469
0.966979086399078 0.596200078725815
0.971463441848755 0.577099943161011
0.975540161132812 0.553600120544434
0.979209125041962 0.526800107955933
0.980432152748108 0.492799991369247
0.981655120849609 0.460500019788742
0.984101116657257 0.41649996638298
0.985731780529022 0.377499979734421
0.988177716732025 0.338400003314018
0.988585412502289 0.30300005376339
0.98980838060379 0.271199983358383
0.990216076374054 0.242800000309944
0.991439044475555 0.212899994850159
0.991439044475555 0.189699985086918
0.991439044475555 0.167399969696999
0.991439044475555 0.145299965143204
0.991439044475555 0.127099993079901
0.992254376411438 0.108700004965067
0.992662072181702 0.0940000012516975
0.993069708347321 0.0813999947160482
0.993477404117584 0.0702999927103519
0.993885040283203 0.0613999888300896
0.993885040283203 0.0528000071644783
0.993885040283203 0.0458999957889318
0.993885040283203 0.0384999971836805
0.993885040283203 0.0335000041872263
0.993885040283203 0.0292000094428658
0.993885040283203 0.0246000036597252
0.993885040283203 0.0210999950766563
0.993885040283203 0.0186000010930002
0.993885040283203 0.0163000041618943
0.994292676448822 0.0148000007495284
0.994292676448822 0.0136999996379018
0.994292676448822 0.0125999985262752
0.994700372219086 0.0119999990798533
0.995108008384705 0.0111999987624586
0.995108008384705 0.0107000004965812
0.995108008384705 0.0100999998860061
0.995108008384705 0.00980000053532422
0.995515704154968 0.00889999778009951
0.995923340320587 0.00839999811723828
0.996331036090851 0.00809999858029187
0.996331036090851 0.00729999770410359
0.996331036090851 0.0066999982111156
0.996331036090851 0.00609999790322036
0.996331036090851 0.00519999966491014
0.996331036090851 0.00449999878183007
0.996331036090851 0.00409999839030206
0.996331036090851 0.00309999897144735
0.99673867225647 0.00239999890327454
0.99673867225647 0.00179999913088977
0.99673867225647 0.00139999899547547
0.99673867225647 0.00109999910928309
0.997146368026733 0.000599999353289604
0.997146368026733 0.000299999699927866
0.997146368026733 0.000199999765027314
0.997146368026733 0.000199999765027314
0.997146368026733 0.000199999765027314
0.997146368026733 9.9999934900552e-05
0.997146368026733 9.9999934900552e-05
0.997146368026733 9.9999934900552e-05
0.997146368026733 9.9999934900552e-05
0.997146368026733 9.9999934900552e-05
0.997146368026733 0
0.997961699962616 0
0.997961699962616 0
0.997961699962616 0
0.998369336128235 0
0.998369336128235 0
0.998369336128235 0
0.998369336128235 0
0.998777031898499 0
0.998777031898499 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999184668064117 0
0.999592363834381 0
0.999592363834381 0
0.999592363834381 0
0.999592363834381 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.211496740579605 0.656900078058243
0.312364816665649 0.641199886798859
0.356833100318909 0.628199887275696
0.381778746843338 0.612600010633469
0.405639857053757 0.596200078725815
0.426247179508209 0.577099943161011
0.45770063996315 0.553600120544434
0.477223455905914 0.526800107955933
0.508676588535309 0.492799991369247
0.531453728675842 0.460500019788742
0.55206024646759 0.41649996638298
0.563990950584412 0.377499979734421
0.575921535491943 0.338400003314018
0.587852478027344 0.30300005376339
0.598698139190674 0.271199983358383
0.613883137702942 0.242800000309944
0.622559726238251 0.212899994850159
0.63232159614563 0.189699985086918
0.650759100914001 0.167399969696999
0.657267212867737 0.145299965143204
0.668112933635712 0.127099993079901
0.676789343357086 0.108700004965067
0.685466349124908 0.0940000012516975
0.693058729171753 0.0813999947160482
0.697397351264954 0.0702999927103519
0.704989016056061 0.0613999888300896
0.712581098079681 0.0528000071644783
0.725596845149994 0.0458999957889318
0.732104241847992 0.0384999971836805
0.740780532360077 0.0335000041872263
0.744034647941589 0.0292000094428658
0.752711236476898 0.0246000036597252
0.759219229221344 0.0210999950766563
0.764642059803009 0.0186000010930002
0.772234380245209 0.0163000041618943
0.780911326408386 0.0148000007495284
0.787418901920319 0.0136999996379018
0.79718005657196 0.0125999985262752
0.806941449642181 0.0119999990798533
0.810195505619049 0.0111999987624586
0.815618336200714 0.0107000004965812
0.821041345596313 0.0100999998860061
0.825379550457001 0.00980000053532422
0.827548921108246 0.00889999778009951
0.830802738666534 0.00839999811723828
0.832971513271332 0.00809999858029187
0.839479386806488 0.00729999770410359
0.84381765127182 0.0066999982111156
0.84598696231842 0.00609999790322036
0.850325226783752 0.00519999966491014
0.852494597434998 0.00449999878183007
0.85900217294693 0.00409999839030206
0.862256050109863 0.00309999897144735
0.863340497016907 0.00239999890327454
0.867678999900818 0.00179999913088977
0.872017204761505 0.00139999899547547
0.874186396598816 0.00109999910928309
0.877440392971039 0.000599999353289604
0.882863223552704 0.000299999699927866
0.883947789669037 0.000199999765027314
0.889370918273926 0.000199999765027314
0.891540110111237 0.000199999765027314
0.898047566413879 9.9999934900552e-05
0.90021675825119 9.9999934900552e-05
0.904555320739746 9.9999934900552e-05
0.907809138298035 9.9999934900552e-05
0.912147521972656 9.9999934900552e-05
0.916485905647278 0
0.917570471763611 0
0.919739723205566 0
0.92299348115921 0
0.926247298717499 0
0.92841649055481 0
0.93058568239212 0
0.93600869178772 0
0.937093257904053 0
0.939262449741364 0
0.942516267299652 0
0.94360089302063 0
0.944685459136963 0
0.947939276695251 0
0.950108468532562 0
0.952277660369873 0
0.955531477928162 0
0.958785235881805 0
0.965292870998383 0
0.968546628952026 0
0.971800446510315 0
0.978308022022247 0
0.978308022022247 0
0.979392647743225 0
0.980477213859558 0
0.981561839580536 0
0.985900223255157 0
0.990238606929779 0
0.991323232650757 0
0.994576990604401 0
0.996746182441711 0
0.997830808162689 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0185660440474749 0.656900078058243
0.0316981114447117 0.641199886798859
0.0466415099799633 0.628199887275696
0.0590188503265381 0.612600010633469
0.0732077062129974 0.596200078725815
0.0861887410283089 0.577099943161011
0.0999245271086693 0.553600120544434
0.11245284974575 0.526800107955933
0.126037910580635 0.492799991369247
0.139773532748222 0.460500019788742
0.152905181050301 0.41649996638298
0.166339844465256 0.377499979734421
0.178565800189972 0.338400003314018
0.188679471611977 0.30300005376339
0.200150907039642 0.271199983358383
0.213735833764076 0.242800000309944
0.226566061377525 0.212899994850159
0.237584874033928 0.189699985086918
0.251169264316559 0.167399969696999
0.262189000844955 0.145299965143204
0.271396458148956 0.127099993079901
0.28316929936409 0.108700004965067
0.293886989355087 0.0940000012516975
0.304301798343658 0.0813999947160482
0.316980570554733 0.0702999927103519
0.328000545501709 0.0613999888300896
0.339924484491348 0.0528000071644783
0.349584609270096 0.0458999957889318
0.36015123128891 0.0384999971836805
0.371622264385223 0.0335000041872263
0.381282836198807 0.0292000094428658
0.391697973012924 0.0246000036597252
0.403170019388199 0.0210999950766563
0.413735508918762 0.0186000010930002
0.422339558601379 0.0163000041618943
0.433056443929672 0.0148000007495284
0.444075614213943 0.0136999996379018
0.452377438545227 0.0125999985262752
0.462792366743088 0.0119999990798533
0.473358452320099 0.0111999987624586
0.485735863447189 0.0107000004965812
0.49599951505661 0.0100999998860061
0.505812227725983 0.00980000053532422
0.517432689666748 0.00889999778009951
0.527999401092529 0.00839999811723828
0.537810027599335 0.00809999858029187
0.547321200370789 0.00729999770410359
0.556829392910004 0.0066999982111156
0.565886616706848 0.00609999790322036
0.575545907020569 0.00519999966491014
0.586565017700195 0.00449999878183007
0.594867885112762 0.00409999839030206
0.604225873947144 0.00309999897144735
0.612981081008911 0.00239999890327454
0.622792482376099 0.00179999913088977
0.632753968238831 0.00139999899547547
0.643018841743469 0.00109999910928309
0.651472747325897 0.000599999353289604
0.658868074417114 0.000299999699927866
0.669734954833984 0.000199999765027314
0.679697036743164 0.000199999765027314
0.688604295253754 0.000199999765027314
0.69977331161499 9.9999934900552e-05
0.70943421125412 9.9999934900552e-05
0.716678261756897 9.9999934900552e-05
0.727246344089508 9.9999934900552e-05
0.736303210258484 9.9999934900552e-05
0.744302153587341 0
0.753962695598602 0
0.761812031269073 0
0.770867645740509 0
0.779623031616211 0
0.787924528121948 0
0.796076059341431 0
0.805434286594391 0
0.814490258693695 0
0.821886956691742 0
0.829433798789978 0
0.838339626789093 0
0.8455850481987 0
0.853433728218079 0
0.862490952014923 0
0.871848702430725 0
0.879396200180054 0
0.885433733463287 0
0.894490838050842 0
0.902641952037811 0
0.910037755966187 0
0.916830062866211 0
0.923622667789459 0
0.930263996124268 0
0.939169883728027 0
0.946264088153839 0
0.953358590602875 0
0.962566018104553 0
0.971320688724518 0
0.977056622505188 0
0.985358476638794 0
0.99305659532547 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/CBTr/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0833999887108803 0.226099923253059
0.0995999798178673 0.210100129246712
0.111399948596954 0.202599912881851
0.12219999730587 0.198699906468391
0.133000299334526 0.195199832320213
0.143299728631973 0.191800311207771
0.153900325298309 0.188299953937531
0.163800090551376 0.185799822211266
0.173200115561485 0.183300018310547
0.182099834084511 0.181300222873688
0.192200049757957 0.178699821233749
0.203500002622604 0.176499828696251
0.212899908423424 0.174399942159653
0.222600117325783 0.173299878835678
0.232299998402596 0.171600073575974
0.241200044751167 0.169499844312668
0.250899642705917 0.166399896144867
0.260501086711884 0.165399849414825
0.269100278615952 0.163999751210213
0.27780094742775 0.162600353360176
0.288300722837448 0.16190005838871
0.297299265861511 0.160100266337395
0.306699812412262 0.158299848437309
0.315099626779556 0.157599687576294
0.323999464511871 0.157100304961205
0.332900136709213 0.155700176954269
0.34170013666153 0.154300004243851
0.35090047121048 0.152900010347366
0.360500305891037 0.150999680161476
0.370599865913391 0.14999982714653
0.38099992275238 0.149099946022034
0.389700084924698 0.145200446248055
0.39979949593544 0.142700433731079
0.409399062395096 0.141400352120399
0.417699992656708 0.14029960334301
0.427099704742432 0.138799980282784
0.435799717903137 0.138100028038025
0.445400387048721 0.13750022649765
0.453899890184402 0.136499911546707
0.464099764823914 0.136099964380264
0.473499894142151 0.135599941015244
0.483000099658966 0.135500013828278
0.490900009870529 0.134899646043777
0.498299986124039 0.134099796414375
0.508699476718903 0.13349986076355
0.517999470233917 0.132599979639053
0.526500999927521 0.131799980998039
0.535398662090302 0.130800276994705
0.545400857925415 0.130000233650208
0.554900467395782 0.129399880766869
0.565100908279419 0.128300234675407
0.575199544429779 0.127400562167168
0.584299445152283 0.126300543546677
0.593401193618774 0.125800356268883
0.602298855781555 0.125099629163742
0.611701488494873 0.124599866569042
0.620599687099457 0.123900108039379
0.63060075044632 0.122899852693081
0.640601217746735 0.122399963438511
0.650498807430267 0.122100003063679
0.659401416778564 0.121800012886524
0.669301748275757 0.121500015258789
0.679000556468964 0.121100008487701
0.688900113105774 0.10819997638464
0.698899805545807 0.104199804365635
0.708098113536835 0.103599950671196
0.71779990196228 0.102799855172634
0.728801071643829 0.102100029587746
0.738000094890594 0.101899951696396
0.747099220752716 0.101000033318996
0.755299270153046 0.0995997861027718
0.763400018215179 0.0989000052213669
0.771700322628021 0.0984000340104103
0.782900810241699 0.0978998094797134
0.790599346160889 0.0971999317407608
0.801199734210968 0.09650007635355
0.810099124908447 0.0959998890757561
0.819801688194275 0.0952001959085464
0.828899681568146 0.0941999852657318
0.837899804115295 0.0933999270200729
0.84670078754425 0.0927999392151833
0.856799304485321 0.0918000862002373
0.864999711513519 0.0908999219536781
0.872900009155273 0.0898999273777008
0.880900204181671 0.0893000736832619
0.888299822807312 0.088999979197979
0.896800577640533 0.088900052011013
0.904700219631195 0.088299997150898
0.912500023841858 0.0878999829292297
0.920400381088257 0.0875001177191734
0.927400171756744 0.0867000073194504
0.935400009155273 0.0861000344157219
0.942599713802338 0.0848999693989754
0.949999988079071 0.0833001062273979
0.957799971103668 0.0818998664617538
0.967899978160858 0.0802001357078552
0.973900020122528 0.0793998762965202
0.981899976730347 0.078299954533577
0.991299986839294 0.0763000026345253
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.879184663295746 0.226099923253059
0.8820960521698 0.210100129246712
0.885007441043854 0.202599912881851
0.886462807655334 0.198699906468391
0.887918591499329 0.195199832320213
0.889374196529388 0.191800311207771
0.890829801559448 0.188299953937531
0.892285406589508 0.185799822211266
0.893740892410278 0.183300018310547
0.893740892410278 0.181300222873688
0.896652102470398 0.178699821233749
0.898107707500458 0.176499828696251
0.898107707500458 0.174399942159653
0.901018917560577 0.173299878835678
0.903930068016052 0.171600073575974
0.905385732650757 0.169499844312668
0.908296883106232 0.166399896144867
0.908296883106232 0.165399849414825
0.908296883106232 0.163999751210213
0.909752547740936 0.162600353360176
0.912663757801056 0.16190005838871
0.914119362831116 0.160100266337395
0.917030572891235 0.158299848437309
0.917030572891235 0.157599687576294
0.917030572891235 0.157100304961205
0.918486177921295 0.155700176954269
0.919941782951355 0.154300004243851
0.921397387981415 0.152900010347366
0.921397387981415 0.150999680161476
0.922852873802185 0.14999982714653
0.924308657646179 0.149099946022034
0.925764203071594 0.145200446248055
0.927219808101654 0.142700433731079
0.927219808101654 0.141400352120399
0.927219808101654 0.14029960334301
0.927219808101654 0.138799980282784
0.928675413131714 0.138100028038025
0.931586623191833 0.13750022649765
0.933042228221893 0.136499911546707
0.934497714042664 0.136099964380264
0.937408924102783 0.135599941015244
0.937408924102783 0.135500013828278
0.937408924102783 0.134899646043777
0.937408924102783 0.134099796414375
0.937408924102783 0.13349986076355
0.938864648342133 0.132599979639053
0.940320253372192 0.131799980998039
0.940320253372192 0.130800276994705
0.940320253372192 0.130000233650208
0.941775858402252 0.129399880766869
0.941775858402252 0.128300234675407
0.946142673492432 0.127400562167168
0.946142673492432 0.126300543546677
0.949053883552551 0.125800356268883
0.949053883552551 0.125099629163742
0.950509488582611 0.124599866569042
0.950509488582611 0.123900108039379
0.951965093612671 0.122899852693081
0.951965093612671 0.122399963438511
0.951965093612671 0.122100003063679
0.951965093612671 0.121800012886524
0.951965093612671 0.121500015258789
0.951965093612671 0.121100008487701
0.953420698642731 0.10819997638464
0.954876244068146 0.104199804365635
0.954876244068146 0.103599950671196
0.954876244068146 0.102799855172634
0.960698664188385 0.102100029587746
0.963609874248505 0.101899951696396
0.965065479278564 0.101000033318996
0.965065479278564 0.0995997861027718
0.967976689338684 0.0989000052213669
0.967976689338684 0.0984000340104103
0.969432294368744 0.0978998094797134
0.972343504428864 0.0971999317407608
0.976710319519043 0.09650007635355
0.976710319519043 0.0959998890757561
0.978165924549103 0.0952001959085464
0.979621529579163 0.0941999852657318
0.979621529579163 0.0933999270200729
0.981077134609222 0.0927999392151833
0.983988344669342 0.0918000862002373
0.985443949699402 0.0908999219536781
0.986899554729462 0.0898999273777008
0.989810764789581 0.0893000736832619
0.989810764789581 0.088999979197979
0.989810764789581 0.088900052011013
0.989810764789581 0.088299997150898
0.989810764789581 0.0878999829292297
0.989810764789581 0.0875001177191734
0.989810764789581 0.0867000073194504
0.989810764789581 0.0861000344157219
0.992721974849701 0.0848999693989754
0.994177579879761 0.0833001062273979
0.994177579879761 0.0818998664617538
0.994177579879761 0.0802001357078552
0.994177579879761 0.0793998762965202
0.995633184909821 0.078299954533577
0.99854439496994 0.0763000026345253
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0784856826066971 0.226099923253059
0.109879955649376 0.210100129246712
0.123730324208736 0.202599912881851
0.134810760617256 0.198699906468391
0.152354598045349 0.195199832320213
0.162511482834816 0.191800311207771
0.174515262246132 0.188299953937531
0.190212368965149 0.185799822211266
0.199445962905884 0.183300018310547
0.210526302456856 0.181300222873688
0.219759911298752 0.178699821233749
0.229916930198669 0.176499828696251
0.237303778529167 0.174399942159653
0.243767306208611 0.173299878835678
0.251154452562332 0.171600073575974
0.260387688875198 0.169499844312668
0.271468132734299 0.166399896144867
0.277931690216064 0.165399849414825
0.285318583250046 0.163999751210213
0.297322541475296 0.162600353360176
0.306555718183517 0.16190005838871
0.312096178531647 0.160100266337395
0.325023114681244 0.158299848437309
0.329639971256256 0.157599687576294
0.338873445987701 0.157100304961205
0.350876957178116 0.155700176954269
0.361957609653473 0.154300004243851
0.371191114187241 0.152900010347366
0.374884456396103 0.150999680161476
0.383194863796234 0.14999982714653
0.393351793289185 0.149099946022034
0.401661992073059 0.145200446248055
0.414589107036591 0.142700433731079
0.425669431686401 0.141400352120399
0.435826420783997 0.14029960334301
0.446906745433807 0.138799980282784
0.457987040281296 0.138100028038025
0.47091406583786 0.13750022649765
0.478301018476486 0.136499911546707
0.48476454615593 0.136099964380264
0.493998199701309 0.135599941015244
0.503232061862946 0.135500013828278
0.506001949310303 0.134899646043777
0.509695112705231 0.134099796414375
0.521699130535126 0.13349986076355
0.530932068824768 0.132599979639053
0.535549461841583 0.131799980998039
0.551246285438538 0.130800276994705
0.559557259082794 0.130000233650208
0.571560919284821 0.129399880766869
0.580794095993042 0.128300234675407
0.587257564067841 0.127400562167168
0.593721508979797 0.126300543546677
0.599261879920959 0.125800356268883
0.610342025756836 0.125099629163742
0.621421754360199 0.124599866569042
0.629732310771942 0.123900108039379
0.639889180660248 0.122899852693081
0.647275507450104 0.122399963438511
0.65373969078064 0.122100003063679
0.663896441459656 0.121800012886524
0.671283543109894 0.121500015258789
0.677747189998627 0.121100008487701
0.686056852340698 0.10819997638464
0.695290565490723 0.104199804365635
0.705447554588318 0.103599950671196
0.719298243522644 0.102799855172634
0.7285315990448 0.102100029587746
0.736841797828674 0.101899951696396
0.746075630187988 0.101000033318996
0.754385948181152 0.0995997861027718
0.761772811412811 0.0989000052213669
0.768236517906189 0.0984000340104103
0.782086849212646 0.0978998094797134
0.789473712444305 0.0971999317407608
0.800553798675537 0.09650007635355
0.80794095993042 0.0959998890757561
0.819944381713867 0.0952001959085464
0.82548463344574 0.0941999852657318
0.831024944782257 0.0933999270200729
0.8374884724617 0.0927999392151833
0.846722006797791 0.0918000862002373
0.854109048843384 0.0908999219536781
0.861495792865753 0.0898999273777008
0.870729327201843 0.0893000736832619
0.87534636259079 0.088999979197979
0.886426568031311 0.088900052011013
0.89289003610611 0.088299997150898
0.901200532913208 0.0878999829292297
0.904893815517426 0.0875001177191734
0.915974080562592 0.0867000073194504
0.921514391899109 0.0861000344157219
0.928901195526123 0.0848999693989754
0.942751586437225 0.0833001062273979
0.953831970691681 0.0818998664617538
0.962142169475555 0.0802001357078552
0.969529092311859 0.0793998762965202
0.979686081409454 0.078299954533577
0.986149609088898 0.0763000026345253
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0176184680312872 0.226099923253059
0.032928328961134 0.210100129246712
0.0452004596590996 0.202599912881851
0.0567436218261719 0.198699906468391
0.0674361661076546 0.195199832320213
0.0784934312105179 0.191800311207771
0.0896718129515648 0.188299953937531
0.0995139554142952 0.185799822211266
0.109599053859711 0.183300018310547
0.118955060839653 0.181300222873688
0.129769012331963 0.178699821233749
0.142041012644768 0.176499828696251
0.152490720152855 0.174399942159653
0.163183569908142 0.173299878835678
0.173754528164864 0.171600073575974
0.183231934905052 0.169499844312668
0.19331718981266 0.166399896144867
0.204131260514259 0.165399849414825
0.213608726859093 0.163999751210213
0.222478702664375 0.162600353360176
0.233778864145279 0.16190005838871
0.243863880634308 0.160100266337395
0.253340631723404 0.158299848437309
0.262939542531967 0.157599687576294
0.27253919839859 0.157100304961205
0.281652480363846 0.155700176954269
0.290766388177872 0.154300004243851
0.300607740879059 0.152900010347366
0.311785876750946 0.150999680161476
0.322842717170715 0.14999982714653
0.334022521972656 0.149099946022034
0.3433777987957 0.145200446248055
0.353827327489853 0.142700433731079
0.36403414607048 0.141400352120399
0.372782617807388 0.14029960334301
0.38274610042572 0.138799980282784
0.391737431287766 0.138100028038025
0.401458084583282 0.13750022649765
0.410692483186722 0.136499911546707
0.422114282846451 0.136099964380264
0.432077586650848 0.135599941015244
0.442405700683594 0.135500013828278
0.451640337705612 0.134899646043777
0.460145831108093 0.134099796414375
0.471202909946442 0.13349986076355
0.481166452169418 0.132599979639053
0.490765511989594 0.131799980998039
0.499514222145081 0.130800276994705
0.51057106256485 0.130000233650208
0.5204136967659 0.129399880766869
0.531593263149261 0.128300234675407
0.542649865150452 0.127400562167168
0.552856147289276 0.126300543546677
0.562940537929535 0.125800356268883
0.572296619415283 0.125099629163742
0.58214008808136 0.124599866569042
0.591858804225922 0.123900108039379
0.602553308010101 0.122899852693081
0.613729655742645 0.122399963438511
0.624908268451691 0.122100003063679
0.634386420249939 0.121800012886524
0.645443439483643 0.121500015258789
0.656377792358398 0.121100008487701
0.667193531990051 0.10819997638464
0.678006827831268 0.104199804365635
0.687848567962646 0.103599950671196
0.697812616825104 0.102799855172634
0.709476351737976 0.102100029587746
0.719320356845856 0.101899951696396
0.729040563106537 0.101000033318996
0.737909078598022 0.0995997861027718
0.746537029743195 0.0989000052213669
0.755771577358246 0.0984000340104103
0.76743620634079 0.0978998094797134
0.775577485561371 0.0971999317407608
0.786634147167206 0.09650007635355
0.796476542949677 0.0959998890757561
0.806560873985291 0.0952001959085464
0.816768050193787 0.0941999852657318
0.826973974704742 0.0933999270200729
0.83669513463974 0.0927999392151833
0.847509443759918 0.0918000862002373
0.856379151344299 0.0908999219536781
0.864884436130524 0.0898999273777008
0.873146772384644 0.0893000736832619
0.881531059741974 0.088999979197979
0.890401244163513 0.088900052011013
0.899149477481842 0.088299997150898
0.907533288002014 0.0878999829292297
0.916646182537079 0.0875001177191734
0.923693776130676 0.0867000073194504
0.932685196399689 0.0861000344157219
0.940218806266785 0.0848999693989754
0.947266221046448 0.0833001062273979
0.955285549163818 0.0818998664617538
0.966464221477509 0.0802001357078552
0.97278243303299 0.0793998762965202
0.981044948101044 0.078299954533577
0.991373002529144 0.0763000026345253
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/CHM/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0780997946858406 0.321199744939804
0.0917002037167549 0.321199744939804
0.105200000107288 0.321199744939804
0.115099973976612 0.321199744939804
0.126499846577644 0.321000337600708
0.137499824166298 0.320899963378906
0.146500065922737 0.320800185203552
0.156500086188316 0.320099472999573
0.166499838232994 0.319800019264221
0.177000030875206 0.318100541830063
0.186500579118729 0.316699951887131
0.197900205850601 0.31499919295311
0.208700001239777 0.312600523233414
0.21819980442524 0.309900164604187
0.227099895477295 0.306600004434586
0.23729994893074 0.303399294614792
0.247600436210632 0.298800557851791
0.257599771022797 0.293299287557602
0.265900135040283 0.28809979557991
0.27580001950264 0.281799554824829
0.286899745464325 0.275899648666382
0.296901524066925 0.269899278879166
0.306700795888901 0.262200385332108
0.315800756216049 0.255999058485031
0.32519993185997 0.248899787664413
0.335400015115738 0.242700099945068
0.344700157642365 0.23489998281002
0.354599863290787 0.228100165724754
0.364499896764755 0.218600004911423
0.374600112438202 0.207599997520447
0.384600132703781 0.20010007917881
0.392499357461929 0.189799889922142
0.402200222015381 0.177599936723709
0.411899864673615 0.16749981045723
0.421700000762939 0.157500043511391
0.431500136852264 0.147799909114838
0.43889981508255 0.137800022959709
0.449499905109406 0.128799960017204
0.457299888134003 0.120000012218952
0.468000054359436 0.110100023448467
0.47760009765625 0.0988999158143997
0.487199991941452 0.0884002074599266
0.495500236749649 0.0780000239610672
0.502997577190399 0.0683001130819321
0.511898159980774 0.0619001761078835
0.520202100276947 0.053999986499548
0.529398798942566 0.0465000011026859
0.53869903087616 0.0400998815894127
0.548401296138763 0.0352000147104263
0.558598697185516 0.0299999825656414
0.568900167942047 0.0262999963015318
0.578201234340668 0.0211000069975853
0.587700664997101 0.0176999792456627
0.598300337791443 0.0149000193923712
0.606000423431396 0.0120000103488564
0.616599440574646 0.00900000240653753
0.626101136207581 0.0071999984793365
0.635099589824677 0.00590000860393047
0.64560067653656 0.00389999803155661
0.655798435211182 0.00349999382160604
0.6644007563591 0.00229999353177845
0.674599528312683 0.00150000036228448
0.684200525283813 0.00119999900925905
0.693499207496643 0.00119999900925905
0.703499317169189 0.000999999814666808
0.71320104598999 0.000599998980760574
0.722401142120361 0.000499999907333404
0.732300221920013 9.99997646431439e-05
0.741301000118256 9.99997646431439e-05
0.750999271869659 0
0.759600341320038 0
0.767699480056763 0
0.776699364185333 0
0.787601172924042 0
0.795400261878967 0
0.805700361728668 0
0.814499795436859 0
0.825200378894806 0
0.834299981594086 0
0.842800378799438 0
0.851498603820801 0
0.861299932003021 0
0.870200216770172 0
0.87749981880188 0
0.88539981842041 0
0.892499923706055 0
0.902299404144287 0
0.909599721431732 0
0.916400015354156 0
0.924499809741974 0
0.932200014591217 0
0.939799785614014 0
0.947799980640411 0
0.955999970436096 0
0.963200211524963 0
0.972299993038177 0
0.978799998760223 0
0.986100018024445 0
0.992399990558624 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.869942307472229 0.321199744939804
0.878612816333771 0.321199744939804
0.884393155574799 0.321199744939804
0.887283325195312 0.321199744939804
0.893063426017761 0.321000337600708
0.89450865983963 0.320899963378906
0.895953774452209 0.320800185203552
0.897398829460144 0.320099472999573
0.900288999080658 0.319800019264221
0.900288999080658 0.318100541830063
0.903179168701172 0.316699951887131
0.904624164104462 0.31499919295311
0.904624164104462 0.312600523233414
0.907514452934265 0.309900164604187
0.910404801368713 0.306600004434586
0.911849737167358 0.303399294614792
0.914739727973938 0.298800557851791
0.914739727973938 0.293299287557602
0.914739727973938 0.28809979557991
0.916184961795807 0.281799554824829
0.919075131416321 0.275899648666382
0.9205202460289 0.269899278879166
0.921965301036835 0.262200385332108
0.921965301036835 0.255999058485031
0.921965301036835 0.248899787664413
0.923410415649414 0.242700099945068
0.924855411052704 0.23489998281002
0.926300644874573 0.228100165724754
0.926300644874573 0.218600004911423
0.927745640277863 0.207599997520447
0.929190754890442 0.20010007917881
0.930635809898376 0.189799889922142
0.930635809898376 0.177599936723709
0.930635809898376 0.16749981045723
0.930635809898376 0.157500043511391
0.930635809898376 0.147799909114838
0.930635809898376 0.137800022959709
0.933526039123535 0.128799960017204
0.93497109413147 0.120000012218952
0.93641608953476 0.110100023448467
0.939306259155273 0.0988999158143997
0.939306259155273 0.0884002074599266
0.939306259155273 0.0780000239610672
0.939306259155273 0.0683001130819321
0.939306259155273 0.0619001761078835
0.940751433372498 0.053999986499548
0.942196547985077 0.0465000011026859
0.942196547985077 0.0400998815894127
0.942196547985077 0.0352000147104263
0.942196547985077 0.0299999825656414
0.942196547985077 0.0262999963015318
0.946531772613525 0.0211000069975853
0.946531772613525 0.0176999792456627
0.949421942234039 0.0149000193923712
0.949421942234039 0.0120000103488564
0.950867056846619 0.00900000240653753
0.950867056846619 0.0071999984793365
0.952312111854553 0.00590000860393047
0.952312111854553 0.00389999803155661
0.952312111854553 0.00349999382160604
0.952312111854553 0.00229999353177845
0.952312111854553 0.00150000036228448
0.952312111854553 0.00119999900925905
0.953757226467133 0.00119999900925905
0.955202341079712 0.000999999814666808
0.955202341079712 0.000599998980760574
0.955202341079712 0.000499999907333404
0.96098268032074 9.99997646431439e-05
0.963872849941254 9.99997646431439e-05
0.965317904949188 0
0.965317904949188 0
0.968208074569702 0
0.968208074569702 0
0.969653189182281 0
0.972543358802795 0
0.976878583431244 0
0.976878583431244 0
0.978323698043823 0
0.979768812656403 0
0.979768812656403 0
0.981213867664337 0
0.984104037284851 0
0.98554915189743 0
0.986994206905365 0
0.989884376525879 0
0.989884376525879 0
0.989884376525879 0
0.989884376525879 0
0.989884376525879 0
0.989884376525879 0
0.989884376525879 0
0.989884376525879 0
0.992774546146393 0
0.994219660758972 0
0.994219660758972 0
0.994219660758972 0
0.994219660758972 0
0.995664715766907 0
0.998554885387421 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0662313997745514 0.321199744939804
0.0970149338245392 0.321199744939804
0.128731459379196 0.321199744939804
0.147387981414795 0.321199744939804
0.165111973881721 0.321000337600708
0.180970177054405 0.320899963378906
0.19309701025486 0.320800185203552
0.212686598300934 0.320099472999573
0.225746273994446 0.319800019264221
0.244402870535851 0.318100541830063
0.254664421081543 0.316699951887131
0.270522505044937 0.31499919295311
0.280783414840698 0.312600523233414
0.286380618810654 0.309900164604187
0.293843269348145 0.306600004434586
0.304104506969452 0.303399294614792
0.315298408269882 0.298800557851791
0.3255595266819 0.293299287557602
0.333022445440292 0.28809979557991
0.342350780963898 0.281799554824829
0.352612137794495 0.275899648666382
0.359141975641251 0.269899278879166
0.374067068099976 0.262200385332108
0.379664123058319 0.255999058485031
0.387127071619034 0.248899787664413
0.401119381189346 0.242700099945068
0.412313461303711 0.23489998281002
0.419775992631912 0.228100165724754
0.424440324306488 0.218600004911423
0.431902974843979 0.207599997520447
0.442164182662964 0.20010007917881
0.449626863002777 0.189799889922142
0.460820943117142 0.177599936723709
0.470149308443069 0.16749981045723
0.479477614164352 0.157500043511391
0.489738792181015 0.147799909114838
0.499067276716232 0.137800022959709
0.513059735298157 0.128799960017204
0.520522356033325 0.120000012218952
0.527985095977783 0.110100023448467
0.535448014736176 0.0988999158143997
0.54384309053421 0.0884002074599266
0.546641647815704 0.0780000239610672
0.550372838973999 0.0683001130819321
0.561567008495331 0.0619001761078835
0.569029748439789 0.053999986499548
0.573694229125977 0.0465000011026859
0.590485274791718 0.0400998815894127
0.597014784812927 0.0352000147104263
0.60634309053421 0.0299999825656414
0.616604566574097 0.0262999963015318
0.624066650867462 0.0211000069975853
0.630596995353699 0.0176999792456627
0.636193990707397 0.0149000193923712
0.647388279438019 0.0120000103488564
0.657649278640747 0.00900000240653753
0.666044592857361 0.0071999984793365
0.67257434129715 0.00590000860393047
0.680037260055542 0.00389999803155661
0.683768451213837 0.00349999382160604
0.69402951002121 0.00229999353177845
0.700559616088867 0.00150000036228448
0.705223739147186 0.00119999900925905
0.712686538696289 0.00119999900925905
0.722014665603638 0.000999999814666808
0.732276082038879 0.000599998980760574
0.742537200450897 0.000499999907333404
0.749999821186066 9.99997646431439e-05
0.757462680339813 9.99997646431439e-05
0.766791224479675 0
0.774253904819489 0
0.782649278640747 0
0.787313520908356 0
0.800373017787933 0
0.807835698127747 0
0.819029927253723 0
0.825559735298157 0
0.83488804101944 0
0.840484976768494 0
0.846082031726837 0
0.851679027080536 0
0.860074639320374 0
0.867537081241608 0
0.874999940395355 0
0.884328305721283 0
0.888992488384247 0
0.901119410991669 0
0.907649338245392 0
0.914179027080536 0
0.91791045665741 0
0.929104447364807 0
0.933768570423126 0
0.940298438072205 0
0.951492488384247 0
0.962686538696289 0
0.970149278640747 0
0.976679086685181 0
0.985074639320374 0
0.990671634674072 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0131131578236818 0.321199744939804
0.0248907245695591 0.321199744939804
0.0366682708263397 0.321199744939804
0.0460175126791 0.321199744939804
0.0570665299892426 0.321000337600708
0.0682370811700821 0.320899963378906
0.0774648264050484 0.320800185203552
0.0869353786110878 0.320099472999573
0.0971345156431198 0.319800019264221
0.107455052435398 0.318100541830063
0.117411352694035 0.316699951887131
0.129067301750183 0.31499919295311
0.140845358371735 0.312600523233414
0.151408493518829 0.309900164604187
0.161000460386276 0.306600004434586
0.171927899122238 0.303399294614792
0.182734370231628 0.298800557851791
0.193540707230568 0.293299287557602
0.202646881341934 0.28809979557991
0.213331699371338 0.281799554824829
0.2252307087183 0.275899648666382
0.236401215195656 0.269899278879166
0.24623604118824 0.262200385332108
0.256556451320648 0.255999058485031
0.266999274492264 0.248899787664413
0.277440279722214 0.242700099945068
0.28715443611145 0.23489998281002
0.29808235168457 0.228100165724754
0.309495210647583 0.218600004911423
0.320665836334229 0.207599997520447
0.331350237131119 0.20010007917881
0.339849501848221 0.189799889922142
0.350170224905014 0.177599936723709
0.360733270645142 0.16749981045723
0.371417999267578 0.157500043511391
0.381981372833252 0.147799909114838
0.389752179384232 0.137800022959709
0.40055850148201 0.128799960017204
0.408936202526093 0.120000012218952
0.420835494995117 0.110100023448467
0.431277304887772 0.0988999158143997
0.441840648651123 0.0884002074599266
0.451554149389267 0.0780000239610672
0.460174798965454 0.0683001130819321
0.469524025917053 0.0619001761078835
0.478508979082108 0.053999986499548
0.488951057195663 0.0465000011026859
0.498057305812836 0.0400998815894127
0.508985817432404 0.0352000147104263
0.520155668258667 0.0299999825656414
0.531324565410614 0.0262999963015318
0.541283249855042 0.0211000069975853
0.551968038082123 0.0176999792456627
0.563865482807159 0.0149000193923712
0.571758508682251 0.0120000103488564
0.583171725273132 0.00900000240653753
0.593613624572754 0.0071999984793365
0.603570640087128 0.00590000860393047
0.615346193313599 0.00389999803155661
0.62724632024765 0.00349999382160604
0.636352837085724 0.00229999353177845
0.647886097431183 0.00150000036228448
0.658936202526093 0.00119999900925905
0.669136226177216 0.00119999900925905
0.679941058158875 0.000999999814666808
0.690383434295654 0.000599998980760574
0.700219452381134 0.000499999907333404
0.710780739784241 9.99997646431439e-05
0.720495641231537 9.99997646431439e-05
0.730937242507935 0
0.740408420562744 0
0.748906970024109 0
0.759227156639099 0
0.770641088485718 0
0.778897285461426 0
0.789582371711731 0
0.799417853355408 0
0.811073184013367 0
0.821272253990173 0
0.830864310264587 0
0.840578079223633 0
0.851141512393951 0
0.860854685306549 0
0.868625402450562 0
0.876760542392731 0
0.884774029254913 0
0.895094811916351 0
0.903108417987823 0
0.910514712333679 0
0.919863998889923 0
0.927756309509277 0
0.936376750469208 0
0.944997429847717 0
0.953375399112701 0
0.960660517215729 0
0.970738232135773 0
0.97778046131134 0
0.98542982339859 0
0.992107808589935 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/List/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0917003154754639 0.320199459791183
0.103800095617771 0.314799696207047
0.114599965512753 0.297500133514404
0.124299935996532 0.2621990442276
0.134299963712692 0.210200294852257
0.144300103187561 0.152899906039238
0.154299795627594 0.100599832832813
0.164100557565689 0.0584999993443489
0.172700151801109 0.0299999993294477
0.181999906897545 0.0147999934852123
0.191699981689453 0.00579999946057796
0.202400043606758 0.00290000275708735
0.212500005960464 0.000399999058572575
0.221900001168251 0
0.231000050902367 0
0.241200000047684 0
0.2510986328125 0
0.261299580335617 0
0.268800020217896 0
0.278400123119354 0
0.289499789476395 0
0.298899620771408 0
0.309699565172195 0
0.31950119137764 0
0.329299658536911 0
0.338799834251404 0
0.347399413585663 0
0.35590010881424 0
0.366099745035172 0
0.376599937677383 0
0.385900437831879 0
0.394699960947037 0
0.404600620269775 0
0.414400011301041 0
0.423900097608566 0
0.433300197124481 0
0.441500097513199 0
0.45159986615181 0
0.459700107574463 0
0.470700085163116 0
0.481099992990494 0
0.490799993276596 0
0.49859955906868 0
0.50709867477417 0
0.515299677848816 0
0.52470064163208 0
0.533399343490601 0
0.54220175743103 0
0.552300572395325 0
0.562399804592133 0
0.572600245475769 0
0.582800269126892 0
0.591399490833282 0
0.600798726081848 0
0.608599841594696 0
0.61809915304184 0
0.627401053905487 0
0.637700438499451 0
0.647600710391998 0
0.65840071439743 0
0.666401326656342 0
0.676799595355988 0
0.686699628829956 0
0.696900606155396 0
0.707299947738647 0
0.716299951076508 0
0.725499391555786 0
0.734900057315826 0
0.743899941444397 0
0.752999305725098 0
0.761499047279358 0
0.770000338554382 0
0.778400361537933 0
0.789699912071228 0
0.798599600791931 0
0.808200418949127 0
0.817400753498077 0
0.82800018787384 0
0.836899399757385 0
0.845599412918091 0
0.85410088300705 0
0.863999724388123 0
0.87299919128418 0
0.880500376224518 0
0.8886998295784 0
0.895899891853333 0
0.903599798679352 0
0.911200106143951 0
0.918000221252441 0
0.925999879837036 0
0.933499991893768 0
0.940999805927277 0
0.94769960641861 0
0.955399990081787 0
0.962700068950653 0
0.972699999809265 0
0.978699803352356 0
0.985499978065491 0
0.992699980735779 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.879008829593658 0.320199459791183
0.881924211978912 0.314799696207047
0.884839534759521 0.297500133514404
0.886297225952148 0.2621990442276
0.886297225952148 0.210200294852257
0.887755215167999 0.152899906039238
0.889212906360626 0.100599832832813
0.890670537948608 0.0584999993443489
0.89212828874588 0.0299999993294477
0.89212828874588 0.0147999934852123
0.895043730735779 0.00579999946057796
0.896501481533051 0.00290000275708735
0.896501481533051 0.000399999058572575
0.899416923522949 0
0.902332365512848 0
0.905247807502747 0
0.908163249492645 0
0.908163249492645 0
0.908163249492645 0
0.909621000289917 0
0.912536442279816 0
0.913994193077087 0
0.915451884269714 0
0.915451884269714 0
0.918367326259613 0
0.919825077056885 0
0.921282708644867 0
0.922740638256073 0
0.922740638256073 0
0.924198269844055 0
0.925655961036682 0
0.927113711833954 0
0.927113711833954 0
0.927113711833954 0
0.927113711833954 0
0.927113711833954 0
0.927113711833954 0
0.930029153823853 0
0.931486904621124 0
0.932944595813751 0
0.93586003780365 0
0.93586003780365 0
0.93586003780365 0
0.93586003780365 0
0.93586003780365 0
0.937317669391632 0
0.938775539398193 0
0.938775539398193 0
0.938775539398193 0
0.938775539398193 0
0.938775539398193 0
0.943148672580719 0
0.943148672580719 0
0.946064114570618 0
0.946064114570618 0
0.947521865367889 0
0.947521865367889 0
0.948979616165161 0
0.948979616165161 0
0.948979616165161 0
0.948979616165161 0
0.948979616165161 0
0.948979616165161 0
0.950437307357788 0
0.95189505815506 0
0.95189505815506 0
0.95189505815506 0
0.957725942134857 0
0.960641384124756 0
0.963556826114655 0
0.963556826114655 0
0.966472327709198 0
0.966472327709198 0
0.967930018901825 0
0.970845460891724 0
0.975218653678894 0
0.975218653678894 0
0.976676404476166 0
0.978134095668793 0
0.978134095668793 0
0.979591846466064 0
0.982507288455963 0
0.983965039253235 0
0.985422730445862 0
0.98833817243576 0
0.98833817243576 0
0.98833817243576 0
0.98833817243576 0
0.98833817243576 0
0.98833817243576 0
0.98833817243576 0
0.98833817243576 0
0.991253674030304 0
0.992711365222931 0
0.992711365222931 0
0.994169116020203 0
0.994169116020203 0
0.99562680721283 0
0.998542249202728 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.167680263519287 0.320199459791183
0.185925245285034 0.314799696207047
0.194613412022591 0.297500133514404
0.207645505666733 0.2621990442276
0.218940064311028 0.210200294852257
0.226759344339371 0.152899906039238
0.235447436571121 0.100599832832813
0.251086056232452 0.0584999993443489
0.258036524057388 0.0299999993294477
0.269331037998199 0.0147999934852123
0.279756754636765 0.00579999946057796
0.291051298379898 0.00290000275708735
0.297133088111877 0.000399999058572575
0.302345633506775 0
0.310164958238602 0
0.321459501981735 0
0.331885159015656 0
0.341442316770554 0
0.347523778676987 0
0.3544742166996 0
0.364900231361389 0
0.370981723070145 0
0.384882777929306 0
0.390964418649673 0
0.39965233206749 0
0.413553446531296 0
0.423110246658325 0
0.430929630994797 0
0.434404879808426 0
0.441355407238007 0
0.449174642562866 0
0.457862615585327 0
0.468288451433182 0
0.478714168071747 0
0.489139884710312 0
0.499565690755844 0
0.509991765022278 0
0.523023545742035 0
0.529974043369293 0
0.536924123764038 0
0.543875396251678 0
0.552562117576599 0
0.554300844669342 0
0.558644711971283 0
0.569070637226105 0
0.576889753341675 0
0.582971453666687 0
0.59861034154892 0
0.60469126701355 0
0.61424857378006 0
0.622936546802521 0
0.629018247127533 0
0.634231388568878 0
0.641181707382202 0
0.653344988822937 0
0.664639413356781 0
0.672458708286285 0
0.679409325122833 0
0.687228500843048 0
0.690703511238098 0
0.700260937213898 0
0.707211136817932 0
0.712423384189606 0
0.719374537467957 0
0.728062510490417 0
0.738488733768463 0
0.749783277511597 0
0.756733417510986 0
0.764552533626556 0
0.773240685462952 0
0.78019118309021 0
0.786272764205933 0
0.790617048740387 0
0.802779912948608 0
0.809730768203735 0
0.820156574249268 0
0.827106356620789 0
0.835795164108276 0
0.841008007526398 0
0.847957968711853 0
0.853171408176422 0
0.860990524291992 0
0.868809759616852 0
0.876629233360291 0
0.885317146778107 0
0.889661192893982 0
0.900086760520935 0
0.907906353473663 0
0.913987815380096 0
0.917463064193726 0
0.929626524448395 0
0.93397045135498 0
0.940920948982239 0
0.952215492725372 0
0.962641179561615 0
0.969591677188873 0
0.976542115211487 0
0.985230207443237 0
0.99131190776825 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.014822980388999 0.320199459791183
0.0268283747136593 0.314799696207047
0.038588747382164 0.297500133514404
0.0485116131603718 0.2621990442276
0.0591694228351116 0.210200294852257
0.0701946616172791 0.152899906039238
0.0810976922512054 0.100599832832813
0.0907754525542259 0.0584999993443489
0.100208304822445 0.0299999993294477
0.110008575022221 0.0147999934852123
0.120176434516907 0.00579999946057796
0.131569191813469 0.00290000275708735
0.143085017800331 0.000399999058572575
0.153619512915611 0
0.163420230150223 0
0.174077942967415 0
0.184491083025932 0
0.195638939738274 0
0.203969165682793 0
0.214626982808113 0
0.226509839296341 0
0.237045347690582 0
0.248193293809891 0
0.259341329336166 0
0.26987686753273 0
0.27943167090416 0
0.288497239351273 0
0.297684669494629 0
0.309690058231354 0
0.321450442075729 0
0.331618070602417 0
0.341050922870636 0
0.351708739995956 0
0.362244158983231 0
0.372411876916885 0
0.382457315921783 0
0.391033142805099 0
0.401323020458221 0
0.410143136978149 0
0.422516226768494 0
0.43403172492981 0
0.444689273834229 0
0.453999876976013 0
0.463800013065338 0
0.472375333309174 0
0.482665777206421 0
0.492343634366989 0
0.50091952085495 0
0.512436091899872 0
0.523458659648895 0
0.534730076789856 0
0.545998811721802 0
0.555800199508667 0
0.566090762615204 0
0.573931455612183 0
0.583853840827942 0
0.594143450260162 0
0.605659246444702 0
0.616684913635254 0
0.629426419734955 0
0.637878239154816 0
0.649638950824738 0
0.661031126976013 0
0.672424018383026 0
0.683816730976105 0
0.69337260723114 0
0.70305073261261 0
0.713095426559448 0
0.722772657871246 0
0.73245108127594 0
0.741883993148804 0
0.751194655895233 0
0.760871589183807 0
0.772877991199493 0
0.782555103302002 0
0.792478501796722 0
0.802768528461456 0
0.814406454563141 0
0.824451923370361 0
0.834129631519318 0
0.843684792518616 0
0.854465365409851 0
0.864265441894531 0
0.872228384017944 0
0.880803763866425 0
0.889011561870575 0
0.896974265575409 0
0.905182063579559 0
0.912654638290405 0
0.921964943408966 0
0.929437577724457 0
0.938012957572937 0
0.944995641708374 0
0.952713429927826 0
0.960186243057251 0
0.971334040164948 0
0.977704286575317 0
0.984687030315399 0
0.992404758930206 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/List/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    % ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.13809996843338 0.21779990196228
0.184500113129616 0.0941999703645706
0.232799932360649 0.0296999700367451
0.281899303197861 0.00619998294860125
0.328099429607391 0.00109999603591859
0.379399955272675 0.000299999490380287
0.430000007152557 0
0.475900083780289 0
0.526400566101074 0
0.572899758815765 0
0.616797804832458 0
0.666398704051971 0
0.712900102138519 0
0.757399559020996 0
0.800800085067749 0
0.846201002597809 0
0.887300908565521 0
0.925000369548798 0
0.964099824428558 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.975728154182434 0.21779990196228
0.975728154182434 0.0941999703645706
0.978964388370514 0.0296999700367451
0.980582535266876 0.00619998294860125
0.980582535266876 0.00109999603591859
0.982200622558594 0.000299999490380287
0.983818769454956 0
0.987055003643036 0
0.987055003643036 0
0.988673150539398 0
0.988673150539398 0
0.99352753162384 0
0.99352753162384 0
0.99352753162384 0
0.995145618915558 0
0.995145618915558 0
0.99676376581192 0
0.99676376581192 0
0.998381853103638 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.378892719745636 0.21779990196228
0.425605475902557 0.0941999703645706
0.461937606334686 0.0296999700367451
0.508650302886963 0.00619998294860125
0.551902949810028 0.00109999603591859
0.591695725917816 0.000299999490380287
0.624567270278931 0
0.659169554710388 0
0.688581347465515 0
0.707612752914429 0
0.73356431722641 0
0.764705657958984 0
0.799307882785797 0
0.825259566307068 0
0.856401264667511 0
0.882352948188782 0
0.908304512500763 0
0.942906558513641 0
0.961937725543976 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0634941086173058 0.21779990196228
0.113130465149879 0.0941999703645706
0.165379628539085 0.0296999700367451
0.217969104647636 0.00619998294860125
0.267604678869247 0.00109999603591859
0.323148727416992 0.000299999490380287
0.378350466489792 0
0.427987605333328 0
0.483416736125946 0
0.534870386123657 0
0.583030104637146 0
0.636982917785645 0
0.687528669834137 0
0.736370325088501 0
0.783507406711578 0
0.833370864391327 0
0.878237307071686 0
0.9187873005867 0
0.961835503578186 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/List_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0918000414967537 0.318799406290054
0.103700198233128 0.311699867248535
0.114699974656105 0.298901319503784
0.123900063335896 0.278200328350067
0.133999943733215 0.252199858427048
0.144300535321236 0.220899924635887
0.153099820017815 0.189099803566933
0.162599965929985 0.159000083804131
0.170900225639343 0.134399771690369
0.181800216436386 0.115399979054928
0.191100224852562 0.0995999127626419
0.201999947428703 0.0879000872373581
0.213200002908707 0.0771000534296036
0.222100093960762 0.0689999908208847
0.231800004839897 0.0606000013649464
0.240299999713898 0.0522000044584274
0.250499963760376 0.042300071567297
0.260900616645813 0.036400031298399
0.269000917673111 0.0303000509738922
0.278900325298309 0.0233000069856644
0.289999812841415 0.0191999953240156
0.300000727176666 0.0153999980539083
0.309000670909882 0.0128999892622232
0.317899197340012 0.0107000125572085
0.326100260019302 0.0094999810680747
0.336599797010422 0.00790000427514315
0.345900505781174 0.00699999695643783
0.356000334024429 0.00650000292807817
0.365899831056595 0.00559999886900187
0.376100212335587 0.00530000310391188
0.386299878358841 0.00449999421834946
0.395499914884567 0.0042000045068562
0.404799968004227 0.00360000086948276
0.41520020365715 0.00329999951645732
0.424599558115005 0.00300000072456896
0.43339991569519 0.00219999602995813
0.441000193357468 0.00200000288896263
0.451100289821625 0.00149999873246998
0.459899693727493 0.00120000110473484
0.470899999141693 0.000900001148693264
0.481200039386749 0.000800001143943518
0.490000009536743 0.000800001143943518
0.497599810361862 0.000800001143943518
0.505302369594574 0.000599998980760574
0.515199542045593 0.000399999669753015
0.524800896644592 0.000299999490380287
0.534600555896759 0.000199999834876508
0.544001340866089 0.000199999834876508
0.553699433803558 9.9999931990169e-05
0.563399851322174 0
0.573599874973297 0
0.583799064159393 0
0.592499792575836 0
0.60160094499588 0
0.609900534152985 0
0.620201110839844 0
0.629099726676941 0
0.638800382614136 0
0.6494020819664 0
0.658899962902069 0
0.668499708175659 0
0.679000556468964 0
0.68740051984787 0
0.696300268173218 0
0.705498218536377 0
0.715099513530731 0
0.72359973192215 0
0.734000265598297 0
0.743598341941833 0
0.753799617290497 0
0.762300550937653 0
0.771301031112671 0
0.780300974845886 0
0.791199147701263 0
0.799600005149841 0
0.809800148010254 0
0.819300174713135 0
0.828999042510986 0
0.837900221347809 0
0.845999777317047 0
0.854199588298798 0
0.863898813724518 0
0.872800409793854 0
0.88049989938736 0
0.887600183486938 0
0.895700216293335 0
0.903999805450439 0
0.912300705909729 0
0.920400202274323 0
0.928799331188202 0
0.936599791049957 0
0.94349992275238 0
0.950200021266937 0
0.957599878311157 0
0.964099824428558 0
0.97299998998642 0
0.978799998760223 0
0.985899984836578 0
0.993099987506866 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.886931002140045 0.318799406290054
0.886931002140045 0.311699867248535
0.889867901802063 0.298901319503784
0.891336441040039 0.278200328350067
0.891336441040039 0.252199858427048
0.892804801464081 0.220899924635887
0.894273221492767 0.189099803566933
0.895741581916809 0.159000083804131
0.897210001945496 0.134399771690369
0.897210001945496 0.115399979054928
0.900146842002869 0.0995999127626419
0.901615262031555 0.0879000872373581
0.901615262031555 0.0771000534296036
0.904552102088928 0.0689999908208847
0.90748918056488 0.0606000013649464
0.908957421779633 0.0522000044584274
0.911894261837006 0.042300071567297
0.911894261837006 0.036400031298399
0.911894261837006 0.0303000509738922
0.913362681865692 0.0233000069856644
0.91629958152771 0.0191999953240156
0.917768001556396 0.0153999980539083
0.919236421585083 0.0128999892622232
0.919236421585083 0.0107000125572085
0.919236421585083 0.0094999810680747
0.92070484161377 0.00790000427514315
0.922173202037811 0.00699999695643783
0.923641800880432 0.00650000292807817
0.923641800880432 0.00559999886900187
0.925110161304474 0.00530000310391188
0.92657858133316 0.00449999421834946
0.928047001361847 0.0042000045068562
0.928047001361847 0.00360000086948276
0.928047001361847 0.00329999951645732
0.928047001361847 0.00300000072456896
0.928047001361847 0.00219999602995813
0.928047001361847 0.00200000288896263
0.93098384141922 0.00149999873246998
0.933920681476593 0.00120000110473484
0.935389161109924 0.000900001148693264
0.938326001167297 0.000800001143943518
0.938326001167297 0.000800001143943518
0.938326001167297 0.000800001143943518
0.938326001167297 0.000599998980760574
0.938326001167297 0.000399999669753015
0.939794301986694 0.000299999490380287
0.94126284122467 0.000199999834876508
0.94126284122467 0.000199999834876508
0.94126284122467 9.9999931990169e-05
0.94126284122467 0
0.94126284122467 0
0.945668160915375 0
0.945668160915375 0
0.948605000972748 0
0.948605000972748 0
0.950073421001434 0
0.950073421001434 0
0.951541841030121 0
0.951541841030121 0
0.951541841030121 0
0.951541841030121 0
0.951541841030121 0
0.951541841030121 0
0.953010261058807 0
0.954478681087494 0
0.954478681087494 0
0.954478681087494 0
0.960352420806885 0
0.963289260864258 0
0.964757680892944 0
0.964757680892944 0
0.967694580554962 0
0.967694580554962 0
0.969163000583649 0
0.972099840641022 0
0.976505160331726 0
0.976505160331726 0
0.977973580360413 0
0.979442000389099 0
0.979442000389099 0
0.980910420417786 0
0.983847260475159 0
0.98531574010849 0
0.986784160137177 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.992657840251923 0
0.994126260280609 0
0.994126260280609 0
0.994126260280609 0
0.994126260280609 0
0.99559473991394 0
0.998531579971313 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.172052472829819 0.318799406290054
0.186026200652122 0.311699867248535
0.195633232593536 0.298901319503784
0.202620059251785 0.278200328350067
0.214847102761269 0.252199858427048
0.226200819015503 0.220899924635887
0.23231440782547 0.189099803566933
0.249782010912895 0.159000083804131
0.25764200091362 0.134399771690369
0.268995523452759 0.115399979054928
0.280349284410477 0.0995999127626419
0.289956480264664 0.0879000872373581
0.299563586711884 0.0771000534296036
0.307423412799835 0.0689999908208847
0.316157102584839 0.0606000013649464
0.323144197463989 0.0522000044584274
0.333624482154846 0.042300071567297
0.339738070964813 0.036400031298399
0.346724718809128 0.0303000509738922
0.35633173584938 0.0233000069856644
0.36681205034256 0.0191999953240156
0.373799204826355 0.0153999980539083
0.385152667760849 0.0128999892622232
0.38951963186264 0.0107000125572085
0.397379904985428 0.0094999810680747
0.411353886127472 0.00790000427514315
0.421834141016006 0.00699999695643783
0.435807824134827 0.00650000292807817
0.43930122256279 0.00559999886900187
0.446288108825684 0.00530000310391188
0.454148530960083 0.00449999421834946
0.461135417222977 0.0042000045068562
0.471615612506866 0.00360000086948276
0.480349332094193 0.00329999951645732
0.489956319332123 0.00300000072456896
0.498690068721771 0.00219999602995813
0.508296847343445 0.00200000288896263
0.521397352218628 0.00149999873246998
0.528384745121002 0.00120000110473484
0.535371005535126 0.000900001148693264
0.54323136806488 0.000800001143943518
0.551964998245239 0.000800001143943518
0.553711533546448 0.000800001143943518
0.558078408241272 0.000599998980760574
0.567685604095459 0.000399999669753015
0.575546324253082 0.000299999490380287
0.580786168575287 0.000199999834876508
0.595633387565613 0.000199999834876508
0.602619767189026 9.9999931990169e-05
0.612227082252502 0
0.620960831642151 0
0.627947330474854 0
0.634060740470886 0
0.639301419258118 0
0.651528418064117 0
0.66113555431366 0
0.668122172355652 0
0.675982177257538 0
0.683843016624451 0
0.688209652900696 0
0.697816431522369 0
0.704803049564362 0
0.710043609142303 0
0.717904150485992 0
0.726637780666351 0
0.73624461889267 0
0.745851576328278 0
0.753711819648743 0
0.760698795318604 0
0.770305097103119 0
0.780785799026489 0
0.787772953510284 0
0.793013155460358 0
0.804366707801819 0
0.81135368347168 0
0.821834206581116 0
0.828820705413818 0
0.837554693222046 0
0.842794597148895 0
0.848908483982086 0
0.855022072792053 0
0.862882077693939 0
0.869868874549866 0
0.876855790615082 0
0.885589599609375 0
0.889956653118134 0
0.900436699390411 0
0.906550407409668 0
0.91353702545166 0
0.917030572891235 0
0.927511036396027 0
0.93275111913681 0
0.938864648342133 0
0.949344992637634 0
0.959825336933136 0
0.967685580253601 0
0.97641921043396 0
0.984279453754425 0
0.989519655704498 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0143136819824576 0.318799406290054
0.0269146077334881 0.311699867248535
0.0387814119458199 0.298901319503784
0.048935629427433 0.278200328350067
0.05957917496562 0.252199858427048
0.0704671889543533 0.220899924635887
0.0802544802427292 0.189099803566933
0.0893076360225677 0.159000083804131
0.0982384011149406 0.134399771690369
0.109982900321484 0.115399979054928
0.119525335729122 0.0995999127626419
0.131392255425453 0.0879000872373581
0.143748328089714 0.0771000534296036
0.153290867805481 0.0689999908208847
0.163689866662025 0.0606000013649464
0.1729876101017 0.0522000044584274
0.183753341436386 0.042300071567297
0.195620283484459 0.036400031298399
0.204550936818123 0.0303000509738922
0.215194717049599 0.0233000069856644
0.227061405777931 0.0191999953240156
0.238194271922112 0.0153999980539083
0.247492045164108 0.0128999892622232
0.257768481969833 0.0107000125572085
0.266699403524399 0.0094999810680747
0.277464658021927 0.00790000427514315
0.28725203871727 0.00699999695643783
0.297528386116028 0.00650000292807817
0.309151113033295 0.00559999886900187
0.320528745651245 0.00530000310391188
0.331783175468445 0.00449999421834946
0.34193754196167 0.0042000045068562
0.351847380399704 0.00360000086948276
0.363347321748734 0.00329999951645732
0.373501598834991 0.00300000072456896
0.38304403424263 0.00219999602995813
0.390996098518372 0.00200000288896263
0.401272356510162 0.00149999873246998
0.410814851522446 0.00120000110473484
0.423171103000641 0.000900001148693264
0.434426248073578 0.000800001143943518
0.443968862295151 0.000800001143943518
0.453021705150604 0.000800001143943518
0.461830258369446 0.000599998980760574
0.472596019506454 0.000399999669753015
0.483117312192917 0.000299999490380287
0.494250237941742 0.000199999834876508
0.503670454025269 0.000199999834876508
0.514557898044586 9.9999931990169e-05
0.525079309940338 0
0.536334812641144 0
0.547469139099121 0
0.557255923748016 0
0.567407548427582 0
0.575850367546082 0
0.586983621120453 0
0.596893310546875 0
0.607535362243652 0
0.619402647018433 0
0.63041216135025 0
0.640812814235687 0
0.652678191661835 0
0.662221193313599 0
0.671886801719666 0
0.681795597076416 0
0.692194521427155 0
0.701246976852417 0
0.712380826473236 0
0.722901582717896 0
0.733913064002991 0
0.742843806743622 0
0.752630531787872 0
0.762906551361084 0
0.774528861045837 0
0.783582210540771 0
0.794225573539734 0
0.804868876934052 0
0.815390050411224 0
0.825421333312988 0
0.834475100040436 0
0.843528032302856 0
0.854049563407898 0
0.863836526870728 0
0.872155606746674 0
0.87937343120575 0
0.888671517372131 0
0.89735746383667 0
0.906655192375183 0
0.915585994720459 0
0.925373136997223 0
0.933447420597076 0
0.941154897212982 0
0.948250412940979 0
0.955713093280792 0
0.962197184562683 0
0.971984326839447 0
0.977856576442719 0
0.985319316387177 0
0.993148982524872 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/List_/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    % ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.136500135064125 0.248399779200554
0.183100089430809 0.153999775648117
0.231699898838997 0.0904000028967857
0.282799899578094 0.0529999621212482
0.329700767993927 0.0297999940812588
0.379300177097321 0.0158000085502863
0.429699718952179 0.0084999967366457
0.475100010633469 0.00419999705627561
0.522398233413696 0.00189999642316252
0.567799687385559 0.000999999814666808
0.614399433135986 0.000199999529286288
0.662600100040436 0.000199999529286288
0.708300352096558 0
0.754899978637695 0
0.799099147319794 0
0.84470009803772 0
0.886199831962585 0
0.92389988899231 0
0.962800025939941 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.977309584617615 0.248399779200554
0.977309584617615 0.153999775648117
0.980551064014435 0.0904000028967857
0.982171773910522 0.0529999621212482
0.982171773910522 0.0297999940812588
0.983792543411255 0.0158000085502863
0.983792543411255 0.0084999967366457
0.987034022808075 0.00419999705627561
0.987034022808075 0.00189999642316252
0.988654792308807 0.000999999814666808
0.988654792308807 0.000199999529286288
0.99351704120636 0.000199999529286288
0.99351704120636 0
0.99351704120636 0
0.995137751102448 0
0.995137751102448 0
0.99675852060318 0
0.99675852060318 0
0.998379230499268 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.374358981847763 0.248399779200554
0.420512795448303 0.153999775648117
0.451282143592834 0.0904000028967857
0.50940203666687 0.0529999621212482
0.552136600017548 0.0297999940812588
0.591453015804291 0.0158000085502863
0.623931705951691 0.0084999967366457
0.658119738101959 0.00419999705627561
0.685470104217529 0.00189999642316252
0.707692444324493 0.000999999814666808
0.73333352804184 0.000199999529286288
0.76581209897995 0.000199999529286288
0.801709771156311 0
0.827350795269012 0
0.858119428157806 0
0.8854700922966 0
0.912820398807526 0
0.941880106925964 0
0.962393164634705 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0617185719311237 0.248399779200554
0.111616350710392 0.153999775648117
0.164583191275597 0.0904000028967857
0.21868622303009 0.0529999621212482
0.26915168762207 0.0297999940812588
0.322800993919373 0.0158000085502863
0.377926677465439 0.0084999967366457
0.427028775215149 0.00419999705627561
0.478972494602203 0.00189999642316252
0.528984248638153 0.000999999814666808
0.580245435237885 0.000199999529286288
0.632531404495239 0.000199999529286288
0.682087242603302 0
0.733348071575165 0
0.781427979469299 0
0.831438601016998 0
0.876676321029663 0
0.917595446109772 0
0.960331916809082 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/List_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0816998407244682 0.321199744939804
0.0958998873829842 0.321199744939804
0.109000071883202 0.321099817752838
0.120100013911724 0.31949970126152
0.131000101566315 0.315499782562256
0.14069989323616 0.305398911237717
0.151300221681595 0.288000613451004
0.161799818277359 0.256599634885788
0.170600116252899 0.217599958181381
0.179599940776825 0.172900199890137
0.188499942421913 0.127200335264206
0.198800042271614 0.087799958884716
0.210499852895737 0.0538000054657459
0.221299901604652 0.0328999385237694
0.230799928307533 0.0200999565422535
0.241300001740456 0.0103000104427338
0.251199394464493 0.00499999802559614
0.261400371789932 0.00249998946674168
0.269899636507034 0.00150000036228448
0.27960017323494 0.000399999058572575
0.290899693965912 9.99997646431439e-05
0.301100611686707 0
0.310099750757217 0
0.318899631500244 0
0.328000575304031 0
0.337100118398666 0
0.345899939537048 0
0.35449954867363 0
0.364500403404236 0
0.376199960708618 0
0.386399745941162 0
0.395300835371017 0
0.40500009059906 0
0.413999706506729 0
0.422500193119049 0
0.431699961423874 0
0.439499795436859 0
0.449799954891205 0
0.459000200033188 0
0.469999998807907 0
0.480700045824051 0
0.489600002765656 0
0.497100353240967 0
0.504200220108032 0
0.514601111412048 0
0.523199081420898 0
0.53209912776947 0
0.542000591754913 0
0.552000284194946 0
0.562299251556396 0
0.57259875535965 0
0.582599699497223 0
0.59080183506012 0
0.600301444530487 0
0.608599185943604 0
0.618999719619751 0
0.627898991107941 0
0.637901365756989 0
0.647701621055603 0
0.657299339771271 0
0.666100084781647 0
0.676101624965668 0
0.684700191020966 0
0.694498836994171 0
0.705499112606049 0
0.71519923210144 0
0.724699139595032 0
0.735900223255157 0
0.744801044464111 0
0.755099296569824 0
0.763799726963043 0
0.771099925041199 0
0.779599666595459 0
0.790599703788757 0
0.798499047756195 0
0.808899819850922 0
0.817800581455231 0
0.827499806880951 0
0.836899816989899 0
0.844700992107391 0
0.853600800037384 0
0.863200008869171 0
0.872000396251678 0
0.880399823188782 0
0.887899994850159 0
0.895000219345093 0
0.902599811553955 0
0.910899877548218 0
0.91899961233139 0
0.927699983119965 0
0.935500264167786 0
0.942399978637695 0
0.948400020599365 0
0.95660001039505 0
0.963800013065338 0
0.973100006580353 0
0.978999972343445 0
0.986199975013733 0
0.992900013923645 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.877551019191742 0.321199744939804
0.880466461181641 0.321199744939804
0.884839653968811 0.321099817752838
0.889212667942047 0.31949970126152
0.89212828874588 0.315499782562256
0.893585979938507 0.305398911237717
0.895043730735779 0.288000613451004
0.896501660346985 0.256599634885788
0.897959172725677 0.217599958181381
0.897959172725677 0.172900199890137
0.900874614715576 0.127200335264206
0.902332365512848 0.087799958884716
0.902332365512848 0.0538000054657459
0.905247747898102 0.0328999385237694
0.908163249492645 0.0200999565422535
0.909620881080627 0.0103000104427338
0.912536442279816 0.00499999802559614
0.913994193077087 0.00249998946674168
0.913994193077087 0.00150000036228448
0.915451884269714 0.000399999058572575
0.918367326259613 9.99997646431439e-05
0.919825077056885 0
0.921282827854156 0
0.921282827854156 0
0.921282827854156 0
0.922740519046783 0
0.924198150634766 0
0.925656080245972 0
0.925656080245972 0
0.927113711833954 0
0.928571403026581 0
0.930029153823853 0
0.930029153823853 0
0.930029153823853 0
0.930029153823853 0
0.930029153823853 0
0.930029153823853 0
0.932944595813751 0
0.934402346611023 0
0.935859978199005 0
0.938775420188904 0
0.938775420188904 0
0.938775420188904 0
0.938775420188904 0
0.938775420188904 0
0.94023323059082 0
0.941690981388092 0
0.941690981388092 0
0.941690981388092 0
0.941690981388092 0
0.941690981388092 0
0.946064114570618 0
0.946064114570618 0
0.948979616165161 0
0.948979616165161 0
0.950437307357788 0
0.950437307357788 0
0.95189505815506 0
0.95189505815506 0
0.95189505815506 0
0.95189505815506 0
0.95189505815506 0
0.95189505815506 0
0.953352749347687 0
0.954810500144958 0
0.954810500144958 0
0.954810500144958 0
0.960641384124756 0
0.963556826114655 0
0.965014576911926 0
0.965014576911926 0
0.967930018901825 0
0.967930018901825 0
0.969387769699097 0
0.972303211688995 0
0.976676404476166 0
0.976676404476166 0
0.978134095668793 0
0.979591846466064 0
0.979591846466064 0
0.981049537658691 0
0.983965039253235 0
0.985422730445862 0
0.986880481243134 0
0.989795923233032 0
0.989795923233032 0
0.989795923233032 0
0.989795923233032 0
0.989795923233032 0
0.989795923233032 0
0.989795923233032 0
0.989795923233032 0
0.992711365222931 0
0.994169116020203 0
0.994169116020203 0
0.994169116020203 0
0.994169116020203 0
0.99562680721283 0
0.998542249202728 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.094323143362999 0.321199744939804
0.130130991339684 0.321199744939804
0.155458465218544 0.321099817752838
0.174672573804855 0.31949970126152
0.193886384367943 0.315499782562256
0.200873404741287 0.305398911237717
0.212227091193199 0.288000613451004
0.23231440782547 0.256599634885788
0.242794781923294 0.217599958181381
0.255021661520004 0.172900199890137
0.262882083654404 0.127200335264206
0.272489190101624 0.087799958884716
0.283842861652374 0.0538000054657459
0.293449580669403 0.0328999385237694
0.301309913396835 0.0200999565422535
0.309170424938202 0.0103000104427338
0.321397393941879 0.00499999802559614
0.328384280204773 0.00249998946674168
0.33449786901474 0.00150000036228448
0.344977974891663 0.000399999058572575
0.355458617210388 9.99997646431439e-05
0.361572057008743 0
0.373799085617065 0
0.380786031484604 0
0.390392959117889 0
0.403493613004684 0
0.412227004766464 0
0.420960605144501 0
0.426200896501541 0
0.434061169624329 0
0.441921353340149 0
0.448908239603043 0
0.460262060165405 0
0.468995630741119 0
0.480349332094193 0
0.48820960521698 0
0.497816473245621 0
0.510043323040009 0
0.518777251243591 0
0.525763630867004 0
0.532751500606537 0
0.542357981204987 0
0.544104874134064 0
0.548471868038177 0
0.558078527450562 0
0.565938889980316 0
0.572925567626953 0
0.58951997756958 0
0.59825325012207 0
0.607860326766968 0
0.616593539714813 0
0.622707426548004 0
0.62882125377655 0
0.635807812213898 0
0.647161602973938 0
0.656768798828125 0
0.663755714893341 0
0.670742273330688 0
0.677729070186615 0
0.682969510555267 0
0.692576467990875 0
0.698689877986908 0
0.704803645610809 0
0.711790144443512 0
0.720524370670319 0
0.730131089687347 0
0.739737927913666 0
0.748471736907959 0
0.75545871257782 0
0.765939295291901 0
0.773799359798431 0
0.779912352561951 0
0.78427928686142 0
0.797379672527313 0
0.804366707801819 0
0.8148472905159 0
0.820960402488708 0
0.829694092273712 0
0.83493447303772 0
0.841047883033752 0
0.847161591053009 0
0.857641875743866 0
0.864628553390503 0
0.871615588665009 0
0.880349159240723 0
0.884716212749481 0
0.896943032741547 0
0.903930127620697 0
0.91004353761673 0
0.917903959751129 0
0.930131018161774 0
0.936244547367096 0
0.942358076572418 0
0.953711807727814 0
0.964192152023315 0
0.972052395343781 0
0.978165924549103 0
0.986026227474213 0
0.991266369819641 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0130982985720038 0.321199744939804
0.0252172742038965 0.321199744939804
0.0373362563550472 0.321099817752838
0.0478638857603073 0.31949970126152
0.058269064873457 0.315499782562256
0.0690414980053902 0.305398911237717
0.0803035721182823 0.288000613451004
0.0902190580964088 0.256599634885788
0.0994001254439354 0.217599958181381
0.108703657984734 0.172900199890137
0.118251986801624 0.127200335264206
0.129391506314278 0.087799958884716
0.142122358083725 0.0538000054657459
0.153751954436302 0.0328999385237694
0.164034828543663 0.0200999565422535
0.175664097070694 0.0103000104427338
0.185824289917946 0.00499999802559614
0.197208926081657 0.00249998946674168
0.206757336854935 0.00150000036228448
0.217040076851845 0.000399999058572575
0.229158982634544 9.99997646431439e-05
0.240665927529335 0
0.24984672665596 0
0.259639352560043 0
0.269432932138443 0
0.27861487865448 0
0.288040339946747 0
0.297220677137375 0
0.308728188276291 0
0.321826368570328 0
0.333088338375092 0
0.342881470918655 0
0.353164404630661 0
0.362957537174225 0
0.371771425008774 0
0.381931871175766 0
0.390133321285248 0
0.400783210992813 0
0.410699158906937 0
0.423062801361084 0
0.434936910867691 0
0.444485247135162 0
0.453421473503113 0
0.46150067448616 0
0.472885310649872 0
0.482188880443573 0
0.491982072591782 0
0.501775503158569 0
0.512793123722076 0
0.52405446767807 0
0.535439431667328 0
0.546455383300781 0
0.555637896060944 0
0.56604140996933 0
0.574611842632294 0
0.585874140262604 0
0.595788478851318 0
0.606929183006287 0
0.617945432662964 0
0.628962159156799 0
0.63838928937912 0
0.649772703647614 0
0.659444570541382 0
0.670339465141296 0
0.682458460330963 0
0.692986190319061 0
0.703268647193909 0
0.715265333652496 0
0.72493577003479 0
0.735953211784363 0
0.745501518249512 0
0.753336846828461 0
0.763129651546478 0
0.774635195732117 0
0.783082544803619 0
0.793976962566376 0
0.804014682769775 0
0.814542412757874 0
0.825192928314209 0
0.833884656429291 0
0.843799591064453 0
0.853837907314301 0
0.863508403301239 0
0.872689425945282 0
0.880401611328125 0
0.888480663299561 0
0.896070659160614 0
0.905251443386078 0
0.914310216903687 0
0.923858463764191 0
0.931692957878113 0
0.939282536506653 0
0.945525646209717 0
0.953849911689758 0
0.961194753646851 0
0.971477508544922 0
0.977843046188354 0
0.985432744026184 0
0.992655158042908 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/List_target/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    % ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.12739984691143 0.285100281238556
0.176699906587601 0.206299901008606
0.226999953389168 0.113400012254715
0.276201039552689 0.0452000051736832
0.323599457740784 0.0125999916344881
0.374300062656403 0.00409999769181013
0.426000088453293 0.00079999933950603
0.473000198602676 0.000199999529286288
0.522098779678345 0
0.568598687648773 0
0.612900853157043 0
0.664599418640137 0
0.709300220012665 0
0.7548987865448 0
0.799099326133728 0
0.846300005912781 0
0.888000965118408 0
0.925800383090973 0
0.963899791240692 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.972580671310425 0.285100281238556
0.972580671310425 0.206299901008606
0.975806474685669 0.113400012254715
0.980645179748535 0.0452000051736832
0.980645179748535 0.0125999916344881
0.982258081436157 0.00409999769181013
0.982258081436157 0.00079999933950603
0.985483884811401 0.000199999529286288
0.985483884811401 0
0.987096786499023 0
0.987096786499023 0
0.99193549156189 0
0.99193549156189 0
0.99193549156189 0
0.993548393249512 0
0.993548393249512 0
0.995161294937134 0
0.996774196624756 0
0.998387098312378 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.298275947570801 0.285100281238556
0.394827634096146 0.206299901008606
0.448275864124298 0.113400012254715
0.501723945140839 0.0452000051736832
0.544827699661255 0.0125999916344881
0.582758486270905 0.00409999769181013
0.620689630508423 0.00079999933950603
0.66034471988678 0.000199999529286288
0.691379189491272 0
0.71034449338913 0
0.734482884407043 0
0.77068966627121 0
0.805172443389893 0
0.831034421920776 0
0.860345005989075 0
0.887931168079376 0
0.913792908191681 0
0.943103432655334 0
0.962068974971771 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0565909333527088 0.285100281238556
0.106249995529652 0.206299901008606
0.159658908843994 0.113400012254715
0.211704447865486 0.0452000051736832
0.262727111577988 0.0125999916344881
0.317727416753769 0.00409999769181013
0.373977214097977 0.00079999933950603
0.424545466899872 0.000199999529286288
0.478295356035233 0
0.529773890972137 0
0.578522086143494 0
0.634546875953674 0
0.683068990707397 0
0.733181715011597 0
0.781363606452942 0
0.833181440830231 0
0.878750622272491 0
0.919658899307251 0
0.961590886116028 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/Markov/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0934999063611031 0.316700428724289
0.104799941182137 0.300899922847748
0.115800023078918 0.260099709033966
0.126600041985512 0.206299811601639
0.136199861764908 0.1369998306036
0.145999908447266 0.078699991106987
0.154800429940224 0.0397999733686447
0.164299920201302 0.0182999689131975
0.173699840903282 0.00680000009015203
0.183599650859833 0.00229999842122197
0.192099750041962 0.000800001027528197
0.202799871563911 9.99999174382538e-05
0.213100045919418 9.99999174382538e-05
0.223700150847435 0
0.23199999332428 0
0.240299955010414 0
0.250500500202179 0
0.259800136089325 0
0.268000543117523 0
0.27759912610054 0
0.288099467754364 0
0.296299964189529 0
0.306000232696533 0
0.314999639987946 0
0.326000094413757 0
0.335200607776642 0
0.345499694347382 0
0.354099571704865 0
0.36550036072731 0
0.377199709415436 0
0.387299805879593 0
0.395799875259399 0
0.405599683523178 0
0.414899408817291 0
0.425299912691116 0
0.434500157833099 0
0.44410029053688 0
0.453399956226349 0
0.461699992418289 0
0.472299814224243 0
0.481400012969971 0
0.489700049161911 0
0.49760028719902 0
0.504800856113434 0
0.513799786567688 0
0.523700773715973 0
0.532199144363403 0
0.541801512241364 0
0.550900399684906 0
0.561300039291382 0
0.571503043174744 0
0.580500602722168 0
0.589298605918884 0
0.598400771617889 0
0.606500327587128 0
0.615601241588593 0
0.625101804733276 0
0.634998619556427 0
0.644400417804718 0
0.654100477695465 0
0.662800073623657 0
0.672699928283691 0
0.681197822093964 0
0.690698444843292 0
0.7011998295784 0
0.711199462413788 0
0.721000611782074 0
0.731099784374237 0
0.740100562572479 0
0.749900221824646 0
0.758800029754639 0
0.767498373985291 0
0.776099681854248 0
0.78700065612793 0
0.794600307941437 0
0.803800165653229 0
0.813799440860748 0
0.823899924755096 0
0.833899438381195 0
0.841601192951202 0
0.850700557231903 0
0.861100018024445 0
0.870599806308746 0
0.878799438476562 0
0.886599600315094 0
0.893700182437897 0
0.901500225067139 0
0.909300208091736 0
0.916299402713776 0
0.925400197505951 0
0.932900607585907 0
0.940299510955811 0
0.947100222110748 0
0.954499781131744 0
0.961399793624878 0
0.969900012016296 0
0.976600110530853 0
0.984399974346161 0
0.99210000038147 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.88563060760498 0.316700428724289
0.88563060760498 0.300899922847748
0.890029430389404 0.260099709033966
0.891495704650879 0.206299811601639
0.891495704650879 0.1369998306036
0.892961800098419 0.078699991106987
0.894428074359894 0.0397999733686447
0.895894587039948 0.0182999689131975
0.897360682487488 0.00680000009015203
0.897360682487488 0.00229999842122197
0.900293231010437 0.000800001027528197
0.901759505271912 9.99999174382538e-05
0.901759505271912 9.99999174382538e-05
0.904692053794861 0
0.907624661922455 0
0.909091114997864 0
0.912023484706879 0
0.912023484706879 0
0.912023484706879 0
0.913489758968353 0
0.916422307491302 0
0.917888581752777 0
0.919354856014252 0
0.919354856014252 0
0.919354856014252 0
0.920821130275726 0
0.922287404537201 0
0.923753559589386 0
0.923753559589386 0
0.925220012664795 0
0.926686227321625 0
0.928152501583099 0
0.928152501583099 0
0.928152501583099 0
0.928152501583099 0
0.928152501583099 0
0.928152501583099 0
0.931085050106049 0
0.932551324367523 0
0.934017598628998 0
0.936950147151947 0
0.936950147151947 0
0.936950147151947 0
0.936950147151947 0
0.936950147151947 0
0.938416421413422 0
0.939882636070251 0
0.939882636070251 0
0.939882636070251 0
0.939882636070251 0
0.939882636070251 0
0.94428151845932 0
0.94428151845932 0
0.947214066982269 0
0.948680341243744 0
0.950146615505219 0
0.950146615505219 0
0.951612889766693 0
0.951612889766693 0
0.951612889766693 0
0.951612889766693 0
0.951612889766693 0
0.951612889766693 0
0.953079164028168 0
0.954545438289642 0
0.954545438289642 0
0.954545438289642 0
0.960410535335541 0
0.96334308385849 0
0.964809358119965 0
0.964809358119965 0
0.967741906642914 0
0.967741906642914 0
0.969208240509033 0
0.972140789031982 0
0.976539611816406 0
0.976539611816406 0
0.978005886077881 0
0.979472160339355 0
0.979472160339355 0
0.98093843460083 0
0.983870983123779 0
0.985337257385254 0
0.986803531646729 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.992668628692627 0
0.994134902954102 0
0.994134902954102 0
0.994134902954102 0
0.994134902954102 0
0.995601177215576 0
0.998533725738525 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.173076868057251 0.316700428724289
0.187937080860138 0.300899922847748
0.197552427649498 0.260099709033966
0.205419600009918 0.206299811601639
0.216783240437508 0.1369998306036
0.224650397896767 0.078699991106987
0.230769231915474 0.0397999733686447
0.24475522339344 0.0182999689131975
0.251748353242874 0.00680000009015203
0.262237817049026 0.00229999842122197
0.273601204156876 0.000800001027528197
0.282342672348022 9.99999174382538e-05
0.291958123445511 9.99999174382538e-05
0.302447527647018 0
0.309440553188324 0
0.318181842565536 0
0.329545557498932 0
0.337412536144257 0
0.344405561685562 0
0.353146821260452 0
0.363636493682861 0
0.37062931060791 0
0.383741319179535 0
0.388111919164658 0
0.398601472377777 0
0.409965038299561 0
0.419580519199371 0
0.428321570158005 0
0.431818217039108 0
0.44230780005455 0
0.449300706386566 0
0.457167834043503 0
0.469405591487885 0
0.477272719144821 0
0.48688817024231 0
0.494755446910858 0
0.506119251251221 0
0.518356680870056 0
0.525349199771881 0
0.531468570232391 0
0.542832434177399 0
0.550699353218079 0
0.553321599960327 0
0.558566212654114 0
0.569055914878845 0
0.577797532081604 0
0.583041727542877 0
0.59877610206604 0
0.604895353317261 0
0.61450982093811 0
0.623251736164093 0
0.629370212554932 0
0.634615361690521 0
0.639860212802887 0
0.65034955739975 0
0.659964740276337 0
0.666958153247833 0
0.673950791358948 0
0.68181836605072 0
0.686189115047455 0
0.697552263736725 0
0.703671455383301 0
0.708915948867798 0
0.71590918302536 0
0.726398885250092 0
0.73688805103302 0
0.746503472328186 0
0.753496527671814 0
0.760489583015442 0
0.770104944705963 0
0.778846561908722 0
0.78496527671814 0
0.78933572769165 0
0.800699353218079 0
0.808566153049469 0
0.81818163394928 0
0.825174927711487 0
0.834790170192719 0
0.841782987117767 0
0.847901940345764 0
0.854020953178406 0
0.862762689590454 0
0.870629131793976 0
0.877622246742249 0
0.886363744735718 0
0.890734136104584 0
0.902097880840302 0
0.908216774463654 0
0.914335668087006 0
0.91783219575882 0
0.929195821285248 0
0.934440553188324 0
0.940559446811676 0
0.951048970222473 0
0.962412595748901 0
0.970279693603516 0
0.976398587226868 0
0.985139846801758 0
0.99125874042511 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0162710957229137 0.316700428724289
0.0280156638473272 0.300899922847748
0.0397602096199989 0.260099709033966
0.0517494082450867 0.206299811601639
0.0619036108255386 0.1369998306036
0.0726694241166115 0.078699991106987
0.0824566259980202 0.0397999733686447
0.0919989719986916 0.0182999689131975
0.102397851645947 0.00680000009015203
0.11304134875536 0.00229999842122197
0.121605202555656 0.000800001027528197
0.133349373936653 9.99999174382538e-05
0.144604906439781 9.99999174382538e-05
0.155859887599945 0
0.164790630340576 0
0.173599362373352 0
0.184242576360703 0
0.194519087672234 0
0.203572258353233 0
0.213971182703972 0
0.22510401904583 0
0.2340347468853 0
0.243944391608238 0
0.254343420267105 0
0.266331970691681 0
0.275873869657516 0
0.287007689476013 0
0.296183317899704 0
0.309640169143677 0
0.322363138198853 0
0.333619028329849 0
0.342794716358185 0
0.353071004152298 0
0.363347351551056 0
0.374725222587585 0
0.384879022836685 0
0.395033031702042 0
0.404453098773956 0
0.413506299257278 0
0.425495594739914 0
0.434793084859848 0
0.443846344947815 0
0.453144162893295 0
0.461218565702438 0
0.470760941505432 0
0.481526792049408 0
0.491069376468658 0
0.500611841678619 0
0.510888040065765 0
0.522265374660492 0
0.533520817756653 0
0.543306112289429 0
0.553339779376984 0
0.563494145870209 0
0.571812212467194 0
0.581476449966431 0
0.592121720314026 0
0.603133261203766 0
0.613530099391937 0
0.624786078929901 0
0.633839011192322 0
0.645093560218811 0
0.654760301113129 0
0.665280282497406 0
0.67653477191925 0
0.687300682067871 0
0.697945296764374 0
0.70883309841156 0
0.718620300292969 0
0.729140520095825 0
0.738806188106537 0
0.748348712921143 0
0.758258044719696 0
0.769880056381226 0
0.777831733226776 0
0.78737461566925 0
0.798629283905029 0
0.809518098831177 0
0.820651054382324 0
0.829214155673981 0
0.839368462562561 0
0.850624144077301 0
0.861023008823395 0
0.869953274726868 0
0.878027677536011 0
0.886102139949799 0
0.894054293632507 0
0.90274041891098 0
0.910447895526886 0
0.921091258525848 0
0.928676187992096 0
0.936995327472687 0
0.944213330745697 0
0.951676070690155 0
0.958527028560638 0
0.967824697494507 0
0.975165128707886 0
0.983361899852753 0
0.991680920124054 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/Markov/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.137199923396111 0.189899504184723
0.183099836111069 0.0651998221874237
0.231000006198883 0.016199991106987
0.278601318597794 0.00229999562725425
0.324700146913528 0.000199999529286288
0.376400291919708 9.99997646431439e-05
0.428299963474274 0
0.474399894475937 0
0.524300873279572 0
0.571001052856445 0
0.61760014295578 0
0.666498899459839 0
0.711899816989899 0
0.755500376224518 0
0.799600541591644 0
0.844298839569092 0
0.886800408363342 0
0.925300002098083 0
0.963699877262115 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.975728154182434 0.189899504184723
0.975728154182434 0.0651998221874237
0.978964388370514 0.016199991106987
0.982200622558594 0.00229999562725425
0.982200622558594 0.000199999529286288
0.983818769454956 9.99997646431439e-05
0.983818769454956 0
0.987055003643036 0
0.987055003643036 0
0.988673150539398 0
0.988673150539398 0
0.99352753162384 0
0.99352753162384 0
0.99352753162384 0
0.995145618915558 0
0.995145618915558 0
0.99676376581192 0
0.99676376581192 0
0.998381853103638 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.383305013179779 0.189899504184723
0.427597999572754 0.0651998221874237
0.461669564247131 0.016199991106987
0.512776672840118 0.00229999562725425
0.555366575717926 0.000199999529286288
0.594548404216766 9.99997646431439e-05
0.623509049415588 0
0.659284293651581 0
0.684838473796844 0
0.708688318729401 0
0.734241724014282 0
0.766610026359558 0
0.800681233406067 0
0.826235055923462 0
0.856899380683899 0
0.885860323905945 0
0.911413967609406 0
0.940374791622162 0
0.960817694664001 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0618532560765743 0.189899504184723
0.111085906624794 0.0651998221874237
0.16304711997509 0.016199991106987
0.213530376553535 0.00229999562725425
0.263104677200317 0.000199999529286288
0.319158226251602 9.99997646431439e-05
0.376236796379089 0
0.426037818193436 0
0.481068968772888 0
0.532461941242218 0
0.583740890026093 0
0.636839330196381 0
0.686184227466583 0
0.734053254127502 0
0.782035112380981 0
0.830926597118378 0
0.877430200576782 0
0.919272243976593 0
0.961455345153809 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/Markov_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0927999690175056 0.296800315380096
0.105500027537346 0.280500173568726
0.116500027477741 0.259499877691269
0.126399636268616 0.229600101709366
0.135800033807755 0.191500157117844
0.146100014448166 0.153299957513809
0.155599638819695 0.120200097560883
0.165800124406815 0.0919998437166214
0.174900054931641 0.0740998983383179
0.184200152754784 0.0596999824047089
0.194799646735191 0.0489000231027603
0.206000044941902 0.0402000211179256
0.215399995446205 0.0320999957621098
0.225899904966354 0.0237999856472015
0.234799951314926 0.0170999858528376
0.243500292301178 0.0111000193282962
0.252799540758133 0.0084999967366457
0.262700021266937 0.00600000144913793
0.271399527788162 0.00449999328702688
0.279999792575836 0.0036000027321279
0.290799826383591 0.00290000275708735
0.299599707126617 0.00249999645166099
0.309099912643433 0.0015000025741756
0.318300306797028 0.00130000256467611
0.327199548482895 0.00119999900925905
0.337400376796722 0.000999999814666808
0.347600221633911 0.000700000789947808
0.357499629259109 0.000499999907333404
0.367300242185593 0.000399999058572575
0.377799808979034 0.000199999529286288
0.387599945068359 0.000199999529286288
0.396299749612808 0.000199999529286288
0.405699878931046 0.000199999529286288
0.415100246667862 9.99997646431439e-05
0.424599409103394 9.99997646431439e-05
0.43429970741272 0
0.442400097846985 0
0.452500402927399 0
0.461299896240234 0
0.471599906682968 0
0.481400012969971 0
0.490399986505508 0
0.497600644826889 0
0.505400419235229 0
0.514801025390625 0
0.524700224399567 0
0.534500420093536 0
0.544500827789307 0
0.553999602794647 0
0.563500940799713 0
0.57349967956543 0
0.582998335361481 0
0.591500818729401 0
0.601599872112274 0
0.610300362110138 0
0.620398998260498 0
0.630300223827362 0
0.639398038387299 0
0.649800300598145 0
0.65979939699173 0
0.669099748134613 0
0.679300546646118 0
0.688500165939331 0
0.697800517082214 0
0.707499623298645 0
0.717200219631195 0
0.726799488067627 0
0.736500144004822 0
0.745198369026184 0
0.755399405956268 0
0.76359885931015 0
0.77190089225769 0
0.781000852584839 0
0.791499197483063 0
0.79909884929657 0
0.809400022029877 0
0.818598508834839 0
0.829500019550323 0
0.839100897312164 0
0.847099781036377 0
0.855300009250641 0
0.864300191402435 0
0.873199582099915 0
0.881200015544891 0
0.8883997797966 0
0.896099925041199 0
0.905199825763702 0
0.912699997425079 0
0.919800102710724 0
0.927600026130676 0
0.935300290584564 0
0.942099690437317 0
0.948800265789032 0
0.955700218677521 0
0.96289998292923 0
0.971399784088135 0
0.976999998092651 0
0.985400021076202 0
0.992500007152557 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.88823527097702 0.296800315380096
0.88823527097702 0.280500173568726
0.891176581382751 0.259499877691269
0.892647266387939 0.229600101709366
0.892647266387939 0.191500157117844
0.894117712974548 0.153299957513809
0.895588338375092 0.120200097560883
0.897058844566345 0.0919998437166214
0.898529410362244 0.0740998983383179
0.898529410362244 0.0596999824047089
0.901470601558685 0.0489000231027603
0.902941167354584 0.0402000211179256
0.902941167354584 0.0320999957621098
0.905882358551025 0.0237999856472015
0.908823728561401 0.0170999858528376
0.910294115543365 0.0111000193282962
0.913235306739807 0.0084999967366457
0.913235306739807 0.00600000144913793
0.913235306739807 0.00449999328702688
0.914705872535706 0.0036000027321279
0.917647063732147 0.00290000275708735
0.919117629528046 0.00249999645166099
0.920588254928589 0.0015000025741756
0.920588254928589 0.00130000256467611
0.920588254928589 0.00119999900925905
0.922058820724487 0.000999999814666808
0.923529326915741 0.000700000789947808
0.925000071525574 0.000499999907333404
0.925000071525574 0.000399999058572575
0.926470577716827 0.000199999529286288
0.927941203117371 0.000199999529286288
0.929411768913269 0.000199999529286288
0.929411768913269 0.000199999529286288
0.929411768913269 9.99997646431439e-05
0.929411768913269 9.99997646431439e-05
0.929411768913269 0
0.929411768913269 0
0.932352960109711 0
0.933823525905609 0
0.935294091701508 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.939705789089203 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.945588231086731 0
0.945588231086731 0
0.948529422283173 0
0.948529422283173 0
0.949999988079071 0
0.949999988079071 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.952941179275513 0
0.954411745071411 0
0.954411745071411 0
0.954411745071411 0
0.960294127464294 0
0.963235318660736 0
0.964705884456635 0
0.964705884456635 0
0.967647075653076 0
0.967647075653076 0
0.969117641448975 0
0.972058832645416 0
0.976470589637756 0
0.976470589637756 0
0.977941155433655 0
0.979411780834198 0
0.979411780834198 0
0.980882346630096 0
0.983823537826538 0
0.985294103622437 0
0.98676472902298 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.992647051811218 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.99558824300766 0
0.998529434204102 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.170924991369247 0.296800315380096
0.188546314835548 0.280500173568726
0.19999997317791 0.259499877691269
0.206167414784431 0.229600101709366
0.218502223491669 0.191500157117844
0.226431712508202 0.153299957513809
0.232599139213562 0.120200097560883
0.249339282512665 0.0919998437166214
0.25814962387085 0.0740998983383179
0.270484745502472 0.0596999824047089
0.282819360494614 0.0489000231027603
0.29251104593277 0.0402000211179256
0.299559623003006 0.0320999957621098
0.30572709441185 0.0237999856472015
0.313656240701675 0.0170999858528376
0.321585774421692 0.0111000193282962
0.332158654928207 0.0084999967366457
0.340088278055191 0.00600000144913793
0.346255451440811 0.00449999328702688
0.355066031217575 0.0036000027321279
0.364757716655731 0.00290000275708735
0.370044082403183 0.00249999645166099
0.383259862661362 0.0015000025741756
0.387665212154388 0.00130000256467611
0.395594596862793 0.00119999900925905
0.407929509878159 0.000999999814666808
0.417621195316315 0.000700000789947808
0.425550639629364 0.000499999907333404
0.428193777799606 0.000399999058572575
0.436123311519623 0.000199999529286288
0.444052785634995 0.000199999529286288
0.452863335609436 0.000199999529286288
0.464317172765732 0.000199999529286288
0.474008798599243 9.99997646431439e-05
0.483700454235077 9.99997646431439e-05
0.491629958152771 0
0.501321732997894 0
0.515418648719788 0
0.524228990077972 0
0.530396521091461 0
0.540088713169098 0
0.548898637294769 0
0.551540911197662 0
0.555066466331482 0
0.565638720989227 0
0.575330436229706 0
0.58061683177948 0
0.595594644546509 0
0.601761519908905 0
0.609691977500916 0
0.619382858276367 0
0.627312898635864 0
0.63436084985733 0
0.639647543430328 0
0.652863442897797 0
0.663435637950897 0
0.670484364032745 0
0.676651835441589 0
0.685462594032288 0
0.688986718654633 0
0.698678731918335 0
0.705727159976959 0
0.710131883621216 0
0.718061685562134 0
0.726872265338898 0
0.736564159393311 0
0.746255218982697 0
0.753304183483124 0
0.760352611541748 0
0.769163131713867 0
0.776211619377136 0
0.78326004743576 0
0.787665367126465 0
0.799118399620056 0
0.806167185306549 0
0.816740095615387 0
0.823788523674011 0
0.8334801197052 0
0.840528547763824 0
0.846695899963379 0
0.851982295513153 0
0.859911739826202 0
0.866960108280182 0
0.8748899102211 0
0.883700311183929 0
0.888986825942993 0
0.900440394878387 0
0.907489001750946 0
0.913656413555145 0
0.917180597782135 0
0.927753329277039 0
0.932158589363098 0
0.939207077026367 0
0.949779748916626 0
0.961233496665955 0
0.969163000583649 0
0.975330412387848 0
0.985903084278107 0
0.991189420223236 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0158827118575573 0.296800315380096
0.0289554130285978 0.280500173568726
0.0405619814991951 0.259499877691269
0.0516798868775368 0.229600101709366
0.0614538975059986 0.191500157117844
0.0728160366415977 0.153299957513809
0.083445280790329 0.120200097560883
0.093463696539402 0.0919998437166214
0.103237628936768 0.0740998983383179
0.11288944631815 0.0596999824047089
0.12388501316309 0.0489000231027603
0.136102616786957 0.0402000211179256
0.146609544754028 0.0320999957621098
0.158338367938995 0.0237999856472015
0.167868509888649 0.0170999858528376
0.177275687456131 0.0111000193282962
0.1869275867939 0.0084999967366457
0.197922974824905 0.00600000144913793
0.207697004079819 0.00449999328702688
0.216860130429268 0.0036000027321279
0.228466704487801 0.00290000275708735
0.238362848758698 0.00249999645166099
0.248015269637108 0.0015000025741756
0.258644133806229 0.00130000256467611
0.268418252468109 0.00119999900925905
0.279046684503555 0.000999999814666808
0.290042579174042 0.000700000789947808
0.300916075706482 0.000499999907333404
0.312522768974304 0.000399999058572575
0.324129313230515 0.000199999529286288
0.334880650043488 0.000199999529286288
0.34416663646698 0.000199999529286288
0.354062139987946 0.000199999529286288
0.364202886819839 9.99997646431439e-05
0.374465316534042 9.99997646431439e-05
0.38521683216095 0
0.393768846988678 0
0.403909713029861 0
0.413316935300827 0
0.424923628568649 0
0.43530860543251 0
0.445082455873489 0
0.453512579202652 0
0.462553381919861 0
0.472571790218353 0
0.483200997114182 0
0.494318872690201 0
0.50445944070816 0
0.515211462974548 0
0.525718748569489 0
0.536591947078705 0
0.546730756759644 0
0.556140601634979 0
0.567500352859497 0
0.576298713684082 0
0.587048709392548 0
0.598169386386871 0
0.608306467533112 0
0.619791626930237 0
0.631520807743073 0
0.641539394855499 0
0.653023719787598 0
0.663652896881104 0
0.67379355430603 0
0.684300601482391 0
0.694807469844818 0
0.70519232749939 0
0.715577960014343 0
0.724984288215637 0
0.736102640628815 0
0.745142996311188 0
0.754062712192535 0
0.764569163322449 0
0.77568781375885 0
0.783751130104065 0
0.794502377510071 0
0.804764807224274 0
0.816615462303162 0
0.827244997024536 0
0.836163938045502 0
0.845327198505402 0
0.854978680610657 0
0.86475282907486 0
0.873304605484009 0
0.880635261535645 0
0.889309883117676 0
0.898839235305786 0
0.907024919986725 0
0.91484409570694 0
0.92388504743576 0
0.931826531887054 0
0.93952339887619 0
0.946487486362457 0
0.953329265117645 0
0.960537552833557 0
0.969822883605957 0
0.975809395313263 0
0.98448383808136 0
0.992180824279785 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/Markov_/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.135699883103371 0.212899953126907
0.18159981071949 0.119100034236908
0.233500048518181 0.0533000230789185
0.282199859619141 0.0231000054627657
0.327600330114365 0.00929997209459543
0.378800272941589 0.00320000224746764
0.430200159549713 0.000800000212620944
0.475799888372421 0.000199999834876508
0.527800321578979 9.9999931990169e-05
0.574099242687225 0
0.61860191822052 0
0.667100369930267 0
0.711399734020233 0
0.756199717521667 0
0.800400376319885 0
0.846400082111359 0
0.887100756168365 0
0.924700081348419 0
0.963500201702118 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.977309584617615 0.212899953126907
0.977309584617615 0.119100034236908
0.980551064014435 0.0533000230789185
0.982171773910522 0.0231000054627657
0.982171773910522 0.00929997209459543
0.983792543411255 0.00320000224746764
0.983792543411255 0.000800000212620944
0.987034022808075 0.000199999834876508
0.987034022808075 9.9999931990169e-05
0.988654792308807 0
0.988654792308807 0
0.99351704120636 0
0.99351704120636 0
0.99351704120636 0
0.995137751102448 0
0.995137751102448 0
0.99675852060318 0
0.99675852060318 0
0.998379230499268 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.385813027620316 0.212899953126907
0.432525873184204 0.119100034236908
0.463667720556259 0.0533000230789185
0.513840734958649 0.0231000054627657
0.557093441486359 0.00929997209459543
0.598616123199463 0.00320000224746764
0.633218109607697 0.000800000212620944
0.667820155620575 0.000199999834876508
0.693771660327911 9.9999931990169e-05
0.712802767753601 0
0.737024307250977 0
0.76989609003067 0
0.804498553276062 0
0.828719675540924 0
0.856401264667511 0
0.882353067398071 0
0.910034596920013 0
0.93944638967514 0
0.961937725543976 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0603066869080067 0.212899953126907
0.109369732439518 0.119100034236908
0.166042014956474 0.0533000230789185
0.217944458127022 0.0231000054627657
0.266666978597641 0.00929997209459543
0.321976184844971 0.00320000224746764
0.378080427646637 0.000800000212620944
0.427370637655258 0.000199999834876508
0.484724700450897 9.9999931990169e-05
0.535944879055023 0
0.584894418716431 0
0.637478411197662 0
0.685519456863403 0
0.734809935092926 0
0.783077895641327 0
0.833616971969604 0
0.877910137176514 0
0.91868257522583 0
0.961158454418182 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/Markov_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0811000913381577 0.321199744939804
0.0970999896526337 0.321099817752838
0.110299952328205 0.319999843835831
0.121899999678135 0.315299600362778
0.132300317287445 0.306199312210083
0.142699614167213 0.286799788475037
0.152900144457817 0.255000352859497
0.162799686193466 0.212599992752075
0.171800002455711 0.1697998046875
0.181699827313423 0.123899951577187
0.191400140523911 0.0834000632166862
0.202399745583534 0.0497000627219677
0.21340024471283 0.0290000084787607
0.223800122737885 0.0147000029683113
0.232800140976906 0.00639999471604824
0.242100045084953 0.00280000315979123
0.252700597047806 0.000999999814666808
0.262700229883194 0.000399999058572575
0.270699977874756 0.000199999529286288
0.27930012345314 0
0.290599554777145 0
0.299899637699127 0
0.30919998884201 0
0.318299502134323 0
0.327501028776169 0
0.337299466133118 0
0.347599506378174 0
0.357199609279633 0
0.366900265216827 0
0.377200245857239 0
0.387299507856369 0
0.394599229097366 0
0.403899639844894 0
0.414299309253693 0
0.422799646854401 0
0.432200193405151 0
0.440299659967422 0
0.449599802494049 0
0.458400189876556 0
0.469199806451797 0
0.479499995708466 0
0.488500088453293 0
0.496499985456467 0
0.504399299621582 0
0.513700425624847 0
0.523201882839203 0
0.532299876213074 0
0.542300999164581 0
0.551499783992767 0
0.560999631881714 0
0.570899724960327 0
0.580899894237518 0
0.588901221752167 0
0.598298490047455 0
0.606300711631775 0
0.616299867630005 0
0.626298785209656 0
0.636400282382965 0
0.645999491214752 0
0.65609884262085 0
0.665900468826294 0
0.675899386405945 0
0.6847003698349 0
0.694599330425262 0
0.704698801040649 0
0.713100254535675 0
0.722900688648224 0
0.732500612735748 0
0.741000533103943 0
0.751200497150421 0
0.760200560092926 0
0.768699824810028 0
0.77790105342865 0
0.790398776531219 0
0.798799633979797 0
0.808099150657654 0
0.817299425601959 0
0.827700614929199 0
0.836800754070282 0
0.844699442386627 0
0.852800607681274 0
0.862200200557709 0
0.871099710464478 0
0.879500567913055 0
0.886900007724762 0
0.894300103187561 0
0.902499973773956 0
0.91049998998642 0
0.917900025844574 0
0.925899922847748 0
0.933399975299835 0
0.941100120544434 0
0.947699904441833 0
0.955399990081787 0
0.962699830532074 0
0.971800029277802 0
0.978500008583069 0
0.985899984836578 0
0.992200016975403 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.875362157821655 0.321199744939804
0.878260850906372 0.321099817752838
0.886956632137299 0.319999843835831
0.892753601074219 0.315299600362778
0.892753601074219 0.306199312210083
0.894202888011932 0.286799788475037
0.895652174949646 0.255000352859497
0.897101640701294 0.212599992752075
0.898550748825073 0.1697998046875
0.898550748825073 0.123899951577187
0.901449263095856 0.0834000632166862
0.902898550033569 0.0497000627219677
0.902898550033569 0.0290000084787607
0.905797004699707 0.0147000029683113
0.908695638179779 0.00639999471604824
0.910145103931427 0.00280000315979123
0.91304349899292 0.000999999814666808
0.91304349899292 0.000399999058572575
0.91304349899292 0.000199999529286288
0.914492547512054 0
0.917391300201416 0
0.91884058713913 0
0.920289874076843 0
0.920289874076843 0
0.920289874076843 0
0.921739101409912 0
0.923188388347626 0
0.924637615680695 0
0.924637615680695 0
0.926087021827698 0
0.927536249160767 0
0.92898553609848 0
0.92898553609848 0
0.92898553609848 0
0.92898553609848 0
0.92898553609848 0
0.92898553609848 0
0.931884050369263 0
0.933333337306976 0
0.93478262424469 0
0.937681138515472 0
0.937681138515472 0
0.937681138515472 0
0.937681138515472 0
0.937681138515472 0
0.939130365848541 0
0.9405797123909 0
0.9405797123909 0
0.9405797123909 0
0.9405797123909 0
0.9405797123909 0
0.944927513599396 0
0.944927513599396 0
0.947826087474823 0
0.947826087474823 0
0.949275374412537 0
0.949275374412537 0
0.95072466135025 0
0.95072466135025 0
0.95072466135025 0
0.95072466135025 0
0.95072466135025 0
0.95072466135025 0
0.953623175621033 0
0.955072462558746 0
0.955072462558746 0
0.955072462558746 0
0.960869550704956 0
0.963768124580383 0
0.965217411518097 0
0.965217411518097 0
0.968115925788879 0
0.968115925788879 0
0.969565212726593 0
0.97246378660202 0
0.976811587810516 0
0.976811587810516 0
0.97826087474823 0
0.979710161685944 0
0.979710161685944 0
0.981159448623657 0
0.98405796289444 0
0.985507249832153 0
0.986956536769867 0
0.989855051040649 0
0.989855051040649 0
0.989855051040649 0
0.989855051040649 0
0.989855051040649 0
0.989855051040649 0
0.989855051040649 0
0.989855051040649 0
0.992753624916077 0
0.99420291185379 0
0.99420291185379 0
0.99420291185379 0
0.99420291185379 0
0.995652198791504 0
0.998550713062286 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0916370674967766 0.321199744939804
0.137010708451271 0.321099817752838
0.16192165017128 0.319999843835831
0.181494563817978 0.315299600362778
0.201067671179771 0.306199312210083
0.210854113101959 0.286799788475037
0.220640599727631 0.255000352859497
0.23665477335453 0.212599992752075
0.245551601052284 0.1697998046875
0.257117331027985 0.123899951577187
0.26868337392807 0.0834000632166862
0.280249267816544 0.0497000627219677
0.286476790904999 0.0290000084787607
0.29448390007019 0.0147000029683113
0.300711750984192 0.00639999471604824
0.310498386621475 0.00280000315979123
0.322953432798386 0.000999999814666808
0.330071061849594 0.000399999058572575
0.338078200817108 0.000199999529286288
0.345195770263672 0
0.355872005224228 0
0.362989336252213 0
0.374554961919785 0
0.38078299164772 0
0.388790130615234 0
0.403025060892105 0
0.413701117038727 0
0.422597795724869 0
0.425266891717911 0
0.433274030685425 0
0.440391451120377 0
0.447508901357651 0
0.458185106515884 0
0.468861222267151 0
0.477758020162582 0
0.485765129327774 0
0.495551556348801 0
0.508007347583771 0
0.5151247382164 0
0.522241652011871 0
0.530249953269958 0
0.539146423339844 0
0.540925443172455 0
0.545373499393463 0
0.557829260826111 0
0.564946591854095 0
0.570285081863403 0
0.58540940284729 0
0.592526793479919 0
0.602313339710236 0
0.611209690570831 0
0.617437839508057 0
0.622775256633759 0
0.628113567829132 0
0.63878983259201 0
0.649465978145599 0
0.657473742961884 0
0.664590060710907 0
0.671708047389984 0
0.676156759262085 0
0.685943305492401 0
0.69217050075531 0
0.697508752346039 0
0.705516278743744 0
0.715302586555481 0
0.725089073181152 0
0.735764682292938 0
0.743771731853485 0
0.751779675483704 0
0.760675966739655 0
0.767793595790863 0
0.774910926818848 0
0.781138837337494 0
0.792704284191132 0
0.801601469516754 0
0.811387896537781 0
0.818505585193634 0
0.830071091651917 0
0.836299061775208 0
0.841637194156647 0
0.846974909305573 0
0.856761634349823 0
0.863879084587097 0
0.870996415615082 0
0.880782902240753 0
0.885231375694275 0
0.895907402038574 0
0.903025209903717 0
0.911032021045685 0
0.915480434894562 0
0.926156580448151 0
0.930604994297028 0
0.93683272600174 0
0.948398590087891 0
0.960854113101959 0
0.968861222267151 0
0.976868331432343 0
0.984875440597534 0
0.990213513374329 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.012704617343843 0.321199744939804
0.0257756896317005 0.321099817752838
0.0377473346889019 0.319999843835831
0.0487417243421078 0.315299600362778
0.0587588474154472 0.306199312210083
0.0699975565075874 0.286799788475037
0.0809918791055679 0.255000352859497
0.090764693915844 0.212599992752075
0.10041531920433 0.1697998046875
0.110921047627926 0.123899951577187
0.120938174426556 0.0834000632166862
0.132665708661079 0.0497000627219677
0.145248308777809 0.0290000084787607
0.156608551740646 0.0147000029683113
0.166503667831421 0.00639999471604824
0.176398724317551 0.00280000315979123
0.187393024563789 0.000999999814666808
0.198631778359413 0.000399999058572575
0.207305088639259 0.000199999529286288
0.216711401939392 0
0.228805243968964 0
0.239066764712334 0
0.248717486858368 0
0.25897803902626 0
0.26911786198616 0
0.279012650251389 0
0.290007144212723 0
0.300391167402267 0
0.311874181032181 0
0.323235124349594 0
0.334473520517349 0
0.342291414737701 0
0.352186471223831 0
0.363425433635712 0
0.372587740421295 0
0.382971256971359 0
0.391522109508514 0
0.400928109884262 0
0.410578846931458 0
0.422672808170319 0
0.433911502361298 0
0.443684339523315 0
0.453212767839432 0
0.462252557277679 0
0.47190323472023 0
0.482409000396729 0
0.492670297622681 0
0.502810418605804 0
0.51307201385498 0
0.523331940174103 0
0.534204483032227 0
0.54519921541214 0
0.554239749908447 0
0.56474506855011 0
0.573051691055298 0
0.583679497241974 0
0.594796180725098 0
0.606034636497498 0
0.616784632205963 0
0.628511965274811 0
0.639139652252197 0
0.650501668453217 0
0.660517990589142 0
0.671268343925476 0
0.682140946388245 0
0.691058158874512 0
0.701563775539398 0
0.711702942848206 0
0.720743179321289 0
0.731858491897583 0
0.741876482963562 0
0.751038610935211 0
0.761422336101532 0
0.774981200695038 0
0.783777415752411 0
0.793427705764771 0
0.803689360618591 0
0.814683854579926 0
0.824823081493378 0
0.833740770816803 0
0.842780292034149 0
0.852675199508667 0
0.86244797706604 0
0.871610105037689 0
0.879061877727509 0
0.887491166591644 0
0.896042048931122 0
0.904837727546692 0
0.912777900695801 0
0.921939790248871 0
0.929635882377625 0
0.938431441783905 0
0.945394575595856 0
0.953090608119965 0
0.960298180580139 0
0.970315039157867 0
0.977400422096252 0
0.985218644142151 0
0.991937458515167 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/Markov_target/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.131299614906311 0.27459979057312
0.1819998472929 0.18020011484623
0.232199981808662 0.0888998806476593
0.279899328947067 0.0295000001788139
0.326999306678772 0.00720000313594937
0.380400240421295 0.00119999772869051
0.432399421930313 9.99997646431439e-05
0.476999998092651 0
0.528699100017548 0
0.575999915599823 0
0.620298802852631 0
0.667499959468842 0
0.713598906993866 0
0.760400176048279 0
0.803801119327545 0
0.849999606609344 0
0.890799820423126 0
0.927700102329254 0
0.963799893856049 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.975728154182434 0.27459979057312
0.975728154182434 0.18020011484623
0.978964388370514 0.0888998806476593
0.980582535266876 0.0295000001788139
0.980582535266876 0.00720000313594937
0.982200622558594 0.00119999772869051
0.982200622558594 9.99997646431439e-05
0.985436916351318 0
0.985436916351318 0
0.987055003643036 0
0.988673150539398 0
0.99352753162384 0
0.99352753162384 0
0.99352753162384 0
0.995145618915558 0
0.995145618915558 0
0.99676376581192 0
0.99676376581192 0
0.998381853103638 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.300518095493317 0.27459979057312
0.402417898178101 0.18020011484623
0.461139887571335 0.0888998806476593
0.516407608985901 0.0295000001788139
0.563039720058441 0.00720000313594937
0.599309384822845 0.00119999772869051
0.626943171024323 9.99997646431439e-05
0.664939761161804 0
0.694300591945648 0
0.715026021003723 0
0.740932524204254 0
0.772020936012268 0
0.804835975170135 0
0.829015493392944 0
0.856649279594421 0
0.884283244609833 0
0.910189986228943 0
0.941278040409088 0
0.962003469467163 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0608883611857891 0.27459979057312
0.111780092120171 0.18020011484623
0.164716556668282 0.0888998806476593
0.215153962373734 0.0295000001788139
0.2655910551548 0.00720000313594937
0.323753535747528 0.00119999772869051
0.381006330251694 9.99997646431439e-05
0.428944498300552 0
0.485743373632431 0
0.537999093532562 0
0.586503744125366 0
0.637737929821014 0
0.687946975231171 0
0.739520668983459 0
0.786891102790833 0
0.837554752826691 0
0.882085502147675 0
0.92195850610733 0
0.961490392684937 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/PCFG/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0953001528978348 0.320300132036209
0.107600048184395 0.314699769020081
0.118600003421307 0.294400244951248
0.128399953246117 0.260398834943771
0.137999445199966 0.203700140118599
0.147999987006187 0.142200171947479
0.15680006146431 0.0893002226948738
0.166099861264229 0.0494000427424908
0.175699725747108 0.0241999868303537
0.185099795460701 0.0113999899476767
0.195600137114525 0.00449999421834946
0.206399708986282 0.00109999801497906
0.217200145125389 0.000299999344861135
0.226399958133698 9.99997646431439e-05
0.235400006175041 0
0.243700191378593 0
0.253300160169601 0
0.26319944858551 0
0.271699488162994 0
0.281000256538391 0
0.291500061750412 0
0.300900459289551 0
0.310799717903137 0
0.319300442934036 0
0.328400135040283 0
0.337400376796722 0
0.346999615430832 0
0.356500536203384 0
0.366600424051285 0
0.376500308513641 0
0.386299878358841 0
0.394800126552582 0
0.404400438070297 0
0.413399994373322 0
0.422099769115448 0
0.4314004778862 0
0.439999908208847 0
0.450800180435181 0
0.458999902009964 0
0.469399899244308 0
0.478500008583069 0
0.488400012254715 0
0.496399998664856 0
0.50429904460907 0
0.514200925827026 0
0.523398995399475 0
0.532098591327667 0
0.540999829769135 0
0.550402283668518 0
0.560400128364563 0
0.570201396942139 0
0.580199778079987 0
0.588699638843536 0
0.598800778388977 0
0.607200026512146 0
0.617799997329712 0
0.628500044345856 0
0.638200879096985 0
0.648999869823456 0
0.658199787139893 0
0.667600512504578 0
0.678200900554657 0
0.687401175498962 0
0.697100579738617 0
0.707099437713623 0
0.716300249099731 0
0.725099623203278 0
0.734799981117249 0
0.744101166725159 0
0.752999782562256 0
0.761100709438324 0
0.769200563430786 0
0.777799308300018 0
0.788599371910095 0
0.795599222183228 0
0.804800450801849 0
0.813900053501129 0
0.823800086975098 0
0.834000408649445 0
0.842000186443329 0
0.851000308990479 0
0.862599790096283 0
0.870900511741638 0
0.879599630832672 0
0.887100577354431 0
0.894600391387939 0
0.902899980545044 0
0.910500407218933 0
0.918200016021729 0
0.925999999046326 0
0.934300005435944 0
0.941100001335144 0
0.948500216007233 0
0.955399692058563 0
0.963500022888184 0
0.972500026226044 0
0.978200018405914 0
0.985699892044067 0
0.993399977684021 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.88823527097702 0.320300132036209
0.88823527097702 0.314699769020081
0.891176581382751 0.294400244951248
0.892647266387939 0.260398834943771
0.892647266387939 0.203700140118599
0.894117712974548 0.142200171947479
0.895588338375092 0.0893002226948738
0.897058844566345 0.0494000427424908
0.898529410362244 0.0241999868303537
0.898529410362244 0.0113999899476767
0.901470601558685 0.00449999421834946
0.902941167354584 0.00109999801497906
0.902941167354584 0.000299999344861135
0.905882358551025 9.99997646431439e-05
0.908823728561401 0
0.910294115543365 0
0.913235306739807 0
0.913235306739807 0
0.913235306739807 0
0.914705872535706 0
0.917647063732147 0
0.919117629528046 0
0.920588254928589 0
0.920588254928589 0
0.920588254928589 0
0.922058820724487 0
0.923529326915741 0
0.925000071525574 0
0.925000071525574 0
0.926470577716827 0
0.927941203117371 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.932352960109711 0
0.933823525905609 0
0.935294091701508 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.939705789089203 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.945588231086731 0
0.945588231086731 0
0.948529422283173 0
0.948529422283173 0
0.949999988079071 0
0.949999988079071 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.952941179275513 0
0.954411745071411 0
0.954411745071411 0
0.954411745071411 0
0.960294127464294 0
0.963235318660736 0
0.964705884456635 0
0.964705884456635 0
0.967647075653076 0
0.967647075653076 0
0.969117641448975 0
0.972058832645416 0
0.976470589637756 0
0.976470589637756 0
0.977941155433655 0
0.979411780834198 0
0.979411780834198 0
0.980882346630096 0
0.983823537826538 0
0.985294103622437 0
0.98676472902298 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.992647051811218 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.99558824300766 0
0.998529434204102 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.177936017513275 0.320300132036209
0.195729553699493 0.314699769020081
0.204626396298409 0.294400244951248
0.214412808418274 0.260398834943771
0.225978657603264 0.203700140118599
0.23309613764286 0.142200171947479
0.241103202104568 0.0893002226948738
0.257117420434952 0.0494000427424908
0.264234930276871 0.0241999868303537
0.274021714925766 0.0113999899476767
0.284697949886322 0.00449999421834946
0.297153115272522 0.00109999801497906
0.303380697965622 0.000299999344861135
0.309608548879623 9.99997646431439e-05
0.317615747451782 0
0.324733018875122 0
0.337188869714737 0
0.34341636300087 0
0.351423472166061 0
0.360320329666138 0
0.370106756687164 0
0.375444740056992 0
0.38790038228035 0
0.392348736524582 0
0.399466067552567 0
0.411032021045685 0
0.421708166599274 0
0.428825467824936 0
0.431494861841202 0
0.438612133264542 0
0.445729583501816 0
0.454626202583313 0
0.466192156076431 0
0.474199295043945 0
0.483985751867294 0
0.492882549762726 0
0.502668261528015 0
0.516014397144318 0
0.524021625518799 0
0.530249238014221 0
0.537366688251495 0
0.546262741088867 0
0.548043429851532 0
0.554270267486572 0
0.564056754112244 0
0.571173489093781 0
0.577402234077454 0
0.592526912689209 0
0.600533723831177 0
0.609430551528931 0
0.618327260017395 0
0.624555170536041 0
0.630783081054688 0
0.636120915412903 0
0.646797120571136 0
0.656583487987518 0
0.664590537548065 0
0.670818626880646 0
0.679715514183044 0
0.683273613452911 0
0.69484007358551 0
0.70195746421814 0
0.706405699253082 0
0.715302228927612 0
0.724199175834656 0
0.735765039920807 0
0.745551884174347 0
0.752669155597687 0
0.761565506458282 0
0.77046275138855 0
0.777579963207245 0
0.783808052539825 0
0.788256168365479 0
0.799821972846985 0
0.806939601898193 0
0.817615568637848 0
0.823843419551849 0
0.832740008831024 0
0.839857459068298 0
0.845195710659027 0
0.850533783435822 0
0.859430313110352 0
0.868327140808105 0
0.875444650650024 0
0.885231375694275 0
0.889679670333862 0
0.900355935096741 0
0.90747332572937 0
0.913701057434082 0
0.917259812355042 0
0.92793595790863 0
0.932384312152863 0
0.939501762390137 0
0.951067507266998 0
0.962633430957794 0
0.970640540122986 0
0.976868331432343 0
0.984875440597534 0
0.991103231906891 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0181796066462994 0.320300132036209
0.0307467244565487 0.314699769020081
0.0427037514746189 0.294400244951248
0.0531966648995876 0.260398834943771
0.0633233040571213 0.203700140118599
0.0744264721870422 0.142200171947479
0.0839433372020721 0.0893002226948738
0.0929721519351006 0.0494000427424908
0.103587128221989 0.0241999868303537
0.113714016973972 0.0113999899476767
0.12481689453125 0.00449999421834946
0.13616406917572 0.00109999801497906
0.148487001657486 0.000299999344861135
0.158613577485085 9.99997646431439e-05
0.168252810835838 0
0.177281603217125 0
0.18704254925251 0
0.198267474770546 0
0.207540258765221 0
0.217545136809349 0
0.228770107030869 0
0.239385053515434 0
0.249633595347404 0
0.259394884109497 0
0.269522190093994 0
0.27879399061203 0
0.288921654224396 0
0.299414277076721 0
0.311370968818665 0
0.322351902723312 0
0.333211421966553 0
0.342239826917648 0
0.352366983890533 0
0.362249791622162 0
0.371522933244705 0
0.381649553775787 0
0.390800267457962 0
0.401903122663498 0
0.410687923431396 0
0.42240110039711 0
0.43228405714035 0
0.44314306974411 0
0.452659904956818 0
0.461444497108459 0
0.472181558609009 0
0.482308208942413 0
0.491948068141937 0
0.500732660293579 0
0.511102259159088 0
0.522085964679718 0
0.532822132110596 0
0.54380065202713 0
0.553318798542023 0
0.5646653175354 0
0.573450446128845 0
0.584918856620789 0
0.596877098083496 0
0.607735097408295 0
0.619691550731659 0
0.630429267883301 0
0.640312075614929 0
0.652269780635834 0
0.662885189056396 0
0.673378169536591 0
0.684236288070679 0
0.693875193595886 0
0.703268706798553 0
0.713640630245209 0
0.723524034023285 0
0.733039498329163 0
0.741946816444397 0
0.750731706619263 0
0.760615468025208 0
0.772083580493927 0
0.77940434217453 0
0.788799405097961 0
0.799048781394958 0
0.809785008430481 0
0.821132481098175 0
0.830161094665527 0
0.840287744998932 0
0.852977514266968 0
0.861762166023254 0
0.871278762817383 0
0.878843665122986 0
0.887384116649628 0
0.896046817302704 0
0.904343485832214 0
0.912884473800659 0
0.921913266181946 0
0.930576145648956 0
0.938262522220612 0
0.946071267127991 0
0.952781856060028 0
0.961078584194183 0
0.970961451530457 0
0.977061986923218 0
0.984992682933807 0
0.993289411067963 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/PCFG_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0937000438570976 0.319800019264221
0.10670006275177 0.313099205493927
0.118199974298477 0.300400406122208
0.127400323748589 0.277601063251495
0.138099506497383 0.252601206302643
0.148200169205666 0.219899952411652
0.157499983906746 0.189100116491318
0.168199956417084 0.157599598169327
0.177399933338165 0.125999748706818
0.186400219798088 0.0990000218153
0.196999877691269 0.0769002065062523
0.208300054073334 0.0579000003635883
0.218800097703934 0.0427999086678028
0.228899970650673 0.0315000116825104
0.23839995265007 0.0238999854773283
0.247399896383286 0.0155000109225512
0.257000416517258 0.00960000418126583
0.267300188541412 0.00600000517442822
0.275499761104584 0.00379999494180083
0.284899771213531 0.00260000303387642
0.295700013637543 0.0015000025741756
0.305199325084686 0.000599998980760574
0.314299613237381 0.000499999907333404
0.322999686002731 0.000399999669753015
0.332699984312057 0.000199999529286288
0.342999696731567 0
0.352199494838715 0
0.360299855470657 0
0.369398862123489 0
0.379500508308411 0
0.389500558376312 0
0.397900551557541 0
0.407099723815918 0
0.415999710559845 0
0.424699991941452 0
0.434900104999542 0
0.443200498819351 0
0.453200101852417 0
0.460799902677536 0
0.471299916505814 0
0.480399996042252 0
0.489699900150299 0
0.497300386428833 0
0.50540018081665 0
0.514399826526642 0
0.523200333118439 0
0.532200694084167 0
0.541399836540222 0
0.550999581813812 0
0.560899436473846 0
0.570699036121368 0
0.580701470375061 0
0.589399755001068 0
0.599299669265747 0
0.607498705387115 0
0.617800414562225 0
0.627299189567566 0
0.636400103569031 0
0.645999491214752 0
0.655299961566925 0
0.6644007563591 0
0.67389988899231 0
0.684099733829498 0
0.693200707435608 0
0.703300654888153 0
0.713398396968842 0
0.723499000072479 0
0.733000874519348 0
0.742099404335022 0
0.752699792385101 0
0.760700464248657 0
0.770000159740448 0
0.778900027275085 0
0.789501070976257 0
0.797598421573639 0
0.807401120662689 0
0.815799415111542 0
0.825700879096985 0
0.834701180458069 0
0.84240049123764 0
0.850500404834747 0
0.861000001430511 0
0.869800567626953 0
0.87749981880188 0
0.88519960641861 0
0.893100023269653 0
0.901700019836426 0
0.909599781036377 0
0.916400015354156 0
0.924599826335907 0
0.931299984455109 0
0.938700020313263 0
0.94539999961853 0
0.953499972820282 0
0.961700022220612 0
0.971300005912781 0
0.977400004863739 0
0.98470002412796 0
0.992500007152557 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.88823527097702 0.319800019264221
0.88823527097702 0.313099205493927
0.891176581382751 0.300400406122208
0.892647266387939 0.277601063251495
0.892647266387939 0.252601206302643
0.894117712974548 0.219899952411652
0.895588338375092 0.189100116491318
0.897058844566345 0.157599598169327
0.898529410362244 0.125999748706818
0.898529410362244 0.0990000218153
0.901470601558685 0.0769002065062523
0.902941167354584 0.0579000003635883
0.902941167354584 0.0427999086678028
0.905882358551025 0.0315000116825104
0.908823728561401 0.0238999854773283
0.910294115543365 0.0155000109225512
0.913235306739807 0.00960000418126583
0.913235306739807 0.00600000517442822
0.913235306739807 0.00379999494180083
0.914705872535706 0.00260000303387642
0.917647063732147 0.0015000025741756
0.919117629528046 0.000599998980760574
0.920588254928589 0.000499999907333404
0.920588254928589 0.000399999669753015
0.920588254928589 0.000199999529286288
0.922058820724487 0
0.923529326915741 0
0.925000071525574 0
0.925000071525574 0
0.926470577716827 0
0.927941203117371 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.932352960109711 0
0.933823525905609 0
0.935294091701508 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.939705789089203 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.945588231086731 0
0.945588231086731 0
0.948529422283173 0
0.948529422283173 0
0.949999988079071 0
0.949999988079071 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.952941179275513 0
0.954411745071411 0
0.954411745071411 0
0.954411745071411 0
0.960294127464294 0
0.963235318660736 0
0.964705884456635 0
0.964705884456635 0
0.967647075653076 0
0.967647075653076 0
0.969117641448975 0
0.972058832645416 0
0.976470589637756 0
0.976470589637756 0
0.977941155433655 0
0.979411780834198 0
0.979411780834198 0
0.980882346630096 0
0.983823537826538 0
0.985294103622437 0
0.98676472902298 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.992647051811218 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.99558824300766 0
0.998529434204102 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.175176009535789 0.319800019264221
0.191021174192429 0.313099205493927
0.1989436596632 0.300400406122208
0.20510570704937 0.277601063251495
0.220070391893387 0.252601206302643
0.228873237967491 0.219899952411652
0.234154924750328 0.189100116491318
0.250880122184753 0.157599598169327
0.258802860975266 0.125999748706818
0.26936611533165 0.0990000218153
0.279049158096313 0.0769002065062523
0.289612501859665 0.0579000003635883
0.297535359859467 0.0427999086678028
0.30281674861908 0.0315000116825104
0.31073921918869 0.0238999854773283
0.320422351360321 0.0155000109225512
0.33186599612236 0.00960000418126583
0.339788764715195 0.00600000517442822
0.346830934286118 0.00379999494180083
0.355633974075317 0.00260000303387642
0.367077589035034 0.0015000025741756
0.375000029802322 0.000599998980760574
0.386443734169006 0.000499999907333404
0.390845000743866 0.000399999669753015
0.399647802114487 0.000199999529286288
0.413732379674911 0
0.424295783042908 0
0.43133807182312 0
0.433978915214539 0
0.441901296377182 0
0.448943674564362 0
0.456866264343262 0
0.468309968709946 0
0.477992951869965 0
0.487676054239273 0
0.497358947992325 0
0.506162047386169 0
0.519366323947906 0
0.526408791542053 0
0.532570779323578 0
0.540493190288544 0
0.549295783042908 0
0.551936447620392 0
0.55633819103241 0
0.566020846366882 0
0.573063611984253 0
0.578344762325287 0
0.593310236930847 0
0.60035228729248 0
0.61003565788269 0
0.618837893009186 0
0.62587982416153 0
0.632042229175568 0
0.640844821929932 0
0.652288854122162 0
0.661971509456635 0
0.669893980026245 0
0.677816808223724 0
0.684859335422516 0
0.688380479812622 0
0.698063313961029 0
0.704225659370422 0
0.708627283573151 0
0.716549336910248 0
0.725352108478546 0
0.735035479068756 0
0.744718372821808 0
0.753521084785461 0
0.760563611984253 0
0.769366383552551 0
0.778169214725494 0
0.785211443901062 0
0.790492951869965 0
0.801936566829681 0
0.808978915214539 0
0.819542169570923 0
0.82658451795578 0
0.836267411708832 0
0.842429399490356 0
0.847711026668549 0
0.853873491287231 0
0.861795723438263 0
0.871478736400604 0
0.879401743412018 0
0.888204097747803 0
0.893486082553864 0
0.904049098491669 0
0.910211026668549 0
0.916373014450073 0
0.919894456863403 0
0.930457770824432 0
0.934859156608582 0
0.941901385784149 0
0.953345060348511 0
0.964788734912872 0
0.97183096408844 0
0.977992951869965 0
0.98591548204422 0
0.991197168827057 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0163734555244446 0.319800019264221
0.0300586335361004 0.313099205493927
0.0427663736045361 0.300400406122208
0.0530302748084068 0.277601063251495
0.064027413725853 0.252601206302643
0.0750242918729782 0.219899952411652
0.0855327323079109 0.189100116491318
0.0961633175611496 0.157599598169327
0.106182798743248 0.125999748706818
0.115713611245155 0.0990000218153
0.127077281475067 0.0769002065062523
0.139295771718025 0.0579000003635883
0.151026576757431 0.0427999086678028
0.16239008307457 0.0315000116825104
0.172653779387474 0.0238999854773283
0.182184785604477 0.0155000109225512
0.192082226276398 0.00960000418126583
0.20356796681881 0.00600000517442822
0.212609976530075 0.00379999494180083
0.222751706838608 0.00260000303387642
0.234115317463875 0.0015000025741756
0.244501292705536 0.000599998980760574
0.253910422325134 0.000499999907333404
0.263929426670074 0.000399999669753015
0.27455934882164 0.000199999529286288
0.285068869590759 0
0.294720411300659 0
0.303519010543823 0
0.314271509647369 0
0.325390875339508 0
0.336510509252548 0
0.345552533864975 0
0.355205148458481 0
0.364736437797546 0
0.37402218580246 0
0.385141611099243 0
0.394061923027039 0
0.40420338511467 0
0.412389785051346 0
0.424242436885834 0
0.434017688035965 0
0.444159299135208 0
0.453079283237457 0
0.462365537881851 0
0.47201856970787 0
0.481671720743179 0
0.491813331842422 0
0.500977039337158 0
0.511728286743164 0
0.522483229637146 0
0.533236443996429 0
0.544110536575317 0
0.553886353969574 0
0.564514815807343 0
0.572947084903717 0
0.584067106246948 0
0.594574570655823 0
0.604472041130066 0
0.615224719047546 0
0.626100420951843 0
0.635875940322876 0
0.64662766456604 0
0.658480584621429 0
0.668376863002777 0
0.679375410079956 0
0.690371096134186 0
0.701368749141693 0
0.711264908313751 0
0.721163153648376 0
0.732770919799805 0
0.7413250207901 0
0.751466155052185 0
0.761608302593231 0
0.772848963737488 0
0.781525194644928 0
0.791666448116302 0
0.800952732563019 0
0.811583697795868 0
0.821602880954742 0
0.830279052257538 0
0.839197993278503 0
0.850684285163879 0
0.859970808029175 0
0.868157744407654 0
0.876099467277527 0
0.885019361972809 0
0.894061684608459 0
0.902859568595886 0
0.910312950611115 0
0.91984349489212 0
0.926564157009125 0
0.934994995594025 0
0.941959917545319 0
0.950146615505219 0
0.958577930927277 0
0.969330430030823 0
0.975928664207458 0
0.9836266040802 0
0.992179870605469 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/PCFG_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0813001096248627 0.321199744939804
0.0960001423954964 0.320900231599808
0.109399974346161 0.320399910211563
0.12109998613596 0.317699939012527
0.131899774074554 0.309499591588974
0.143600165843964 0.291999667882919
0.153400152921677 0.26489993929863
0.164200112223625 0.225500002503395
0.174000024795532 0.180300250649452
0.183499962091446 0.133000150322914
0.192199870944023 0.0917000249028206
0.203200146555901 0.0585999861359596
0.21419994533062 0.0333000347018242
0.224599897861481 0.0192000083625317
0.234400004148483 0.0109000029042363
0.243699908256531 0.00560000538825989
0.253599524497986 0.00219999602995813
0.264201551675797 0.00079999933950603
0.272899866104126 0.000299999752314761
0.282599300146103 0.000199999834876508
0.293899387121201 9.99999174382538e-05
0.302999407052994 0
0.312100023031235 0
0.320899963378906 0
0.329900145530701 0
0.339500159025192 0
0.348799914121628 0
0.358500331640244 0
0.368600457906723 0
0.379500478506088 0
0.38959988951683 0
0.397600412368774 0
0.407300263643265 0
0.416200190782547 0
0.425799816846848 0
0.434899896383286 0
0.443300247192383 0
0.45300018787384 0
0.461600303649902 0
0.471799910068512 0
0.48100009560585 0
0.489600002765656 0
0.497499912977219 0
0.506301701068878 0
0.516099631786346 0
0.525100946426392 0
0.534600973129272 0
0.543601155281067 0
0.553499639034271 0
0.563300371170044 0
0.573499381542206 0
0.583600163459778 0
0.591400444507599 0
0.600898265838623 0
0.609800577163696 0
0.620298981666565 0
0.629899084568024 0
0.639199912548065 0
0.649201214313507 0
0.659699857234955 0
0.668501198291779 0
0.67900013923645 0
0.687899231910706 0
0.69760000705719 0
0.707799971103668 0
0.717599391937256 0
0.726698875427246 0
0.736501097679138 0
0.745700061321259 0
0.754901051521301 0
0.762898802757263 0
0.771498799324036 0
0.781400859355927 0
0.792699337005615 0
0.800700068473816 0
0.810498893260956 0
0.820699036121368 0
0.830699980258942 0
0.839200556278229 0
0.846900224685669 0
0.855200171470642 0
0.865100026130676 0
0.874100983142853 0
0.88230037689209 0
0.889800071716309 0
0.897600114345551 0
0.905300080776215 0
0.912800192832947 0
0.920300126075745 0
0.928699612617493 0
0.935999810695648 0
0.943099915981293 0
0.949399888515472 0
0.956500172615051 0
0.963400185108185 0
0.972400009632111 0
0.977999806404114 0
0.985300004482269 0
0.99260002374649 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.876453459262848 0.321199744939804
0.880814015865326 0.320900231599808
0.886627912521362 0.320399910211563
0.889534950256348 0.317699939012527
0.889534950256348 0.309499591588974
0.893895328044891 0.291999667882919
0.895348846912384 0.26489993929863
0.896802484989166 0.225500002503395
0.898255825042725 0.180300250649452
0.898255825042725 0.133000150322914
0.901162803173065 0.0917000249028206
0.902616262435913 0.0585999861359596
0.902616262435913 0.0333000347018242
0.905523180961609 0.0192000083625317
0.908430218696594 0.0109000029042363
0.909883916378021 0.00560000538825989
0.912790715694427 0.00219999602995813
0.912790715694427 0.00079999933950603
0.912790715694427 0.000299999752314761
0.914244174957275 0.000199999834876508
0.917151153087616 9.99999174382538e-05
0.918604671955109 0
0.920058131217957 0
0.921511650085449 0
0.921511650085449 0
0.922965109348297 0
0.9244185090065 0
0.925872206687927 0
0.925872206687927 0
0.92732560634613 0
0.928779065608978 0
0.930232584476471 0
0.930232584476471 0
0.930232584476471 0
0.930232584476471 0
0.930232584476471 0
0.930232584476471 0
0.933139562606812 0
0.934593021869659 0
0.936046421527863 0
0.938953399658203 0
0.938953399658203 0
0.938953399658203 0
0.938953399658203 0
0.938953399658203 0
0.940406978130341 0
0.941860437393188 0
0.941860437393188 0
0.941860437393188 0
0.941860437393188 0
0.941860437393188 0
0.946220934391022 0
0.946220934391022 0
0.949127912521362 0
0.949127912521362 0
0.95058137178421 0
0.95058137178421 0
0.952034890651703 0
0.952034890651703 0
0.952034890651703 0
0.952034890651703 0
0.952034890651703 0
0.952034890651703 0
0.953488349914551 0
0.954941868782043 0
0.954941868782043 0
0.954941868782043 0
0.960755825042725 0
0.963662803173065 0
0.965116262435913 0
0.965116262435913 0
0.968023240566254 0
0.968023240566254 0
0.969476759433746 0
0.972383737564087 0
0.976744174957275 0
0.976744174957275 0
0.978197693824768 0
0.979651153087616 0
0.979651153087616 0
0.981104671955109 0
0.984011650085449 0
0.985465109348297 0
0.98691862821579 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.992732584476471 0
0.994186043739319 0
0.994186043739319 0
0.994186043739319 0
0.994186043739319 0
0.995639562606812 0
0.998546540737152 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0872600004076958 0.321199744939804
0.126527070999146 0.320900231599808
0.1518325060606 0.320399910211563
0.170157089829445 0.317699939012527
0.18673649430275 0.309499591588974
0.201570704579353 0.291999667882919
0.215532273054123 0.26489993929863
0.230366498231888 0.225500002503395
0.239965096116066 0.180300250649452
0.249563783407211 0.133000150322914
0.25916263461113 0.0917000249028206
0.270505964756012 0.0585999861359596
0.279232293367386 0.0333000347018242
0.28446763753891 0.0192000083625317
0.293193817138672 0.0109000029042363
0.303664773702621 0.00560000538825989
0.315008878707886 0.00219999602995813
0.324607342481613 0.00079999933950603
0.331588119268417 0.000299999752314761
0.34118664264679 0.000199999834876508
0.351658165454865 9.99999174382538e-05
0.357766181230545 0
0.370855152606964 0
0.376963198184967 0
0.388307243585587 0
0.399650990962982 0
0.409249812364578 0
0.418848067522049 0
0.422338455915451 0
0.433682262897491 0
0.442408472299576 0
0.449389189481735 0
0.460732996463776 0
0.468586385250092 0
0.478184998035431 0
0.486038386821747 0
0.499127566814423 0
0.511343479156494 0
0.52006995677948 0
0.527051329612732 0
0.534031867980957 0
0.542757749557495 0
0.544502139091492 0
0.550611019134521 0
0.561954915523529 0
0.5698082447052 0
0.575043857097626 0
0.589878082275391 0
0.595986008644104 0
0.604712545871735 0
0.613438069820404 0
0.620418965816498 0
0.62652713060379 0
0.632635354995728 0
0.643979012966156 0
0.654450118541718 0
0.661430954933167 0
0.668411791324615 0
0.676264941692352 0
0.681500494480133 0
0.691972315311432 0
0.698952853679657 0
0.703315734863281 0
0.710296511650085 0
0.719895243644714 0
0.730366587638855 0
0.740837156772614 0
0.749564051628113 0
0.756544232368469 0
0.766142904758453 0
0.773123860359192 0
0.780104756355286 0
0.785340547561646 0
0.79755687713623 0
0.805410265922546 0
0.815008640289307 0
0.8219895362854 0
0.832460939884186 0
0.838568866252899 0
0.844676911830902 0
0.849912464618683 0
0.8586385846138 0
0.86649215221405 0
0.874345481395721 0
0.883071601390839 0
0.887434601783752 0
0.898778557777405 0
0.904886543750763 0
0.911867260932922 0
0.915357768535614 0
0.928446769714355 0
0.93280953168869 0
0.939790546894073 0
0.95287960767746 0
0.963350772857666 0
0.971204161643982 0
0.978184998035431 0
0.986038386821747 0
0.991273999214172 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0134704736992717 0.321199744939804
0.0255939159542322 0.320900231599808
0.0379622243344784 0.320399910211563
0.0494734346866608 0.317699939012527
0.060372281819582 0.309499591588974
0.0722508281469345 0.291999667882919
0.0821701064705849 0.26489993929863
0.0931913405656815 0.225500002503395
0.103722751140594 0.180300250649452
0.114009328186512 0.133000150322914
0.12307134270668 0.0917000249028206
0.134827122092247 0.0585999861359596
0.147072821855545 0.0333000347018242
0.158829510211945 0.0192000083625317
0.169360518455505 0.0109000029042363
0.179157391190529 0.00560000538825989
0.18944376707077 0.00219999602995813
0.201077699661255 0.00079999933950603
0.210751891136169 0.000299999752314761
0.221160992980003 0.000199999834876508
0.233284473419189 9.99999174382538e-05
0.243448302149773 0
0.252632051706314 0
0.262429893016815 0
0.271859228610992 0
0.281900674104691 0
0.291820198297501 0
0.302228927612305 0
0.314107447862625 0
0.325740814208984 0
0.336761951446533 0
0.345457017421722 0
0.355742841959 0
0.365540355443954 0
0.375948876142502 0
0.385990619659424 0
0.394440144300461 0
0.404359817504883 0
0.413544118404388 0
0.424932658672333 0
0.434974402189255 0
0.444280982017517 0
0.453710615634918 0
0.463629752397537 0
0.474038690328598 0
0.483835428953171 0
0.494612008333206 0
0.503552258014679 0
0.514817118644714 0
0.525594353675842 0
0.536861479282379 0
0.547880411148071 0
0.556576788425446 0
0.567107617855072 0
0.576412856578827 0
0.587680518627167 0
0.598456084728241 0
0.608743190765381 0
0.619888067245483 0
0.632010638713837 0
0.641317248344421 0
0.65319550037384 0
0.663482964038849 0
0.674259424209595 0
0.685280561447144 0
0.69581139087677 0
0.705485701560974 0
0.715772092342377 0
0.725813627243042 0
0.735610604286194 0
0.744427502155304 0
0.753734886646271 0
0.765123128890991 0
0.777124285697937 0
0.785574376583099 0
0.795860290527344 0
0.807371437549591 0
0.818025827407837 0
0.827455341815948 0
0.836027324199677 0
0.845334649085999 0
0.855988144874573 0
0.86578506231308 0
0.874601662158966 0
0.882316946983337 0
0.89125645160675 0
0.899093449115753 0
0.907421171665192 0
0.915625631809235 0
0.925422430038452 0
0.932524979114532 0
0.940607190132141 0
0.947097599506378 0
0.953832864761353 0
0.960813105106354 0
0.97073233127594 0
0.976610362529755 0
0.984325230121613 0
0.992285072803497 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/RNN/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0917002782225609 0.319999843835831
0.104000076651573 0.311399728059769
0.11520005017519 0.287700355052948
0.124499961733818 0.24549999833107
0.135099709033966 0.18609981238842
0.145699962973595 0.125000134110451
0.153799891471863 0.0718998983502388
0.162900194525719 0.0374000184237957
0.172299891710281 0.0167999844998121
0.1819998472929 0.00799999851733446
0.19160008430481 0.00330000161193311
0.201800480484962 0.00109999941196293
0.211700096726418 0.000399999669753015
0.222199976444244 9.99997646431439e-05
0.231799945235252 9.99997646431439e-05
0.240099996328354 0
0.250699877738953 0
0.261100232601166 0
0.268999636173248 0
0.277300029993057 0
0.288898944854736 0
0.298200279474258 0
0.306900054216385 0
0.31630003452301 0
0.326000511646271 0
0.33580020070076 0
0.346399635076523 0
0.355099409818649 0
0.365400165319443 0
0.376300722360611 0
0.38689923286438 0
0.395100176334381 0
0.405699402093887 0
0.415600478649139 0
0.424500197172165 0
0.433199614286423 0
0.441099613904953 0
0.45089989900589 0
0.460200011730194 0
0.470400005578995 0
0.479699909687042 0
0.489800006151199 0
0.498999744653702 0
0.506698906421661 0
0.515602231025696 0
0.524200022220612 0
0.533300220966339 0
0.543200552463531 0
0.55229926109314 0
0.562101423740387 0
0.572401285171509 0
0.582499742507935 0
0.591000258922577 0
0.600798904895782 0
0.608801603317261 0
0.618999719619751 0
0.62819892168045 0
0.637599408626556 0
0.647800803184509 0
0.657499670982361 0
0.666801452636719 0
0.677101075649261 0
0.68589973449707 0
0.695800721645355 0
0.70560222864151 0
0.715600609779358 0
0.725400626659393 0
0.735499620437622 0
0.744400024414062 0
0.753398656845093 0
0.761800825595856 0
0.770899891853333 0
0.779101073741913 0
0.789900660514832 0
0.798000335693359 0
0.807600200176239 0
0.816900610923767 0
0.826499223709106 0
0.83569872379303 0
0.843700110912323 0
0.852400183677673 0
0.862500607967377 0
0.871199607849121 0
0.879900276660919 0
0.887199401855469 0
0.895200192928314 0
0.904100179672241 0
0.911700010299683 0
0.91869980096817 0
0.927299797534943 0
0.935400187969208 0
0.94219982624054 0
0.94870001077652 0
0.955500364303589 0
0.963100075721741 0
0.972100019454956 0
0.97790002822876 0
0.985499978065491 0
0.99260002374649 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.883040964603424 0.319999843835831
0.883040964603424 0.311399728059769
0.885964930057526 0.287700355052948
0.887426912784576 0.24549999833107
0.887426912784576 0.18609981238842
0.888888955116272 0.125000134110451
0.890350937843323 0.0718998983502388
0.891812860965729 0.0374000184237957
0.894737005233765 0.0167999844998121
0.894737005233765 0.00799999851733446
0.897660791873932 0.00330000161193311
0.899122834205627 0.00109999941196293
0.899122834205627 0.000399999669753015
0.902046799659729 9.99997646431439e-05
0.904970765113831 9.99997646431439e-05
0.906432747840881 0
0.909356713294983 0
0.909356713294983 0
0.909356713294983 0
0.910818696022034 0
0.913742661476135 0
0.915204703807831 0
0.916666686534882 0
0.916666686534882 0
0.916666686534882 0
0.918128669261932 0
0.921052634716034 0
0.923976540565491 0
0.923976540565491 0
0.925438702106476 0
0.926900565624237 0
0.928362548351288 0
0.928362548351288 0
0.928362548351288 0
0.928362548351288 0
0.928362548351288 0
0.928362548351288 0
0.931286573410034 0
0.932748556137085 0
0.934210538864136 0
0.937134504318237 0
0.937134504318237 0
0.937134504318237 0
0.937134504318237 0
0.937134504318237 0
0.938596487045288 0
0.940058410167694 0
0.940058410167694 0
0.940058410167694 0
0.940058410167694 0
0.940058410167694 0
0.944444417953491 0
0.944444417953491 0
0.947368443012238 0
0.948830425739288 0
0.950292408466339 0
0.950292408466339 0
0.95175439119339 0
0.95175439119339 0
0.95175439119339 0
0.95175439119339 0
0.95175439119339 0
0.95175439119339 0
0.953216373920441 0
0.954678356647491 0
0.954678356647491 0
0.954678356647491 0
0.960526287555695 0
0.963450312614441 0
0.964912295341492 0
0.964912295341492 0
0.967836260795593 0
0.967836260795593 0
0.969298243522644 0
0.972222208976746 0
0.976608216762543 0
0.976608216762543 0
0.978070199489594 0
0.979532182216644 0
0.979532182216644 0
0.980994164943695 0
0.983918130397797 0
0.985380113124847 0
0.986842095851898 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.992690086364746 0
0.994152069091797 0
0.994152069091797 0
0.994152069091797 0
0.994152069091797 0
0.995614051818848 0
0.998538017272949 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.171833455562592 0.319999843835831
0.186891064047813 0.311399728059769
0.196634188294411 0.287700355052948
0.203720092773438 0.24549999833107
0.216120347380638 0.18609981238842
0.223206385970116 0.125000134110451
0.229406550526619 0.0718998983502388
0.24357844889164 0.0374000184237957
0.250664681196213 0.0167999844998121
0.262178927659988 0.00799999851733446
0.275465279817581 0.00330000161193311
0.283436417579651 0.00109999941196293
0.290522456169128 0.000399999669753015
0.29672247171402 9.99997646431439e-05
0.306465655565262 9.99997646431439e-05
0.314437389373779 0
0.324180752038956 0
0.333038091659546 0
0.340124160051346 0
0.347209870815277 0
0.356067329645157 0
0.36226749420166 0
0.3746677339077 0
0.379982113838196 0
0.38883963227272 0
0.402125746011734 0
0.411868929862976 0
0.420726269483566 0
0.423383593559265 0
0.431355088949203 0
0.438441038131714 0
0.444641292095184 0
0.456155955791473 0
0.465013295412064 0
0.474756479263306 0
0.482728064060211 0
0.493357002735138 0
0.508414030075073 0
0.519043803215027 0
0.526129126548767 0
0.534101188182831 0
0.542073130607605 0
0.544729769229889 0
0.548273265361786 0
0.558015882968903 0
0.567759394645691 0
0.573959469795227 0
0.589016199111938 0
0.596102356910706 0
0.604074537754059 0
0.613817453384399 0
0.621789038181305 0
0.62798935174942 0
0.633303761482239 0
0.644818663597107 0
0.656332850456238 0
0.663418710231781 0
0.670504689216614 0
0.677590370178223 0
0.682019233703613 0
0.693533658981323 0
0.699734210968018 0
0.704163074493408 0
0.712134420871735 0
0.721877634525299 0
0.733392655849457 0
0.743135511875153 0
0.751107037067413 0
0.759078621864319 0
0.767936050891876 0
0.775022149085999 0
0.782107830047607 0
0.78742241859436 0
0.798937261104584 0
0.806908428668976 0
0.817537724971771 0
0.823737740516663 0
0.833480954170227 0
0.83879542350769 0
0.844109773635864 0
0.851195573806763 0
0.860053300857544 0
0.868025064468384 0
0.875996172428131 0
0.884853661060333 0
0.891053915023804 0
0.902568519115448 0
0.908768713474274 0
0.915854752063751 0
0.920283317565918 0
0.931798040866852 0
0.936226844787598 0
0.942426919937134 0
0.953055799007416 0
0.963684678077698 0
0.970770597457886 0
0.976970791816711 0
0.984942436218262 0
0.991142630577087 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.01453522965312 0.319999843835831
0.0274825971573591 0.311399728059769
0.0395749658346176 0.287700355052948
0.0498351417481899 0.24549999833107
0.0610724054276943 0.18609981238842
0.0729203969240189 0.125000134110451
0.0818369388580322 0.0718998983502388
0.0908757373690605 0.0374000184237957
0.101135917007923 0.0167999844998121
0.111396141350269 0.00799999851733446
0.12104556709528 0.00330000161193311
0.132283344864845 0.00109999941196293
0.143397703766823 0.000399999669753015
0.155124053359032 9.99997646431439e-05
0.165262088179588 9.99997646431439e-05
0.174178779125214 0
0.18553814291954 0
0.19701974093914 0
0.205691933631897 0
0.214730605483055 0
0.227433800697327 0
0.237816229462624 0
0.246610417962074 0
0.257358372211456 0
0.267986297607422 0
0.278002828359604 0
0.289361417293549 0
0.298521757125854 0
0.310736775398254 0
0.322828948497772 0
0.334677428007126 0
0.343715518712997 0
0.355075150728226 0
0.365945637226105 0
0.375473201274872 0
0.385000258684158 0
0.393184036016464 0
0.402833521366119 0
0.41260552406311 0
0.423964768648148 0
0.433980762958527 0
0.445217996835709 0
0.456088930368423 0
0.465005546808243 0
0.474532753229141 0
0.483571529388428 0
0.493709772825241 0
0.503724455833435 0
0.513863563537598 0
0.52473396062851 0
0.535972476005554 0
0.546844124794006 0
0.556368768215179 0
0.567362666130066 0
0.575424075126648 0
0.586171507835388 0
0.596433222293854 0
0.606815993785858 0
0.618297398090363 0
0.629533767700195 0
0.639305114746094 0
0.651031672954559 0
0.661170601844788 0
0.672041058540344 0
0.682545185089111 0
0.693171799182892 0
0.703798830509186 0
0.714547216892242 0
0.724074423313141 0
0.733723819255829 0
0.743007302284241 0
0.752901494503021 0
0.762183964252472 0
0.773664951324463 0
0.782215595245361 0
0.792109131813049 0
0.802614331245422 0
0.812874436378479 0
0.823256611824036 0
0.832295417785645 0
0.841822445392609 0
0.852693796157837 0
0.862098455429077 0
0.871503531932831 0
0.878954410552979 0
0.887871146202087 0
0.897153794765472 0
0.905581951141357 0
0.913154780864716 0
0.923048913478851 0
0.931354582309723 0
0.939049959182739 0
0.945889830589294 0
0.952607810497284 0
0.960425078868866 0
0.970440924167633 0
0.976670324802399 0
0.984731912612915 0
0.992304861545563 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/RNN/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.136400356888771 0.204900056123734
0.183399796485901 0.0831001549959183
0.231900051236153 0.024499973282218
0.282000064849854 0.00639999471604824
0.330998867750168 0.000699998810887337
0.381700456142426 9.99997646431439e-05
0.433000236749649 9.99997646431439e-05
0.478299915790558 0
0.527198851108551 0
0.573799610137939 0
0.619101405143738 0
0.668598473072052 0
0.715200543403625 0
0.759199202060699 0
0.801299154758453 0
0.846300780773163 0
0.886799991130829 0
0.923999905586243 0
0.962000012397766 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.977309584617615 0.204900056123734
0.977309584617615 0.0831001549959183
0.980551064014435 0.024499973282218
0.982171773910522 0.00639999471604824
0.982171773910522 0.000699998810887337
0.983792543411255 9.99997646431439e-05
0.983792543411255 9.99997646431439e-05
0.987034022808075 0
0.987034022808075 0
0.988654792308807 0
0.988654792308807 0
0.99351704120636 0
0.99351704120636 0
0.99351704120636 0
0.995137751102448 0
0.995137751102448 0
0.99675852060318 0
0.99675852060318 0
0.998379230499268 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.373083502054214 0.204900056123734
0.413969308137894 0.0831001549959183
0.456558763980865 0.024499973282218
0.505962371826172 0.00639999471604824
0.555366098880768 0.000699998810887337
0.59284508228302 9.99997646431439e-05
0.623509645462036 9.99997646431439e-05
0.655877470970154 0
0.68313455581665 0
0.703577160835266 0
0.72913122177124 0
0.763202905654907 0
0.802384793758392 0
0.827938675880432 0
0.855195939540863 0
0.882453143596649 0
0.911413967609406 0
0.940374791622162 0
0.960817694664001 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0616188421845436 0.204900056123734
0.112323775887489 0.0831001549959183
0.164393082261086 0.024499973282218
0.217940077185631 0.00639999471604824
0.270350366830826 0.000699998810887337
0.325375378131866 9.99997646431439e-05
0.381650596857071 9.99997646431439e-05
0.430764138698578 0
0.484538435935974 0
0.536038160324097 0
0.585833013057709 0
0.639494717121124 0
0.689858376979828 0
0.738175928592682 0
0.784106254577637 0
0.833446741104126 0
0.877444267272949 0
0.917803287506104 0
0.95952707529068 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/RNN_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0924000218510628 0.304299712181091
0.103299915790558 0.286699235439301
0.114200003445148 0.267400205135345
0.124600060284138 0.240199968218803
0.134899884462357 0.207799851894379
0.14459952712059 0.177499994635582
0.155099898576736 0.151400119066238
0.165300354361534 0.129099994897842
0.174799993634224 0.112899996340275
0.18489982187748 0.098700039088726
0.194400042295456 0.0878000259399414
0.20479978621006 0.0799001306295395
0.21459998190403 0.0714999660849571
0.223699957132339 0.0634998381137848
0.232600003480911 0.0538000017404556
0.241700023412704 0.0462000109255314
0.252400189638138 0.0393000282347202
0.262300103902817 0.0328999646008015
0.270499676465988 0.0261999871581793
0.279900223016739 0.0207000225782394
0.290600597858429 0.0163000114262104
0.300699859857559 0.0136000011116266
0.310500174760818 0.0115000056102872
0.320000410079956 0.00959997903555632
0.328200489282608 0.0078999912366271
0.338100135326385 0.00690000131726265
0.346799820661545 0.0059999949298799
0.355999886989594 0.00519999070093036
0.365999519824982 0.0042999885044992
0.376700341701508 0.00390000641345978
0.386200696229935 0.00330000231042504
0.394900679588318 0.00279999896883965
0.40500009059906 0.00260000512935221
0.413600087165833 0.00210000015795231
0.4231998026371 0.0018000032287091
0.432500004768372 0.00139999762177467
0.440699994564056 0.000699999742209911
0.450599908828735 0.000599998980760574
0.459699988365173 0.000499999907333404
0.470700055360794 0.000499999907333404
0.480400085449219 0.000399999058572575
0.490500092506409 0.000299999490380287
0.49779999256134 0.000199999529286288
0.505600273609161 9.99997646431439e-05
0.515501081943512 0
0.524599194526672 0
0.533801138401031 0
0.542698681354523 0
0.553399682044983 0
0.563199996948242 0
0.57430100440979 0
0.583999812602997 0
0.59190160036087 0
0.600901186466217 0
0.608300685882568 0
0.618898808956146 0
0.62930154800415 0
0.638998866081238 0
0.649898767471313 0
0.659999370574951 0
0.669400691986084 0
0.679200172424316 0
0.68880021572113 0
0.698999524116516 0
0.709799408912659 0
0.719700813293457 0
0.728500366210938 0
0.738899648189545 0
0.747599482536316 0
0.757299959659576 0
0.764800488948822 0
0.773900270462036 0
0.78290057182312 0
0.793100714683533 0
0.799799680709839 0
0.809000313282013 0
0.817201018333435 0
0.828100085258484 0
0.837200224399567 0
0.845700562000275 0
0.854600012302399 0
0.864401340484619 0
0.87330037355423 0
0.881300210952759 0
0.888999998569489 0
0.896300792694092 0
0.904000222682953 0
0.910999774932861 0
0.91810017824173 0
0.926199972629547 0
0.934000313282013 0
0.941600024700165 0
0.948199987411499 0
0.955800116062164 0
0.963699817657471 0
0.972599983215332 0
0.977800011634827 0
0.98580002784729 0
0.9932000041008 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.886931002140045 0.304299712181091
0.886931002140045 0.286699235439301
0.889867842197418 0.267400205135345
0.891336381435394 0.240199968218803
0.891336381435394 0.207799851894379
0.892804622650146 0.177499994635582
0.894273042678833 0.151400119066238
0.895741581916809 0.129099994897842
0.89721018075943 0.112899996340275
0.89721018075943 0.098700039088726
0.900146842002869 0.0878000259399414
0.901615262031555 0.0799001306295395
0.901615262031555 0.0714999660849571
0.904552102088928 0.0634998381137848
0.907489001750946 0.0538000017404556
0.908957302570343 0.0462000109255314
0.911894261837006 0.0393000282347202
0.911894261837006 0.0328999646008015
0.911894261837006 0.0261999871581793
0.913362503051758 0.0207000225782394
0.91629958152771 0.0163000114262104
0.917768001556396 0.0136000011116266
0.919236421585083 0.0115000056102872
0.92070484161377 0.00959997903555632
0.92070484161377 0.0078999912366271
0.922173261642456 0.00690000131726265
0.923641622066498 0.0059999949298799
0.925110220909119 0.00519999070093036
0.925110220909119 0.0042999885044992
0.92657858133316 0.00390000641345978
0.928047001361847 0.00330000231042504
0.929515421390533 0.00279999896883965
0.929515421390533 0.00260000512935221
0.929515421390533 0.00210000015795231
0.929515421390533 0.0018000032287091
0.929515421390533 0.00139999762177467
0.929515421390533 0.000699999742209911
0.932452261447906 0.000599998980760574
0.933920681476593 0.000499999907333404
0.935389161109924 0.000499999907333404
0.938326001167297 0.000399999058572575
0.938326001167297 0.000299999490380287
0.938326001167297 0.000199999529286288
0.938326001167297 9.99997646431439e-05
0.938326001167297 0
0.939794301986694 0
0.94126284122467 0
0.94126284122467 0
0.94126284122467 0
0.94126284122467 0
0.94126284122467 0
0.945668160915375 0
0.945668160915375 0
0.948605000972748 0
0.948605000972748 0
0.950073421001434 0
0.950073421001434 0
0.951541841030121 0
0.951541841030121 0
0.951541841030121 0
0.951541841030121 0
0.951541841030121 0
0.951541841030121 0
0.953010261058807 0
0.954478681087494 0
0.954478681087494 0
0.954478681087494 0
0.960352420806885 0
0.963289260864258 0
0.964757680892944 0
0.964757680892944 0
0.967694580554962 0
0.967694580554962 0
0.969163000583649 0
0.972099840641022 0
0.976505160331726 0
0.976505160331726 0
0.977973580360413 0
0.979442000389099 0
0.979442000389099 0
0.980910420417786 0
0.983847260475159 0
0.98531574010849 0
0.986784160137177 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.98972100019455 0
0.992657840251923 0
0.994126260280609 0
0.994126260280609 0
0.994126260280609 0
0.994126260280609 0
0.99559473991394 0
0.998531579971313 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.171155527234077 0.304299712181091
0.185056522488594 0.286699235439301
0.195482239127159 0.267400205135345
0.205039083957672 0.240199968218803
0.216333642601967 0.207799851894379
0.222415313124657 0.177499994635582
0.231972202658653 0.151400119066238
0.247610822319984 0.129099994897842
0.255429893732071 0.112899996340275
0.267593443393707 0.098700039088726
0.278887957334518 0.0878000259399414
0.288444817066193 0.0799001306295395
0.296264201402664 0.0714999660849571
0.302345871925354 0.0634998381137848
0.309296369552612 0.0538000017404556
0.317984193563461 0.0462000109255314
0.329278916120529 0.0393000282347202
0.336229532957077 0.0328999646008015
0.344917297363281 0.0261999871581793
0.3536057472229 0.0207000225782394
0.366637587547302 0.0163000114262104
0.377931982278824 0.0136000011116266
0.390095621347427 0.0115000056102872
0.395308345556259 0.00959997903555632
0.402258962392807 0.0078999912366271
0.414422273635864 0.00690000131726265
0.423979252576828 0.0059999949298799
0.431798309087753 0.00519999070093036
0.434404879808426 0.0042999885044992
0.442224204540253 0.00390000641345978
0.450912237167358 0.00330000231042504
0.459600359201431 0.00279999896883965
0.471763670444489 0.00260000512935221
0.479583084583282 0.00210000015795231
0.488271057605743 0.0018000032287091
0.496090292930603 0.00139999762177467
0.505647480487823 0.000699999742209911
0.517810642719269 0.000599998980760574
0.525630116462708 0.000499999907333404
0.532580375671387 0.000499999907333404
0.540399730205536 0.000399999058572575
0.549956977367401 0.000299999490380287
0.551694631576538 0.000199999529286288
0.556038379669189 9.99997646431439e-05
0.565595269203186 0
0.573414981365204 0
0.578627586364746 0
0.593397200107574 0
0.600347578525543 0
0.60990434885025 0
0.618592500686646 0
0.626411974430084 0
0.631624698638916 0
0.636837720870972 0
0.647263169288635 0
0.657688856124878 0
0.666377365589142 0
0.672459006309509 0
0.68114697933197 0
0.684622466564178 0
0.694179058074951 0
0.700261056423187 0
0.706342220306396 0
0.715030610561371 0
0.724586963653564 0
0.736750841140747 0
0.746307373046875 0
0.753257930278778 0
0.761077344417572 0
0.770634472370148 0
0.777584493160248 0
0.784534692764282 0
0.78887927532196 0
0.800173759460449 0
0.807992994785309 0
0.817550241947174 0
0.824500501155853 0
0.834925830364227 0
0.840138792991638 0
0.847089529037476 0
0.854909002780914 0
0.86272805929184 0
0.869678437709808 0
0.876628935337067 0
0.885317027568817 0
0.890529990196228 0
0.900955557823181 0
0.907037556171417 0
0.914856672286987 0
0.918331861495972 0
0.929626405239105 0
0.93397045135498 0
0.940920948982239 0
0.953084290027618 0
0.963509976863861 0
0.970460474491119 0
0.976542115211487 0
0.985230207443237 0
0.990443110466003 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0150587493553758 0.304299712181091
0.026444673538208 0.286699235439301
0.0380754806101322 0.267400205135345
0.0493389032781124 0.240199968218803
0.0603575184941292 0.207799851894379
0.071253702044487 0.177499994635582
0.0826394930481911 0.151400119066238
0.0928012207150459 0.129099994897842
0.103207565844059 0.112899996340275
0.113858975470066 0.098700039088726
0.123653344810009 0.0878000259399414
0.134917199611664 0.0799001306295395
0.145812854170799 0.0714999660849571
0.155851811170578 0.0634998381137848
0.165524184703827 0.0538000017404556
0.175318270921707 0.0462000109255314
0.186581969261169 0.0393000282347202
0.197722911834717 0.0328999646008015
0.206537693738937 0.0261999871581793
0.216699287295341 0.0207000225782394
0.227717936038971 0.0163000114262104
0.238369300961494 0.0136000011116266
0.248530849814415 0.0115000056102872
0.259304970502853 0.00959997903555632
0.268363863229752 0.0078999912366271
0.278648436069489 0.00690000131726265
0.287830382585526 0.0059999949298799
0.297869324684143 0.00519999070093036
0.309745401144028 0.0042999885044992
0.321621060371399 0.00390000641345978
0.331904798746109 0.00330000231042504
0.341209888458252 0.00279999896883965
0.351860791444778 0.00260000512935221
0.361288189888 0.00210000015795231
0.371817022562027 0.0018000032287091
0.382100880146027 0.00139999762177467
0.390793174505234 0.000699999742209911
0.400954753160477 0.000599998980760574
0.410871714353561 0.000499999907333404
0.423236906528473 0.000499999907333404
0.433765977621078 0.000399999058572575
0.444784462451935 0.000299999490380287
0.453476995229721 0.000199999529286288
0.462414294481277 9.99997646431439e-05
0.473187983036041 0
0.483104646205902 0
0.493511080741882 0
0.502325654029846 0
0.514448046684265 0
0.525097966194153 0
0.53746509552002 0
0.54786890745163 0
0.556806683540344 0
0.566848278045654 0
0.574436843395233 0
0.58582329750061 0
0.597331166267395 0
0.608228206634521 0
0.62034797668457 0
0.632223188877106 0
0.642384707927704 0
0.653526246547699 0
0.664422988891602 0
0.675562798976898 0
0.687316477298737 0
0.697722792625427 0
0.707149267196655 0
0.718413293361664 0
0.727717816829681 0
0.738125324249268 0
0.746327579021454 0
0.756243646144867 0
0.766650557518005 0
0.777423858642578 0
0.784280002117157 0
0.793829798698425 0
0.802889108657837 0
0.814641952514648 0
0.824926435947418 0
0.83435332775116 0
0.844025492668152 0
0.854676902294159 0
0.864471137523651 0
0.873163282871246 0
0.881121575832367 0
0.889324069023132 0
0.897282183170319 0
0.904995024204254 0
0.91258579492569 0
0.922012984752655 0
0.929970622062683 0
0.938663125038147 0
0.945519089698792 0
0.952987253665924 0
0.961189866065979 0
0.971106767654419 0
0.976616084575653 0
0.985063672065735 0
0.993143975734711 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/RNN_/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.135699778795242 0.22139997780323
0.18489982187748 0.137000009417534
0.23150010406971 0.0781999602913857
0.281300485134125 0.0427999943494797
0.328499794006348 0.0238000117242336
0.376100122928619 0.0139000033959746
0.426800012588501 0.00669999094679952
0.474000006914139 0.00380000844597816
0.523999214172363 0.00180000078398734
0.571401000022888 0.000499999907333404
0.616899371147156 0.000199999529286288
0.666699707508087 0
0.711799442768097 0
0.756400108337402 0
0.802300810813904 0
0.848000764846802 0
0.887400269508362 0
0.924399614334106 0
0.962700009346008 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.977309584617615 0.22139997780323
0.977309584617615 0.137000009417534
0.980551064014435 0.0781999602913857
0.982171773910522 0.0427999943494797
0.982171773910522 0.0238000117242336
0.983792543411255 0.0139000033959746
0.983792543411255 0.00669999094679952
0.987034022808075 0.00380000844597816
0.987034022808075 0.00180000078398734
0.988654792308807 0.000499999907333404
0.988654792308807 0.000199999529286288
0.99351704120636 0
0.99351704120636 0
0.99351704120636 0
0.995137751102448 0
0.995137751102448 0
0.99675852060318 0
0.99675852060318 0
0.998379230499268 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.370118767023087 0.22139997780323
0.427843749523163 0.137000009417534
0.463497459888458 0.0781999602913857
0.516129076480865 0.0427999943494797
0.558574497699738 0.0238000117242336
0.595925271511078 0.0139000033959746
0.629881024360657 0.00669999094679952
0.662139177322388 0.00380000844597816
0.689303934574127 0.00180000078398734
0.709677338600159 0.000499999907333404
0.733446359634399 0.000199999529286288
0.767402589321136 0
0.801358103752136 0
0.825127243995667 0
0.852291941642761 0
0.88285219669342 0
0.908319175243378 0
0.938879430294037 0
0.957555174827576 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0609506480395794 0.22139997780323
0.113031648099422 0.137000009417534
0.163406729698181 0.0781999602913857
0.2163977175951 0.0427999943494797
0.267227798700333 0.0238000117242336
0.318740546703339 0.0139000033959746
0.37411841750145 0.00669999094679952
0.425403505563736 0.00380000844597816
0.48044142127037 0.00180000078398734
0.532864332199097 0.000499999907333404
0.583011150360107 0.000199999529286288
0.637024581432343 0
0.686036229133606 0
0.73516058921814 0
0.785421669483185 0
0.835342288017273 0
0.878325998783112 0
0.918353617191315 0
0.960541069507599 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/RNN_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.080999881029129 0.321199744939804
0.0949999541044235 0.321099817752838
0.107799924910069 0.320299685001373
0.118500009179115 0.31849992275238
0.130100294947624 0.310699731111526
0.140699818730354 0.29699969291687
0.152099534869194 0.272600084543228
0.162499755620956 0.238100007176399
0.172199860215187 0.192800030112267
0.181399509310722 0.147200375795364
0.190699994564056 0.103399954736233
0.201999932527542 0.0689998492598534
0.213000193238258 0.041399959474802
0.222699955105782 0.0239999890327454
0.232299953699112 0.0129000060260296
0.241000056266785 0.00469999620690942
0.250500619411469 0.0015000025741756
0.260899215936661 0.000999999814666808
0.269500821828842 0.000199999529286288
0.278699964284897 0.000199999529286288
0.289900362491608 0
0.300099819898605 0
0.308599859476089 0
0.318700134754181 0
0.32799968123436 0
0.33770015835762 0
0.347200065851212 0
0.357500344514847 0
0.366799741983414 0
0.377599865198135 0
0.38739949464798 0
0.396100044250488 0
0.406799912452698 0
0.41649979352951 0
0.425499945878983 0
0.434500008821487 0
0.443099915981293 0
0.453600138425827 0
0.46219989657402 0
0.473100006580353 0
0.482700109481812 0
0.491699695587158 0
0.498900979757309 0
0.507199287414551 0
0.516900658607483 0
0.525999963283539 0
0.534499704837799 0
0.543801724910736 0
0.553497731685638 0
0.563300371170044 0
0.573299586772919 0
0.582899272441864 0
0.591197192668915 0
0.601600170135498 0
0.60929936170578 0
0.619698703289032 0
0.629700481891632 0
0.639702200889587 0
0.650501012802124 0
0.660200476646423 0
0.668900907039642 0
0.679099917411804 0
0.68830007314682 0
0.698899149894714 0
0.708798706531525 0
0.718300461769104 0
0.72769969701767 0
0.737700641155243 0
0.746700465679169 0
0.757199823856354 0
0.765699446201324 0
0.774599552154541 0
0.783600509166718 0
0.794701337814331 0
0.802700281143188 0
0.811800122261047 0
0.82050096988678 0
0.829900026321411 0
0.83899998664856 0
0.847300589084625 0
0.855799794197083 0
0.865099191665649 0
0.873900473117828 0
0.881599605083466 0
0.888999402523041 0
0.89579963684082 0
0.904300391674042 0
0.911599636077881 0
0.918299973011017 0
0.926200211048126 0
0.933799982070923 0
0.941299974918365 0
0.947799980640411 0
0.955399930477142 0
0.962799608707428 0
0.971300005912781 0
0.977599799633026 0
0.984899997711182 0
0.99260002374649 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.883040964603424 0.321199744939804
0.88596498966217 0.321099817752838
0.890350937843323 0.320299685001373
0.891812860965729 0.31849992275238
0.891812860965729 0.310699731111526
0.893274784088135 0.29699969291687
0.896198987960815 0.272600084543228
0.897660791873932 0.238100007176399
0.899122834205627 0.192800030112267
0.899122834205627 0.147200375795364
0.902046799659729 0.103399954736233
0.90350878238678 0.0689998492598534
0.90350878238678 0.041399959474802
0.906432747840881 0.0239999890327454
0.909356653690338 0.0129000060260296
0.910818696022034 0.00469999620690942
0.913742661476135 0.0015000025741756
0.913742661476135 0.000999999814666808
0.913742661476135 0.000199999529286288
0.915204703807831 0.000199999529286288
0.918128669261932 0
0.919590651988983 0
0.921052634716034 0
0.921052634716034 0
0.921052634716034 0
0.922514617443085 0
0.923976540565491 0
0.925438702106476 0
0.925438702106476 0
0.926900565624237 0
0.928362548351288 0
0.929824590682983 0
0.929824590682983 0
0.929824590682983 0
0.929824590682983 0
0.929824590682983 0
0.929824590682983 0
0.932748556137085 0
0.934210538864136 0
0.935672521591187 0
0.938596487045288 0
0.938596487045288 0
0.938596487045288 0
0.938596487045288 0
0.938596487045288 0
0.940058410167694 0
0.94152045249939 0
0.94152045249939 0
0.94152045249939 0
0.94152045249939 0
0.94152045249939 0
0.945906460285187 0
0.945906460285187 0
0.948830425739288 0
0.948830425739288 0
0.950292408466339 0
0.950292408466339 0
0.95175439119339 0
0.95175439119339 0
0.95175439119339 0
0.95175439119339 0
0.95175439119339 0
0.95175439119339 0
0.953216373920441 0
0.954678356647491 0
0.954678356647491 0
0.954678356647491 0
0.960526287555695 0
0.963450312614441 0
0.964912295341492 0
0.964912295341492 0
0.967836260795593 0
0.967836260795593 0
0.969298243522644 0
0.972222208976746 0
0.976608216762543 0
0.976608216762543 0
0.978070199489594 0
0.979532182216644 0
0.979532182216644 0
0.980994164943695 0
0.983918130397797 0
0.985380113124847 0
0.986842095851898 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.989766061306 0
0.992690086364746 0
0.994152069091797 0
0.994152069091797 0
0.994152069091797 0
0.994152069091797 0
0.995614051818848 0
0.998538017272949 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0949868261814117 0.321199744939804
0.134564638137817 0.321099817752838
0.160070329904556 0.320299685001373
0.175021901726723 0.31849992275238
0.197889193892479 0.310699731111526
0.208443343639374 0.29699969291687
0.221635907888412 0.272600084543228
0.237467020750046 0.238100007176399
0.245382562279701 0.192800030112267
0.259454727172852 0.147200375795364
0.268249839544296 0.103399954736233
0.281442493200302 0.0689998492598534
0.288478583097458 0.041399959474802
0.292875975370407 0.0239999890327454
0.300791501998901 0.0129000060260296
0.309586644172668 0.00469999620690942
0.321020245552063 0.0015000025741756
0.330694854259491 0.000999999814666808
0.339489936828613 0.000199999529286288
0.35004398226738 0.000199999529286288
0.359718501567841 0
0.366754680871964 0
0.378188252449036 0
0.383465141057968 0
0.392260402441025 0
0.404573410749435 0
0.416007101535797 0
0.425681561231613 0
0.429199546575546 0
0.436235636472702 0
0.444151192903519 0
0.451187342405319 0
0.464379996061325 0
0.474934041500092 0
0.484608620405197 0
0.495162695646286 0
0.503958404064178 0
0.518029510974884 0
0.525066077709198 0
0.532101988792419 0
0.540017783641815 0
0.549692094326019 0
0.554090082645416 0
0.558487355709076 0
0.569920599460602 0
0.577836394309998 0
0.582234442234039 0
0.597185730934143 0
0.604221820831299 0
0.612137079238892 0
0.620932340621948 0
0.627968192100525 0
0.634124875068665 0
0.640281736850739 0
0.652594864368439 0
0.66314834356308 0
0.67018449306488 0
0.676341116428375 0
0.683377504348755 0
0.686895489692688 0
0.697449743747711 0
0.704485714435577 0
0.709762632846832 0
0.716798424720764 0
0.725593328475952 0
0.735268533229828 0
0.744942665100098 0
0.753737807273865 0
0.760774195194244 0
0.770448744297028 0
0.778363823890686 0
0.78540027141571 0
0.789797782897949 0
0.801230907440186 0
0.808267116546631 0
0.817941844463348 0
0.824098527431488 0
0.832893550395966 0
0.839049875736237 0
0.845206618309021 0
0.853122353553772 0
0.861037731170654 0
0.868953168392181 0
0.877748548984528 0
0.88654363155365 0
0.890940845012665 0
0.901495158672333 0
0.907651901245117 0
0.913808286190033 0
0.918205916881561 0
0.930518925189972 0
0.934916436672211 0
0.941073000431061 0
0.95162707567215 0
0.96394020318985 0
0.970976233482361 0
0.977132797241211 0
0.985927879810333 0
0.991204917430878 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0119819026440382 0.321199744939804
0.02335250005126 0.321099817752838
0.0350898317992687 0.320299685001373
0.0459713898599148 0.31849992275238
0.056975182145834 0.310699731111526
0.0683456659317017 0.29699969291687
0.0802053138613701 0.272600084543228
0.0905979350209236 0.238100007176399
0.101234942674637 0.192800030112267
0.110526978969574 0.147200375795364
0.120430499315262 0.103399954736233
0.132289826869965 0.0689998492598534
0.144760921597481 0.041399959474802
0.155764698982239 0.0239999890327454
0.166156873106956 0.0129000060260296
0.175449341535568 0.00469999620690942
0.185230553150177 0.0015000025741756
0.196601018309593 0.000999999814666808
0.205893114209175 0.000199999529286288
0.215552017092705 0.000199999529286288
0.227656185626984 0
0.239026844501495 0
0.24770824611187 0
0.259322822093964 0
0.269470155239105 0
0.279497176408768 0
0.289400279521942 0
0.300526201725006 0
0.311406791210175 0
0.323511630296707 0
0.334270864725113 0
0.343807369470596 0
0.355055272579193 0
0.365447849035263 0
0.375107228755951 0
0.384643793106079 0
0.39393562078476 0
0.404572576284409 0
0.41398686170578 0
0.426213353872299 0
0.436605870723724 0
0.446264833211899 0
0.45445653796196 0
0.46399313211441 0
0.474263370037079 0
0.484166771173477 0
0.493825644254684 0
0.503115952014923 0
0.513999044895172 0
0.52488124370575 0
0.535884618759155 0
0.546276330947876 0
0.555568873882294 0
0.567184031009674 0
0.574887752532959 0
0.586013436317444 0
0.597261250019073 0
0.608509480953217 0
0.620736241340637 0
0.632106363773346 0
0.641275584697723 0
0.652769029140472 0
0.663283586502075 0
0.675142884254456 0
0.685902774333954 0
0.696172893047333 0
0.706320405006409 0
0.71683543920517 0
0.726617455482483 0
0.737987756729126 0
0.747280061244965 0
0.756938755512238 0
0.767331182956696 0
0.7791907787323 0
0.787749230861664 0
0.797163069248199 0
0.806944251060486 0
0.817092299461365 0
0.827240407466888 0
0.836532711982727 0
0.845702171325684 0
0.855728447437286 0
0.865264356136322 0
0.873333811759949 0
0.880914628505707 0
0.888617217540741 0
0.897542536258698 0
0.905611932277679 0
0.912947773933411 0
0.921995460987091 0
0.929575622081757 0
0.938134133815765 0
0.944981038570404 0
0.952683568000793 0
0.960019469261169 0
0.969433784484863 0
0.976280689239502 0
0.983861088752747 0
0.992297351360321 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/RNN_target/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.129500418901443 0.279199331998825
0.179299861192703 0.1825001090765
0.227000042796135 0.0909998491406441
0.275199741125107 0.0330999530851841
0.323400527238846 0.00970000028610229
0.376300066709518 0.00280000315979123
0.428800046443939 0.000599998980760574
0.474800050258636 9.9999931990169e-05
0.522401452064514 9.9999931990169e-05
0.570299327373505 0
0.615901291370392 0
0.663900315761566 0
0.709698736667633 0
0.755800545215607 0
0.800900340080261 0
0.845500409603119 0
0.88640022277832 0
0.923600196838379 0
0.962800025939941 0
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.970967769622803 0.279199331998825
0.974193572998047 0.1825001090765
0.979032278060913 0.0909998491406441
0.980645179748535 0.0330999530851841
0.980645179748535 0.00970000028610229
0.982258081436157 0.00280000315979123
0.982258081436157 0.000599998980760574
0.985483884811401 9.9999931990169e-05
0.985483884811401 9.9999931990169e-05
0.987096786499023 0
0.987096786499023 0
0.99193549156189 0
0.993548393249512 0
0.993548393249512 0
0.995161294937134 0
0.995161294937134 0
0.996774196624756 0
0.996774196624756 0
0.998387098312378 0
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.304794520139694 0.279199331998825
0.409246623516083 0.1825001090765
0.445205479860306 0.0909998491406441
0.501712560653687 0.0330999530851841
0.549658000469208 0.00970000028610229
0.592465817928314 0.00280000315979123
0.625000238418579 0.000599998980760574
0.660958826541901 9.9999931990169e-05
0.686643898487091 9.9999931990169e-05
0.707191705703735 0
0.732876896858215 0
0.765410840511322 0
0.79965752363205 0
0.827054917812347 0
0.856164515018463 0
0.88184928894043 0
0.909246563911438 0
0.941780805587769 0
0.962328791618347 0
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0585493482649326 0.279199331998825
0.108003690838814 0.1825001090765
0.159504234790802 0.0909998491406441
0.210436701774597 0.0330999530851841
0.262051045894623 0.00970000028610229
0.319236546754837 0.00280000315979123
0.376762539148331 0.000599998980760574
0.426443934440613 9.9999931990169e-05
0.478854030370712 9.9999931990169e-05
0.531832933425903 0
0.581967711448669 0
0.634037554264069 0
0.683719456195831 0
0.734311759471893 0
0.783538341522217 0
0.832537770271301 0
0.877103090286255 0
0.917234718799591 0
0.960322856903076 0
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/Tweak/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0777998268604279 0.228100028634071
0.0907999724149704 0.20509998947382
0.103900022804737 0.186299981176853
0.114900052547455 0.169299980998039
0.12420017272234 0.152999988943338
0.13419982790947 0.138800005614758
0.144299745559692 0.126900035142899
0.154200106859207 0.112900002300739
0.163699805736542 0.102199999243021
0.172800049185753 0.0914000064134598
0.182099968194962 0.0791999898850918
0.191799804568291 0.0704999841749668
0.202000007033348 0.0626000113785267
0.212200090289116 0.0540000040084124
0.221100091934204 0.0451999984681606
0.22999994456768 0.0386000027880073
0.240200072526932 0.0315000034868717
0.250399887561798 0.0253000056371093
0.259200990200043 0.0194999970495701
0.268800288438797 0.01529999980703
0.280499905347824 0.0117999998852611
0.2892005443573 0.00949999801814556
0.298700392246246 0.00799999935552478
0.308299988508224 0.00629999912343919
0.317799955606461 0.00469999860506505
0.327599197626114 0.00329999912064523
0.336600065231323 0.00259999940171838
0.345900565385818 0.00169999952195212
0.355500787496567 0.000999999651685357
0.366600304841995 0.000899999716784805
0.376699805259705 0.000899999716784805
0.385099768638611 0.00049999967450276
0.395400255918503 0.00049999967450276
0.405299574136734 0.000299999804701656
0.413700103759766 0.000299999804701656
0.42399999499321 0.000199999869801104
0.433000355958939 0.000199999869801104
0.444300085306168 0.000199999869801104
0.452200204133987 0.000199999869801104
0.462500095367432 0.000199999869801104
0.472800046205521 9.9999934900552e-05
0.482699900865555 9.9999934900552e-05
0.491200000047684 0
0.498999714851379 0
0.509101092815399 0
0.51850038766861 0
0.527199685573578 0
0.537099599838257 0
0.546599686145782 0
0.557100713253021 0
0.568099081516266 0
0.578100442886353 0
0.586198627948761 0
0.595599412918091 0
0.603798389434814 0
0.613300204277039 0
0.623701214790344 0
0.633700609207153 0
0.643500983715057 0
0.652401149272919 0
0.6609006524086 0
0.6715008020401 0
0.680600702762604 0
0.690899968147278 0
0.700799524784088 0
0.71060049533844 0
0.719998598098755 0
0.730098485946655 0
0.738899648189545 0
0.748999834060669 0
0.75849974155426 0
0.767700850963593 0
0.777100205421448 0
0.787499785423279 0
0.794799566268921 0
0.804500997066498 0
0.815099954605103 0
0.826000213623047 0
0.835300028324127 0
0.843400001525879 0
0.853400111198425 0
0.86279970407486 0
0.871800184249878 0
0.879400193691254 0
0.887199997901917 0
0.895900785923004 0
0.904899775981903 0
0.91210001707077 0
0.919500410556793 0
0.928099930286407 0
0.934900283813477 0
0.942600309848785 0
0.949899971485138 0
0.957099795341492 0
0.964399993419647 0
0.973200023174286 0
0.978999972343445 0
0.986599981784821 0
0.992900013923645 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.849295794963837 0.228100028634071
0.856337666511536 0.20509998947382
0.866197168827057 0.186299981176853
0.874647974967957 0.169299980998039
0.876056432723999 0.152999988943338
0.877464771270752 0.138800005614758
0.881690144538879 0.126900035142899
0.884507119655609 0.112900002300739
0.887323915958405 0.102199999243021
0.887323915958405 0.0914000064134598
0.892957746982574 0.0791999898850918
0.894366383552551 0.0704999841749668
0.895774483680725 0.0626000113785267
0.898591578006744 0.0540000040084124
0.902816891670227 0.0451999984681606
0.904225289821625 0.0386000027880073
0.90704208612442 0.0315000034868717
0.90704208612442 0.0253000056371093
0.908450603485107 0.0194999970495701
0.909859180450439 0.01529999980703
0.915492951869965 0.0117999998852611
0.916901409626007 0.00949999801814556
0.91830986738205 0.00799999935552478
0.919718205928802 0.00629999912343919
0.919718205928802 0.00469999860506505
0.921126782894135 0.00329999912064523
0.922535300254822 0.00259999940171838
0.923943638801575 0.00169999952195212
0.925352096557617 0.000999999651685357
0.92676055431366 0.000899999716784805
0.928169012069702 0.000899999716784805
0.929577469825745 0.00049999967450276
0.930985927581787 0.00049999967450276
0.930985927581787 0.000299999804701656
0.930985927581787 0.000299999804701656
0.930985927581787 0.000199999869801104
0.930985927581787 0.000199999869801104
0.933802843093872 0.000199999869801104
0.93521124124527 0.000199999869801104
0.936619699001312 0.000199999869801104
0.939436614513397 9.9999934900552e-05
0.939436614513397 9.9999934900552e-05
0.939436614513397 0
0.939436614513397 0
0.939436614513397 0
0.94084507226944 0
0.942253530025482 0
0.943661987781525 0
0.943661987781525 0
0.943661987781525 0
0.943661987781525 0
0.947887301445007 0
0.947887301445007 0
0.950704216957092 0
0.950704216957092 0
0.952112674713135 0
0.952112674713135 0
0.953521132469177 0
0.953521132469177 0
0.953521132469177 0
0.953521132469177 0
0.953521132469177 0
0.953521132469177 0
0.95492959022522 0
0.956338047981262 0
0.956338047981262 0
0.956338047981262 0
0.961971819400787 0
0.964788734912872 0
0.966197192668915 0
0.966197192668915 0
0.969014108181 0
0.969014108181 0
0.970422506332397 0
0.973239421844482 0
0.97746479511261 0
0.97746479511261 0
0.978873252868652 0
0.980281710624695 0
0.980281710624695 0
0.981690168380737 0
0.984507024288177 0
0.98591548204422 0
0.987323939800262 0
0.990140855312347 0
0.990140855312347 0
0.990140855312347 0
0.990140855312347 0
0.990140855312347 0
0.990140855312347 0
0.990140855312347 0
0.990140855312347 0
0.992957770824432 0
0.99436616897583 0
0.99436616897583 0
0.99436616897583 0
0.99436616897583 0
0.995774626731873 0
0.998591542243958 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0766320526599884 0.228100028634071
0.10217597335577 0.20509998947382
0.12298958003521 0.186299981176853
0.139072969555855 0.169299980998039
0.157048255205154 0.152999988943338
0.166509032249451 0.138800005614758
0.178808033466339 0.126900035142899
0.197729423642159 0.112900002300739
0.205297991633415 0.102199999243021
0.219489112496376 0.0914000064134598
0.230842009186745 0.0791999898850918
0.240302726626396 0.0704999841749668
0.247871339321136 0.0626000113785267
0.255439907312393 0.0540000040084124
0.262062579393387 0.0451999984681606
0.269631147384644 0.0386000027880073
0.280037701129913 0.0315000034868717
0.290444701910019 0.0253000056371093
0.298013150691986 0.0194999970495701
0.305581748485565 0.01529999980703
0.316934913396835 0.0117999998852611
0.323557138442993 0.00949999801814556
0.335856318473816 0.00799999935552478
0.343424737453461 0.00629999912343919
0.350993186235428 0.00469999860506505
0.364238351583481 0.00329999912064523
0.374645084142685 0.00259999940171838
0.385998100042343 0.00169999952195212
0.389782190322876 0.000999999651685357
0.398297071456909 0.000899999716784805
0.405865639448166 0.000899999716784805
0.416272550821304 0.00049999967450276
0.428571462631226 0.00049999967450276
0.438032180070877 0.000299999804701656
0.447492867708206 0.000299999804701656
0.456007599830627 0.000199999869801104
0.467360466718674 0.000199999869801104
0.480605512857437 0.000199999869801104
0.488174080848694 0.000199999869801104
0.494796723127365 0.000199999869801104
0.506149530410767 9.9999934900552e-05
0.519394814968109 9.9999934900552e-05
0.522233009338379 0
0.526017248630524 0
0.537370264530182 0
0.546830654144287 0
0.551560342311859 0
0.568590641021729 0
0.575213134288788 0
0.586565852165222 0
0.596026837825775 0
0.602649092674255 0
0.609271287918091 0
0.616840243339539 0
0.630085229873657 0
0.640491664409637 0
0.648060202598572 0
0.655629396438599 0
0.665089786052704 0
0.668874263763428 0
0.679281115531921 0
0.686849355697632 0
0.692525863647461 0
0.701986610889435 0
0.712393522262573 0
0.722800195217133 0
0.733207225799561 0
0.741721928119659 0
0.749290466308594 0
0.759697496891022 0
0.768212020397186 0
0.774834334850311 0
0.780510902404785 0
0.792809903621674 0
0.801324725151062 0
0.811731219291687 0
0.818353950977325 0
0.82781457901001 0
0.833491027355194 0
0.841059505939484 0
0.847681999206543 0
0.856196820735931 0
0.863765299320221 0
0.87133401632309 0
0.880794823169708 0
0.885524868965149 0
0.896877944469452 0
0.903500497341156 0
0.910122811794281 0
0.91390722990036 0
0.926206231117249 0
0.930936694145203 0
0.937559127807617 0
0.949858069419861 0
0.962157130241394 0
0.969725608825684 0
0.976348161697388 0
0.984862804412842 0
0.990539252758026 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.011417462490499 0.228100028634071
0.023320771753788 0.20509998947382
0.0357098579406738 0.186299981176853
0.0462772287428379 0.169299980998039
0.0551439374685287 0.152999988943338
0.0659540146589279 0.138800005614758
0.076278381049633 0.126900035142899
0.0856310278177261 0.112900002300739
0.0959554463624954 0.102199999243021
0.105186492204666 0.0914000064134598
0.114539064466953 0.0791999898850918
0.124984815716743 0.0704999841749668
0.136280998587608 0.0626000113785267
0.147455170750618 0.0540000040084124
0.157050892710686 0.0451999984681606
0.166767820715904 0.0386000027880073
0.177577987313271 0.0315000034868717
0.188631266355515 0.0253000056371093
0.198226675391197 0.0194999970495701
0.208793938159943 0.01529999980703
0.221061632037163 0.0117999998852611
0.230657085776329 0.00949999801814556
0.240495771169662 0.00799999935552478
0.251062452793121 0.00629999912343919
0.261630356311798 0.00469999860506505
0.271710634231567 0.00329999912064523
0.281185299158096 0.00259999940171838
0.290901869535446 0.00169999952195212
0.301956295967102 0.000999999651685357
0.31422221660614 0.000899999716784805
0.325397551059723 0.000899999716784805
0.334143131971359 0.00049999967450276
0.344953179359436 0.00049999967450276
0.355763405561447 0.000299999804701656
0.364751666784286 0.000299999804701656
0.376169413328171 0.000199999869801104
0.385643035173416 0.000199999869801104
0.39742511510849 0.000199999869801104
0.40592747926712 0.000199999869801104
0.417466163635254 0.000199999869801104
0.42827633023262 9.9999934900552e-05
0.438600808382034 9.9999934900552e-05
0.448560684919357 0
0.457548946142197 0
0.468359053134918 0
0.478440314531326 0
0.488279283046722 0
0.497995764017105 0
0.50868433713913 0
0.51997983455658 0
0.532126426696777 0
0.543057382106781 0
0.552046895027161 0
0.562247574329376 0
0.570508301258087 0
0.580590069293976 0
0.592250943183899 0
0.603303790092468 0
0.61399257183075 0
0.624317109584808 0
0.63330489397049 0
0.645208358764648 0
0.655533194541931 0
0.666707515716553 0
0.677273452281952 0
0.687841773033142 0
0.697922766208649 0
0.70861154794693 0
0.718086361885071 0
0.728895545005798 0
0.739342629909515 0
0.749422371387482 0
0.760112106800079 0
0.771043479442596 0
0.778574645519257 0
0.788654923439026 0
0.800679624080658 0
0.812583744525909 0
0.823029398918152 0
0.83189582824707 0
0.843070328235626 0
0.85315215587616 0
0.862990498542786 0
0.871128499507904 0
0.87914502620697 0
0.889104902744293 0
0.898578763008118 0
0.906473815441132 0
0.91461169719696 0
0.924571871757507 0
0.931252300739288 0
0.939997613430023 0
0.947771310806274 0
0.954815983772278 0
0.962103724479675 0
0.971820712089539 0
0.978015244007111 0
0.986031830310822 0
0.992712259292603 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/chaffing3/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0851998254656792 0.264400839805603
0.099899984896183 0.218400090932846
0.112500049173832 0.194799914956093
0.123799912631512 0.182499974966049
0.134600207209587 0.174600303173065
0.144799873232841 0.169200092554092
0.15469978749752 0.165500178933144
0.164800092577934 0.163700118660927
0.173900187015533 0.162799805402756
0.181899696588516 0.162100180983543
0.191000029444695 0.161600053310394
0.201299861073494 0.160799741744995
0.212200000882149 0.159700065851212
0.222599998116493 0.157600298523903
0.231000050902367 0.155799999833107
0.240700095891953 0.152199819684029
0.25030106306076 0.148399889469147
0.260300010442734 0.144799843430519
0.268599659204483 0.139300286769867
0.276600122451782 0.134499579668045
0.287599325180054 0.130000188946724
0.296900033950806 0.12479991465807
0.307000398635864 0.122099936008453
0.316199600696564 0.117600001394749
0.325299382209778 0.114699929952621
0.334999799728394 0.113099902868271
0.343899965286255 0.112100012600422
0.352799624204636 0.111400038003922
0.362000674009323 0.111200034618378
0.372599512338638 0.111100070178509
0.382299661636353 0.110800035297871
0.391300648450851 0.110200002789497
0.400299966335297 0.10989997535944
0.409300208091736 0.109499923884869
0.418400138616562 0.109399951994419
0.4280004799366 0.109399951994419
0.435700207948685 0.109200082719326
0.444899797439575 0.108999900519848
0.453999936580658 0.108899898827076
0.463799893856049 0.10869986563921
0.472899913787842 0.108599998056889
0.481799989938736 0.108500048518181
0.490299999713898 0.108500048518181
0.498300105333328 0.108400046825409
0.507600963115692 0.108400046825409
0.517099916934967 0.108400046825409
0.526400804519653 0.108400046825409
0.535501182079315 0.108400046825409
0.546300172805786 0.108400046825409
0.55620002746582 0.108400046825409
0.566700577735901 0.108400046825409
0.576499044895172 0.108400046825409
0.584999978542328 0.108400046825409
0.593998908996582 0.108400046825409
0.602701246738434 0.108400046825409
0.613600611686707 0.108400046825409
0.623700082302094 0.108400046825409
0.633800268173218 0.108400046825409
0.642998337745667 0.108400046825409
0.652500033378601 0.108400046825409
0.661600470542908 0.108400046825409
0.67119961977005 0.108400046825409
0.680099368095398 0.108400046825409
0.689900755882263 0.108400046825409
0.700600743293762 0.108400046825409
0.710299015045166 0.108400046825409
0.720000684261322 0.108400046825409
0.7289999127388 0.108400046825409
0.738200902938843 0.108400046825409
0.747999727725983 0.108400046825409
0.756098806858063 0.108400046825409
0.764601051807404 0.108400046825409
0.773400366306305 0.108400046825409
0.784599602222443 0.108400046825409
0.79200154542923 0.108400046825409
0.801899969577789 0.108400046825409
0.811499416828156 0.108400046825409
0.821800410747528 0.108400046825409
0.830599129199982 0.108400046825409
0.838399887084961 0.108400046825409
0.84759920835495 0.108400046825409
0.857499122619629 0.108400046825409
0.866299986839294 0.108400046825409
0.874299585819244 0.108400046825409
0.881999433040619 0.108400046825409
0.889799892902374 0.108400046825409
0.898800492286682 0.108400046825409
0.906299829483032 0.108400046825409
0.91349983215332 0.108400046825409
0.921399712562561 0.108400046825409
0.929399311542511 0.108400046825409
0.936500370502472 0.108400046825409
0.945000171661377 0.108400046825409
0.952799677848816 0.108400046825409
0.960799992084503 0.108400046825409
0.97079998254776 0.108400046825409
0.977199971675873 0.108400046825409
0.984200000762939 0.108400046825409
0.99260002374649 0.108400046825409
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.886931002140045 0.264400839805603
0.886931002140045 0.218400090932846
0.889867842197418 0.194799914956093
0.892804861068726 0.182499974966049
0.892804861068726 0.174600303173065
0.894273102283478 0.169200092554092
0.895741581916809 0.165500178933144
0.89721018075943 0.163700118660927
0.898678421974182 0.162799805402756
0.898678421974182 0.162100180983543
0.901615262031555 0.161600053310394
0.903083682060242 0.160799741744995
0.903083682060242 0.159700065851212
0.90602058172226 0.157600298523903
0.908957600593567 0.155799999833107
0.910425841808319 0.152199819684029
0.913362681865692 0.148399889469147
0.913362681865692 0.144799843430519
0.913362681865692 0.139300286769867
0.914831101894379 0.134499579668045
0.917768001556396 0.130000188946724
0.919236421585083 0.12479991465807
0.92070484161377 0.122099936008453
0.92070484161377 0.117600001394749
0.92070484161377 0.114699929952621
0.922173261642456 0.113099902868271
0.923641622066498 0.112100012600422
0.925110220909119 0.111400038003922
0.925110220909119 0.111200034618378
0.92657858133316 0.111100070178509
0.928047001361847 0.110800035297871
0.929515421390533 0.110200002789497
0.929515421390533 0.10989997535944
0.929515421390533 0.109499923884869
0.929515421390533 0.109399951994419
0.929515421390533 0.109399951994419
0.929515421390533 0.109200082719326
0.932452261447906 0.108999900519848
0.933920681476593 0.108899898827076
0.935389161109924 0.10869986563921
0.938326001167297 0.108599998056889
0.938326001167297 0.108500048518181
0.938326001167297 0.108500048518181
0.938326001167297 0.108400046825409
0.938326001167297 0.108400046825409
0.939794301986694 0.108400046825409
0.94126284122467 0.108400046825409
0.94126284122467 0.108400046825409
0.94126284122467 0.108400046825409
0.94126284122467 0.108400046825409
0.94126284122467 0.108400046825409
0.945668160915375 0.108400046825409
0.945668160915375 0.108400046825409
0.948605000972748 0.108400046825409
0.948605000972748 0.108400046825409
0.950073421001434 0.108400046825409
0.950073421001434 0.108400046825409
0.951541841030121 0.108400046825409
0.951541841030121 0.108400046825409
0.951541841030121 0.108400046825409
0.951541841030121 0.108400046825409
0.951541841030121 0.108400046825409
0.951541841030121 0.108400046825409
0.953010261058807 0.108400046825409
0.954478681087494 0.108400046825409
0.954478681087494 0.108400046825409
0.954478681087494 0.108400046825409
0.960352420806885 0.108400046825409
0.963289260864258 0.108400046825409
0.964757680892944 0.108400046825409
0.964757680892944 0.108400046825409
0.967694580554962 0.108400046825409
0.967694580554962 0.108400046825409
0.969163000583649 0.108400046825409
0.972099840641022 0.108400046825409
0.976505160331726 0.108400046825409
0.976505160331726 0.108400046825409
0.977973580360413 0.108400046825409
0.979442000389099 0.108400046825409
0.979442000389099 0.108400046825409
0.980910420417786 0.108400046825409
0.983847260475159 0.108400046825409
0.98531574010849 0.108400046825409
0.986784160137177 0.108400046825409
0.98972100019455 0.108400046825409
0.98972100019455 0.108400046825409
0.98972100019455 0.108400046825409
0.98972100019455 0.108400046825409
0.98972100019455 0.108400046825409
0.98972100019455 0.108400046825409
0.98972100019455 0.108400046825409
0.98972100019455 0.108400046825409
0.992657840251923 0.108400046825409
0.994126260280609 0.108400046825409
0.994126260280609 0.108400046825409
0.994126260280609 0.108400046825409
0.994126260280609 0.108400046825409
0.99559473991394 0.108400046825409
0.998531579971313 0.108400046825409
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.112888015806675 0.264400839805603
0.142991587519646 0.218400090932846
0.164628386497498 0.194799914956093
0.175917208194733 0.182499974966049
0.190028235316277 0.174600303173065
0.200376257300377 0.169200092554092
0.208842903375626 0.165500178933144
0.226716816425323 0.163700118660927
0.23424269258976 0.162799805402756
0.247413158416748 0.162100180983543
0.256820350885391 0.161600053310394
0.266227900981903 0.160799741744995
0.273753374814987 0.159700065851212
0.28127920627594 0.157600298523903
0.287864416837692 0.155799999833107
0.296330988407135 0.152199819684029
0.306679308414459 0.148399889469147
0.313264191150665 0.144799843430519
0.321730852127075 0.139300286769867
0.329256922006607 0.134499579668045
0.338664293289185 0.130000188946724
0.344308346509933 0.12479991465807
0.356537908315659 0.122099936008453
0.363123297691345 0.117600001394749
0.371589720249176 0.114699929952621
0.383819371461868 0.113099902868271
0.394167393445969 0.112100012600422
0.402634054422379 0.111400038003922
0.406396985054016 0.111200034618378
0.414863556623459 0.111100070178509
0.423330128192902 0.110800035297871
0.432737469673157 0.110200002789497
0.444026380777359 0.10989997535944
0.453433722257614 0.109499923884869
0.464722484350204 0.109399951994419
0.473189145326614 0.109399951994419
0.482596427202225 0.109200082719326
0.495766639709473 0.108999900519848
0.504233717918396 0.108899898827076
0.510818541049957 0.10869986563921
0.518344581127167 0.108599998056889
0.527751743793488 0.108500048518181
0.530573785305023 0.108500048518181
0.534336686134338 0.108400046825409
0.545625329017639 0.108400046825409
0.553151428699493 0.108400046825409
0.55785459280014 0.108400046825409
0.574788331985474 0.108400046825409
0.581373870372772 0.108400046825409
0.589840292930603 0.108400046825409
0.600188434123993 0.108400046825409
0.606773495674133 0.108400046825409
0.615239679813385 0.108400046825409
0.621825158596039 0.108400046825409
0.633114278316498 0.108400046825409
0.643462300300598 0.108400046825409
0.651928544044495 0.108400046825409
0.659454166889191 0.108400046825409
0.666979789733887 0.108400046825409
0.670742869377136 0.108400046825409
0.682972848415375 0.108400046825409
0.689557552337646 0.108400046825409
0.694261431694031 0.108400046825409
0.701787531375885 0.108400046825409
0.712135672569275 0.108400046825409
0.722483575344086 0.108400046825409
0.733772039413452 0.108400046825409
0.741298317909241 0.108400046825409
0.748823881149292 0.108400046825409
0.758231282234192 0.108400046825409
0.765757203102112 0.108400046825409
0.772342562675476 0.108400046825409
0.777046144008636 0.108400046825409
0.790216207504272 0.108400046825409
0.797742366790771 0.108400046825409
0.808090388774872 0.108400046825409
0.814675390720367 0.108400046825409
0.824082851409912 0.108400046825409
0.829726994037628 0.108400046825409
0.835371434688568 0.108400046825409
0.841956615447998 0.108400046825409
0.850423336029053 0.108400046825409
0.857949376106262 0.108400046825409
0.865475058555603 0.108400046825409
0.875823259353638 0.108400046825409
0.881467461585999 0.108400046825409
0.892756164073944 0.108400046825409
0.899341464042664 0.108400046825409
0.906867384910583 0.108400046825409
0.910630345344543 0.108400046825409
0.921919167041779 0.108400046825409
0.927563488483429 0.108400046825409
0.934148669242859 0.108400046825409
0.946378171443939 0.108400046825409
0.958607733249664 0.108400046825409
0.966133594512939 0.108400046825409
0.973659455776215 0.108400046825409
0.98212605714798 0.108400046825409
0.987770438194275 0.108400046825409
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0155038889497519 0.264400839805603
0.0294331442564726 0.218400090932846
0.0416666716337204 0.194799914956093
0.0536579452455044 0.182499974966049
0.0649226754903793 0.174600303173065
0.0758237466216087 0.169200092554092
0.0866036638617516 0.165500178933144
0.096414789557457 0.163700118660927
0.10634683817625 0.162799805402756
0.114341095089912 0.162100180983543
0.123910002410412 0.161600053310394
0.13505320250988 0.160799741744995
0.147286951541901 0.159700065851212
0.158672466874123 0.157600298523903
0.167756751179695 0.155799999833107
0.178294643759727 0.152199819684029
0.188347846269608 0.148399889469147
0.199612438678741 0.144799843430519
0.208575546741486 0.139300286769867
0.217175424098969 0.134499579668045
0.229045554995537 0.130000188946724
0.239462062716484 0.12479991465807
0.250000357627869 0.122099936008453
0.260295063257217 0.117600001394749
0.270227938890457 0.114699929952621
0.280280232429504 0.113099902868271
0.289606600999832 0.112100012600422
0.299176752567291 0.111400038003922
0.309834271669388 0.111200034618378
0.321462661027908 0.111100070178509
0.33200079202652 0.110800035297871
0.341570198535919 0.110200002789497
0.351017564535141 0.10989997535944
0.360707193613052 0.109499923884869
0.370275795459747 0.109399951994419
0.380814135074615 0.109399951994419
0.388929039239883 0.109200082719326
0.398134827613831 0.108999900519848
0.407945692539215 0.108899898827076
0.418846845626831 0.10869986563921
0.428658068180084 0.108599998056889
0.438226819038391 0.108500048518181
0.448158860206604 0.108500048518181
0.457364290952682 0.108400046825409
0.467175394296646 0.108400046825409
0.477592021226883 0.108400046825409
0.488129794597626 0.108400046825409
0.496971666812897 0.108400046825409
0.509203910827637 0.108400046825409
0.520105481147766 0.108400046825409
0.531491339206696 0.108400046825409
0.542151749134064 0.108400046825409
0.551356375217438 0.108400046825409
0.561168670654297 0.108400046825409
0.57025134563446 0.108400046825409
0.582000255584717 0.108400046825409
0.593144357204437 0.108400046825409
0.604288041591644 0.108400046825409
0.614461839199066 0.108400046825409
0.625484824180603 0.108400046825409
0.634930729866028 0.108400046825409
0.645712196826935 0.108400046825409
0.655886113643646 0.108400046825409
0.666666448116302 0.108400046825409
0.678173959255219 0.108400046825409
0.688590943813324 0.108400046825409
0.698884963989258 0.108400046825409
0.708333671092987 0.108400046825409
0.718266069889069 0.108400046825409
0.728803157806396 0.108400046825409
0.737646102905273 0.108400046825409
0.746851086616516 0.108400046825409
0.756903767585754 0.108400046825409
0.768652439117432 0.108400046825409
0.776404976844788 0.108400046825409
0.786700248718262 0.108400046825409
0.797479927539825 0.108400046825409
0.808624148368835 0.108400046825409
0.818435430526733 0.108400046825409
0.827155947685242 0.108400046825409
0.83733069896698 0.108400046825409
0.84798938035965 0.108400046825409
0.857557773590088 0.108400046825409
0.86615777015686 0.108400046825409
0.873910009860992 0.108400046825409
0.882630705833435 0.108400046825409
0.892078638076782 0.108400046825409
0.900314927101135 0.108400046825409
0.908067107200623 0.108400046825409
0.917151510715485 0.108400046825409
0.925387680530548 0.108400046825409
0.933260679244995 0.108400046825409
0.942466199398041 0.108400046825409
0.950218021869659 0.108400046825409
0.958333373069763 0.108400046825409
0.969476759433746 0.108400046825409
0.976259708404541 0.108400046825409
0.98352712392807 0.108400046825409
0.992732584476471 0.108400046825409
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/chaffing3/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
        
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
    \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
    table {%
0.132399901747704 0.19770011305809
0.180300086736679 0.163900017738342
0.228699952363968 0.149400055408478
0.277700185775757 0.134300127625465
0.325600057840347 0.12289997190237
0.375000476837158 0.11619994789362
0.426899939775467 0.111700020730495
0.471800059080124 0.109500050544739
0.5197993516922 0.108699984848499
0.565398514270782 0.108499996364117
0.611200153827667 0.108499996364117
0.660800516605377 0.108400046825409
0.705498456954956 0.108400046825409
0.750199973583221 0.108400046825409
0.797300934791565 0.108400046825409
0.842699825763702 0.108400046825409
0.885299026966095 0.108400046825409
0.922300100326538 0.108400046825409
0.962000012397766 0.108400046825409
};
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.977309584617615 0.19770011305809
0.977309584617615 0.163900017738342
0.980551064014435 0.149400055408478
0.982171773910522 0.134300127625465
0.982171773910522 0.12289997190237
0.983792543411255 0.11619994789362
0.983792543411255 0.111700020730495
0.987034022808075 0.109500050544739
0.987034022808075 0.108699984848499
0.988654792308807 0.108499996364117
0.988654792308807 0.108499996364117
0.99351704120636 0.108400046825409
0.99351704120636 0.108400046825409
0.99351704120636 0.108400046825409
0.995137751102448 0.108400046825409
0.995137751102448 0.108400046825409
0.99675852060318 0.108400046825409
0.99675852060318 0.108400046825409
0.998379230499268 0.108400046825409
};
\addplot [line width=3, mediumseagreen85168104, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.315696686506271 0.19770011305809
0.382716149091721 0.163900017738342
0.419753134250641 0.149400055408478
0.47089958190918 0.134300127625465
0.518518924713135 0.12289997190237
0.559082865715027 0.11619994789362
0.597883403301239 0.111700020730495
0.631393313407898 0.109500050544739
0.661375641822815 0.108699984848499
0.682539761066437 0.108499996364117
0.712522029876709 0.108499996364117
0.746031939983368 0.108400046825409
0.783068656921387 0.108400046825409
0.809523820877075 0.108400046825409
0.839506149291992 0.108400046825409
0.865961313247681 0.108400046825409
0.897707343101501 0.108400046825409
0.931216955184937 0.108400046825409
0.955908298492432 0.108400046825409
};
\addplot [line width=3, indianred1967882, dotted, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0614791549742222 0.19770011305809
0.111501790583134 0.163900017738342
0.163793087005615 0.149400055408478
0.215970933437347 0.134300127625465
0.267241895198822 0.12289997190237
0.320554405450821 0.11619994789362
0.376928567886353 0.111700020730495
0.425476521253586 0.109500050544739
0.477994441986084 0.108699984848499
0.528243958950043 0.108499996364117
0.578267753124237 0.108499996364117
0.632031619548798 0.108400046825409
0.68035477399826 0.108400046825409
0.729356229305267 0.108400046825409
0.780740678310394 0.108400046825409
0.830535113811493 0.108400046825409
0.876701474189758 0.108400046825409
0.916515409946442 0.108400046825409
0.959845721721649 0.108400046825409
};

\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/chaffing4/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0905000194907188 0.134699866175652
0.104099996387959 0.110100023448467
0.115699999034405 0.100000075995922
0.126100197434425 0.0941999182105064
0.136500179767609 0.0898000001907349
0.145300015807152 0.0856999158859253
0.153400078415871 0.0794000253081322
0.164899870753288 0.0706997886300087
0.173600271344185 0.0615000054240227
0.18319995701313 0.0497000180184841
0.193400084972382 0.0385999344289303
0.20389997959137 0.0254999846220016
0.214199900627136 0.0173000022768974
0.223499909043312 0.0109000224620104
0.232999995350838 0.00629999861121178
0.241699859499931 0.0037999942433089
0.251600712537766 0.00230000261217356
0.261799931526184 0.000799998117145151
0.269699156284332 0.000499999907333404
0.280099481344223 0.000399999058572575
0.290000736713409 9.99997646431439e-05
0.299099087715149 0
0.308900326490402 0
0.317300409078598 0
0.32580092549324 0
0.335600018501282 0
0.345100075006485 0
0.353899836540222 0
0.363500148057938 0
0.373800307512283 0
0.383700162172318 0
0.391199499368668 0
0.400700211524963 0
0.410699665546417 0
0.419500201940536 0
0.428699404001236 0
0.436700195074081 0
0.447000205516815 0
0.455299705266953 0
0.466200202703476 0
0.476099997758865 0
0.484899997711182 0
0.49250003695488 0
0.500499665737152 0
0.509101629257202 0
0.519000709056854 0
0.527800142765045 0
0.536700010299683 0
0.547001600265503 0
0.557299852371216 0
0.566701412200928 0
0.576101243495941 0
0.584599554538727 0
0.593599319458008 0
0.60229903459549 0
0.611999332904816 0
0.621700167655945 0
0.631499767303467 0
0.641199886798859 0
0.650399267673492 0
0.660000562667847 0
0.670201182365417 0
0.679999828338623 0
0.690000593662262 0
0.700301706790924 0
0.710501194000244 0
0.719800174236298 0
0.729700267314911 0
0.739500463008881 0
0.748898804187775 0
0.757799744606018 0
0.766399800777435 0
0.774899780750275 0
0.78529953956604 0
0.793399155139923 0
0.803799092769623 0
0.813898324966431 0
0.823399603366852 0
0.832400023937225 0
0.840799629688263 0
0.850199997425079 0
0.860000014305115 0
0.868300557136536 0
0.876300275325775 0
0.883499979972839 0
0.891200184822083 0
0.90060019493103 0
0.90839958190918 0
0.916200220584869 0
0.924200415611267 0
0.931500196456909 0
0.938899993896484 0
0.945700168609619 0
0.953199982643127 0
0.960799813270569 0
0.970699906349182 0
0.976999998092651 0
0.984799981117249 0
0.991699993610382 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.88823527097702 0.134699866175652
0.88823527097702 0.110100023448467
0.891176581382751 0.100000075995922
0.892647266387939 0.0941999182105064
0.892647266387939 0.0898000001907349
0.894117712974548 0.0856999158859253
0.895588338375092 0.0794000253081322
0.897058844566345 0.0706997886300087
0.898529410362244 0.0615000054240227
0.898529410362244 0.0497000180184841
0.901470601558685 0.0385999344289303
0.902941167354584 0.0254999846220016
0.902941167354584 0.0173000022768974
0.905882358551025 0.0109000224620104
0.908823728561401 0.00629999861121178
0.910294115543365 0.0037999942433089
0.913235306739807 0.00230000261217356
0.913235306739807 0.000799998117145151
0.913235306739807 0.000499999907333404
0.914705872535706 0.000399999058572575
0.917647063732147 9.99997646431439e-05
0.919117629528046 0
0.920588254928589 0
0.920588254928589 0
0.920588254928589 0
0.922058820724487 0
0.923529326915741 0
0.925000071525574 0
0.925000071525574 0
0.926470577716827 0
0.927941203117371 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.932352960109711 0
0.933823525905609 0
0.935294091701508 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.939705789089203 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.945588231086731 0
0.945588231086731 0
0.948529422283173 0
0.948529422283173 0
0.949999988079071 0
0.949999988079071 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.952941179275513 0
0.954411745071411 0
0.954411745071411 0
0.954411745071411 0
0.960294127464294 0
0.963235318660736 0
0.964705884456635 0
0.964705884456635 0
0.967647075653076 0
0.967647075653076 0
0.969117641448975 0
0.972058832645416 0
0.976470589637756 0
0.976470589637756 0
0.977941155433655 0
0.979411780834198 0
0.979411780834198 0
0.980882346630096 0
0.983823537826538 0
0.985294103622437 0
0.98676472902298 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.992647051811218 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.99558824300766 0
0.998529434204102 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.146204307675362 0.134699866175652
0.170571699738503 0.110100023448467
0.180880904197693 0.100000075995922
0.18931582570076 0.0941999182105064
0.203373938798904 0.0898000001907349
0.210871607065201 0.0856999158859253
0.217432051897049 0.0794000253081322
0.234301745891571 0.0706997886300087
0.241799458861351 0.0615000054240227
0.253982961177826 0.0497000180184841
0.264292389154434 0.0385999344289303
0.27460178732872 0.0254999846220016
0.283973634243011 0.0173000022768974
0.288659691810608 0.0109000224620104
0.296157509088516 0.00629999861121178
0.304592609405518 0.0037999942433089
0.316776067018509 0.00230000261217356
0.326148182153702 0.000799998117145151
0.333645731210709 0.000499999907333404
0.342080414295197 0.000399999058572575
0.3514524102211 9.99997646431439e-05
0.357075899839401 0
0.369259595870972 0
0.374882936477661 0
0.382380545139313 0
0.395501434803009 0
0.405810683965683 0
0.413308352231979 0
0.416119992733002 0
0.423617571592331 0
0.43111526966095 0
0.437675803899765 0
0.449859380722046 0
0.459231525659561 0
0.469540804624557 0
0.478912830352783 0
0.488284915685654 0
0.501406192779541 0
0.508903443813324 0
0.515463888645172 0
0.524836242198944 0
0.533270716667175 0
0.535144925117493 0
0.53889399766922 0
0.549203932285309 0
0.556700825691223 0
0.561387479305267 0
0.579194307327271 0
0.585754454135895 0
0.594189047813416 0
0.603561103343964 0
0.610122263431549 0
0.61574524641037 0
0.621367990970612 0
0.63261479139328 0
0.642924129962921 0
0.650421500205994 0
0.657919645309448 0
0.66541713476181 0
0.669165730476379 0
0.679474949836731 0
0.686035633087158 0
0.690721750259399 0
0.698219478130341 0
0.707591593265533 0
0.71790075302124 0
0.72914719581604 0
0.736644685268402 0
0.744142174720764 0
0.753514647483826 0
0.761012375354767 0
0.76757276058197 0
0.772258698940277 0
0.784442067146301 0
0.791940093040466 0
0.802249193191528 0
0.809747040271759 0
0.820056438446045 0
0.826616585254669 0
0.832239925861359 0
0.838800311088562 0
0.847235262393951 0
0.855670094490051 0
0.864104986190796 0
0.873477160930634 0
0.87816309928894 0
0.890346705913544 0
0.897844433784485 0
0.904404938220978 0
0.910028159618378 0
0.922211885452271 0
0.927834987640381 0
0.93626993894577 0
0.948453664779663 0
0.959700107574463 0
0.967197775840759 0
0.974695384502411 0
0.983130276203156 0
0.990627944469452 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0175693910568953 0.134699866175652
0.0308978632092476 0.110100023448467
0.0433781631290913 0.100000075995922
0.0547679588198662 0.0941999182105064
0.0655519962310791 0.0898000001907349
0.0751242116093636 0.0856999158859253
0.0839695781469345 0.0794000253081322
0.0956016406416893 0.0706997886300087
0.105052702128887 0.0615000054240227
0.115109674632549 0.0497000180184841
0.125893592834473 0.0385999344289303
0.137162566184998 0.0254999846220016
0.148430809378624 0.0173000022768974
0.158851429820061 0.0109000224620104
0.169150710105896 0.00629999861121178
0.178480535745621 0.0037999942433089
0.188658580183983 0.00230000261217356
0.1998061388731 0.000799998117145151
0.208409041166306 0.000499999907333404
0.219798877835274 0.000399999058572575
0.230340480804443 9.99997646431439e-05
0.240518242120743 0
0.250696271657944 0
0.260147392749786 0
0.269476979970932 0
0.279535055160522 0
0.28959122300148 0
0.29916450381279 0
0.310432851314545 0
0.321821838617325 0
0.332727342844009 0
0.340846002101898 0
0.350781589746475 0
0.361686944961548 0
0.371016830205917 0
0.380952209234238 0
0.389434039592743 0
0.399975895881653 0
0.408942312002182 0
0.421180337667465 0
0.431721806526184 0
0.441293954849243 0
0.450260609388351 0
0.459469318389893 0
0.468556821346283 0
0.479462027549744 0
0.489397495985031 0
0.497880101203918 0
0.509512603282928 0
0.52090185880661 0
0.531081259250641 0
0.54125714302063 0
0.550830185413361 0
0.560766816139221 0
0.569854080677032 0
0.580151259899139 0
0.590937077999115 0
0.601720750331879 0
0.612504959106445 0
0.623168230056763 0
0.633465647697449 0
0.644976794719696 0
0.656246840953827 0
0.667271792888641 0
0.67842036485672 0
0.689446628093719 0
0.69926118850708 0
0.709802746772766 0
0.720465540885925 0
0.730522096157074 0
0.740336775779724 0
0.749667823314667 0
0.759360611438751 0
0.77026504278183 0
0.778868079185486 0
0.789773225784302 0
0.801041483879089 0
0.811098873615265 0
0.82103443145752 0
0.830485761165619 0
0.840905964374542 0
0.851448237895966 0
0.860293328762054 0
0.868774652481079 0
0.876045167446136 0
0.884769320487976 0
0.894583940505981 0
0.90306556224823 0
0.91166877746582 0
0.920634806156158 0
0.927905142307281 0
0.936144292354584 0
0.943050801753998 0
0.95044219493866 0
0.958196997642517 0
0.969223260879517 0
0.975887537002563 0
0.98412698507309 0
0.99127596616745 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/combination/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0923999547958374 0.319199800491333
0.104900144040585 0.310899257659912
0.117499962449074 0.286400347948074
0.127299919724464 0.242300003767014
0.138199701905251 0.18469999730587
0.148499727249146 0.125899910926819
0.158200085163116 0.0747001320123672
0.167899876832962 0.0426000691950321
0.176599591970444 0.0214000251144171
0.185799717903137 0.00789999589323997
0.194399863481522 0.00360000040382147
0.205299824476242 0.00140000157989562
0.215500041842461 0.000399999058572575
0.225900053977966 0
0.234899997711182 0
0.244200140237808 0
0.254300206899643 0
0.263500183820724 0
0.271800309419632 0
0.28070056438446 0
0.292199403047562 0
0.300899475812912 0
0.310999780893326 0
0.320599645376205 0
0.329300135374069 0
0.338900655508041 0
0.348299741744995 0
0.358099550008774 0
0.367400944232941 0
0.378100037574768 0
0.387700021266937 0
0.396100103855133 0
0.405599415302277 0
0.415599912405014 0
0.424899816513062 0
0.435300052165985 0
0.444299906492233 0
0.454299986362457 0
0.462500005960464 0
0.473699986934662 0
0.483799964189529 0
0.493600010871887 0
0.501500308513641 0
0.509000301361084 0
0.51819896697998 0
0.527499198913574 0
0.536400616168976 0
0.545899391174316 0
0.555301070213318 0
0.565902352333069 0
0.576400935649872 0
0.586201071739197 0
0.59379768371582 0
0.603199362754822 0
0.611700832843781 0
0.6214998960495 0
0.631299197673798 0
0.641299724578857 0
0.650600910186768 0
0.660799026489258 0
0.669498860836029 0
0.679200649261475 0
0.688099265098572 0
0.698600172996521 0
0.708600103855133 0
0.717499911785126 0
0.728201150894165 0
0.738400042057037 0
0.74729859828949 0
0.757099568843842 0
0.766600906848907 0
0.774700164794922 0
0.783299922943115 0
0.793500125408173 0
0.801499545574188 0
0.810899615287781 0
0.820299923419952 0
0.829999387264252 0
0.838600099086761 0
0.846199989318848 0
0.854800760746002 0
0.864100217819214 0
0.873299598693848 0
0.881099581718445 0
0.887899816036224 0
0.895799994468689 0
0.903800189495087 0
0.911400020122528 0
0.918500363826752 0
0.926999807357788 0
0.934599697589874 0
0.941999971866608 0
0.947600126266479 0
0.955500185489655 0
0.963100016117096 0
0.971700012683868 0
0.97759997844696 0
0.985199987888336 0
0.992999970912933 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.88563060760498 0.319199800491333
0.88563060760498 0.310899257659912
0.88856303691864 0.286400347948074
0.890029430389404 0.242300003767014
0.890029430389404 0.18469999730587
0.891495704650879 0.125899910926819
0.892961978912354 0.0747001320123672
0.894428312778473 0.0426000691950321
0.895894587039948 0.0214000251144171
0.895894587039948 0.00789999589323997
0.898826956748962 0.00360000040382147
0.900293231010437 0.00140000157989562
0.900293231010437 0.000399999058572575
0.903225779533386 0
0.906158328056335 0
0.907624661922455 0
0.910557210445404 0
0.910557210445404 0
0.910557210445404 0
0.913489758968353 0
0.916422307491302 0
0.917888581752777 0
0.919354856014252 0
0.919354856014252 0
0.919354856014252 0
0.920821130275726 0
0.922287404537201 0
0.923753559589386 0
0.923753559589386 0
0.925220012664795 0
0.926686227321625 0
0.928152501583099 0
0.928152501583099 0
0.928152501583099 0
0.928152501583099 0
0.928152501583099 0
0.928152501583099 0
0.931085050106049 0
0.932551324367523 0
0.934017598628998 0
0.936950147151947 0
0.936950147151947 0
0.936950147151947 0
0.936950147151947 0
0.936950147151947 0
0.938416421413422 0
0.939882636070251 0
0.939882636070251 0
0.939882636070251 0
0.939882636070251 0
0.939882636070251 0
0.94428151845932 0
0.94428151845932 0
0.947214066982269 0
0.947214066982269 0
0.948680341243744 0
0.948680341243744 0
0.951612889766693 0
0.951612889766693 0
0.951612889766693 0
0.951612889766693 0
0.951612889766693 0
0.951612889766693 0
0.953079164028168 0
0.954545438289642 0
0.954545438289642 0
0.954545438289642 0
0.960410535335541 0
0.96334308385849 0
0.964809358119965 0
0.964809358119965 0
0.967741906642914 0
0.967741906642914 0
0.969208240509033 0
0.972140789031982 0
0.976539611816406 0
0.976539611816406 0
0.978005886077881 0
0.979472160339355 0
0.979472160339355 0
0.98093843460083 0
0.983870983123779 0
0.985337257385254 0
0.986803531646729 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.989736080169678 0
0.992668628692627 0
0.994134902954102 0
0.994134902954102 0
0.994134902954102 0
0.994134902954102 0
0.995601177215576 0
0.998533725738525 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.166666701436043 0.319199800491333
0.183333277702332 0.310899257659912
0.195614069700241 0.286400347948074
0.204385966062546 0.242300003767014
0.215789422392845 0.18469999730587
0.223684176802635 0.125899910926819
0.229824557900429 0.0747001320123672
0.245614066720009 0.0426000691950321
0.251754373311996 0.0214000251144171
0.264912128448486 0.00789999589323997
0.274561494588852 0.00360000040382147
0.285965025424957 0.00140000157989562
0.293859601020813 0.000399999058572575
0.299999922513962 0
0.307894676923752 0
0.315789461135864 0
0.327193200588226 0
0.334210723638535 0
0.342105180025101 0
0.349122852087021 0
0.357894778251648 0
0.364912301301956 0
0.377193182706833 0
0.383333444595337 0
0.391228079795837 0
0.403508812189102 0
0.413157880306244 0
0.42280712723732 0
0.427193015813828 0
0.435087770223618 0
0.4438596367836 0
0.449999958276749 0
0.461403399705887 0
0.470175445079803 0
0.47982457280159 0
0.488596498966217 0
0.498245656490326 0
0.51140296459198 0
0.519298434257507 0
0.525439262390137 0
0.534210324287415 0
0.542982757091522 0
0.545614004135132 0
0.549122869968414 0
0.560526907444 0
0.567544102668762 0
0.572806596755981 0
0.588596940040588 0
0.595613360404968 0
0.604385852813721 0
0.613158285617828 0
0.619297862052917 0
0.624561429023743 0
0.630701780319214 0
0.642105340957642 0
0.652631998062134 0
0.659649312496185 0
0.665789544582367 0
0.673683881759644 0
0.680701553821564 0
0.691227972507477 0
0.699122190475464 0
0.704385697841644 0
0.711403369903564 0
0.721052408218384 0
0.730701684951782 0
0.740350902080536 0
0.747368216514587 0
0.754386126995087 0
0.764912366867065 0
0.77456134557724 0
0.781578898429871 0
0.785964787006378 0
0.797368764877319 0
0.806140124797821 0
0.818420708179474 0
0.824561536312103 0
0.833333253860474 0
0.838596284389496 0
0.844736635684967 0
0.852631628513336 0
0.860526084899902 0
0.867543935775757 0
0.875438451766968 0
0.884210526943207 0
0.889473617076874 0
0.900876998901367 0
0.907017767429352 0
0.914035081863403 0
0.917543888092041 0
0.928070187568665 0
0.932456135749817 0
0.939473688602448 0
0.949999988079071 0
0.961403489112854 0
0.968421041965485 0
0.975438475608826 0
0.983333349227905 0
0.990350902080536 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0158963017165661 0.319199800491333
0.0288579110056162 0.310899257659912
0.0423086434602737 0.286400347948074
0.0529469288885593 0.242300003767014
0.0646855384111404 0.18469999730587
0.0760576874017715 0.125899910926819
0.0869406163692474 0.0747001320123672
0.0964783132076263 0.0426000691950321
0.106138415634632 0.0214000251144171
0.115553915500641 0.00789999589323997
0.124480344355106 0.00360000040382147
0.136096581816673 0.00140000157989562
0.147468939423561 0.000399999058572575
0.159085407853127 0
0.168745696544647 0
0.178894504904747 0
0.189410552382469 0
0.199682116508484 0
0.208730697631836 0
0.218390807509422 0
0.230985596776009 0
0.240523442625999 0
0.251039147377014 0
0.261921346187592 0
0.271460562944412 0
0.281363695859909 0
0.291391313076019 0
0.301907747983932 0
0.312667906284332 0
0.324528813362122 0
0.334923028945923 0
0.344216018915176 0
0.354243218898773 0
0.3652483522892 0
0.37527534365654 0
0.386769413948059 0
0.396429032087326 0
0.406578630208969 0
0.41538268327713 0
0.428099721670151 0
0.43898269534111 0
0.449743330478668 0
0.459036380052567 0
0.46771827340126 0
0.477378338575363 0
0.487649828195572 0
0.4976766705513 0
0.507090389728546 0
0.517605602741241 0
0.529346466064453 0
0.540963351726532 0
0.551723718643188 0
0.560283303260803 0
0.57067734003067 0
0.579481840133667 0
0.589875876903534 0
0.600881218910217 0
0.612006843090057 0
0.622280478477478 0
0.633773922920227 0
0.642944037914276 0
0.65370512008667 0
0.6638543009758 0
0.675592482089996 0
0.686352908611298 0
0.695891678333282 0
0.707630217075348 0
0.718635559082031 0
0.728295803070068 0
0.738689303398132 0
0.748961091041565 0
0.757642865180969 0
0.767547070980072 0
0.778308153152466 0
0.786622822284698 0
0.796038150787354 0
0.806676685810089 0
0.817192256450653 0
0.826852321624756 0
0.835289537906647 0
0.844583034515381 0
0.854609906673431 0
0.864758968353271 0
0.873074233531952 0
0.879921615123749 0
0.888847768306732 0
0.897040843963623 0
0.905478000640869 0
0.913181602954865 0
0.923086285591125 0
0.93091231584549 0
0.939349472522736 0
0.944974303245544 0
0.953044652938843 0
0.960748374462128 0
0.970286190509796 0
0.976522386074066 0
0.984592795372009 0
0.992907822132111 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/combination_/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0921000763773918 0.317099571228027
0.104600094258785 0.308099567890167
0.115500003099442 0.291599571704865
0.125400304794312 0.266700506210327
0.134900286793709 0.23870000243187
0.14570027589798 0.207799807190895
0.15489998459816 0.171199843287468
0.165299788117409 0.139600247144699
0.174400180578232 0.11329997330904
0.184200152754784 0.0909998789429665
0.193700104951859 0.0749998986721039
0.204699799418449 0.0628998726606369
0.214899927377701 0.0529999621212482
0.225400045514107 0.0444000214338303
0.234799951314926 0.0368000082671642
0.244399860501289 0.029000012204051
0.255000174045563 0.0215000193566084
0.264700353145599 0.0167000088840723
0.272400945425034 0.0129000041633844
0.281500458717346 0.00889996904879808
0.292000353336334 0.00549999671056867
0.301199913024902 0.00380000844597816
0.309999793767929 0.00230000261217356
0.318999767303467 0.00139999762177467
0.328899890184402 0.00109999882988632
0.337599724531174 0.000799998117145151
0.347299635410309 0.000599998980760574
0.35549995303154 9.99997646431439e-05
0.365200191736221 0
0.375699669122696 0
0.385300040245056 0
0.393499612808228 0
0.402300238609314 0
0.412399619817734 0
0.421399503946304 0
0.431500136852264 0
0.438900381326675 0
0.448899894952774 0
0.457700133323669 0
0.468400001525879 0
0.478200107812881 0
0.487300008535385 0
0.494700014591217 0
0.502800047397614 0
0.511500060558319 0
0.520399928092957 0
0.529200255870819 0
0.538899481296539 0
0.547999978065491 0
0.558899402618408 0
0.56890082359314 0
0.578599154949188 0
0.587099611759186 0
0.597299158573151 0
0.604900777339935 0
0.614999890327454 0
0.624600172042847 0
0.634299874305725 0
0.643500149250031 0
0.653299927711487 0
0.662099957466125 0
0.672397971153259 0
0.681200325489044 0
0.690500438213348 0
0.701402008533478 0
0.711100578308105 0
0.720399975776672 0
0.730399429798126 0
0.739699304103851 0
0.748999834060669 0
0.758500576019287 0
0.766700804233551 0
0.775400400161743 0
0.78700065612793 0
0.79570072889328 0
0.805100798606873 0
0.815699875354767 0
0.825600206851959 0
0.834900200366974 0
0.843299806118011 0
0.852600395679474 0
0.862199246883392 0
0.871599495410919 0
0.880100190639496 0
0.886699974536896 0
0.894699811935425 0
0.903099894523621 0
0.911000370979309 0
0.918200016021729 0
0.925899982452393 0
0.933000206947327 0
0.940500199794769 0
0.946800172328949 0
0.954500019550323 0
0.961899876594543 0
0.971300005912781 0
0.978100001811981 0
0.985499978065491 0
0.993099987506866 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.88823527097702 0.317099571228027
0.88823527097702 0.308099567890167
0.891176581382751 0.291599571704865
0.892647266387939 0.266700506210327
0.892647266387939 0.23870000243187
0.894117712974548 0.207799807190895
0.895588338375092 0.171199843287468
0.897058844566345 0.139600247144699
0.898529410362244 0.11329997330904
0.898529410362244 0.0909998789429665
0.901470601558685 0.0749998986721039
0.902941167354584 0.0628998726606369
0.902941167354584 0.0529999621212482
0.905882358551025 0.0444000214338303
0.908823728561401 0.0368000082671642
0.910294115543365 0.029000012204051
0.913235306739807 0.0215000193566084
0.913235306739807 0.0167000088840723
0.913235306739807 0.0129000041633844
0.914705872535706 0.00889996904879808
0.917647063732147 0.00549999671056867
0.919117629528046 0.00380000844597816
0.920588254928589 0.00230000261217356
0.920588254928589 0.00139999762177467
0.920588254928589 0.00109999882988632
0.922058820724487 0.000799998117145151
0.923529326915741 0.000599998980760574
0.925000071525574 9.99997646431439e-05
0.925000071525574 0
0.926470577716827 0
0.927941203117371 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.929411768913269 0
0.932352960109711 0
0.933823525905609 0
0.935294091701508 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.938235282897949 0
0.939705789089203 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.941176474094391 0
0.945588231086731 0
0.945588231086731 0
0.948529422283173 0
0.948529422283173 0
0.949999988079071 0
0.949999988079071 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.951470613479614 0
0.952941179275513 0
0.954411745071411 0
0.954411745071411 0
0.954411745071411 0
0.960294127464294 0
0.963235318660736 0
0.964705884456635 0
0.964705884456635 0
0.967647075653076 0
0.967647075653076 0
0.969117641448975 0
0.972058832645416 0
0.976470589637756 0
0.976470589637756 0
0.977941155433655 0
0.979411780834198 0
0.979411780834198 0
0.980882346630096 0
0.983823537826538 0
0.985294103622437 0
0.98676472902298 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.989705860614777 0
0.992647051811218 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.994117617607117 0
0.99558824300766 0
0.998529434204102 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.172925770282745 0.317099571228027
0.185152918100357 0.308099567890167
0.19388647377491 0.291599571704865
0.202620059251785 0.266700506210327
0.213973864912987 0.23870000243187
0.223580837249756 0.207799807190895
0.234934493899345 0.171199843287468
0.248908430337906 0.139600247144699
0.255895256996155 0.11329997330904
0.268995434045792 0.0909998789429665
0.279475808143616 0.0749998986721039
0.289083063602448 0.0628998726606369
0.296943515539169 0.0529999621212482
0.303930044174194 0.0444000214338303
0.310916811227798 0.0368000082671642
0.321397393941879 0.029000012204051
0.333624571561813 0.0215000193566084
0.341484814882278 0.0167000088840723
0.348471492528915 0.0129000041633844
0.359825521707535 0.00889996904879808
0.370305627584457 0.00549999671056867
0.377292484045029 0.00380000844597816
0.388646215200424 0.00230000261217356
0.39388644695282 0.00139999762177467
0.402620166540146 0.00109999882988632
0.413973867893219 0.000799998117145151
0.424454241991043 0.000599998980760574
0.432314246892929 9.99997646431439e-05
0.435807913541794 0
0.443668216466904 0
0.45065513253212 0
0.456768572330475 0
0.467248916625977 0
0.476855903863907 0
0.487336248159409 0
0.496943324804306 0
0.506550192832947 0
0.518777847290039 0
0.527510821819305 0
0.535371363162994 0
0.544104754924774 0
0.551965236663818 0
0.553711950778961 0
0.558952391147614 0
0.568558990955353 0
0.575546145439148 0
0.580785870552063 0
0.597380220890045 0
0.604367315769196 0
0.613973677158356 0
0.622707426548004 0
0.629694581031799 0
0.635807991027832 0
0.642794787883759 0
0.653275668621063 0
0.662882268428802 0
0.671615481376648 0
0.679475903511047 0
0.686463057994843 0
0.690829634666443 0
0.700436532497406 0
0.707423150539398 0
0.711790144443512 0
0.718777298927307 0
0.730130910873413 0
0.740611910820007 0
0.750218152999878 0
0.757204949855804 0
0.764192044734955 0
0.772925853729248 0
0.779912233352661 0
0.786026060581207 0
0.790392756462097 0
0.80262017250061 0
0.810480535030365 0
0.820087194442749 0
0.82707405090332 0
0.836681127548218 0
0.841921269893646 0
0.848908305168152 0
0.855021834373474 0
0.863755583763123 0
0.870742440223694 0
0.878602623939514 0
0.887336194515228 0
0.891703188419342 0
0.902183592319489 0
0.908297181129456 0
0.915284037590027 0
0.918777287006378 0
0.92925763130188 0
0.933624446392059 0
0.939738094806671 0
0.951091706752777 0
0.961572051048279 0
0.969432294368744 0
0.977292597293854 0
0.985152840614319 0
0.991266369819641 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.014556554146111 0.317099571228027
0.0281345639377832 0.308099567890167
0.0400000251829624 0.291599571704865
0.0507644526660442 0.266700506210327
0.060795146971941 0.23870000243187
0.07253797352314 0.207799807190895
0.0820793285965919 0.171199843287468
0.0927217081189156 0.139600247144699
0.102752283215523 0.11329997330904
0.112905241549015 0.0909998789429665
0.122813411056995 0.0749998986721039
0.134801611304283 0.0628998726606369
0.14617732167244 0.0529999621212482
0.157798200845718 0.0444000214338303
0.168073371052742 0.0368000082671642
0.178226128220558 0.029000012204051
0.189235508441925 0.0215000193566084
0.200000092387199 0.0167000088840723
0.208440437912941 0.0129000041633844
0.217859297990799 0.00889996904879808
0.228990882635117 0.00549999671056867
0.239143714308739 0.00380000844597816
0.248195961117744 0.00230000261217356
0.258470743894577 0.00139999762177467
0.269357740879059 0.00109999882988632
0.278288185596466 0.000799998117145151
0.288563191890717 0.000599998980760574
0.297369956970215 9.99997646431439e-05
0.308746129274368 0
0.320367455482483 0
0.331009119749069 0
0.340061634778976 0
0.349357783794403 0
0.360367387533188 0
0.369908422231674 0
0.380917429924011 0
0.388624131679535 0
0.398898839950562 0
0.408318102359772 0
0.420183479785919 0
0.430703401565552 0
0.440733939409256 0
0.44954127073288 0
0.458715587854385 0
0.468012303113937 0
0.477798193693161 0
0.487706363201141 0
0.497246593236923 0
0.507401347160339 0
0.519388258457184 0
0.530397653579712 0
0.540916264057159 0
0.550459086894989 0
0.561712443828583 0
0.569541275501251 0
0.580428600311279 0
0.590949237346649 0
0.601591289043427 0
0.611864745616913 0
0.623242497444153 0
0.632661283016205 0
0.644280612468719 0
0.654433727264404 0
0.664709150791168 0
0.67632919549942 0
0.686728179454803 0
0.696758329868317 0
0.707522690296173 0
0.717676103115082 0
0.72770631313324 0
0.738348364830017 0
0.747277915477753 0
0.7573082447052 0
0.769663751125336 0
0.778960585594177 0
0.788746774196625 0
0.80073356628418 0
0.811375916004181 0
0.821895897388458 0
0.831192195415497 0
0.841590464115143 0
0.851865708827972 0
0.862263083457947 0
0.871437132358551 0
0.878043115139008 0
0.887217104434967 0
0.896024405956268 0
0.904831647872925 0
0.912660717964172 0
0.921590328216553 0
0.928807139396667 0
0.937369883060455 0
0.943975389003754 0
0.951681971549988 0
0.959266066551208 0
0.969663619995117 0
0.976880729198456 0
0.984709501266479 0
0.99290519952774 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/combination_target/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0804001316428185 0.321199744939804
0.0952000319957733 0.321099817752838
0.10739990323782 0.319899678230286
0.118400022387505 0.317500174045563
0.129099905490875 0.31139999628067
0.140200212597847 0.296999365091324
0.148900121450424 0.271600037813187
0.159899815917015 0.237200051546097
0.170200154185295 0.190999925136566
0.179399788379669 0.143199697136879
0.188999623060226 0.0989998206496239
0.198699966073036 0.0641999095678329
0.210100248456001 0.0393999144434929
0.220099955797195 0.0220000091940165
0.230299919843674 0.0111999958753586
0.238999992609024 0.00569999217987061
0.248600855469704 0.00239999545738101
0.258800238370895 0.000999999814666808
0.266999393701553 0.000699998810887337
0.276600122451782 0.000199999529286288
0.287798881530762 9.99997646431439e-05
0.297099530696869 0
0.306800812482834 0
0.316300004720688 0
0.325599521398544 0
0.335799664258957 0
0.345400333404541 0
0.354799926280975 0
0.364899456501007 0
0.375199794769287 0
0.384600520133972 0
0.393799990415573 0
0.403700292110443 0
0.412899941205978 0
0.422099947929382 0
0.431600391864777 0
0.43989971280098 0
0.449800103902817 0
0.4578997194767 0
0.469399988651276 0
0.479099899530411 0
0.48879998922348 0
0.497500002384186 0
0.50529932975769 0
0.514399588108063 0
0.523399651050568 0
0.531501114368439 0
0.542301833629608 0
0.552199959754944 0
0.562601268291473 0
0.572899580001831 0
0.582099199295044 0
0.591500639915466 0
0.60060065984726 0
0.608200967311859 0
0.618099272251129 0
0.627699732780457 0
0.637499392032623 0
0.647499978542328 0
0.656600177288055 0
0.665899753570557 0
0.675299227237701 0
0.684400975704193 0
0.694399058818817 0
0.704398155212402 0
0.714199483394623 0
0.723299443721771 0
0.733300447463989 0
0.743400990962982 0
0.753899693489075 0
0.763801097869873 0
0.772900521755219 0
0.781098484992981 0
0.791501045227051 0
0.799399077892303 0
0.808700859546661 0
0.816900312900543 0
0.827498853206635 0
0.837100028991699 0
0.845199823379517 0
0.853699684143066 0
0.863099634647369 0
0.872500598430634 0
0.880900025367737 0
0.887899875640869 0
0.894900321960449 0
0.904600203037262 0
0.91239982843399 0
0.919700026512146 0
0.928300380706787 0
0.936099827289581 0
0.942799985408783 0
0.948700189590454 0
0.956499993801117 0
0.963900029659271 0
0.972599983215332 0
0.977799892425537 0
0.985000014305115 0
0.992999970912933 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.877906799316406 0.321199744939804
0.883721113204956 0.321099817752838
0.889534950256348 0.319899678230286
0.890988349914551 0.317500174045563
0.890988349914551 0.31139999628067
0.893895506858826 0.296999365091324
0.895349025726318 0.271600037813187
0.896802306175232 0.237200051546097
0.898255825042725 0.190999925136566
0.898255825042725 0.143199697136879
0.901162803173065 0.0989998206496239
0.902616202831268 0.0641999095678329
0.902616202831268 0.0393999144434929
0.905523240566254 0.0220000091940165
0.908430397510529 0.0111999958753586
0.909883737564087 0.00569999217987061
0.912790715694427 0.00239999545738101
0.912790715694427 0.000999999814666808
0.912790715694427 0.000699998810887337
0.914244174957275 0.000199999529286288
0.917151153087616 9.99997646431439e-05
0.918604671955109 0
0.920058131217957 0
0.920058131217957 0
0.920058131217957 0
0.921511650085449 0
0.922965049743652 0
0.924418687820435 0
0.924418687820435 0
0.925872087478638 0
0.92732560634613 0
0.928779065608978 0
0.928779065608978 0
0.930232584476471 0
0.930232584476471 0
0.930232584476471 0
0.930232584476471 0
0.933139562606812 0
0.934593021869659 0
0.936046421527863 0
0.938953399658203 0
0.938953399658203 0
0.938953399658203 0
0.938953399658203 0
0.938953399658203 0
0.940406978130341 0
0.941860437393188 0
0.941860437393188 0
0.941860437393188 0
0.941860437393188 0
0.941860437393188 0
0.946220934391022 0
0.946220934391022 0
0.949127912521362 0
0.949127912521362 0
0.95058137178421 0
0.95058137178421 0
0.952034890651703 0
0.952034890651703 0
0.952034890651703 0
0.952034890651703 0
0.952034890651703 0
0.952034890651703 0
0.953488349914551 0
0.954941868782043 0
0.954941868782043 0
0.954941868782043 0
0.960755825042725 0
0.963662803173065 0
0.965116262435913 0
0.965116262435913 0
0.968023240566254 0
0.968023240566254 0
0.969476759433746 0
0.972383737564087 0
0.976744174957275 0
0.976744174957275 0
0.978197693824768 0
0.979651153087616 0
0.979651153087616 0
0.981104671955109 0
0.984011650085449 0
0.985465109348297 0
0.98691862821579 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.98982560634613 0
0.992732584476471 0
0.994186043739319 0
0.994186043739319 0
0.994186043739319 0
0.994186043739319 0
0.995639562606812 0
0.998546540737152 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0909090936183929 0.321199744939804
0.131015911698341 0.321099817752838
0.1515152156353 0.319899678230286
0.173796758055687 0.317500174045563
0.196078464388847 0.31139999628067
0.213012471795082 0.296999365091324
0.223707720637321 0.271600037813187
0.241532981395721 0.237200051546097
0.247771993279457 0.190999925136566
0.258466899394989 0.143199697136879
0.266488611698151 0.0989998206496239
0.27629229426384 0.0641999095678329
0.285205066204071 0.0393999144434929
0.293226510286331 0.0220000091940165
0.304812908172607 0.0111999958753586
0.313725560903549 0.00569999217987061
0.326203286647797 0.00239999545738101
0.332442134618759 0.000999999814666808
0.338680982589722 0.000699998810887337
0.347593575716019 0.000199999529286288
0.358288764953613 9.99997646431439e-05
0.366309970617294 0
0.381461650133133 0
0.387700468301773 0
0.395722001791 0
0.409982264041901 0
0.41889476776123 0
0.426916152238846 0
0.430481284856796 0
0.43761146068573 0
0.445632845163345 0
0.453654199838638 0
0.465240627527237 0
0.473262041807175 0
0.482174694538116 0
0.491087347269058 0
0.5 0
0.513368308544159 0
0.520499110221863 0
0.527629137039185 0
0.535650014877319 0
0.546345472335815 0
0.550802171230316 0
0.554367125034332 0
0.564171195030212 0
0.572192072868347 0
0.576648771762848 0
0.592691719532013 0
0.599821925163269 0
0.608734428882599 0
0.619429290294647 0
0.62566876411438 0
0.631016075611115 0
0.63725483417511 0
0.647950172424316 0
0.657754063606262 0
0.66488391160965 0
0.672013580799103 0
0.68092668056488 0
0.686274588108063 0
0.696969628334045 0
0.704991042613983 0
0.709447205066681 0
0.716577410697937 0
0.725490629673004 0
0.735294103622437 0
0.745098173618317 0
0.753119647502899 0
0.760249614715576 0
0.769162118434906 0
0.777183651924133 0
0.783422648906708 0
0.78787887096405 0
0.799465119838715 0
0.807486712932587 0
0.817290365695953 0
0.823529183864594 0
0.83422464132309 0
0.84046345949173 0
0.84670215845108 0
0.852941155433655 0
0.860962569713593 0
0.868092596530914 0
0.875222682952881 0
0.884135246276855 0
0.888591587543488 0
0.899286985397339 0
0.906417191028595 0
0.913547217845917 0
0.918003559112549 0
0.928698778152466 0
0.933155059814453 0
0.940285205841064 0
0.951871633529663 0
0.963458120822906 0
0.970588207244873 0
0.976827085018158 0
0.984848499298096 0
0.991087317466736 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0119658028706908 0.321199744939804
0.0240537468343973 0.321099817752838
0.0356531292200089 0.319899678230286
0.0459096543490887 0.317500174045563
0.0559218674898148 0.31139999628067
0.0669110864400864 0.296999365091324
0.0759463608264923 0.271600037813187
0.0868131443858147 0.237200051546097
0.0984126999974251 0.190999925136566
0.108180701732635 0.143199697136879
0.118559278547764 0.0989998206496239
0.128937900066376 0.0641999095678329
0.141635611653328 0.0393999144434929
0.152503162622452 0.0220000091940165
0.163125619292259 0.0111999958753586
0.172405183315277 0.00569999217987061
0.182173535227776 0.00239999545738101
0.19377301633358 0.000999999814666808
0.202930420637131 0.000699998810887337
0.21330888569355 0.000199999529286288
0.22527477145195 9.99997646431439e-05
0.235408961772919 0
0.245055183768272 0
0.255799949169159 0
0.266056209802628 0
0.276434600353241 0
0.286813616752625 0
0.297069549560547 0
0.308912813663483 0
0.320390522480011 0
0.330647081136703 0
0.340659290552139 0
0.351160079240799 0
0.36117222905159 0
0.371184289455414 0
0.381562799215317 0
0.390476614236832 0
0.400488436222076 0
0.409279555082321 0
0.422222167253494 0
0.432723015546799 0
0.4431012570858 0
0.453113317489624 0
0.462149024009705 0
0.471917003393173 0
0.481684863567352 0
0.490842789411545 0
0.501831293106079 0
0.512941777706146 0
0.524420619010925 0
0.535533428192139 0
0.545543909072876 0
0.55628889799118 0
0.566300630569458 0
0.574115455150604 0
0.584736406803131 0
0.5954829454422 0
0.606348812580109 0
0.617338716983795 0
0.627716958522797 0
0.637606859207153 0
0.647984802722931 0
0.658487141132355 0
0.669597327709198 0
0.680463850498199 0
0.69108659029007 0
0.700854957103729 0
0.711477100849152 0
0.722588539123535 0
0.734066545963287 0
0.745054960250854 0
0.755066633224487 0
0.764469087123871 0
0.775457978248596 0
0.783760130405426 0
0.79340648651123 0
0.802564382553101 0
0.813919067382812 0
0.824663996696472 0
0.833699524402618 0
0.843101561069489 0
0.85323566198349 0
0.86361426115036 0
0.872771322727203 0
0.879853487014771 0
0.887790203094482 0
0.898168385028839 0
0.906715512275696 0
0.914651989936829 0
0.924542248249054 0
0.932600975036621 0
0.94017094373703 0
0.94615375995636 0
0.953968226909637 0
0.961416304111481 0
0.971062123775482 0
0.976556777954102 0
0.98412698507309 0
0.992796063423157 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/gpt/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0798053592443466 0.120194643735886
0.0948904678225517 0.0836984142661095
0.10900241881609 0.0666666254401207
0.119221411645412 0.058880802243948
0.132360100746155 0.0527980849146843
0.143552288413048 0.0489050783216953
0.153041377663612 0.0462286807596684
0.163503602147102 0.0437956415116787
0.174695894122124 0.0406325720250607
0.185157984495163 0.0345498248934746
0.196350380778313 0.0316301845014095
0.207542583346367 0.028953779488802
0.220924541354179 0.0274939239025116
0.229683712124825 0.0260340590029955
0.239172786474228 0.0250608455389738
0.248661831021309 0.023357667028904
0.262287646532059 0.0226277261972427
0.27007257938385 0.022141108289361
0.277615189552307 0.0214112009853125
0.28686112165451 0.0211678650230169
0.297567069530487 0.0187348052859306
0.307542324066162 0.0184914954006672
0.315571665763855 0.0184914954006672
0.324087530374527 0.0184914954006672
0.333090037107468 0.0184914954006672
0.342092424631119 0.0180048607289791
0.351095110177994 0.0180048607289791
0.359854012727737 0.0177615508437157
0.369343012571335 0.0172749422490597
0.381751954555511 0.0172749422490597
0.392214268445969 0.0172749422490597
0.400486528873444 0.0163017138838768
0.409975647926331 0.0160584058612585
0.4192214012146 0.0160584058612585
0.426763951778412 0.0158151015639305
0.435036540031433 0.0138686159625649
0.441119134426117 0.0131386909633875
0.453284680843353 0.0126520777121186
0.461557239294052 0.012408759444952
0.470559597015381 0.0119221359491348
0.478588819503784 0.0109488973394036
0.488077908754349 0.00997565872967243
0.495864033699036 0.00997565872967243
0.505351483821869 0.00973235163837671
0.515327990055084 0.00924573466181755
0.525061070919037 0.00900242570787668
0.534061253070831 0.00851580966264009
0.541849792003632 0.00827249884605408
0.550608515739441 0.00802918616682291
0.560340642929077 0.00705596292391419
0.569343566894531 0.00656934408470988
0.579318761825562 0.00608272943645716
0.587104737758636 0.00583942048251629
0.597324430942535 0.00583942048251629
0.604865968227386 0.00583942048251629
0.612408339977264 0.00486618652939796
0.621167778968811 0.00413624756038189
0.633819758892059 0.00389294675551355
0.643795371055603 0.00364963035099208
0.654500663280487 0.00364963035099208
0.663017153739929 0.00340632698498666
0.671775817871094 0.00291970977559686
0.68248188495636 0.00291970977559686
0.690997660160065 0.00267639686353505
0.702189385890961 0.00218977825716138
0.712651669979095 0.00218977825716138
0.723357915878296 0.00218977825716138
0.733819782733917 0.00170316232834011
0.744282364845276 0.00170316232834011
0.754258036613464 0.00170316232834011
0.763503670692444 0.00145985302515328
0.771289348602295 0.00121654500253499
0.778102159500122 0.00121654500253499
0.788078129291534 0.000973234651610255
0.797810554504395 0.000973234651610255
0.806812644004822 0.000973234651610255
0.815328478813171 0.000973234651610255
0.827007234096527 0.000729926687199622
0.838442802429199 0.000729926687199622
0.846715152263641 0.000729926687199622
0.854257822036743 0.000729926687199622
0.864233613014221 0.000729926687199622
0.871289432048798 0.000729926687199622
0.878345608711243 0.000729926687199622
0.886861443519592 0.000729926687199622
0.893673837184906 0.000486617325805128
0.90024322271347 0.000486617325805128
0.906569480895996 0.000486617325805128
0.912895202636719 0.000486617325805128
0.920194625854492 0.000243308662902564
0.927980542182922 0.000243308662902564
0.935036480426788 0.000243308662902564
0.943065702915192 0
0.949878394603729 0
0.956204354763031 0
0.967883229255676 0
0.97323602437973 0
0.982968389987946 0
0.990267634391785 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.823943614959717 0.120194643735886
0.852112650871277 0.0836984142661095
0.866197288036346 0.0666666254401207
0.869718313217163 0.058880802243948
0.869718313217163 0.0527980849146843
0.869718313217163 0.0489050783216953
0.876760542392731 0.0462286807596684
0.876760542392731 0.0437956415116787
0.880281805992126 0.0406325720250607
0.880281805992126 0.0345498248934746
0.890845119953156 0.0316301845014095
0.894366264343262 0.028953779488802
0.894366264343262 0.0274939239025116
0.894366264343262 0.0260340590029955
0.904929578304291 0.0250608455389738
0.904929578304291 0.023357667028904
0.911971807479858 0.0226277261972427
0.911971807479858 0.022141108289361
0.915492951869965 0.0214112009853125
0.922535240650177 0.0211678650230169
0.926056325435638 0.0187348052859306
0.926056325435638 0.0184914954006672
0.926056325435638 0.0184914954006672
0.926056325435638 0.0184914954006672
0.926056325435638 0.0184914954006672
0.929577469825745 0.0180048607289791
0.933098614215851 0.0180048607289791
0.933098614215851 0.0177615508437157
0.933098614215851 0.0172749422490597
0.936619699001312 0.0172749422490597
0.936619699001312 0.0172749422490597
0.940140843391418 0.0163017138838768
0.943661987781525 0.0160584058612585
0.943661987781525 0.0160584058612585
0.943661987781525 0.0158151015639305
0.943661987781525 0.0138686159625649
0.943661987781525 0.0131386909633875
0.943661987781525 0.0126520777121186
0.947183072566986 0.012408759444952
0.950704216957092 0.0119221359491348
0.954225361347198 0.0109488973394036
0.954225361347198 0.00997565872967243
0.954225361347198 0.00997565872967243
0.954225361347198 0.00973235163837671
0.954225361347198 0.00924573466181755
0.954225361347198 0.00900242570787668
0.957746505737305 0.00851580966264009
0.957746505737305 0.00827249884605408
0.957746505737305 0.00802918616682291
0.957746505737305 0.00705596292391419
0.957746505737305 0.00656934408470988
0.964788734912872 0.00608272943645716
0.964788734912872 0.00583942048251629
0.964788734912872 0.00583942048251629
0.964788734912872 0.00583942048251629
0.964788734912872 0.00486618652939796
0.964788734912872 0.00413624756038189
0.964788734912872 0.00389294675551355
0.964788734912872 0.00364963035099208
0.964788734912872 0.00364963035099208
0.964788734912872 0.00340632698498666
0.964788734912872 0.00291970977559686
0.964788734912872 0.00291970977559686
0.964788734912872 0.00267639686353505
0.964788734912872 0.00218977825716138
0.964788734912872 0.00218977825716138
0.964788734912872 0.00218977825716138
0.975352108478546 0.00170316232834011
0.978873252868652 0.00170316232834011
0.978873252868652 0.00170316232834011
0.978873252868652 0.00145985302515328
0.978873252868652 0.00121654500253499
0.978873252868652 0.00121654500253499
0.978873252868652 0.000973234651610255
0.978873252868652 0.000973234651610255
0.978873252868652 0.000973234651610255
0.978873252868652 0.000973234651610255
0.982394337654114 0.000729926687199622
0.982394337654114 0.000729926687199622
0.982394337654114 0.000729926687199622
0.982394337654114 0.000729926687199622
0.98591548204422 0.000729926687199622
0.98591548204422 0.000729926687199622
0.98591548204422 0.000729926687199622
0.98591548204422 0.000729926687199622
0.98591548204422 0.000486617325805128
0.98591548204422 0.000486617325805128
0.98591548204422 0.000486617325805128
0.98591548204422 0.000486617325805128
0.98591548204422 0.000243308662902564
0.98591548204422 0.000243308662902564
0.98591548204422 0.000243308662902564
0.989436626434326 0
0.992957770824432 0
0.992957770824432 0
0.992957770824432 0
0.992957770824432 0
0.992957770824432 0
1 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0627802833914757 0.120194643735886
0.0919282510876656 0.0836984142661095
0.105381175875664 0.0666666254401207
0.125560626387596 0.058880802243948
0.141255617141724 0.0527980849146843
0.147982120513916 0.0489050783216953
0.161434948444366 0.0462286807596684
0.177130073308945 0.0437956415116787
0.186098694801331 0.0406325720250607
0.199551552534103 0.0345498248934746
0.213004484772682 0.0316301845014095
0.224215269088745 0.028953779488802
0.230941623449326 0.0274939239025116
0.235426008701324 0.0260340590029955
0.244394570589066 0.0250608455389738
0.248878970742226 0.023357667028904
0.26681587100029 0.0226277261972427
0.273542881011963 0.022141108289361
0.278027176856995 0.0214112009853125
0.286995589733124 0.0211678650230169
0.293722182512283 0.0187348052859306
0.295964270830154 0.0184914954006672
0.307174831628799 0.0184914954006672
0.313901335000992 0.0184914954006672
0.322869956493378 0.0184914954006672
0.336322814226151 0.0180048607289791
0.347533643245697 0.0180048607289791
0.358744353055954 0.0177615508437157
0.360986560583115 0.0172749422490597
0.367713004350662 0.0172749422490597
0.378923773765564 0.0172749422490597
0.383408039808273 0.0163017138838768
0.394618839025497 0.0160584058612585
0.403587430715561 0.0160584058612585
0.410313904285431 0.0158151015639305
0.417040437459946 0.0138686159625649
0.432735353708267 0.0131386909633875
0.450672656297684 0.0126520777121186
0.459641247987747 0.012408759444952
0.466367781162262 0.0119221359491348
0.473094195127487 0.0109488973394036
0.479820638895035 0.00997565872967243
0.486547201871872 0.00997565872967243
0.493273466825485 0.00973235163837671
0.50000011920929 0.00924573466181755
0.508969128131866 0.00900242570787668
0.515695333480835 0.00851580966264009
0.531390070915222 0.00827249884605408
0.538116693496704 0.00802918616682291
0.553811550140381 0.00705596292391419
0.5627800822258 0.00656934408470988
0.57623279094696 0.00608272943645716
0.585201680660248 0.00583942048251629
0.589686214923859 0.00583942048251629
0.600896954536438 0.00583942048251629
0.612107753753662 0.00486618652939796
0.61659163236618 0.00413624756038189
0.6300448179245 0.00389294675551355
0.639013469219208 0.00364963035099208
0.641255378723145 0.00364963035099208
0.652466237545013 0.00340632698498666
0.659192681312561 0.00291970977559686
0.661434710025787 0.00291970977559686
0.663677036762238 0.00267639686353505
0.674887835979462 0.00218977825716138
0.692825198173523 0.00218977825716138
0.710762321949005 0.00218977825716138
0.726457417011261 0.00170316232834011
0.730941712856293 0.00170316232834011
0.744394600391388 0.00170316232834011
0.757847547531128 0.00145985302515328
0.762331962585449 0.00121654500253499
0.766816079616547 0.00121654500253499
0.780269086360931 0.000973234651610255
0.789237797260284 0.000973234651610255
0.807174861431122 0.000973234651610255
0.811659216880798 0.000973234651610255
0.822869956493378 0.000729926687199622
0.829596340656281 0.000729926687199622
0.836322784423828 0.000729926687199622
0.845291495323181 0.000729926687199622
0.85650223493576 0.000729926687199622
0.863228678703308 0.000729926687199622
0.874439477920532 0.000729926687199622
0.883408069610596 0.000729926687199622
0.887892425060272 0.000486617325805128
0.894618809223175 0.000486617325805128
0.903587460517883 0.000486617325805128
0.905829608440399 0.000486617325805128
0.908071756362915 0.000243308662902564
0.923766791820526 0.000243308662902564
0.926008939743042 0.000243308662902564
0.930493295192719 0
0.939461886882782 0
0.950672626495361 0
0.961883425712585 0
0.968609869480133 0
0.984304904937744 0
0.991031408309937 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0195266548544168 0.120194643735886
0.031656738370657 0.0836984142661095
0.0458579882979393 0.0666666254401207
0.0553254336118698 0.058880802243948
0.0692308023571968 0.0527980849146843
0.0819527432322502 0.0489050783216953
0.0911242812871933 0.0462286807596684
0.101775117218494 0.0437956415116787
0.11390532553196 0.0406325720250607
0.124852016568184 0.0345498248934746
0.135798722505569 0.0316301845014095
0.147632896900177 0.028953779488802
0.163017749786377 0.0274939239025116
0.173076927661896 0.0260340590029955
0.182544454932213 0.0250608455389738
0.193491131067276 0.023357667028904
0.207100555300713 0.0226277261972427
0.215680435299873 0.022141108289361
0.223964497447014 0.0214112009853125
0.233431875705719 0.0211678650230169
0.245265856385231 0.0187348052859306
0.257100403308868 0.0184914954006672
0.265384286642075 0.0184914954006672
0.274851351976395 0.0184914954006672
0.284615695476532 0.0184914954006672
0.293490827083588 0.0180048607289791
0.302662700414658 0.0180048607289791
0.311834812164307 0.0177615508437157
0.323076635599136 0.0172749422490597
0.336981952190399 0.0172749422490597
0.348224848508835 0.0172749422490597
0.357396513223648 0.0163017138838768
0.367159843444824 0.0160584058612585
0.377218782901764 0.0160584058612585
0.385503113269806 0.0158151015639305
0.394674569368362 0.0138686159625649
0.399999797344208 0.0131386909633875
0.41242578625679 0.0126520777121186
0.42100590467453 0.012408759444952
0.430769234895706 0.0119221359491348
0.439349174499512 0.0109488973394036
0.449999988079071 0.00997565872967243
0.458579957485199 0.00997565872967243
0.469230800867081 0.00973235163837671
0.480473339557648 0.00924573466181755
0.491124123334885 0.00900242570787668
0.500887036323547 0.00851580966264009
0.508284032344818 0.00827249884605408
0.518046855926514 0.00802918616682291
0.527810454368591 0.00705596292391419
0.5375736951828 0.00656934408470988
0.547337472438812 0.00608272943645716
0.555620968341827 0.00583942048251629
0.567455887794495 0.00583942048251629
0.575147807598114 0.00583942048251629
0.582838475704193 0.00486618652939796
0.592899441719055 0.00413624756038189
0.606508016586304 0.00389294675551355
0.617454767227173 0.00364963035099208
0.630178511142731 0.00364963035099208
0.639053106307983 0.00340632698498666
0.648816287517548 0.00291970977559686
0.661539494991302 0.00291970977559686
0.67159777879715 0.00267639686353505
0.68372768163681 0.00218977825716138
0.694082677364349 0.00218977825716138
0.704734027385712 0.00218977825716138
0.714497447013855 0.00170316232834011
0.726330935955048 0.00170316232834011
0.736685812473297 0.00170316232834011
0.746153831481934 0.00145985302515328
0.755029737949371 0.00121654500253499
0.762721598148346 0.00121654500253499
0.773076951503754 0.000973234651610255
0.7837273478508 0.000973234651610255
0.792307794094086 0.000973234651610255
0.802071392536163 0.000973234651610255
0.814497172832489 0.000729926687199622
0.827515244483948 0.000729926687199622
0.836686253547668 0.000729926687199622
0.844674408435822 0.000729926687199622
0.855029702186584 0.000729926687199622
0.862721800804138 0.000729926687199622
0.869822442531586 0.000729926687199622
0.878994345664978 0.000729926687199622
0.886686384677887 0.000486617325805128
0.8937868475914 0.000486617325805128
0.900295853614807 0.000486617325805128
0.907692134380341 0.000486617325805128
0.916272282600403 0.000243308662902564
0.923668622970581 0.000243308662902564
0.931952595710754 0.000243308662902564
0.940828561782837 0
0.947632968425751 0
0.953846156597137 0
0.966568052768707 0
0.972189247608185 0
0.981952667236328 0
0.989349126815796 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/mixed_0.67/pass2path/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{indianred1967882}{RGB}{196,78,82}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumseagreen85168104}{RGB}{85,168,104}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{FNR},
xmajorgrids,
xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{FPR},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
\addplot [very thick, steelblue76114176, mark=+, mark size=5, mark options={solid}]
table {%
0.0757000371813774 0.313599893450737
0.092199981212616 0.306399983167648
0.104799903929234 0.299699929356575
0.115399979054928 0.292900052666664
0.125999912619591 0.286300054192543
0.13620038330555 0.277199968695641
0.145599529147148 0.266300064325333
0.15640015900135 0.252499990165234
0.166300117969513 0.235199995338917
0.176000192761421 0.216700010001659
0.186300128698349 0.198099999129772
0.197600066661835 0.179600004851818
0.208099856972694 0.162399986386299
0.217300072312355 0.145000021159649
0.225700095295906 0.130100008845329
0.235599994659424 0.1148999966681
0.245800629258156 0.102300003170967
0.255799889564514 0.0891999952495098
0.264899283647537 0.076599982380867
0.274000287055969 0.0682999983429909
0.285000026226044 0.0588000040501356
0.293799430131912 0.0505999993532896
0.3048996925354 0.0454000022262335
0.313601136207581 0.0394999986514449
0.323200106620789 0.0339000012725592
0.333000183105469 0.0300000036135316
0.342999368906021 0.0253000041469932
0.352199494838715 0.0212000017054379
0.361799210309982 0.0191000013612211
0.373300135135651 0.0161999999545515
0.384300500154495 0.0141999986022711
0.392700403928757 0.0114000007510185
0.403200656175613 0.0101000007707626
0.412799745798111 0.0091000022366643
0.42160040140152 0.00800000047311187
0.431200534105301 0.00709999864920974
0.439199805259705 0.00679999920539558
0.449299991130829 0.00600000014528632
0.457899808883667 0.00529999947175384
0.467999964952469 0.00520000010728836
0.478200137615204 0.00460000028833747
0.487899959087372 0.00440000044181943
0.495600670576096 0.00410000002011657
0.502998650074005 0.0039000001270324
0.511800527572632 0.00359999965876341
0.521501243114471 0.00349999964237213
0.530599534511566 0.00319999970961362
0.540199518203735 0.00289999966043979
0.550297856330872 0.00239999935729429
0.560801148414612 0.00209999919170514
0.571699380874634 0.00179999932879582
0.581398963928223 0.00159999913303182
0.590199589729309 0.00119999923044816
0.599500119686127 0.0010999992955476
0.608001828193665 0.000699999451171607
0.617799460887909 0.000599999516271055
0.627701580524445 0.000499999686144292
0.637601017951965 0.000299999804701656
0.64840179681778 0.000199999869801104
0.658299505710602 9.9999934900552e-05
0.667300164699554 0
0.678099393844604 0
0.687299847602844 0
0.696099579334259 0
0.706599414348602 0
0.717700242996216 0
0.726998805999756 0
0.737100541591644 0
0.746100544929504 0
0.756199240684509 0
0.763799905776978 0
0.772300779819489 0
0.780700027942657 0
0.791199386119843 0
0.799499034881592 0
0.809900164604187 0
0.820099413394928 0
0.830101370811462 0
0.839200973510742 0
0.846800804138184 0
0.85569953918457 0
0.865500211715698 0
0.874100029468536 0
0.882699906826019 0
0.890200316905975 0
0.897799611091614 0
0.90559983253479 0
0.912900388240814 0
0.920600175857544 0
0.928400218486786 0
0.935799598693848 0
0.943199992179871 0
0.949599981307983 0
0.956099987030029 0
0.963399827480316 0
0.972599983215332 0
0.977800011634827 0
0.985199928283691 0
0.992699980735779 0
};
\addlegendentry{averaged}
\addplot [very thick, peru22113282, mark=+, mark size=5, mark options={solid}]
table {%
0.809139966964722 0.313599893450737
0.838709831237793 0.306399983167648
0.853494703769684 0.299699929356575
0.86827939748764 0.292900052666664
0.875 0.286300054192543
0.88172060251236 0.277199968695641
0.889785051345825 0.266300064325333
0.897849440574646 0.252499990165234
0.903225779533386 0.235199995338917
0.903225779533386 0.216700010001659
0.905913949012756 0.198099999129772
0.907258093357086 0.179600004851818
0.907258093357086 0.162399986386299
0.909946143627167 0.145000021159649
0.913978517055511 0.130100008845329
0.915322601795197 0.1148999966681
0.918010771274567 0.102300003170967
0.918010771274567 0.0891999952495098
0.918010771274567 0.076599982380867
0.919354856014252 0.0682999983429909
0.922043025493622 0.0588000040501356
0.923387110233307 0.0505999993532896
0.924731254577637 0.0454000022262335
0.924731254577637 0.0394999986514449
0.924731254577637 0.0339000012725592
0.926075279712677 0.0300000036135316
0.927419364452362 0.0253000041469932
0.928763449192047 0.0212000017054379
0.928763449192047 0.0191000013612211
0.930107533931732 0.0161999999545515
0.931451618671417 0.0141999986022711
0.932795703411102 0.0114000007510185
0.935483872890472 0.0101000007707626
0.935483872890472 0.0091000022366643
0.935483872890472 0.00800000047311187
0.935483872890472 0.00709999864920974
0.935483872890472 0.00679999920539558
0.938172042369843 0.00600000014528632
0.939516127109528 0.00529999947175384
0.940860211849213 0.00520000010728836
0.943548381328583 0.00460000028833747
0.943548381328583 0.00440000044181943
0.943548381328583 0.00410000002011657
0.943548381328583 0.0039000001270324
0.943548381328583 0.00359999965876341
0.944892466068268 0.00349999964237213
0.946236550807953 0.00319999970961362
0.946236550807953 0.00289999966043979
0.946236550807953 0.00239999935729429
0.946236550807953 0.00209999919170514
0.946236550807953 0.00179999932879582
0.950268805027008 0.00159999913303182
0.950268805027008 0.00119999923044816
0.952956974506378 0.0010999992955476
0.952956974506378 0.000699999451171607
0.954301059246063 0.000599999516271055
0.954301059246063 0.000499999686144292
0.955645143985748 0.000299999804701656
0.955645143985748 0.000199999869801104
0.955645143985748 9.9999934900552e-05
0.955645143985748 0
0.955645143985748 0
0.955645143985748 0
0.956989228725433 0
0.958333313465118 0
0.958333313465118 0
0.958333313465118 0
0.963709652423859 0
0.966397821903229 0
0.967741906642914 0
0.967741906642914 0
0.970430135726929 0
0.970430135726929 0
0.971774220466614 0
0.974462389945984 0
0.978494644165039 0
0.978494644165039 0
0.979838728904724 0
0.981182813644409 0
0.981182813644409 0
0.982526898384094 0
0.985215067863464 0
0.986559152603149 0
0.987903237342834 0
0.990591406822205 0
0.990591406822205 0
0.990591406822205 0
0.990591406822205 0
0.990591406822205 0
0.990591406822205 0
0.990591406822205 0
0.990591406822205 0
0.993279576301575 0
0.99462366104126 0
0.99462366104126 0
0.99462366104126 0
0.99462366104126 0
0.995967745780945 0
0.998655915260315 0
};
\addlegendentry{easy}
\addplot [very thick, mediumseagreen85168104, mark=+, mark size=5, mark options={solid}]
table {%
0.0573689416050911 0.313599893450737
0.0979228094220161 0.306399983167648
0.118694365024567 0.299699929356575
0.1315528601408 0.292900052666664
0.144411563873291 0.286300054192543
0.154302671551704 0.277199968695641
0.164193898439407 0.266300064325333
0.181998118758202 0.252499990165234
0.191889241337776 0.235199995338917
0.205736890435219 0.216700010001659
0.216617181897163 0.198099999129772
0.226508378982544 0.179600004851818
0.234421372413635 0.162399986386299
0.239366963505745 0.145000021159649
0.247279867529869 0.130100008845329
0.25717094540596 0.1148999966681
0.270029604434967 0.102300003170967
0.277942568063736 0.0891999952495098
0.287833780050278 0.076599982380867
0.295746684074402 0.0682999983429909
0.308605343103409 0.0588000040501356
0.316518247127533 0.0505999993532896
0.331355005502701 0.0454000022262335
0.336300700902939 0.0394999986514449
0.344213575124741 0.0339000012725592
0.357072085142136 0.0300000036135316
0.367952406406403 0.0253000041469932
0.378832906484604 0.0212000017054379
0.381800204515457 0.0191000013612211
0.391691237688065 0.0161999999545515
0.39960440993309 0.0141999986022711
0.406528204679489 0.0114000007510185
0.418397665023804 0.0101000007707626
0.429277926683426 0.0091000022366643
0.440158247947693 0.00800000047311187
0.450049459934235 0.00709999864920974
0.461918860673904 0.00679999920539558
0.477744817733765 0.00600000014528632
0.486646890640259 0.00529999947175384
0.493570923805237 0.00520000010728836
0.503462314605713 0.00460000028833747
0.51236367225647 0.00440000044181943
0.514341771602631 0.00410000002011657
0.518299162387848 0.0039000001270324
0.530168533325195 0.00359999965876341
0.538081109523773 0.00349999964237213
0.544016480445862 0.00319999970961362
0.560831069946289 0.00289999966043979
0.567754924297333 0.00239999935729429
0.576656639575958 0.00209999919170514
0.586548209190369 0.00179999932879582
0.595450043678284 0.00159999913303182
0.60138475894928 0.00119999923044816
0.607319235801697 0.0010999992955476
0.620178163051605 0.000699999451171607
0.633036613464355 0.000599999516271055
0.640949487686157 0.000499999686144292
0.648863196372986 0.000299999804701656
0.657764375209808 0.000199999869801104
0.663699328899384 9.9999934900552e-05
0.676557600498199 0
0.683481574058533 0
0.688426911830902 0
0.696340143680573 0
0.707220673561096 0
0.718100905418396 0
0.728981196880341 0
0.736894369125366 0
0.744806945323944 0
0.75469833612442 0
0.762611150741577 0
0.769535064697266 0
0.775470077991486 0
0.788328170776367 0
0.796241462230682 0
0.807121634483337 0
0.814045488834381 0
0.823936581611633 0
0.830860555171967 0
0.836795151233673 0
0.842729985713959 0
0.851631939411163 0
0.859544992446899 0
0.867457985877991 0
0.877349138259888 0
0.882294833660126 0
0.894164144992828 0
0.901088058948517 0
0.908011913299561 0
0.911968410015106 0
0.923837780952454 0
0.928783357143402 0
0.935707211494446 0
0.947576582431793 0
0.95944607257843 0
0.967359066009521 0
0.97428286075592 0
0.983184993267059 0
0.990108788013458 0
};
\addlegendentry{medium}
\addplot [very thick, indianred1967882, mark=+, mark size=5, mark options={solid}]
table {%
0.0117646995931864 0.313599893450737
0.0241358391940594 0.306399983167648
0.0355367213487625 0.299699929356575
0.045482125133276 0.292900052666664
0.0561552420258522 0.286300054192543
0.0667069107294083 0.277199968695641
0.0761673450469971 0.266300064325333
0.0863553360104561 0.252499990165234
0.0966647192835808 0.235199995338917
0.106731355190277 0.216700010001659
0.117647081613541 0.198099999129772
0.130017846822739 0.179600004851818
0.141782596707344 0.162399986386299
0.152092203497887 0.145000021159649
0.160946235060692 0.130100008845329
0.171618804335594 0.1148999966681
0.182171121239662 0.102300003170967
0.193329304456711 0.0891999952495098
0.20315346121788 0.076599982380867
0.213098883628845 0.0682999983429909
0.22462098300457 0.0588000040501356
0.234202370047569 0.0505999993532896
0.245724573731422 0.0454000022262335
0.255670726299286 0.0394999986514449
0.26634293794632 0.0339000012725592
0.276531338691711 0.0300000036135316
0.287204653024673 0.0253000041469932
0.29690757393837 0.0212000017054379
0.308186769485474 0.0191000013612211
0.320799976587296 0.0161999999545515
0.333050191402435 0.0141999986022711
0.342267900705338 0.0114000007510185
0.353304505348206 0.0101000007707626
0.363614201545715 0.0091000022366643
0.372953295707703 0.00800000047311187
0.383383721113205 0.00709999864920974
0.391631484031677 0.00679999920539558
0.401698112487793 0.00600000014528632
0.410915642976761 0.00529999947175384
0.42219540476799 0.00520000010728836
0.433110982179642 0.00460000028833747
0.443784236907959 0.00440000044181943
0.452880412340164 0.00410000002011657
0.461370557546616 0.0039000001270324
0.470588237047195 0.00359999965876341
0.481261253356934 0.00349999964237213
0.491449534893036 0.00319999970961362
0.501031935214996 0.00289999966043979
0.512431800365448 0.00239999935729429
0.524074614048004 0.00209999919170514
0.536082148551941 0.00179999932879582
0.546392977237701 0.00159999913303182
0.556339025497437 0.00119999923044816
0.566646456718445 0.0010999992955476
0.575378656387329 0.000699999451171607
0.585567593574524 0.000599999516271055
0.596603631973267 0.000499999686144292
0.607520699501038 0.000299999804701656
0.619527280330658 0.000199999869801104
0.630807280540466 9.9999934900552e-05
0.640145182609558 0
0.652395248413086 0
0.662948548793793 0
0.672529339790344 0
0.683807790279388 0
0.695936441421509 0
0.705882430076599 0
0.71667605638504 0
0.726380467414856 0
0.73729544878006 0
0.745542824268341 0
0.754760563373566 0
0.76422131061554 0
0.775257706642151 0
0.784111440181732 0
0.795027375221252 0
0.80654913187027 0
0.817343354225159 0
0.827410638332367 0
0.835900664329529 0
0.845845937728882 0
0.85639762878418 0
0.865736663341522 0
0.875076055526733 0
0.882716774940491 0
0.891328155994415 0
0.899332940578461 0
0.907337725162506 0
0.915827870368958 0
0.924802899360657 0
0.93232274055481 0
0.940691351890564 0
0.947362065315247 0
0.953668832778931 0
0.961067378520966 0
0.971255242824554 0
0.976713180541992 0
0.984475433826447 0
0.992480278015137 0
};
\addlegendentry{hard}
\end{axis}

\end{tikzpicture}


==> figure/random_generated/Alg_gen/trade-off_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
% legend cell align={left},
% legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick pos=left,
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
xmajorgrids,
% xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
ymajorgrids,
ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
% \addplot [very thick, steelblue76114176, mark=*, mark size=5, mark options={solid}]
% table {%
% 0.0109000029042363 0
% 0.0234000254422426 0
% 0.0325000360608101 0
% 0.0449000336229801 0
% 0.0553000122308731 0
% 0.0651999786496162 0
% 0.0753001272678375 0
% 0.0841998681426048 0
% 0.097100093960762 0
% 0.105100125074387 0
% 0.114099949598312 0
% 0.12440025806427 0
% 0.135399505496025 0
% 0.145499974489212 0
% 0.154100373387337 0
% 0.16539990901947 0
% 0.174600213766098 0
% 0.184299871325493 0
% 0.194899812340736 0
% 0.205400004982948 0
% 0.214700073003769 0
% 0.223999753594398 0
% 0.233300104737282 0
% 0.243299946188927 0
% 0.254599511623383 0
% 0.266299694776535 0
% 0.275999963283539 0
% 0.284801125526428 0
% 0.293800115585327 0
% 0.303598970174789 0
% 0.313800513744354 0
% 0.324499636888504 0
% 0.333400189876556 0
% 0.343100696802139 0
% 0.353399187326431 0
% 0.363600820302963 0
% 0.371500194072723 0
% 0.38000026345253 0
% 0.390599340200424 0
% 0.399500072002411 0
% 0.408400058746338 0
% 0.416299909353256 0
% 0.426799803972244 0
% 0.435400485992432 0
% 0.444199800491333 0
% 0.454699903726578 0
% 0.464399844408035 0
% 0.475100010633469 0
% 0.486799985170364 0
% 0.496400088071823 0
% 0.505700170993805 0
% 0.515601933002472 0
% 0.525799930095673 0
% 0.537900626659393 0
% 0.547900438308716 0
% 0.557297766208649 0
% 0.568399369716644 0
% 0.578399538993835 0
% 0.589200019836426 0
% 0.598397612571716 0
% 0.608499705791473 0
% 0.618101596832275 0
% 0.628900706768036 0
% 0.638098478317261 0
% 0.64639937877655 0
% 0.656799733638763 0
% 0.667000889778137 0
% 0.677699685096741 0
% 0.68740040063858 0
% 0.697500169277191 0
% 0.708299815654755 0
% 0.717699468135834 0
% 0.728898286819458 0
% 0.739700496196747 0
% 0.750000953674316 0
% 0.759600758552551 0
% 0.769299745559692 0
% 0.780400991439819 0
% 0.790400624275208 0
% 0.799498736858368 0
% 0.8084996342659 0
% 0.818200290203094 0
% 0.829200208187103 0
% 0.838900208473206 0
% 0.848301351070404 0
% 0.859299600124359 0
% 0.871299624443054 0
% 0.882800221443176 0
% 0.891799807548523 0
% 0.902600288391113 0
% 0.910699605941772 0
% 0.921300292015076 0
% 0.931400001049042 0
% 0.941299736499786 0
% 0.951000094413757 0
% 0.960899889469147 0
% 0.97020012140274 0
% 0.981400012969971 0
% 0.990400016307831 0
% };
% \addlegendentry{num(X)=1, malicous user=F}
\addplot [very thick, steelblue76114176, mark=*, mark size=5, mark options={solid}]
table {%
0.0109000029042363 0
0.0234000254422426 0
0.0325000360608101 0
0.0449000336229801 0
0.0553000122308731 0
0.0651999786496162 0
0.0753001272678375 0
0.0841998681426048 0
0.097100093960762 0
0.105100125074387 0
0.114099949598312 0
0.12440025806427 0
0.135399505496025 0
0.145499974489212 0
0.154100373387337 0
0.16539990901947 0
0.174600213766098 0
0.184299871325493 0
0.194899812340736 0
0.205400004982948 0
0.214700073003769 0
0.223999753594398 0
0.233300104737282 0
0.243299946188927 0
0.254599511623383 0
0.266299694776535 0
0.275999963283539 0
0.284801125526428 0
0.293800115585327 0
0.303598970174789 0
0.313800513744354 0
0.324499636888504 0
0.333400189876556 0
0.343100696802139 0
0.353399187326431 0
0.363600820302963 0
0.371500194072723 0
0.38000026345253 0
0.390599340200424 0
0.399500072002411 0
0.408400058746338 0
0.416299909353256 0
0.426799803972244 0
0.435400485992432 0
0.444199800491333 0
0.454699903726578 0
0.464399844408035 0
0.475100010633469 0
0.486799985170364 0
0.496400088071823 0
0.505700170993805 0
0.515601933002472 0
0.525799930095673 0
0.537900626659393 0
0.547900438308716 0
0.557297766208649 0
0.568399369716644 0
0.578399538993835 0
0.589200019836426 0
0.598397612571716 0
0.608499705791473 0
0.618101596832275 0
0.628900706768036 0
0.638098478317261 0
0.64639937877655 0
0.656799733638763 0
0.667000889778137 0
0.677699685096741 0
0.68740040063858 0
0.697500169277191 0
0.708299815654755 0
0.717699468135834 0
0.728898286819458 0
0.739700496196747 0
0.750000953674316 0
0.759600758552551 0
0.769299745559692 0
0.780400991439819 0
0.790400624275208 0
0.799498736858368 0
0.8084996342659 0
0.818200290203094 0
0.829200208187103 0
0.838900208473206 0
0.848301351070404 0
0.859299600124359 0
0.871299624443054 0
0.882800221443176 0
0.891799807548523 0
0.902600288391113 0
0.910699605941772 0
0.921300292015076 0
0.931400001049042 0
0.941299736499786 0
0.951000094413757 0
0.960899889469147 0
0.97020012140274 0
0.981400012969971 0
0.990400016307831 0
};
% \addlegendentry{num(X)=1, malicous user=T}
\end{axis}

\end{tikzpicture}


==> figure/random_generated/Alg_gen/trade-off_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{peru22113282}{RGB}{221,132,82}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkslategray38},
% legend cell align={left},
% legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick pos=left,
tick align=outside,
x grid style={lightgray204},
xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
xmajorgrids,
% xmajorticks=false,
xmin=-0.01, xmax=1.01,
xtick style={color=darkslategray38},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
ymajorgrids,
% ymajorticks=false,
ymin=-0.01, ymax=1.01,
ytick style={color=darkslategray38}
]
% \addplot [very thick, steelblue76114176, mark=*, mark size=5, mark options={solid}]
% table {%
% 0.0551999807357788 0
% 0.104399830102921 0
% 0.153600201010704 0
% 0.203500136733055 0
% 0.256399422883987 0
% 0.305600136518478 0
% 0.354499667882919 0
% 0.400999844074249 0
% 0.44979989528656 0
% 0.498500108718872 0
% 0.547301292419434 0
% 0.597000539302826 0
% 0.650499939918518 0
% 0.69830048084259 0
% 0.750100612640381 0
% 0.797300755977631 0
% 0.850900113582611 0
% 0.900400578975677 0
% 0.952099919319153 0
% };
% \addlegendentry{num(X)=1, malicous user=F}
\addplot [very thick, steelblue76114176, mark=*, mark size=5, mark options={solid}]
table {%
0.0551999807357788 0
0.104399830102921 0
0.153600201010704 0
0.203500136733055 0
0.256399422883987 0
0.305600136518478 0
0.354499667882919 0
0.400999844074249 0
0.44979989528656 0
0.498500108718872 0
0.547301292419434 0
0.597000539302826 0
0.650499939918518 0
0.69830048084259 0
0.750100612640381 0
0.797300755977631 0
0.850900113582611 0
0.900400578975677 0
0.952099919319153 0
};
% \addlegendentry{num(X)=1, malicous user=T}
\end{axis}

\end{tikzpicture}


==> figure/random_generated/Alg_gen_/trade_off_curve_100.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

\definecolor{black25}{RGB}{25,25,25}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
    axis line style={darkslategray38},
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(0.99,0.99)},
      anchor=north east,
      draw=lightgray204
    },
    tick align=outside,
    x grid style={lightgray204},
    %ylabel=\textcolor{darkslategray38}{Probability},
    xmajorgrids,
    % xmajorticks=false,
    xmin=0.55, xmax=10.45,
    xtick pos=bottom,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    %ylabel=\textcolor{darkslategray38}{Probability},
    ymajorgrids,
    % ymajorticks=false,
    ymin=-.01, ymax=1.01,   
    ytick pos=left,
    ytick style={color=darkslategray38}
    ]
\addplot [line width=2, black25]
table {%
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
};
%\addlegendentry{\fpProbWOParams ($\attackBudget=10$)}
\addplot [line width=2, black25, dashed]
table {%
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
};
%\addlegendentry{\fpProbWOParams ($\attackBudget=100$)}
\addplot [line width=2, black25, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
};
%\addlegendentry{\fpProbWOParams ($\attackBudget=1000$)}
\addplot [line width=2, black25, mark=x, mark size=3, mark options={solid}]
table {%
1 0.0109000029042363
2 0.0234000254422426
3 0.0325000360608101
4 0.0449000336229801
5 0.0553000122308731
6 0.0651999786496162
7 0.0753001272678375
8 0.0841998681426048
9 0.097100093960762
10 0.105100125074387
};
%\addlegendentry{\fnProbWOParams}
\end{axis}

\end{tikzpicture}


==> figure/random_generated/Alg_gen_/trade_off_curve_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

\definecolor{black25}{RGB}{25,25,25}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
    axis line style={darkslategray38},
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(0.99,0.99)},
      anchor=north east,
      draw=lightgray204
    },
    tick align=outside,
    x grid style={lightgray204},
    %ylabel=\textcolor{darkslategray38}{Probability},
    xmajorgrids,
    % xmajorticks=false,
    xmin=0.55, xmax=10.45,
    xtick pos=bottom,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    %ylabel=\textcolor{darkslategray38}{Probability},
    ymajorgrids,
    % ymajorticks=false,
    ymin=-.01, ymax=1.01,   
    ytick pos=left,
    ytick style={color=darkslategray38}
    ]
\addplot [line width=2, black25]
table {%
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
};
%\addlegendentry{\fpProbWOParams ($\attackBudget=10$)}
\addplot [line width=2, black25, dashed]
table {%
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
};
%\addlegendentry{\fpProbWOParams ($\attackBudget=100$)}
\addplot [line width=2, black25, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
};
%\addlegendentry{\fpProbWOParams ($\attackBudget=1000$)}
\addplot [line width=2, black25, mark=x, mark size=3, mark options={solid}]
table {%
1 0.0551999807357788
2 0.104399830102921
3 0.153600201010704
4 0.203500136733055
5 0.256399422883987
6 0.305600136518478
7 0.354499667882919
8 0.400999844074249
9 0.44979989528656
10 0.498500108718872
};
%\addlegendentry{\fnProbWOParams}
\end{axis}

\end{tikzpicture}


==> figure/random_generated/RNN/trade-off_100.tex <==
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
     ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
%     \addplot [very thick, steelblue76114176, mark=*, mark size=5, mark options={solid}]
% table {%
% 0.988200008869171 0.996399998664856
% 0.999400019645691 0.968400180339813
% 1 0.894200801849365
% 1 0.749200224876404
% 1 0.56979888677597
% 1 0.382099866867065
% 1 0.231899946928024
% 1 0.119799979031086
% 1 0.0562000311911106
% 1 0.0257999934256077
% 1 0.0105000045150518
% 1 0.00299999746493995
% 1 0.00119999900925905
% 1 0.000499999907333404
% 1 0.000199999834876508
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% };
% \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
% table {%
% 0.992200016975403 0.996399998664856
% 0.999599993228912 0.968400180339813
% 1 0.894200801849365
% 1 0.749200224876404
% 1 0.56979888677597
% 1 0.382099866867065
% 1 0.231899946928024
% 1 0.119799979031086
% 1 0.0562000311911106
% 1 0.0257999934256077
% 1 0.0105000045150518
% 1 0.00299999746493995
% 1 0.00119999900925905
% 1 0.000499999907333404
% 1 0.000199999834876508
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% };
\addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
table {%
0.989000022411346 0.996399998664856
0.999499976634979 0.968400180339813
1 0.894200801849365
1 0.749200224876404
1 0.56979888677597
1 0.382099866867065
1 0.231899946928024
1 0.119799979031086
1 0.0562000311911106
1 0.0257999934256077
1 0.0105000045150518
1 0.00299999746493995
1 0.00119999900925905
1 0.000499999907333404
1 0.000199999834876508
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
};
\end{axis}

\end{tikzpicture}


==> figure/random_generated/RNN/trade-off_20.tex <==
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
     ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
%     \addplot [very thick, steelblue76114176, mark=*, mark size=5, mark options={solid}]
% table {%
% 0.997600018978119 0.646202027797699
% 0.999800026416779 0.264401257038116
% 1 0.0739002078771591
% 1 0.0141000002622604
% 1 0.0030999961309135
% 1 0.000199999834876508
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% };
% \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
% table {%
% 0.998399972915649 0.646202027797699
% 1 0.264401257038116
% 1 0.0739002078771591
% 1 0.0141000002622604
% 1 0.0030999961309135
% 1 0.000199999834876508
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% };
\addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
table {%
0.997600018978119 0.646202027797699
0.999800026416779 0.264401257038116
1 0.0739002078771591
1 0.0141000002622604
1 0.0030999961309135
1 0.000199999834876508
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
};
\end{axis}

\end{tikzpicture}


==> figure/random_generated/RNN_/trade-off_100.tex <==
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
     ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
%     \addplot [very thick, steelblue76114176, mark=*, mark size=5, mark options={solid}]
% table {%
% 0.778801262378693 0.451599895954132
% 0.867900609970093 0.114500045776367
% 0.904801189899445 0.0190000236034393
% 0.928099989891052 0.00220000138506293
% 0.943400263786316 0.000399999058572575
% 0.95419979095459 9.99997646431439e-05
% 0.962699830532074 0
% 0.967999994754791 0
% 0.972299993038177 0
% 0.975399971008301 0
% 0.977799892425537 0
% 0.979499995708466 0
% 0.98089998960495 0
% 0.981400012969971 0
% 0.982100009918213 0
% 0.982899904251099 0
% 0.983399987220764 0
% 0.98419988155365 0
% 0.984499990940094 0
% 0.984899997711182 0
% 0.985599994659424 0
% 0.986200094223022 0
% 0.986500024795532 0
% 0.986799895763397 0
% 0.986899971961975 0
% 0.986999988555908 0
% 0.987500011920929 0
% 0.987800002098083 0
% 0.988099992275238 0
% 0.988600015640259 0
% 0.98879998922348 0
% 0.989099979400635 0
% 0.989300012588501 0
% 0.989600002765656 0
% 0.98989999294281 0
% 0.990000009536743 0
% 0.990199983119965 0
% 0.990299999713898 0
% 0.990700006484985 0
% 0.991500020027161 0
% 0.99210000038147 0
% 0.992500007152557 0
% 0.992999970912933 0
% 0.993399977684021 0
% 0.994099974632263 0
% 0.994599997997284 0
% 0.994799971580505 0
% 0.995100021362305 0
% 0.995899975299835 0
% 0.995999991893768 0
% 0.996500015258789 0
% 0.996900022029877 0
% 0.997099995613098 0
% 0.997200012207031 0
% 0.997399985790253 0
% 0.997600018978119 0
% 0.998399972915649 0
% 0.998700022697449 0
% 0.998799979686737 0
% 0.999000012874603 0
% 0.999199986457825 0
% 0.999199986457825 0
% 0.999599993228912 0
% 0.999700009822845 0
% 0.999700009822845 0
% 0.999700009822845 0
% 0.999800026416779 0
% 0.999800026416779 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% };
% \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
% table {%
% 0.80359947681427 0.451599895954132
% 0.890999615192413 0.114500045776367
% 0.925199806690216 0.0190000236034393
% 0.945899903774261 0.00220000138506293
% 0.957400023937225 0.000399999058572575
% 0.965900003910065 9.99997646431439e-05
% 0.972000002861023 0
% 0.975900113582611 0
% 0.979099988937378 0
% 0.980400025844574 0
% 0.981899976730347 0
% 0.982900023460388 0
% 0.983500003814697 0
% 0.984099984169006 0
% 0.984499990940094 0
% 0.984799981117249 0
% 0.985000014305115 0
% 0.985400021076202 0
% 0.985499978065491 0
% 0.985700011253357 0
% 0.986100077629089 0
% 0.986500024795532 0
% 0.986699879169464 0
% 0.986800014972687 0
% 0.986899971961975 0
% 0.986999988555908 0
% 0.987399995326996 0
% 0.98769998550415 0
% 0.987999975681305 0
% 0.988499999046326 0
% 0.988699972629547 0
% 0.989199995994568 0
% 0.989400029182434 0
% 0.989700019359589 0
% 0.990000009536743 0
% 0.990100026130676 0
% 0.990299999713898 0
% 0.990499973297119 0
% 0.990800023078918 0
% 0.991599977016449 0
% 0.99210000038147 0
% 0.992399990558624 0
% 0.992900013923645 0
% 0.993300020694733 0
% 0.994199991226196 0
% 0.994599997997284 0
% 0.994799971580505 0
% 0.995199978351593 0
% 0.996100008487701 0
% 0.996200025081635 0
% 0.996800005435944 0
% 0.997399985790253 0
% 0.997500002384186 0
% 0.997600018978119 0
% 0.99779999256134 0
% 0.998099982738495 0
% 0.998600006103516 0
% 0.99889999628067 0
% 0.999100029468536 0
% 0.999300003051758 0
% 0.999300003051758 0
% 0.999300003051758 0
% 0.999700009822845 0
% 0.999800026416779 0
% 0.999800026416779 0
% 0.999800026416779 0
% 0.999899983406067 0
% 0.999899983406067 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% 1 0
% };
\addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
table {%
0.784899950027466 0.451599895954132
0.874600172042847 0.114500045776367
0.910600006580353 0.0190000236034393
0.93280017375946 0.00220000138506293
0.947500109672546 0.000399999058572575
0.957999885082245 9.99997646431439e-05
0.965900003910065 0
0.970700025558472 0
0.974900007247925 0
0.977700173854828 0
0.97979998588562 0
0.981199979782104 0
0.982400119304657 0
0.982900023460388 0
0.983399987220764 0
0.983999907970428 0
0.984600007534027 0
0.985099971294403 0
0.985400021076202 0
0.98580002784729 0
0.986500024795532 0
0.986999988555908 0
0.987299978733063 0
0.987500011920929 0
0.987600028514862 0
0.98769998550415 0
0.988199889659882 0
0.988499999046326 0
0.98879998922348 0
0.989300012588501 0
0.989499986171722 0
0.989799976348877 0
0.990000009536743 0
0.990299999713898 0
0.990599989891052 0
0.990700006484985 0
0.990899980068207 0
0.99099999666214 0
0.991299986839294 0
0.991999983787537 0
0.992500007152557 0
0.992799997329712 0
0.993300020694733 0
0.99370002746582 0
0.994400024414062 0
0.994899988174438 0
0.995100021362305 0
0.995400011539459 0
0.996200025081635 0
0.996299982070923 0
0.996800005435944 0
0.997200012207031 0
0.997399985790253 0
0.997500002384186 0
0.997699975967407 0
0.997900009155273 0
0.998499989509583 0
0.998799979686737 0
0.99889999628067 0
0.999100029468536 0
0.999300003051758 0
0.999300003051758 0
0.999700009822845 0
0.999800026416779 0
0.999800026416779 0
0.999800026416779 0
0.999899983406067 0
0.999899983406067 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
1 0
};
\end{axis}

\end{tikzpicture}


==> figure/random_generated/RNN_/trade-off_20.tex <==
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
     ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
%     \addplot [very thick, steelblue76114176, mark=*, mark size=5, mark options={solid}]
% table {%
% 0.902100086212158 0.108199998736382
% 0.960899591445923 0.00469999015331268
% 0.97759997844696 9.99997646431439e-05
% 0.98360002040863 0
% 0.98580002784729 0
% 0.98769998550415 0
% 0.989400029182434 0
% 0.991900026798248 0
% 0.993399977684021 0
% 0.994799971580505 0
% 0.996500015258789 0
% 0.997600018978119 0
% 0.998399972915649 0
% 0.99889999628067 0
% 0.999499976634979 0
% 0.999800026416779 0
% 0.999800026416779 0
% 0.999899983406067 0
% 0.999899983406067 0
% };
% \addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
% table {%
% 0.917400002479553 0.108199998736382
% 0.967899978160858 0.00469999015331268
% 0.981199979782104 9.99997646431439e-05
% 0.985000014305115 0
% 0.986599981784821 0
% 0.988199889659882 0
% 0.990000009536743 0
% 0.992500007152557 0
% 0.993900001049042 0
% 0.995400011539459 0
% 0.996999979019165 0
% 0.99779999256134 0
% 0.998499989509583 0
% 0.99889999628067 0
% 0.999400019645691 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% 0.999899983406067 0
% };
\addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
table {%
0.905799984931946 0.108199998736382
0.962400019168854 0.00469999015331268
0.978500008583069 9.99997646431439e-05
0.983799993991852 0
0.985599994659424 0
0.987399995326996 0
0.989199995994568 0
0.991599977016449 0
0.9932000041008 0
0.994700014591217 0
0.996500015258789 0
0.997600018978119 0
0.998300015926361 0
0.998799979686737 0
0.999400019645691 0
0.999800026416779 0
0.999800026416779 0
0.999899983406067 0
0.999899983406067 0
};
\end{axis}

\end{tikzpicture}


==> figure/user_chosen/RNN/trade-off_varyingX_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    
    \begin{axis}[
        axis line style={darkslategray38},
        % legend cell align={left},
        % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
        tick pos=left,
        tick align=outside,
        x grid style={lightgray204},
        % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
        xmajorgrids,
        % xmajorticks=false,
        xmin=-0.01, xmax=1.01,
        xtick style={color=darkslategray38},
        y grid style={lightgray204},
        ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
        ymajorgrids,
        % ymajorticks=false,
        ymin=-0.01, ymax=1.01,
        ytick style={color=darkslategray38}
        ]
\addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
table {%
0.586299240589142 0.643299698829651
0.637000858783722 0.259601205587387
0.67449939250946 0.072700135409832
0.709499478340149 0.0134999882429838
0.742099046707153 0.00210000388324261
0.773300468921661 0.000199999834876508
0.799500703811646 9.99997646431439e-05
0.820500016212463 0
0.841500401496887 0
0.860800385475159 0
0.878299117088318 0
0.896600008010864 0
0.91430002450943 0
0.927900016307831 0
0.941700220108032 0
0.953599989414215 0
0.966799974441528 0
0.979100108146667 0
0.990599989891052 0
};
% \addlegendentry{X=1}
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.635800421237946 0.643299698829651
0.683100044727325 0.259601205587387
0.718300223350525 0.072700135409832
0.750600516796112 0.0134999882429838
0.779901087284088 0.00210000388324261
0.809299349784851 0.000199999834876508
0.831399619579315 9.99997646431439e-05
0.850100517272949 0
0.867200016975403 0
0.883799433708191 0
0.898600101470947 0
0.913799822330475 0
0.928899824619293 0
0.94109982252121 0
0.952300012111664 0
0.962400019168854 0
0.973899781703949 0
0.983200013637543 0
0.992200016975403 0
};
% \addlegendentry{X>=1}
\end{axis}

\end{tikzpicture}


==> figure/user_chosen/RNN_/trade-off_varyingX_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
\addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
table {%
0.581499457359314 0.692100167274475
0.633500993251801 0.424899756908417
0.676001071929932 0.243699997663498
0.708200335502625 0.138600260019302
0.738399922847748 0.0771999359130859
0.767799437046051 0.0428000167012215
0.792001366615295 0.0219000186771154
0.81520003080368 0.0111000193282962
0.839199900627136 0.00479998299852014
0.858300089836121 0.00189999944996089
0.878099620342255 0.000699999742209911
0.896399974822998 0.000299999752314761
0.912899792194366 9.99997646431439e-05
0.926900207996368 0
0.940900385379791 0
0.95419979095459 0
0.967400014400482 0
0.980700016021729 0
0.99099999666214 0
};
% \addlegendentry{X=1}
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.632799386978149 0.692100167274475
0.67929995059967 0.424899756908417
0.718599200248718 0.243699997663498
0.749100506305695 0.138600260019302
0.776500284671783 0.0771999359130859
0.802599608898163 0.0428000167012215
0.824099242687225 0.0219000186771154
0.844599425792694 0.0111000193282962
0.864900767803192 0.00479998299852014
0.881700217723846 0.00189999944996089
0.898100614547729 0.000699999742209911
0.914500117301941 0.000299999752314761
0.92820018529892 9.99997646431439e-05
0.940499901771545 0
0.952600598335266 0
0.963999927043915 0
0.974399924278259 0
0.985000014305115 0
0.993300020694733 0
};
% \addlegendentry{X>=1}
\end{axis}

\end{tikzpicture}


==> figure/user_chosen/RNN_target/trade-off_varyingX_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
      axis line style={darkslategray38},
      % legend cell align={left},
      % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
      tick pos=left,
      tick align=outside,
      x grid style={lightgray204},
      % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
      xmajorgrids,
      % xmajorticks=false,
      xmin=-0.01, xmax=1.01,
      xtick style={color=darkslategray38},
      y grid style={lightgray204},
      ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
      ymajorgrids,
      % ymajorticks=false,
      ymin=-0.01, ymax=1.01,
      ytick style={color=darkslategray38}
      ]
\addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
table {%
0.532097697257996 0.86989963054657
0.608199775218964 0.581799387931824
0.660199880599976 0.295099377632141
0.703400313854218 0.112799949944019
0.73600035905838 0.0333000086247921
0.767400681972504 0.0080999843776226
0.793999850749969 0.00150000129360706
0.819499015808105 9.9999931990169e-05
0.841300368309021 9.9999931990169e-05
0.861499428749084 0
0.881300091743469 0
0.898799777030945 0
0.915799975395203 0
0.9309002161026 0
0.945999801158905 0
0.959200024604797 0
0.971399903297424 0
0.984000027179718 0
0.993099987506866 0
};
% \addlegendentry{X=1}
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.587600529193878 0.86989963054657
0.657400727272034 0.581799387931824
0.707800030708313 0.295099377632141
0.746099948883057 0.112799949944019
0.775199353694916 0.0333000086247921
0.801200389862061 0.0080999843776226
0.824899792671204 0.00150000129360706
0.847099602222443 9.9999931990169e-05
0.867100179195404 9.9999931990169e-05
0.884100019931793 0
0.900899827480316 0
0.915500223636627 0
0.929499983787537 0
0.943100392818451 0
0.955800175666809 0
0.967299997806549 0
0.977199792861938 0
0.987100005149841 0
0.994400024414062 0
};
% \addlegendentry{X>=1}
\end{axis}

\end{tikzpicture}


==> figure/user_chosen/chaffing3/trade-off_varyingX_20.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[font=\huge]

    \definecolor{darkslategray38}{RGB}{38,38,38}
    \definecolor{indianred1967882}{RGB}{196,78,82}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
    \definecolor{peru22113282}{RGB}{221,132,82}
    \definecolor{steelblue76114176}{RGB}{76,114,176}
    
    \begin{axis}[
    axis line style={darkslategray38},
    % legend cell align={left},
    % legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
    tick pos=left,
    tick align=outside,
    x grid style={lightgray204},
    % xlabel=\textcolor{darkslategray38}{\fnProbWParams(\breachAttacker)},
    xmajorgrids,
    % xmajorticks=false,
    xmin=-0.01, xmax=1.01,
    xtick style={color=darkslategray38},
    y grid style={lightgray204},
    % ylabel=\textcolor{darkslategray38}{\fpProbWParams(\alarmAttacker)},
    ymajorgrids,
    ymajorticks=false,
    ymin=-0.01, ymax=1.01,
    ytick style={color=darkslategray38}
    ]
\addplot [line width=3, steelblue76114176, mark=*, mark size=3, mark options={solid}]
table {%
0.56089973449707 0.602299630641937
0.61789870262146 0.50069934129715
0.660400032997131 0.45740008354187
0.694398701190948 0.41730010509491
0.720699489116669 0.384900450706482
0.741900026798248 0.360599786043167
0.76300048828125 0.346899956464767
0.782800137996674 0.339899748563766
0.800500988960266 0.337200254201889
0.820499002933502 0.336500912904739
0.836400389671326 0.335900127887726
0.852400600910187 0.335599631071091
0.867399632930756 0.335599631071091
0.884200572967529 0.335599631071091
0.899099826812744 0.335599631071091
0.914099991321564 0.335599631071091
0.931599497795105 0.335599631071091
0.949599623680115 0.335599631071091
0.971300005912781 0.335599631071091
};
% \addlegendentry{X=1}
\addplot [line width=3, peru22113282, densely dotted, mark=square*, mark size=3, mark options={solid}]
table {%
0.612600028514862 0.602299630641937
0.665200591087341 0.50069934129715
0.705399334430695 0.45740008354187
0.735199868679047 0.41730010509491
0.757899940013885 0.384900450706482
0.776899874210358 0.360599786043167
0.795399963855743 0.346899956464767
0.812699735164642 0.339899748563766
0.828399002552032 0.337200254201889
0.846599638462067 0.336500912904739
0.860300004482269 0.335900127887726
0.874799609184265 0.335599631071091
0.887900173664093 0.335599631071091
0.903099894523621 0.335599631071091
0.917899608612061 0.335599631071091
0.931099832057953 0.335599631071091
0.945700109004974 0.335599631071091
0.960300028324127 0.335599631071091
0.977100074291229 0.335599631071091
};
% \addlegendentry{X>=1}
\end{axis}

\end{tikzpicture}

